Self-Assessment and Correction of Sensor Synchronization

We propose an approach to assess the synchronization of rigidly mounted sensors based on their rotational motion. Using function similarity measures combined with a sliding window approach, our approach is capable of estimating time-varying time offsets. Further, the estimated offset allows the correction of erroneously assigned time stamps on measurements. This mitigates the effect of synchronization issues on subsequent modules in autonomous software stacks, such as tracking systems that heavily rely on accurate measurement time stamps. Additionally, a self-assessment based on an uncertainty measure is derived, and correction strategies are described. Our approach is evaluated with Monte Carlo experiments containing different error patterns. The results show that our approach accurately estimates time offsets and, thus, is able to detect and assess synchronization issues. To further embrace the importance of our approach for autonomous systems, we investigate the effect of synchronization inconsistencies in tracking systems in more detail and demonstrate the beneficial effect of our proposed offset correction.

==> img/raw/exp/ramp_high_error.tex <==
\addplot [name path=error, color=errorColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 2.000000000000010450e-02
1.100000000000000000e+01, 9.999999999999896125e-03
1.200000000000000000e+01, 1.499999999999989536e-02
1.300000000000000000e+01, 1.999999999999989633e-02
1.400000000000000000e+01, 2.000000000000010450e-02
1.500000000000000000e+01, 1.040834085586084257e-16
1.600000000000000000e+01, 1.499999999999989536e-02
1.700000000000000000e+01, 5.000000000000104187e-03
1.800000000000000000e+01, 2.499999999999989730e-02
1.900000000000000000e+01, 5.999999999999990064e-02
2.000000000000000000e+01, 1.040834085586084257e-16
2.100000000000000000e+01, 2.000000000000010103e-02
2.200000000000000000e+01, 1.000000000000010256e-02
2.300000000000000000e+01, 1.040834085586084257e-16
2.400000000000000000e+01, 9.999999999999897859e-03
2.500000000000000000e+01, 1.499999999999990230e-02
2.600000000000000000e+01, 2.499999999999989730e-02
2.700000000000000000e+01, 2.999999999999990175e-02
2.800000000000000000e+01, 3.999999999999989675e-02
2.900000000000000000e+01, 4.999999999999989175e-02
3.000000000000000000e+01, 5.999999999999990064e-02
3.100000000000000000e+01, 6.999999999999989564e-02
3.200000000000000000e+01, 7.999999999999989064e-02
3.300000000000000000e+01, 7.999999999999990452e-02
3.400000000000000000e+01, 5.999999999999991451e-02
3.500000000000000000e+01, 1.499999999999987454e-02
3.600000000000000000e+01, 2.000000000000010103e-02
3.700000000000000000e+01, 5.000000000000087708e-03
3.800000000000000000e+01, 5.000000000000115463e-03
3.900000000000000000e+01, 3.000000000000010991e-02
4.000000000000000000e+01, 1.000000000000009215e-02
4.100000000000000000e+01, 2.000000000000012879e-02
4.200000000000000000e+01, 3.000000000000010991e-02
4.300000000000000000e+01, 1.000000000000009215e-02
4.400000000000000000e+01, 1.000000000000011990e-02
4.500000000000000000e+01, 3.500000000000014211e-02
4.600000000000000000e+01, 3.500000000000008660e-02
4.700000000000000000e+01, 1.999999999999990674e-02
4.800000000000000000e+01, 5.999999999999991451e-02
4.900000000000000000e+01, 2.999999999999986011e-02
5.000000000000000000e+01, 1.110223024625156540e-16
5.100000000000000000e+01, 1.499999999999990230e-02
5.200000000000000000e+01, 1.500000000000012434e-02
5.300000000000000000e+01, 3.999999999999992450e-02
5.400000000000000000e+01, 1.999999999999990674e-02
5.500000000000000000e+01, 2.999999999999986011e-02
5.600000000000000000e+01, 3.999999999999986899e-02
5.700000000000000000e+01, 4.999999999999987788e-02
5.800000000000000000e+01, 5.999999999999988676e-02
5.900000000000000000e+01, 6.499999999999989120e-02
6.000000000000000000e+01, 7.999999999999990452e-02
6.100000000000000000e+01, 7.999999999999984901e-02
6.200000000000000000e+01, 8.999999999999985789e-02
6.300000000000000000e+01, 7.999999999999990452e-02
6.400000000000000000e+01, 8.499999999999990896e-02
6.500000000000000000e+01, 1.499999999999990230e-02
6.600000000000000000e+01, 4.000000000000009104e-02
6.700000000000000000e+01, 1.665334536937734811e-16
6.800000000000000000e+01, 1.499999999999984679e-02
6.900000000000000000e+01, 2.499999999999985567e-02
7.000000000000000000e+01, 3.999999999999986899e-02
7.100000000000000000e+01, 4.999999999999987788e-02
7.200000000000000000e+01, 1.999999999999990674e-02
7.300000000000000000e+01, 2.499999999999991118e-02
7.400000000000000000e+01, 3.499999999999992006e-02
7.500000000000000000e+01, 2.999999999999991562e-02
7.600000000000000000e+01, 3.499999999999992006e-02
7.700000000000000000e+01, 6.999999999999984013e-02
7.800000000000000000e+01, 1.499999999999979128e-02
7.900000000000000000e+01, 5.499999999999982681e-02
8.000000000000000000e+01, 1.499999999999990230e-02
8.100000000000000000e+01, 9.999999999999897859e-03
8.200000000000000000e+01, 1.999999999999990674e-02
8.300000000000000000e+01, 1.999999999999990674e-02
8.400000000000000000e+01, 1.999999999999990674e-02
8.500000000000000000e+01, 1.999999999999990674e-02
8.600000000000000000e+01, 9.999999999999897859e-03
8.700000000000000000e+01, 2.999999999999991562e-02
8.800000000000000000e+01, 4.499999999999992895e-02
8.900000000000000000e+01, 5.999999999999983125e-02
9.000000000000000000e+01, 2.999999999999980460e-02
9.100000000000000000e+01, 3.499999999999980904e-02
9.200000000000000000e+01, 3.999999999999981348e-02
9.300000000000000000e+01, 4.999999999999982236e-02
9.400000000000000000e+01, 4.500000000000015099e-02
9.500000000000000000e+01, 4.000000000000014655e-02
9.600000000000000000e+01, 2.500000000000013323e-02
9.700000000000000000e+01, 2.000000000000012879e-02
9.800000000000000000e+01, 4.999999999999893419e-03
9.900000000000000000e+01, 1.000000000000011990e-02
1.000000000000000000e+02, 1.110223024625156540e-16
1.010000000000000000e+02, 4.999999999999893419e-03
1.020000000000000000e+02, 1.499999999999979128e-02
1.030000000000000000e+02, 2.499999999999980016e-02
1.040000000000000000e+02, 2.999999999999980460e-02
1.050000000000000000e+02, 3.999999999999981348e-02
1.060000000000000000e+02, 4.999999999999982236e-02
1.070000000000000000e+02, 3.999999999999992450e-02
1.080000000000000000e+02, 6.499999999999983569e-02
1.090000000000000000e+02, 6.999999999999984013e-02
1.100000000000000000e+02, 3.000000000000013767e-02
1.110000000000000000e+02, 1.000000000000001998e-01
1.120000000000000000e+02, 3.000000000000013767e-02
1.130000000000000000e+02, 4.999999999999893419e-03
1.140000000000000000e+02, 1.000000000000023093e-02
1.150000000000000000e+02, 2.499999999999980016e-02
1.160000000000000000e+02, 2.499999999999980016e-02
1.170000000000000000e+02, 1.499999999999990230e-02
1.180000000000000000e+02, 3.999999999999981348e-02
1.190000000000000000e+02, 2.999999999999991562e-02
1.200000000000000000e+02, 3.499999999999992006e-02
1.210000000000000000e+02, 3.499999999999992006e-02
1.220000000000000000e+02, 5.499999999999993783e-02
1.230000000000000000e+02, 8.499999999999985345e-02
1.240000000000000000e+02, 3.999999999999981348e-02
1.250000000000000000e+02, 5.000000000000115463e-03
1.260000000000000000e+02, 4.999999999999893419e-03
1.270000000000000000e+02, 1.000000000000000888e-02
1.280000000000000000e+02, 2.000000000000001776e-02
1.290000000000000000e+02, 3.000000000000002665e-02
1.300000000000000000e+02, 3.000000000000002665e-02
1.310000000000000000e+02, 4.000000000000003553e-02
1.320000000000000000e+02, 5.000000000000004441e-02
1.330000000000000000e+02, 5.999999999999983125e-02
1.340000000000000000e+02, 6.999999999999984013e-02
1.350000000000000000e+02, 7.999999999999984901e-02
1.360000000000000000e+02, 8.999999999999985789e-02
1.370000000000000000e+02, 8.999999999999985789e-02
1.380000000000000000e+02, 9.999999999999986677e-02
1.390000000000000000e+02, 8.499999999999996447e-02
1.400000000000000000e+02, 9.499999999999997335e-02
1.410000000000000000e+02, 7.000000000000028422e-02
1.420000000000000000e+02, 1.499999999999990230e-02
1.430000000000000000e+02, 4.499999999999992895e-02
1.440000000000000000e+02, 6.499999999999972466e-02
1.450000000000000000e+02, 5.999999999999983125e-02
1.460000000000000000e+02, 4.499999999999970690e-02
1.470000000000000000e+02, 1.999999999999979572e-02
1.480000000000000000e+02, 4.999999999999982236e-02
1.490000000000000000e+02, 5.499999999999971578e-02
1.500000000000000000e+02, 4.999999999999982236e-02
1.510000000000000000e+02, 5.499999999999971578e-02
1.520000000000000000e+02, 5.999999999999983125e-02
1.530000000000000000e+02, 5.000000000000004441e-02
1.540000000000000000e+02, 5.000000000000004441e-02
1.550000000000000000e+02, 3.500000000000014211e-02
1.560000000000000000e+02, 4.000000000000003553e-02
1.570000000000000000e+02, 2.499999999999991118e-02
1.580000000000000000e+02, 2.999999999999980460e-02
1.590000000000000000e+02, 4.999999999999982236e-02
1.600000000000000000e+02, 2.999999999999980460e-02
1.610000000000000000e+02, 4.999999999999982236e-02
1.620000000000000000e+02, 2.999999999999980460e-02
1.630000000000000000e+02, 5.499999999999993783e-02
1.640000000000000000e+02, 7.999999999999984901e-02
1.650000000000000000e+02, 7.999999999999984901e-02
1.660000000000000000e+02, 4.999999999999982236e-02
1.670000000000000000e+02, 6.999999999999984013e-02
1.680000000000000000e+02, 5.999999999999983125e-02
1.690000000000000000e+02, 1.999999999999979572e-02
1.700000000000000000e+02, 1.100000000000000977e-01
1.710000000000000000e+02, 1.050000000000002043e-01
1.720000000000000000e+02, 4.499999999999992895e-02
1.730000000000000000e+02, 9.999999999999786837e-03
1.740000000000000000e+02, 2.000000000000001776e-02
1.750000000000000000e+02, 2.999999999999980460e-02
1.760000000000000000e+02, 2.000000000000001776e-02
1.770000000000000000e+02, 3.000000000000002665e-02
1.780000000000000000e+02, 4.000000000000003553e-02
1.790000000000000000e+02, 4.500000000000015099e-02
1.800000000000000000e+02, 5.000000000000004441e-02
1.810000000000000000e+02, 6.000000000000005329e-02
1.820000000000000000e+02, 7.500000000000017764e-02
1.830000000000000000e+02, 6.499999999999994671e-02
1.840000000000000000e+02, 7.499999999999995559e-02
1.850000000000000000e+02, 5.500000000000015987e-02
1.860000000000000000e+02, 4.500000000000015099e-02
1.870000000000000000e+02, 5.000000000000026645e-02
1.880000000000000000e+02, 4.500000000000015099e-02
1.890000000000000000e+02, 5.500000000000015987e-02
1.900000000000000000e+02, 3.500000000000036415e-02
1.910000000000000000e+02, 6.500000000000039080e-02
1.920000000000000000e+02, 5.500000000000038192e-02
1.930000000000000000e+02, 1.499999999999968026e-02
1.940000000000000000e+02, 2.999999999999980460e-02
};

\addlegendentry{error}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_high_estimation.tex <==
\addplot [name path=estimationlower, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, -1.299999999999998934e-01
1.100000000000000000e+01, -1.424999999999999045e-01
1.200000000000000000e+01, -1.499999999999999112e-01
1.300000000000000000e+01, -1.624999999999998945e-01
1.400000000000000000e+01, -1.749999999999999056e-01
1.500000000000000000e+01, -2.124999999999999112e-01
1.600000000000000000e+01, -1.999999999999999001e-01
1.700000000000000000e+01, -2.124999999999999112e-01
1.800000000000000000e+01, -2.699999999999999067e-01
1.900000000000000000e+01, -2.524999999999998912e-01
2.000000000000000000e+01, -1.324999999999998956e-01
2.100000000000000000e+01, -4.999999999999989869e-02
2.200000000000000000e+01, -9.999999999999896125e-03
2.300000000000000000e+01, -2.499999999999895969e-03
2.400000000000000000e+01, 1.040834085586084257e-16
2.500000000000000000e+01, -9.999999999999896125e-03
2.600000000000000000e+01, -9.999999999999896125e-03
2.700000000000000000e+01, 1.040834085586084257e-16
2.800000000000000000e+01, 7.500000000000103806e-03
2.900000000000000000e+01, 1.000000000000010429e-02
3.000000000000000000e+01, 7.500000000000103806e-03
3.100000000000000000e+01, 1.000000000000010429e-02
3.200000000000000000e+01, 7.500000000000103806e-03
3.300000000000000000e+01, 7.500000000000103806e-03
3.400000000000000000e+01, -1.249999999999989661e-02
3.500000000000000000e+01, -1.224999999999999006e-01
3.600000000000000000e+01, -1.049999999999998990e-01
3.700000000000000000e+01, -1.224999999999999006e-01
3.800000000000000000e+01, -1.324999999999998956e-01
3.900000000000000000e+01, -5.499999999999989619e-02
4.000000000000000000e+01, 2.500000000000104569e-03
4.100000000000000000e+01, 5.000000000000010686e-02
4.200000000000000000e+01, 4.750000000000010464e-02
4.300000000000000000e+01, 7.750000000000009659e-02
4.400000000000000000e+01, 5.750000000000010658e-02
4.500000000000000000e+01, 1.750000000000010575e-02
4.600000000000000000e+01, 2.000000000000010450e-02
4.700000000000000000e+01, -4.999999999999896888e-03
4.800000000000000000e+01, 7.500000000000103806e-03
4.900000000000000000e+01, -2.499999999999989730e-02
5.000000000000000000e+01, 1.975000000000001199e-01
5.100000000000000000e+01, 2.500000000000001110e-01
5.200000000000000000e+01, 2.900000000000000910e-01
5.300000000000000000e+01, 2.575000000000001177e-01
5.400000000000000000e+01, 2.900000000000000910e-01
5.500000000000000000e+01, 2.900000000000000910e-01
5.600000000000000000e+01, 2.900000000000000910e-01
5.700000000000000000e+01, 2.900000000000000910e-01
5.800000000000000000e+01, 2.900000000000000910e-01
5.900000000000000000e+01, 2.900000000000000910e-01
6.000000000000000000e+01, 2.900000000000000910e-01
6.100000000000000000e+01, 2.800000000000001377e-01
6.200000000000000000e+01, 2.875000000000000888e-01
6.300000000000000000e+01, 2.775000000000001354e-01
6.400000000000000000e+01, 1.950000000000001177e-01
6.500000000000000000e+01, 2.400000000000001021e-01
6.600000000000000000e+01, 3.000000000000000999e-01
6.700000000000000000e+01, 2.700000000000001288e-01
6.800000000000000000e+01, 2.800000000000001377e-01
6.900000000000000000e+01, 2.775000000000001354e-01
7.000000000000000000e+01, 3.275000000000001243e-01
7.100000000000000000e+01, 3.375000000000001332e-01
7.200000000000000000e+01, 3.450000000000000844e-01
7.300000000000000000e+01, 3.675000000000001044e-01
7.400000000000000000e+01, 3.575000000000000955e-01
7.500000000000000000e+01, 3.700000000000001066e-01
7.600000000000000000e+01, 3.775000000000001132e-01
7.700000000000000000e+01, 3.700000000000001066e-01
7.800000000000000000e+01, 3.775000000000001132e-01
7.900000000000000000e+01, 3.700000000000001066e-01
8.000000000000000000e+01, 4.000000000000001332e-01
8.100000000000000000e+01, 4.200000000000000955e-01
8.200000000000000000e+01, 4.775000000000000910e-01
8.300000000000000000e+01, 4.575000000000001288e-01
8.400000000000000000e+01, 4.700000000000001399e-01
8.500000000000000000e+01, 5.300000000000001377e-01
8.600000000000000000e+01, 5.300000000000001377e-01
8.700000000000000000e+01, 5.475000000000000977e-01
8.800000000000000000e+01, 5.375000000000000888e-01
8.900000000000000000e+01, 5.375000000000000888e-01
9.000000000000000000e+01, 5.400000000000001465e-01
9.100000000000000000e+01, 5.300000000000001377e-01
9.200000000000000000e+01, 5.300000000000001377e-01
9.300000000000000000e+01, 5.100000000000001199e-01
9.400000000000000000e+01, 4.850000000000000977e-01
9.500000000000000000e+01, 5.400000000000001465e-01
9.600000000000000000e+01, 6.900000000000001688e-01
9.700000000000000000e+01, 7.500000000000001110e-01
9.800000000000000000e+01, 7.300000000000000933e-01
9.900000000000000000e+01, 7.675000000000000711e-01
1.000000000000000000e+02, 7.700000000000001288e-01
1.010000000000000000e+02, 7.700000000000001288e-01
1.020000000000000000e+02, 7.700000000000001288e-01
1.030000000000000000e+02, 7.700000000000001288e-01
1.040000000000000000e+02, 7.700000000000001288e-01
1.050000000000000000e+02, 7.700000000000001288e-01
1.060000000000000000e+02, 7.700000000000001288e-01
1.070000000000000000e+02, 7.800000000000001377e-01
1.080000000000000000e+02, 7.700000000000001288e-01
1.090000000000000000e+02, 7.475000000000000533e-01
1.100000000000000000e+02, 7.200000000000000844e-01
1.110000000000000000e+02, 6.700000000000001510e-01
1.120000000000000000e+02, 7.475000000000000533e-01
1.130000000000000000e+02, 7.100000000000000755e-01
1.140000000000000000e+02, 7.250000000000000888e-01
1.150000000000000000e+02, 7.650000000000001243e-01
1.160000000000000000e+02, 7.275000000000000355e-01
1.170000000000000000e+02, 7.175000000000000266e-01
1.180000000000000000e+02, 7.100000000000000755e-01
1.190000000000000000e+02, 7.300000000000000933e-01
1.200000000000000000e+02, 7.150000000000000799e-01
1.210000000000000000e+02, 7.000000000000000666e-01
1.220000000000000000e+02, 6.725000000000000977e-01
1.230000000000000000e+02, 6.675000000000002043e-01
1.240000000000000000e+02, 7.725000000000001865e-01
1.250000000000000000e+02, 8.775000000000001688e-01
1.260000000000000000e+02, 9.600000000000000755e-01
1.270000000000000000e+02, 1.017500000000000071e+00
1.280000000000000000e+02, 1.020000000000000018e+00
1.290000000000000000e+02, 1.030000000000000027e+00
1.300000000000000000e+02, 1.050000000000000044e+00
1.310000000000000000e+02, 1.050000000000000044e+00
1.320000000000000000e+02, 1.050000000000000044e+00
1.330000000000000000e+02, 1.050000000000000044e+00
1.340000000000000000e+02, 1.040000000000000036e+00
1.350000000000000000e+02, 1.050000000000000044e+00
1.360000000000000000e+02, 1.050000000000000044e+00
1.370000000000000000e+02, 1.050000000000000044e+00
1.380000000000000000e+02, 1.047500000000000098e+00
1.390000000000000000e+02, 9.900000000000001021e-01
1.400000000000000000e+02, 9.250000000000001554e-01
1.410000000000000000e+02, 1.035000000000000142e+00
1.420000000000000000e+02, 1.010000000000000231e+00
1.430000000000000000e+02, 1.027500000000000080e+00
1.440000000000000000e+02, 1.017500000000000071e+00
1.450000000000000000e+02, 1.027500000000000080e+00
1.460000000000000000e+02, 1.090000000000000080e+00
1.470000000000000000e+02, 1.087500000000000133e+00
1.480000000000000000e+02, 1.107500000000000151e+00
1.490000000000000000e+02, 1.100000000000000089e+00
1.500000000000000000e+02, 1.127500000000000169e+00
1.510000000000000000e+02, 1.090000000000000080e+00
1.520000000000000000e+02, 1.095000000000000195e+00
1.530000000000000000e+02, 1.100000000000000089e+00
1.540000000000000000e+02, 1.110000000000000098e+00
1.550000000000000000e+02, 1.150000000000000133e+00
1.560000000000000000e+02, 1.187500000000000222e+00
1.570000000000000000e+02, 1.207500000000000240e+00
1.580000000000000000e+02, 1.220000000000000195e+00
1.590000000000000000e+02, 1.220000000000000195e+00
1.600000000000000000e+02, 1.240000000000000213e+00
1.610000000000000000e+02, 1.250000000000000222e+00
1.620000000000000000e+02, 1.237500000000000266e+00
1.630000000000000000e+02, 1.240000000000000213e+00
1.640000000000000000e+02, 1.240000000000000213e+00
1.650000000000000000e+02, 1.230000000000000204e+00
1.660000000000000000e+02, 1.210000000000000187e+00
1.670000000000000000e+02, 1.210000000000000187e+00
1.680000000000000000e+02, 1.207500000000000240e+00
1.690000000000000000e+02, 1.237500000000000266e+00
1.700000000000000000e+02, 1.297500000000000098e+00
1.710000000000000000e+02, 1.400000000000000133e+00
1.720000000000000000e+02, 1.437500000000000222e+00
1.730000000000000000e+02, 1.477500000000000258e+00
1.740000000000000000e+02, 1.500000000000000222e+00
1.750000000000000000e+02, 1.480000000000000204e+00
1.760000000000000000e+02, 1.510000000000000231e+00
1.770000000000000000e+02, 1.510000000000000231e+00
1.780000000000000000e+02, 1.510000000000000231e+00
1.790000000000000000e+02, 1.510000000000000231e+00
1.800000000000000000e+02, 1.510000000000000231e+00
1.810000000000000000e+02, 1.520000000000000240e+00
1.820000000000000000e+02, 1.497500000000000275e+00
1.830000000000000000e+02, 1.510000000000000231e+00
1.840000000000000000e+02, 1.500000000000000222e+00
1.850000000000000000e+02, 1.457500000000000240e+00
1.860000000000000000e+02, 1.502500000000000169e+00
1.870000000000000000e+02, 1.502500000000000169e+00
1.880000000000000000e+02, 1.507500000000000284e+00
1.890000000000000000e+02, 1.527500000000000080e+00
1.900000000000000000e+02, 1.550000000000000044e+00
1.910000000000000000e+02, 1.540000000000000036e+00
1.920000000000000000e+02, 1.557500000000000107e+00
1.930000000000000000e+02, 1.590000000000000080e+00
1.940000000000000000e+02, 1.555000000000000160e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationupper, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 1.700000000000000955e-01
1.100000000000000000e+01, 1.325000000000001177e-01
1.200000000000000000e+01, 1.325000000000001177e-01
1.300000000000000000e+01, 1.300000000000001155e-01
1.400000000000000000e+01, 1.500000000000001055e-01
1.500000000000000000e+01, 1.625000000000001166e-01
1.600000000000000000e+01, 2.125000000000001055e-01
1.700000000000000000e+01, 2.075000000000001288e-01
1.800000000000000000e+01, 2.125000000000001055e-01
1.900000000000000000e+01, 2.225000000000001144e-01
2.000000000000000000e+01, 2.125000000000001055e-01
2.100000000000000000e+01, 1.000000000000001027e-01
2.200000000000000000e+01, 6.000000000000010880e-02
2.300000000000000000e+01, 6.000000000000010880e-02
2.400000000000000000e+01, 7.000000000000010381e-02
2.500000000000000000e+01, 6.250000000000011102e-02
2.600000000000000000e+01, 6.250000000000011102e-02
2.700000000000000000e+01, 7.000000000000010381e-02
2.800000000000000000e+01, 7.000000000000010381e-02
2.900000000000000000e+01, 7.000000000000010381e-02
3.000000000000000000e+01, 7.000000000000010381e-02
3.100000000000000000e+01, 7.000000000000010381e-02
3.200000000000000000e+01, 8.000000000000009881e-02
3.300000000000000000e+01, 9.250000000000010991e-02
3.400000000000000000e+01, 1.975000000000001199e-01
3.500000000000000000e+01, 3.225000000000001199e-01
3.600000000000000000e+01, 4.000000000000001332e-01
3.700000000000000000e+01, 3.900000000000001243e-01
3.800000000000000000e+01, 4.025000000000001354e-01
3.900000000000000000e+01, 3.850000000000001199e-01
4.000000000000000000e+01, 4.200000000000000955e-01
4.100000000000000000e+01, 4.150000000000000910e-01
4.200000000000000000e+01, 4.300000000000001044e-01
4.300000000000000000e+01, 4.500000000000001221e-01
4.400000000000000000e+01, 4.625000000000001332e-01
4.500000000000000000e+01, 4.725000000000001421e-01
4.600000000000000000e+01, 4.625000000000001332e-01
4.700000000000000000e+01, 4.500000000000001221e-01
4.800000000000000000e+01, 4.525000000000001243e-01
4.900000000000000000e+01, 4.725000000000001421e-01
5.000000000000000000e+01, 4.500000000000001221e-01
5.100000000000000000e+01, 3.600000000000000977e-01
5.200000000000000000e+01, 3.800000000000001155e-01
5.300000000000000000e+01, 3.400000000000001354e-01
5.400000000000000000e+01, 3.500000000000000888e-01
5.500000000000000000e+01, 3.500000000000000888e-01
5.600000000000000000e+01, 3.500000000000000888e-01
5.700000000000000000e+01, 3.500000000000000888e-01
5.800000000000000000e+01, 3.500000000000000888e-01
5.900000000000000000e+01, 3.500000000000000888e-01
6.000000000000000000e+01, 3.500000000000000888e-01
6.100000000000000000e+01, 3.525000000000000910e-01
6.200000000000000000e+01, 3.725000000000001088e-01
6.300000000000000000e+01, 4.000000000000001332e-01
6.400000000000000000e+01, 5.800000000000000711e-01
6.500000000000000000e+01, 7.025000000000001243e-01
6.600000000000000000e+01, 7.625000000000001776e-01
6.700000000000000000e+01, 7.200000000000000844e-01
6.800000000000000000e+01, 6.925000000000001155e-01
6.900000000000000000e+01, 6.600000000000001421e-01
7.000000000000000000e+01, 6.625000000000000888e-01
7.100000000000000000e+01, 6.625000000000000888e-01
7.200000000000000000e+01, 6.325000000000000622e-01
7.300000000000000000e+01, 6.400000000000001243e-01
7.400000000000000000e+01, 6.500000000000001332e-01
7.500000000000000000e+01, 6.625000000000000888e-01
7.600000000000000000e+01, 7.000000000000000666e-01
7.700000000000000000e+01, 7.075000000000000178e-01
7.800000000000000000e+01, 7.400000000000001021e-01
7.900000000000000000e+01, 7.300000000000000933e-01
8.000000000000000000e+01, 7.475000000000000533e-01
8.100000000000000000e+01, 7.500000000000001110e-01
8.200000000000000000e+01, 7.425000000000001599e-01
8.300000000000000000e+01, 7.800000000000001377e-01
8.400000000000000000e+01, 7.525000000000001688e-01
8.500000000000000000e+01, 7.400000000000001021e-01
8.600000000000000000e+01, 7.400000000000001021e-01
8.700000000000000000e+01, 7.500000000000001110e-01
8.800000000000000000e+01, 7.625000000000001776e-01
8.900000000000000000e+01, 7.800000000000001377e-01
9.000000000000000000e+01, 8.500000000000000888e-01
9.100000000000000000e+01, 8.800000000000001155e-01
9.200000000000000000e+01, 8.925000000000000711e-01
9.300000000000000000e+01, 9.225000000000000977e-01
9.400000000000000000e+01, 1.002500000000000169e+00
9.500000000000000000e+01, 1.090000000000000080e+00
9.600000000000000000e+01, 9.325000000000001066e-01
9.700000000000000000e+01, 8.400000000000000799e-01
9.800000000000000000e+01, 8.100000000000001643e-01
9.900000000000000000e+01, 8.325000000000000178e-01
1.000000000000000000e+02, 8.300000000000000711e-01
1.010000000000000000e+02, 8.325000000000000178e-01
1.020000000000000000e+02, 8.300000000000000711e-01
1.030000000000000000e+02, 8.300000000000000711e-01
1.040000000000000000e+02, 8.300000000000000711e-01
1.050000000000000000e+02, 8.325000000000000178e-01
1.060000000000000000e+02, 8.400000000000000799e-01
1.070000000000000000e+02, 8.600000000000000977e-01
1.080000000000000000e+02, 8.425000000000000266e-01
1.090000000000000000e+02, 9.000000000000001332e-01
1.100000000000000000e+02, 1.282499999999999973e+00
1.110000000000000000e+02, 1.267500000000000071e+00
1.120000000000000000e+02, 1.180000000000000160e+00
1.130000000000000000e+02, 1.150000000000000133e+00
1.140000000000000000e+02, 1.160000000000000142e+00
1.150000000000000000e+02, 1.140000000000000124e+00
1.160000000000000000e+02, 1.142500000000000071e+00
1.170000000000000000e+02, 1.120000000000000107e+00
1.180000000000000000e+02, 1.092500000000000027e+00
1.190000000000000000e+02, 1.102500000000000036e+00
1.200000000000000000e+02, 1.130000000000000115e+00
1.210000000000000000e+02, 1.170000000000000151e+00
1.220000000000000000e+02, 1.170000000000000151e+00
1.230000000000000000e+02, 1.162500000000000089e+00
1.240000000000000000e+02, 1.220000000000000195e+00
1.250000000000000000e+02, 1.302499999999999991e+00
1.260000000000000000e+02, 1.182500000000000107e+00
1.270000000000000000e+02, 1.112500000000000044e+00
1.280000000000000000e+02, 1.090000000000000080e+00
1.290000000000000000e+02, 1.100000000000000089e+00
1.300000000000000000e+02, 1.100000000000000089e+00
1.310000000000000000e+02, 1.100000000000000089e+00
1.320000000000000000e+02, 1.110000000000000098e+00
1.330000000000000000e+02, 1.110000000000000098e+00
1.340000000000000000e+02, 1.110000000000000098e+00
1.350000000000000000e+02, 1.110000000000000098e+00
1.360000000000000000e+02, 1.110000000000000098e+00
1.370000000000000000e+02, 1.122500000000000053e+00
1.380000000000000000e+02, 1.150000000000000133e+00
1.390000000000000000e+02, 1.347500000000000142e+00
1.400000000000000000e+02, 1.772500000000000187e+00
1.410000000000000000e+02, 1.564999999999999947e+00
1.420000000000000000e+02, 1.460000000000000187e+00
1.430000000000000000e+02, 1.400000000000000133e+00
1.440000000000000000e+02, 1.392500000000000071e+00
1.450000000000000000e+02, 1.392500000000000071e+00
1.460000000000000000e+02, 1.340000000000000080e+00
1.470000000000000000e+02, 1.342500000000000027e+00
1.480000000000000000e+02, 1.362500000000000044e+00
1.490000000000000000e+02, 1.380000000000000115e+00
1.500000000000000000e+02, 1.382500000000000062e+00
1.510000000000000000e+02, 1.410000000000000142e+00
1.520000000000000000e+02, 1.422500000000000098e+00
1.530000000000000000e+02, 1.420000000000000151e+00
1.540000000000000000e+02, 1.460000000000000187e+00
1.550000000000000000e+02, 1.472500000000000142e+00
1.560000000000000000e+02, 1.500000000000000222e+00
1.570000000000000000e+02, 1.490000000000000213e+00
1.580000000000000000e+02, 1.470000000000000195e+00
1.590000000000000000e+02, 1.502500000000000169e+00
1.600000000000000000e+02, 1.500000000000000222e+00
1.610000000000000000e+02, 1.472500000000000142e+00
1.620000000000000000e+02, 1.500000000000000222e+00
1.630000000000000000e+02, 1.512500000000000178e+00
1.640000000000000000e+02, 1.512500000000000178e+00
1.650000000000000000e+02, 1.552499999999999991e+00
1.660000000000000000e+02, 1.604999999999999982e+00
1.670000000000000000e+02, 1.632500000000000062e+00
1.680000000000000000e+02, 1.592500000000000027e+00
1.690000000000000000e+02, 1.750000000000000222e+00
1.700000000000000000e+02, 1.957500000000000240e+00
1.710000000000000000e+02, 1.860000000000000098e+00
1.720000000000000000e+02, 1.662500000000000089e+00
1.730000000000000000e+02, 1.552499999999999991e+00
1.740000000000000000e+02, 1.582500000000000018e+00
1.750000000000000000e+02, 1.550000000000000044e+00
1.760000000000000000e+02, 1.570000000000000062e+00
1.770000000000000000e+02, 1.570000000000000062e+00
1.780000000000000000e+02, 1.570000000000000062e+00
1.790000000000000000e+02, 1.570000000000000062e+00
1.800000000000000000e+02, 1.580000000000000071e+00
1.810000000000000000e+02, 1.590000000000000080e+00
1.820000000000000000e+02, 1.600000000000000089e+00
1.830000000000000000e+02, 1.620000000000000107e+00
1.840000000000000000e+02, 1.680000000000000160e+00
1.850000000000000000e+02, 1.982500000000000151e+00
1.860000000000000000e+02, 2.012500000000000178e+00
1.870000000000000000e+02, 1.955000000000000071e+00
1.880000000000000000e+02, 1.922500000000000098e+00
1.890000000000000000e+02, 1.942500000000000115e+00
1.900000000000000000e+02, 1.942500000000000115e+00
1.910000000000000000e+02, 1.912500000000000089e+00
1.920000000000000000e+02, 1.892500000000000071e+00
1.930000000000000000e+02, 1.872500000000000053e+00
1.940000000000000000e+02, 1.890000000000000124e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationmedian, color=estimationColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 2.000000000000010450e-02
1.100000000000000000e+01, -9.999999999999896125e-03
1.200000000000000000e+01, -1.499999999999989536e-02
1.300000000000000000e+01, -1.999999999999989633e-02
1.400000000000000000e+01, 2.000000000000010450e-02
1.500000000000000000e+01, 1.040834085586084257e-16
1.600000000000000000e+01, -1.499999999999989536e-02
1.700000000000000000e+01, 5.000000000000104187e-03
1.800000000000000000e+01, -2.499999999999989730e-02
1.900000000000000000e+01, -5.999999999999990064e-02
2.000000000000000000e+01, 1.040834085586084257e-16
2.100000000000000000e+01, 3.000000000000010297e-02
2.200000000000000000e+01, 3.000000000000010297e-02
2.300000000000000000e+01, 3.000000000000010297e-02
2.400000000000000000e+01, 3.000000000000010297e-02
2.500000000000000000e+01, 3.500000000000010048e-02
2.600000000000000000e+01, 3.500000000000010048e-02
2.700000000000000000e+01, 4.000000000000010492e-02
2.800000000000000000e+01, 4.000000000000010492e-02
2.900000000000000000e+01, 4.000000000000010492e-02
3.000000000000000000e+01, 4.000000000000010492e-02
3.100000000000000000e+01, 4.000000000000010492e-02
3.200000000000000000e+01, 4.000000000000010492e-02
3.300000000000000000e+01, 5.000000000000010686e-02
3.400000000000000000e+01, 8.000000000000009881e-02
3.500000000000000000e+01, 1.350000000000001199e-01
3.600000000000000000e+01, 1.800000000000001044e-01
3.700000000000000000e+01, 1.750000000000000999e-01
3.800000000000000000e+01, 1.850000000000001088e-01
3.900000000000000000e+01, 2.200000000000001121e-01
4.000000000000000000e+01, 2.100000000000001033e-01
4.100000000000000000e+01, 2.300000000000001210e-01
4.200000000000000000e+01, 2.500000000000001110e-01
4.300000000000000000e+01, 2.400000000000001021e-01
4.400000000000000000e+01, 2.500000000000001110e-01
4.500000000000000000e+01, 2.850000000000001421e-01
4.600000000000000000e+01, 2.950000000000000955e-01
4.700000000000000000e+01, 2.500000000000001110e-01
4.800000000000000000e+01, 2.200000000000001121e-01
4.900000000000000000e+01, 2.600000000000001199e-01
5.000000000000000000e+01, 3.000000000000000999e-01
5.100000000000000000e+01, 2.950000000000000955e-01
5.200000000000000000e+01, 3.350000000000001310e-01
5.300000000000000000e+01, 2.900000000000000910e-01
5.400000000000000000e+01, 3.200000000000001177e-01
5.500000000000000000e+01, 3.200000000000001177e-01
5.600000000000000000e+01, 3.200000000000001177e-01
5.700000000000000000e+01, 3.200000000000001177e-01
5.800000000000000000e+01, 3.200000000000001177e-01
5.900000000000000000e+01, 3.250000000000001221e-01
6.000000000000000000e+01, 3.200000000000001177e-01
6.100000000000000000e+01, 3.300000000000001266e-01
6.200000000000000000e+01, 3.300000000000001266e-01
6.300000000000000000e+01, 3.500000000000000888e-01
6.400000000000000000e+01, 3.550000000000000933e-01
6.500000000000000000e+01, 4.350000000000001088e-01
6.600000000000000000e+01, 5.000000000000001110e-01
6.700000000000000000e+01, 4.700000000000001399e-01
6.800000000000000000e+01, 4.650000000000001354e-01
6.900000000000000000e+01, 4.650000000000001354e-01
7.000000000000000000e+01, 4.600000000000001310e-01
7.100000000000000000e+01, 4.600000000000001310e-01
7.200000000000000000e+01, 5.000000000000001110e-01
7.300000000000000000e+01, 5.050000000000001155e-01
7.400000000000000000e+01, 5.050000000000001155e-01
7.500000000000000000e+01, 5.200000000000001288e-01
7.600000000000000000e+01, 5.250000000000001332e-01
7.700000000000000000e+01, 5.000000000000001110e-01
7.800000000000000000e+01, 5.650000000000001688e-01
7.900000000000000000e+01, 5.350000000000001421e-01
8.000000000000000000e+01, 5.850000000000000755e-01
8.100000000000000000e+01, 6.000000000000000888e-01
8.200000000000000000e+01, 6.000000000000000888e-01
8.300000000000000000e+01, 6.100000000000000977e-01
8.400000000000000000e+01, 6.200000000000001066e-01
8.500000000000000000e+01, 6.300000000000001155e-01
8.600000000000000000e+01, 6.500000000000001332e-01
8.700000000000000000e+01, 6.400000000000001243e-01
8.800000000000000000e+01, 6.350000000000001199e-01
8.900000000000000000e+01, 6.300000000000001155e-01
9.000000000000000000e+01, 6.700000000000001510e-01
9.100000000000000000e+01, 6.750000000000001554e-01
9.200000000000000000e+01, 6.800000000000001599e-01
9.300000000000000000e+01, 6.800000000000001599e-01
9.400000000000000000e+01, 7.850000000000001421e-01
9.500000000000000000e+01, 7.900000000000001465e-01
9.600000000000000000e+01, 7.850000000000001421e-01
9.700000000000000000e+01, 7.900000000000001465e-01
9.800000000000000000e+01, 7.750000000000001332e-01
9.900000000000000000e+01, 8.000000000000001554e-01
1.000000000000000000e+02, 8.000000000000001554e-01
1.010000000000000000e+02, 8.050000000000001599e-01
1.020000000000000000e+02, 8.050000000000001599e-01
1.030000000000000000e+02, 8.050000000000001599e-01
1.040000000000000000e+02, 8.100000000000001643e-01
1.050000000000000000e+02, 8.100000000000001643e-01
1.060000000000000000e+02, 8.100000000000001643e-01
1.070000000000000000e+02, 8.300000000000000711e-01
1.080000000000000000e+02, 8.150000000000001688e-01
1.090000000000000000e+02, 8.200000000000001732e-01
1.100000000000000000e+02, 9.300000000000001599e-01
1.110000000000000000e+02, 1.010000000000000231e+00
1.120000000000000000e+02, 9.500000000000001776e-01
1.130000000000000000e+02, 9.250000000000001554e-01
1.140000000000000000e+02, 9.500000000000001776e-01
1.150000000000000000e+02, 9.250000000000001554e-01
1.160000000000000000e+02, 9.350000000000001643e-01
1.170000000000000000e+02, 9.550000000000000711e-01
1.180000000000000000e+02, 9.400000000000001688e-01
1.190000000000000000e+02, 9.600000000000000755e-01
1.200000000000000000e+02, 9.650000000000000799e-01
1.210000000000000000e+02, 9.750000000000000888e-01
1.220000000000000000e+02, 9.650000000000000799e-01
1.230000000000000000e+02, 9.450000000000001732e-01
1.240000000000000000e+02, 1.000000000000000222e+00
1.250000000000000000e+02, 1.055000000000000160e+00
1.260000000000000000e+02, 1.064999999999999947e+00
1.270000000000000000e+02, 1.060000000000000053e+00
1.280000000000000000e+02, 1.060000000000000053e+00
1.290000000000000000e+02, 1.060000000000000053e+00
1.300000000000000000e+02, 1.070000000000000062e+00
1.310000000000000000e+02, 1.070000000000000062e+00
1.320000000000000000e+02, 1.070000000000000062e+00
1.330000000000000000e+02, 1.070000000000000062e+00
1.340000000000000000e+02, 1.070000000000000062e+00
1.350000000000000000e+02, 1.070000000000000062e+00
1.360000000000000000e+02, 1.070000000000000062e+00
1.370000000000000000e+02, 1.080000000000000071e+00
1.380000000000000000e+02, 1.080000000000000071e+00
1.390000000000000000e+02, 1.104999999999999982e+00
1.400000000000000000e+02, 1.294999999999999929e+00
1.410000000000000000e+02, 1.280000000000000249e+00
1.420000000000000000e+02, 1.205000000000000071e+00
1.430000000000000000e+02, 1.185000000000000053e+00
1.440000000000000000e+02, 1.175000000000000266e+00
1.450000000000000000e+02, 1.190000000000000169e+00
1.460000000000000000e+02, 1.215000000000000302e+00
1.470000000000000000e+02, 1.250000000000000222e+00
1.480000000000000000e+02, 1.230000000000000204e+00
1.490000000000000000e+02, 1.235000000000000320e+00
1.500000000000000000e+02, 1.250000000000000222e+00
1.510000000000000000e+02, 1.255000000000000338e+00
1.520000000000000000e+02, 1.260000000000000231e+00
1.530000000000000000e+02, 1.280000000000000027e+00
1.540000000000000000e+02, 1.290000000000000036e+00
1.550000000000000000e+02, 1.314999999999999947e+00
1.560000000000000000e+02, 1.320000000000000062e+00
1.570000000000000000e+02, 1.345000000000000195e+00
1.580000000000000000e+02, 1.350000000000000089e+00
1.590000000000000000e+02, 1.340000000000000080e+00
1.600000000000000000e+02, 1.370000000000000107e+00
1.610000000000000000e+02, 1.360000000000000098e+00
1.620000000000000000e+02, 1.390000000000000124e+00
1.630000000000000000e+02, 1.375000000000000000e+00
1.640000000000000000e+02, 1.360000000000000098e+00
1.650000000000000000e+02, 1.370000000000000107e+00
1.660000000000000000e+02, 1.410000000000000142e+00
1.670000000000000000e+02, 1.400000000000000133e+00
1.680000000000000000e+02, 1.420000000000000151e+00
1.690000000000000000e+02, 1.470000000000000195e+00
1.700000000000000000e+02, 1.610000000000000098e+00
1.710000000000000000e+02, 1.615000000000000213e+00
1.720000000000000000e+02, 1.564999999999999947e+00
1.730000000000000000e+02, 1.520000000000000240e+00
1.740000000000000000e+02, 1.560000000000000053e+00
1.750000000000000000e+02, 1.520000000000000240e+00
1.760000000000000000e+02, 1.540000000000000036e+00
1.770000000000000000e+02, 1.540000000000000036e+00
1.780000000000000000e+02, 1.540000000000000036e+00
1.790000000000000000e+02, 1.544999999999999929e+00
1.800000000000000000e+02, 1.550000000000000044e+00
1.810000000000000000e+02, 1.550000000000000044e+00
1.820000000000000000e+02, 1.544999999999999929e+00
1.830000000000000000e+02, 1.564999999999999947e+00
1.840000000000000000e+02, 1.564999999999999947e+00
1.850000000000000000e+02, 1.705000000000000071e+00
1.860000000000000000e+02, 1.705000000000000071e+00
1.870000000000000000e+02, 1.720000000000000195e+00
1.880000000000000000e+02, 1.725000000000000089e+00
1.890000000000000000e+02, 1.745000000000000107e+00
1.900000000000000000e+02, 1.735000000000000320e+00
1.910000000000000000e+02, 1.775000000000000355e+00
1.920000000000000000e+02, 1.775000000000000355e+00
1.930000000000000000e+02, 1.715000000000000302e+00
1.940000000000000000e+02, 1.710000000000000187e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addlegendentry{estimation}

\addplot [backGray, fill opacity=0.9, forget plot] fill between[of=estimationlower and estimationupper];

\addplot [name path=ground-truth, color=ground-truthColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 0.000000000000000000e+00
1.100000000000000000e+01, 0.000000000000000000e+00
1.200000000000000000e+01, 0.000000000000000000e+00
1.300000000000000000e+01, 0.000000000000000000e+00
1.400000000000000000e+01, 0.000000000000000000e+00
1.500000000000000000e+01, 0.000000000000000000e+00
1.600000000000000000e+01, 0.000000000000000000e+00
1.700000000000000000e+01, 0.000000000000000000e+00
1.800000000000000000e+01, 0.000000000000000000e+00
1.900000000000000000e+01, 0.000000000000000000e+00
2.000000000000000000e+01, 0.000000000000000000e+00
2.100000000000000000e+01, 1.000000000000000021e-02
2.200000000000000000e+01, 2.000000000000000042e-02
2.300000000000000000e+01, 2.999999999999999889e-02
2.400000000000000000e+01, 4.000000000000000083e-02
2.500000000000000000e+01, 5.000000000000000278e-02
2.600000000000000000e+01, 5.999999999999999778e-02
2.700000000000000000e+01, 7.000000000000000666e-02
2.800000000000000000e+01, 8.000000000000000167e-02
2.900000000000000000e+01, 8.999999999999999667e-02
3.000000000000000000e+01, 1.000000000000000056e-01
3.100000000000000000e+01, 1.100000000000000006e-01
3.200000000000000000e+01, 1.199999999999999956e-01
3.300000000000000000e+01, 1.300000000000000044e-01
3.400000000000000000e+01, 1.400000000000000133e-01
3.500000000000000000e+01, 1.499999999999999944e-01
3.600000000000000000e+01, 1.600000000000000033e-01
3.700000000000000000e+01, 1.700000000000000122e-01
3.800000000000000000e+01, 1.799999999999999933e-01
3.900000000000000000e+01, 1.900000000000000022e-01
4.000000000000000000e+01, 2.000000000000000111e-01
4.100000000000000000e+01, 2.099999999999999922e-01
4.200000000000000000e+01, 2.200000000000000011e-01
4.300000000000000000e+01, 2.300000000000000100e-01
4.400000000000000000e+01, 2.399999999999999911e-01
4.500000000000000000e+01, 2.500000000000000000e-01
4.600000000000000000e+01, 2.600000000000000089e-01
4.700000000000000000e+01, 2.700000000000000178e-01
4.800000000000000000e+01, 2.800000000000000266e-01
4.900000000000000000e+01, 2.899999999999999800e-01
5.000000000000000000e+01, 2.999999999999999889e-01
5.100000000000000000e+01, 3.099999999999999978e-01
5.200000000000000000e+01, 3.200000000000000067e-01
5.300000000000000000e+01, 3.300000000000000155e-01
5.400000000000000000e+01, 3.400000000000000244e-01
5.500000000000000000e+01, 3.499999999999999778e-01
5.600000000000000000e+01, 3.599999999999999867e-01
5.700000000000000000e+01, 3.699999999999999956e-01
5.800000000000000000e+01, 3.800000000000000044e-01
5.900000000000000000e+01, 3.900000000000000133e-01
6.000000000000000000e+01, 4.000000000000000222e-01
6.100000000000000000e+01, 4.099999999999999756e-01
6.200000000000000000e+01, 4.199999999999999845e-01
6.300000000000000000e+01, 4.299999999999999933e-01
6.400000000000000000e+01, 4.400000000000000022e-01
6.500000000000000000e+01, 4.500000000000000111e-01
6.600000000000000000e+01, 4.600000000000000200e-01
6.700000000000000000e+01, 4.699999999999999734e-01
6.800000000000000000e+01, 4.799999999999999822e-01
6.900000000000000000e+01, 4.899999999999999911e-01
7.000000000000000000e+01, 5.000000000000000000e-01
7.100000000000000000e+01, 5.100000000000000089e-01
7.200000000000000000e+01, 5.200000000000000178e-01
7.300000000000000000e+01, 5.300000000000000266e-01
7.400000000000000000e+01, 5.400000000000000355e-01
7.500000000000000000e+01, 5.500000000000000444e-01
7.600000000000000000e+01, 5.600000000000000533e-01
7.700000000000000000e+01, 5.699999999999999512e-01
7.800000000000000000e+01, 5.799999999999999600e-01
7.900000000000000000e+01, 5.899999999999999689e-01
8.000000000000000000e+01, 5.999999999999999778e-01
8.100000000000000000e+01, 6.099999999999999867e-01
8.200000000000000000e+01, 6.199999999999999956e-01
8.300000000000000000e+01, 6.300000000000000044e-01
8.400000000000000000e+01, 6.400000000000000133e-01
8.500000000000000000e+01, 6.500000000000000222e-01
8.600000000000000000e+01, 6.600000000000000311e-01
8.700000000000000000e+01, 6.700000000000000400e-01
8.800000000000000000e+01, 6.800000000000000488e-01
8.900000000000000000e+01, 6.899999999999999467e-01
9.000000000000000000e+01, 6.999999999999999556e-01
9.100000000000000000e+01, 7.099999999999999645e-01
9.200000000000000000e+01, 7.199999999999999734e-01
9.300000000000000000e+01, 7.299999999999999822e-01
9.400000000000000000e+01, 7.399999999999999911e-01
9.500000000000000000e+01, 7.500000000000000000e-01
9.600000000000000000e+01, 7.600000000000000089e-01
9.700000000000000000e+01, 7.700000000000000178e-01
9.800000000000000000e+01, 7.800000000000000266e-01
9.900000000000000000e+01, 7.900000000000000355e-01
1.000000000000000000e+02, 8.000000000000000444e-01
1.010000000000000000e+02, 8.100000000000000533e-01
1.020000000000000000e+02, 8.199999999999999512e-01
1.030000000000000000e+02, 8.299999999999999600e-01
1.040000000000000000e+02, 8.399999999999999689e-01
1.050000000000000000e+02, 8.499999999999999778e-01
1.060000000000000000e+02, 8.599999999999999867e-01
1.070000000000000000e+02, 8.699999999999999956e-01
1.080000000000000000e+02, 8.800000000000000044e-01
1.090000000000000000e+02, 8.900000000000000133e-01
1.100000000000000000e+02, 9.000000000000000222e-01
1.110000000000000000e+02, 9.100000000000000311e-01
1.120000000000000000e+02, 9.200000000000000400e-01
1.130000000000000000e+02, 9.300000000000000488e-01
1.140000000000000000e+02, 9.399999999999999467e-01
1.150000000000000000e+02, 9.499999999999999556e-01
1.160000000000000000e+02, 9.599999999999999645e-01
1.170000000000000000e+02, 9.699999999999999734e-01
1.180000000000000000e+02, 9.799999999999999822e-01
1.190000000000000000e+02, 9.899999999999999911e-01
1.200000000000000000e+02, 1.000000000000000000e+00
1.210000000000000000e+02, 1.010000000000000009e+00
1.220000000000000000e+02, 1.020000000000000018e+00
1.230000000000000000e+02, 1.030000000000000027e+00
1.240000000000000000e+02, 1.040000000000000036e+00
1.250000000000000000e+02, 1.050000000000000044e+00
1.260000000000000000e+02, 1.060000000000000053e+00
1.270000000000000000e+02, 1.070000000000000062e+00
1.280000000000000000e+02, 1.080000000000000071e+00
1.290000000000000000e+02, 1.090000000000000080e+00
1.300000000000000000e+02, 1.100000000000000089e+00
1.310000000000000000e+02, 1.110000000000000098e+00
1.320000000000000000e+02, 1.120000000000000107e+00
1.330000000000000000e+02, 1.129999999999999893e+00
1.340000000000000000e+02, 1.139999999999999902e+00
1.350000000000000000e+02, 1.149999999999999911e+00
1.360000000000000000e+02, 1.159999999999999920e+00
1.370000000000000000e+02, 1.169999999999999929e+00
1.380000000000000000e+02, 1.179999999999999938e+00
1.390000000000000000e+02, 1.189999999999999947e+00
1.400000000000000000e+02, 1.199999999999999956e+00
1.410000000000000000e+02, 1.209999999999999964e+00
1.420000000000000000e+02, 1.219999999999999973e+00
1.430000000000000000e+02, 1.229999999999999982e+00
1.440000000000000000e+02, 1.239999999999999991e+00
1.450000000000000000e+02, 1.250000000000000000e+00
1.460000000000000000e+02, 1.260000000000000009e+00
1.470000000000000000e+02, 1.270000000000000018e+00
1.480000000000000000e+02, 1.280000000000000027e+00
1.490000000000000000e+02, 1.290000000000000036e+00
1.500000000000000000e+02, 1.300000000000000044e+00
1.510000000000000000e+02, 1.310000000000000053e+00
1.520000000000000000e+02, 1.320000000000000062e+00
1.530000000000000000e+02, 1.330000000000000071e+00
1.540000000000000000e+02, 1.340000000000000080e+00
1.550000000000000000e+02, 1.350000000000000089e+00
1.560000000000000000e+02, 1.360000000000000098e+00
1.570000000000000000e+02, 1.370000000000000107e+00
1.580000000000000000e+02, 1.379999999999999893e+00
1.590000000000000000e+02, 1.389999999999999902e+00
1.600000000000000000e+02, 1.399999999999999911e+00
1.610000000000000000e+02, 1.409999999999999920e+00
1.620000000000000000e+02, 1.419999999999999929e+00
1.630000000000000000e+02, 1.429999999999999938e+00
1.640000000000000000e+02, 1.439999999999999947e+00
1.650000000000000000e+02, 1.449999999999999956e+00
1.660000000000000000e+02, 1.459999999999999964e+00
1.670000000000000000e+02, 1.469999999999999973e+00
1.680000000000000000e+02, 1.479999999999999982e+00
1.690000000000000000e+02, 1.489999999999999991e+00
1.700000000000000000e+02, 1.500000000000000000e+00
1.710000000000000000e+02, 1.510000000000000009e+00
1.720000000000000000e+02, 1.520000000000000018e+00
1.730000000000000000e+02, 1.530000000000000027e+00
1.740000000000000000e+02, 1.540000000000000036e+00
1.750000000000000000e+02, 1.550000000000000044e+00
1.760000000000000000e+02, 1.560000000000000053e+00
1.770000000000000000e+02, 1.570000000000000062e+00
1.780000000000000000e+02, 1.580000000000000071e+00
1.790000000000000000e+02, 1.590000000000000080e+00
1.800000000000000000e+02, 1.600000000000000089e+00
1.810000000000000000e+02, 1.610000000000000098e+00
1.820000000000000000e+02, 1.620000000000000107e+00
1.830000000000000000e+02, 1.629999999999999893e+00
1.840000000000000000e+02, 1.639999999999999902e+00
1.850000000000000000e+02, 1.649999999999999911e+00
1.860000000000000000e+02, 1.659999999999999920e+00
1.870000000000000000e+02, 1.669999999999999929e+00
1.880000000000000000e+02, 1.679999999999999938e+00
1.890000000000000000e+02, 1.689999999999999947e+00
1.900000000000000000e+02, 1.699999999999999956e+00
1.910000000000000000e+02, 1.709999999999999964e+00
1.920000000000000000e+02, 1.719999999999999973e+00
1.930000000000000000e+02, 1.729999999999999982e+00
1.940000000000000000e+02, 1.739999999999999991e+00
};

\addlegendentry{ground-truth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_high_filter.tex <==
\addplot [name path=target-velocity, color=target-velocityColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 4.000000000000000222e-01
1.000000000000000000e+00, 4.000000000000000222e-01
2.000000000000000000e+00, 4.096465259120290470e-01
3.000000000000000000e+00, 4.004859211640439676e-01
4.000000000000000000e+00, 3.979848234988722644e-01
5.000000000000000000e+00, 3.964103354974548576e-01
6.000000000000000000e+00, 3.952458537096633640e-01
7.000000000000000000e+00, 3.978584175311586923e-01
8.000000000000000000e+00, 3.958995663954071875e-01
9.000000000000000000e+00, 3.972599946022654094e-01
1.000000000000000000e+01, 3.972614756932498215e-01
1.100000000000000000e+01, 3.986717090966401256e-01
1.200000000000000000e+01, 3.980869110411040523e-01
1.300000000000000000e+01, 3.987534407947318504e-01
1.400000000000000000e+01, 3.978414664548208801e-01
1.500000000000000000e+01, 3.973218001713236247e-01
1.600000000000000000e+01, 3.978031878892201445e-01
1.700000000000000000e+01, 3.975465200012910927e-01
1.800000000000000000e+01, 3.990188368619430048e-01
1.900000000000000000e+01, 3.982263950163748012e-01
2.000000000000000000e+01, 3.982011017271399611e-01
2.100000000000000000e+01, 3.971573984190709394e-01
2.200000000000000000e+01, 3.969335020356693500e-01
2.300000000000000000e+01, 3.975902743051631383e-01
2.400000000000000000e+01, 3.980713639320325736e-01
2.500000000000000000e+01, 3.985461941915937611e-01
2.600000000000000000e+01, 3.992753669132665939e-01
2.700000000000000000e+01, 3.983631652407547685e-01
2.800000000000000000e+01, 3.976789591207153807e-01
2.900000000000000000e+01, 3.980275299432546321e-01
3.000000000000000000e+01, 3.983890742367798277e-01
3.100000000000000000e+01, 3.984177937796493651e-01
3.200000000000000000e+01, 3.991135190460427529e-01
3.300000000000000000e+01, 3.989675121595712137e-01
3.400000000000000000e+01, 3.991455114790580794e-01
3.500000000000000000e+01, 3.988834465158338505e-01
3.600000000000000000e+01, 3.982592346924699322e-01
3.700000000000000000e+01, 3.985532619789000641e-01
3.800000000000000000e+01, 3.996305925409254778e-01
3.900000000000000000e+01, 3.994996931046606026e-01
4.000000000000000000e+01, 3.983568322419012153e-01
4.100000000000000000e+01, 3.985890736526084277e-01
4.200000000000000000e+01, 3.979072519049423051e-01
4.300000000000000000e+01, 3.976987554078622589e-01
4.400000000000000000e+01, 3.981332553609510105e-01
4.500000000000000000e+01, 3.986878986282996751e-01
4.600000000000000000e+01, 3.975251903477113880e-01
4.700000000000000000e+01, 3.989860092396121938e-01
4.800000000000000000e+01, 3.988696540707948879e-01
4.900000000000000000e+01, 3.991446394633832995e-01
5.000000000000000000e+01, 3.986132113698807045e-01
5.100000000000000000e+01, 4.001885577620113432e-01
5.200000000000000000e+01, 3.992595869834637545e-01
5.300000000000000000e+01, 3.995661856607466422e-01
5.400000000000000000e+01, 3.977609405432541712e-01
5.500000000000000000e+01, 3.992323838434975181e-01
5.600000000000000000e+01, 3.981893827865133906e-01
5.700000000000000000e+01, 3.998703377515419044e-01
5.800000000000000000e+01, 3.985782800598058895e-01
5.900000000000000000e+01, 4.001139568908969046e-01
6.000000000000000000e+01, 3.983623435070973717e-01
6.100000000000000000e+01, 4.005290608586158374e-01
6.200000000000000000e+01, 3.980756719543565025e-01
6.300000000000000000e+01, 4.001144242395819894e-01
6.400000000000000000e+01, 3.975317724220319704e-01
6.500000000000000000e+01, 3.996448340116024456e-01
6.600000000000000000e+01, 3.966141463652432808e-01
6.700000000000000000e+01, 3.991194033314365841e-01
6.800000000000000000e+01, 3.972285884428595759e-01
6.900000000000000000e+01, 3.998780383259664117e-01
7.000000000000000000e+01, 3.980443840172145920e-01
7.100000000000000000e+01, 4.006353450996025245e-01
7.200000000000000000e+01, 3.984686515695831099e-01
7.300000000000000000e+01, 4.011646502582484342e-01
7.400000000000000000e+01, 3.970149253623692642e-01
7.500000000000000000e+01, 4.000312289787292253e-01
7.600000000000000000e+01, 3.964550908731536705e-01
7.700000000000000000e+01, 4.003832666196153189e-01
7.800000000000000000e+01, 3.965736637174674950e-01
7.900000000000000000e+01, 4.010395721548193348e-01
8.000000000000000000e+01, 3.973770997795901261e-01
8.100000000000000000e+01, 4.005057005444952467e-01
8.200000000000000000e+01, 3.954610667453654083e-01
8.300000000000000000e+01, 3.994115041777934749e-01
8.400000000000000000e+01, 3.952250647055547406e-01
8.500000000000000000e+01, 3.999848517765822176e-01
8.600000000000000000e+01, 3.943798627781404664e-01
8.700000000000000000e+01, 3.990818834479566979e-01
8.800000000000000000e+01, 3.948015607136516891e-01
8.900000000000000000e+01, 3.990353296704308717e-01
9.000000000000000000e+01, 3.950794252493815550e-01
9.100000000000000000e+01, 3.995540513176423225e-01
9.200000000000000000e+01, 3.950847502120951038e-01
9.300000000000000000e+01, 4.001991751674555120e-01
9.400000000000000000e+01, 3.951231685833659357e-01
9.500000000000000000e+01, 4.003185609054666916e-01
9.600000000000000000e+01, 3.935898112779735447e-01
9.700000000000000000e+01, 3.992986102489878286e-01
9.800000000000000000e+01, 3.936867394251660213e-01
9.900000000000000000e+01, 3.992573822272151851e-01
1.000000000000000000e+02, 3.941770156276571679e-01
1.010000000000000000e+02, 4.001247727986970704e-01
1.020000000000000000e+02, 3.940845785245193911e-01
1.030000000000000000e+02, 4.000473674994012852e-01
1.040000000000000000e+02, 3.940524962489239669e-01
1.050000000000000000e+02, 3.997475671797638963e-01
1.060000000000000000e+02, 3.933155450673926357e-01
1.070000000000000000e+02, 4.003184694248873021e-01
1.080000000000000000e+02, 3.927754968986907347e-01
1.090000000000000000e+02, 3.992099225950295205e-01
1.100000000000000000e+02, 3.938053323140038309e-01
1.110000000000000000e+02, 4.004131733700428963e-01
1.120000000000000000e+02, 3.944611248565835226e-01
1.130000000000000000e+02, 4.005675034845624927e-01
1.140000000000000000e+02, 3.930364908128930468e-01
1.150000000000000000e+02, 3.988185347446840945e-01
1.160000000000000000e+02, 3.922517660207632262e-01
1.170000000000000000e+02, 3.996914972136111910e-01
1.180000000000000000e+02, 3.919801270349779210e-01
1.190000000000000000e+02, 3.985272815503068111e-01
1.200000000000000000e+02, 3.926696465266329428e-01
1.210000000000000000e+02, 4.000380014040749721e-01
1.220000000000000000e+02, 3.931395887373712594e-01
1.230000000000000000e+02, 4.007914716526816967e-01
1.240000000000000000e+02, 3.921445284959212407e-01
1.250000000000000000e+02, 3.990311786119646875e-01
1.260000000000000000e+02, 3.912762138122226618e-01
1.270000000000000000e+02, 3.994499498904409140e-01
1.280000000000000000e+02, 3.919813130161838299e-01
1.290000000000000000e+02, 4.009685755658788375e-01
1.300000000000000000e+02, 3.917286742890659368e-01
1.310000000000000000e+02, 3.997785812324761712e-01
1.320000000000000000e+02, 3.911413832252860767e-01
1.330000000000000000e+02, 4.011594994290004212e-01
1.340000000000000000e+02, 3.913737818894841292e-01
1.350000000000000000e+02, 3.998960439066439054e-01
1.360000000000000000e+02, 3.909120362747331434e-01
1.370000000000000000e+02, 3.990411663297620537e-01
1.380000000000000000e+02, 3.897870513267717718e-01
1.390000000000000000e+02, 3.988404450579997595e-01
1.400000000000000000e+02, 3.898898624750783970e-01
1.410000000000000000e+02, 3.996673291849230925e-01
1.420000000000000000e+02, 3.910836383208712297e-01
1.430000000000000000e+02, 3.998145032328316306e-01
1.440000000000000000e+02, 3.907478187609318976e-01
1.450000000000000000e+02, 4.009802243096414198e-01
1.460000000000000000e+02, 3.908430672178332954e-01
1.470000000000000000e+02, 4.006072308892383305e-01
1.480000000000000000e+02, 3.909782456401365014e-01
1.490000000000000000e+02, 4.002930586568163029e-01
1.500000000000000000e+02, 3.895653287021910716e-01
1.510000000000000000e+02, 4.004926798122569465e-01
1.520000000000000000e+02, 3.891748974878711520e-01
1.530000000000000000e+02, 4.004966462344282663e-01
1.540000000000000000e+02, 3.894835773666206480e-01
1.550000000000000000e+02, 3.994152786427785373e-01
1.560000000000000000e+02, 3.888098095235383300e-01
1.570000000000000000e+02, 4.008428703583256092e-01
1.580000000000000000e+02, 3.873941925643072937e-01
1.590000000000000000e+02, 3.984173244430072036e-01
1.600000000000000000e+02, 3.886113944669831177e-01
1.610000000000000000e+02, 3.993314316234666261e-01
1.620000000000000000e+02, 3.873746499861592807e-01
1.630000000000000000e+02, 4.001883948827195114e-01
1.640000000000000000e+02, 3.883457532338190354e-01
1.650000000000000000e+02, 4.009270302554306387e-01
1.660000000000000000e+02, 3.890181634988846837e-01
1.670000000000000000e+02, 4.004574166981343941e-01
1.680000000000000000e+02, 3.880121848099881698e-01
1.690000000000000000e+02, 3.995461228025778966e-01
1.700000000000000000e+02, 3.881460667951404098e-01
1.710000000000000000e+02, 4.000764593618568732e-01
1.720000000000000000e+02, 3.871496004780700106e-01
1.730000000000000000e+02, 4.005975248261758881e-01
1.740000000000000000e+02, 3.877919696303593344e-01
1.750000000000000000e+02, 3.999886328407920022e-01
1.760000000000000000e+02, 3.877177333139047444e-01
1.770000000000000000e+02, 3.998852285421218289e-01
1.780000000000000000e+02, 3.869899770008310425e-01
1.790000000000000000e+02, 4.000043523114915622e-01
1.800000000000000000e+02, 3.867727953263801477e-01
1.810000000000000000e+02, 4.009674248195788104e-01
1.820000000000000000e+02, 3.872963664914828574e-01
1.830000000000000000e+02, 4.009651695236836622e-01
1.840000000000000000e+02, 3.867311911747167152e-01
1.850000000000000000e+02, 4.008990902714557047e-01
1.860000000000000000e+02, 3.869865109872274167e-01
1.870000000000000000e+02, 4.008714994551572652e-01
1.880000000000000000e+02, 3.870624748188825626e-01
1.890000000000000000e+02, 4.002196835477760950e-01
1.900000000000000000e+02, 3.856242106916692447e-01
1.910000000000000000e+02, 4.008523194843088833e-01
1.920000000000000000e+02, 3.846789715640079876e-01
1.930000000000000000e+02, 3.998620934482051137e-01
1.940000000000000000e+02, 3.854454952972055093e-01
1.950000000000000000e+02, 4.006377154329301971e-01
1.960000000000000000e+02, 3.847478155775264641e-01
1.970000000000000000e+02, 3.983847579758216240e-01
1.980000000000000000e+02, 3.847857241573011677e-01
1.990000000000000000e+02, 3.994637421661402232e-01
2.000000000000000000e+02, 3.852631672013647757e-01
2.010000000000000000e+02, 4.000166342873099912e-01
2.020000000000000000e+02, 3.838402884716465291e-01
2.030000000000000000e+02, 3.990514596885188503e-01
2.040000000000000000e+02, 3.839622533981613128e-01
2.050000000000000000e+02, 3.994483147510481391e-01
2.060000000000000000e+02, 3.856132313907915665e-01
2.070000000000000000e+02, 4.007791244432614142e-01
2.080000000000000000e+02, 3.840983345112206071e-01
2.090000000000000000e+02, 3.996500029924541231e-01
2.100000000000000000e+02, 3.837582601823117390e-01
2.110000000000000000e+02, 3.995843753247608765e-01
2.120000000000000000e+02, 3.836483176339272605e-01
2.130000000000000000e+02, 4.002297793527279657e-01
2.140000000000000000e+02, 3.836984205292005568e-01
2.150000000000000000e+02, 4.003258615112987306e-01
2.160000000000000000e+02, 3.837021998916587684e-01
2.170000000000000000e+02, 4.005301302207494585e-01
2.180000000000000000e+02, 3.830245558020083374e-01
2.190000000000000000e+02, 4.003170577922234852e-01
2.200000000000000000e+02, 3.830321788175778952e-01
2.210000000000000000e+02, 4.002420679958270666e-01
2.220000000000000000e+02, 3.832425852988057824e-01
2.230000000000000000e+02, 4.007065862307147008e-01
2.240000000000000000e+02, 3.826797983354127131e-01
2.250000000000000000e+02, 4.003753761108853060e-01
2.260000000000000000e+02, 3.824450187832800774e-01
2.270000000000000000e+02, 3.997621977128614779e-01
2.280000000000000000e+02, 3.829022680331877759e-01
2.290000000000000000e+02, 4.008069321631981818e-01
2.300000000000000000e+02, 3.819566344790669143e-01
2.310000000000000000e+02, 3.990213105117362824e-01
2.320000000000000000e+02, 3.818991879940571987e-01
2.330000000000000000e+02, 3.995121896781355098e-01
2.340000000000000000e+02, 3.823631312029371343e-01
2.350000000000000000e+02, 4.012081232686378618e-01
2.360000000000000000e+02, 3.818532714033794351e-01
2.370000000000000000e+02, 4.004713395856996927e-01
2.380000000000000000e+02, 3.817050434087299049e-01
2.390000000000000000e+02, 4.006795307378077098e-01
2.400000000000000000e+02, 3.807597600127243798e-01
2.410000000000000000e+02, 3.999141940123199790e-01
2.420000000000000000e+02, 3.816870707237249860e-01
2.430000000000000000e+02, 4.006909280900302628e-01
2.440000000000000000e+02, 3.813311504177712141e-01
2.450000000000000000e+02, 4.004434457008103632e-01
2.460000000000000000e+02, 3.804848371323883427e-01
2.470000000000000000e+02, 3.993667726901886095e-01
2.480000000000000000e+02, 3.805168020975352450e-01
2.490000000000000000e+02, 3.997314543520167351e-01
2.500000000000000000e+02, 3.797443243066745966e-01
2.510000000000000000e+02, 3.996246383896644438e-01
2.520000000000000000e+02, 3.804030533639974898e-01
2.530000000000000000e+02, 3.992967323723790596e-01
2.540000000000000000e+02, 3.794770199864851423e-01
2.550000000000000000e+02, 3.982012960630052500e-01
2.560000000000000000e+02, 3.793346759093242371e-01
2.570000000000000000e+02, 4.000270892482123974e-01
2.580000000000000000e+02, 3.793447457726042971e-01
2.590000000000000000e+02, 4.000647821593750209e-01
2.600000000000000000e+02, 3.793392111970843028e-01
2.610000000000000000e+02, 3.995430757074676098e-01
2.620000000000000000e+02, 3.794195552704077157e-01
2.630000000000000000e+02, 4.001377598301409932e-01
2.640000000000000000e+02, 3.796339338041380129e-01
2.650000000000000000e+02, 3.994579535306779228e-01
2.660000000000000000e+02, 3.777332147335231705e-01
2.670000000000000000e+02, 3.993671638751438158e-01
2.680000000000000000e+02, 3.783474975641370475e-01
2.690000000000000000e+02, 4.000610010189611376e-01
2.700000000000000000e+02, 3.788939574256267040e-01
2.710000000000000000e+02, 4.011444563099970662e-01
2.720000000000000000e+02, 3.788556414430678809e-01
2.730000000000000000e+02, 4.011311634903566015e-01
2.740000000000000000e+02, 3.779612974232764433e-01
2.750000000000000000e+02, 4.002856478528545314e-01
2.760000000000000000e+02, 3.770855008670919717e-01
2.770000000000000000e+02, 3.991485736786455907e-01
2.780000000000000000e+02, 3.767461747559714969e-01
2.790000000000000000e+02, 3.990735615866756181e-01
2.800000000000000000e+02, 3.770234553107851827e-01
2.810000000000000000e+02, 4.000110033837128709e-01
2.820000000000000000e+02, 3.759833998465412774e-01
2.830000000000000000e+02, 3.988511856689506696e-01
2.840000000000000000e+02, 3.757300568113307593e-01
2.850000000000000000e+02, 3.995915495285536911e-01
2.860000000000000000e+02, 3.761390577297438198e-01
2.870000000000000000e+02, 3.999813068525893689e-01
2.880000000000000000e+02, 3.764781632823571700e-01
2.890000000000000000e+02, 3.998742873604114179e-01
2.900000000000000000e+02, 3.768456188521484007e-01
2.910000000000000000e+02, 4.003190560990059765e-01
2.920000000000000000e+02, 3.767089411961694889e-01
2.930000000000000000e+02, 4.007911070313264768e-01
2.940000000000000000e+02, 3.776412567121808506e-01
2.950000000000000000e+02, 4.007759169360949336e-01
2.960000000000000000e+02, 3.768719865131613389e-01
2.970000000000000000e+02, 4.002386146925201449e-01
2.980000000000000000e+02, 3.777628540041201299e-01
2.990000000000000000e+02, 4.022095476157800942e-01
3.000000000000000000e+02, 3.752885322065522278e-01
3.010000000000000000e+02, 3.998995026926358554e-01
3.020000000000000000e+02, 3.751749143530745956e-01
3.030000000000000000e+02, 3.994438647874390957e-01
3.040000000000000000e+02, 3.751890526291519201e-01
3.050000000000000000e+02, 3.996522786515677717e-01
3.060000000000000000e+02, 3.750322800852752270e-01
3.070000000000000000e+02, 4.001789243939123386e-01
3.080000000000000000e+02, 3.748789104005507133e-01
3.090000000000000000e+02, 3.995340560738985247e-01
3.100000000000000000e+02, 3.735473681483240105e-01
3.110000000000000000e+02, 3.985599754773049286e-01
3.120000000000000000e+02, 3.738788194247484320e-01
3.130000000000000000e+02, 3.996276628899391170e-01
3.140000000000000000e+02, 3.719889333479723947e-01
3.150000000000000000e+02, 3.989241416256064099e-01
3.160000000000000000e+02, 3.722598075734864231e-01
3.170000000000000000e+02, 3.998039923563047049e-01
3.180000000000000000e+02, 3.749461488056944347e-01
3.190000000000000000e+02, 4.005336792555588277e-01
3.200000000000000000e+02, 3.752192226464148295e-01
3.210000000000000000e+02, 4.014218804869841284e-01
3.220000000000000000e+02, 3.745135878493055515e-01
3.230000000000000000e+02, 4.011229181918658515e-01
3.240000000000000000e+02, 3.739143314851650635e-01
3.250000000000000000e+02, 4.007136640559274543e-01
3.260000000000000000e+02, 3.737168699921858961e-01
3.270000000000000000e+02, 4.007779503163275692e-01
3.280000000000000000e+02, 3.725330612046795498e-01
3.290000000000000000e+02, 4.008381217996156987e-01
3.300000000000000000e+02, 3.726541102595104515e-01
3.310000000000000000e+02, 3.999369959034059230e-01
3.320000000000000000e+02, 3.724310430233181424e-01
3.330000000000000000e+02, 3.994464016222702973e-01
3.340000000000000000e+02, 3.713330427279734613e-01
3.350000000000000000e+02, 4.002058888742902054e-01
3.360000000000000000e+02, 3.726100182504152869e-01
3.370000000000000000e+02, 4.002204938643928456e-01
3.380000000000000000e+02, 3.713496522992019155e-01
3.390000000000000000e+02, 3.988956334004207793e-01
3.400000000000000000e+02, 3.709725007763751137e-01
3.410000000000000000e+02, 4.002536429006183782e-01
3.420000000000000000e+02, 3.722704014806708650e-01
3.430000000000000000e+02, 4.010854926842725154e-01
3.440000000000000000e+02, 3.719934869154669643e-01
3.450000000000000000e+02, 4.002455346086071231e-01
3.460000000000000000e+02, 3.707924027150280022e-01
3.470000000000000000e+02, 3.997024992100072227e-01
3.480000000000000000e+02, 3.705646807500789230e-01
3.490000000000000000e+02, 3.992481471086297695e-01
3.500000000000000000e+02, 3.707445247243016384e-01
3.510000000000000000e+02, 4.000064873136705557e-01
3.520000000000000000e+02, 3.713645510097488556e-01
3.530000000000000000e+02, 3.997258579759987995e-01
3.540000000000000000e+02, 3.698454819592541520e-01
3.550000000000000000e+02, 3.996114649597078960e-01
3.560000000000000000e+02, 3.694148191659453184e-01
3.570000000000000000e+02, 3.996063558067842192e-01
3.580000000000000000e+02, 3.713728396584964342e-01
3.590000000000000000e+02, 4.007799225766646156e-01
3.600000000000000000e+02, 3.706457892184391589e-01
3.610000000000000000e+02, 4.001939026385023523e-01
3.620000000000000000e+02, 3.697286545466604846e-01
3.630000000000000000e+02, 3.988006202775332687e-01
3.640000000000000000e+02, 3.691165278914931847e-01
3.650000000000000000e+02, 3.997099778083165189e-01
3.660000000000000000e+02, 3.681618194419750134e-01
3.670000000000000000e+02, 3.987001050030037907e-01
3.680000000000000000e+02, 3.673273881303883437e-01
3.690000000000000000e+02, 3.988044960410889184e-01
3.700000000000000000e+02, 3.693967890970849544e-01
3.710000000000000000e+02, 3.998450965290053505e-01
3.720000000000000000e+02, 3.681089703484478060e-01
3.730000000000000000e+02, 3.991155752680807245e-01
3.740000000000000000e+02, 3.685545122504160220e-01
3.750000000000000000e+02, 4.005026429108249908e-01
3.760000000000000000e+02, 3.695877474393060025e-01
3.770000000000000000e+02, 4.012308301095898200e-01
3.780000000000000000e+02, 3.680991767943543325e-01
3.790000000000000000e+02, 4.002916832136972358e-01
3.800000000000000000e+02, 3.684347659116699036e-01
3.810000000000000000e+02, 4.016384807763809794e-01
3.820000000000000000e+02, 3.679531668063504291e-01
3.830000000000000000e+02, 3.992816949011915861e-01
3.840000000000000000e+02, 3.668365848365894299e-01
3.850000000000000000e+02, 3.993415043345198701e-01
3.860000000000000000e+02, 3.678424701504492411e-01
3.870000000000000000e+02, 3.993199440805198508e-01
3.880000000000000000e+02, 3.693790551200925032e-01
3.890000000000000000e+02, 4.011061918897765866e-01
3.900000000000000000e+02, 3.669900468721792874e-01
3.910000000000000000e+02, 3.995749322506493284e-01
3.920000000000000000e+02, 3.665852278974688350e-01
3.930000000000000000e+02, 4.006678490706385709e-01
3.940000000000000000e+02, 3.661022822044002201e-01
};

\addlegendentry{target-velocity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=target-velocity-corrected, color=target-velocity-correctedColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 4.000000000000000222e-01
1.000000000000000000e+00, 4.000000000000000222e-01
2.000000000000000000e+00, 3.932906937243531020e-01
3.000000000000000000e+00, 3.989260881890229760e-01
4.000000000000000000e+00, 3.938217227582009317e-01
5.000000000000000000e+00, 3.954109810712709283e-01
6.000000000000000000e+00, 3.951224637761395764e-01
7.000000000000000000e+00, 3.948034659829893211e-01
8.000000000000000000e+00, 3.961558551871992018e-01
9.000000000000000000e+00, 3.965626293230756771e-01
1.000000000000000000e+01, 3.963917738370932309e-01
1.100000000000000000e+01, 3.969829668348017759e-01
1.200000000000000000e+01, 3.971635421386530140e-01
1.300000000000000000e+01, 3.970312202162068482e-01
1.400000000000000000e+01, 3.976205324983638212e-01
1.500000000000000000e+01, 3.973848360438041460e-01
1.600000000000000000e+01, 3.979904030814504501e-01
1.700000000000000000e+01, 3.978413926150303759e-01
1.800000000000000000e+01, 3.984541022146507738e-01
1.900000000000000000e+01, 3.975765894498042297e-01
2.000000000000000000e+01, 4.003645891724883499e-01
2.100000000000000000e+01, 3.981002921062399835e-01
2.200000000000000000e+01, 4.007796525590241465e-01
2.300000000000000000e+01, 3.976445107023224845e-01
2.400000000000000000e+01, 4.005870427894264729e-01
2.500000000000000000e+01, 3.991023693226708469e-01
2.600000000000000000e+01, 4.024512856455153553e-01
2.700000000000000000e+01, 3.991938412289866012e-01
2.800000000000000000e+01, 4.009724605966425992e-01
2.900000000000000000e+01, 3.980308207718514235e-01
3.000000000000000000e+01, 4.000645608104232975e-01
3.100000000000000000e+01, 3.956935524926256664e-01
3.200000000000000000e+01, 3.999501386003787018e-01
3.300000000000000000e+01, 3.970119884834559243e-01
3.400000000000000000e+01, 3.996682664496258308e-01
3.500000000000000000e+01, 3.959244652795633201e-01
3.600000000000000000e+01, 4.006531379493929457e-01
3.700000000000000000e+01, 3.977488588362925181e-01
3.800000000000000000e+01, 4.019796662194701220e-01
3.900000000000000000e+01, 3.976672394160241097e-01
4.000000000000000000e+01, 3.967390707460370924e-01
4.100000000000000000e+01, 3.936853113747830202e-01
4.200000000000000000e+01, 3.962911919692536644e-01
4.300000000000000000e+01, 3.931287922298108972e-01
4.400000000000000000e+01, 3.956739405232052587e-01
4.500000000000000000e+01, 3.959046718208993343e-01
4.600000000000000000e+01, 3.961378262155378915e-01
4.700000000000000000e+01, 3.979964311182237480e-01
4.800000000000000000e+01, 3.999837995636423837e-01
4.900000000000000000e+01, 3.984879133260991191e-01
5.000000000000000000e+01, 4.001120102590268734e-01
5.100000000000000000e+01, 3.993398166291282636e-01
5.200000000000000000e+01, 3.995028124676993087e-01
5.300000000000000000e+01, 3.996842236709821083e-01
5.400000000000000000e+01, 3.990172500178715831e-01
5.500000000000000000e+01, 3.988718855196065061e-01
5.600000000000000000e+01, 3.998063705856373939e-01
5.700000000000000000e+01, 4.004110736022925554e-01
5.800000000000000000e+01, 4.012528307048153220e-01
5.900000000000000000e+01, 4.011540961583555109e-01
6.000000000000000000e+01, 3.992140043275724803e-01
6.100000000000000000e+01, 3.994320447118677730e-01
6.200000000000000000e+01, 3.986620770059922103e-01
6.300000000000000000e+01, 3.990206777565338814e-01
6.400000000000000000e+01, 3.988758550483308962e-01
6.500000000000000000e+01, 3.990900302676668732e-01
6.600000000000000000e+01, 3.985613300567216744e-01
6.700000000000000000e+01, 3.997683579847752799e-01
6.800000000000000000e+01, 3.996922422538752295e-01
6.900000000000000000e+01, 3.967452891113660840e-01
7.000000000000000000e+01, 3.992239397205107898e-01
7.100000000000000000e+01, 3.965533131311040349e-01
7.200000000000000000e+01, 3.989346604751602410e-01
7.300000000000000000e+01, 3.962935786149151540e-01
7.400000000000000000e+01, 3.940219164200524093e-01
7.500000000000000000e+01, 3.944657703014229355e-01
7.600000000000000000e+01, 3.952886136515730842e-01
7.700000000000000000e+01, 3.935219994157234669e-01
7.800000000000000000e+01, 3.944002467110456212e-01
7.900000000000000000e+01, 3.933813540645381135e-01
8.000000000000000000e+01, 3.975163426199663785e-01
8.100000000000000000e+01, 3.933267322336223004e-01
8.200000000000000000e+01, 3.944648353651778461e-01
8.300000000000000000e+01, 3.945506475066563601e-01
8.400000000000000000e+01, 3.982384634809985613e-01
8.500000000000000000e+01, 3.943921961362222839e-01
8.600000000000000000e+01, 3.980235767285277837e-01
8.700000000000000000e+01, 3.955519397900961187e-01
8.800000000000000000e+01, 4.002414812426919322e-01
8.900000000000000000e+01, 3.971162660708131842e-01
9.000000000000000000e+01, 3.979357711651030360e-01
9.100000000000000000e+01, 3.983698585652740154e-01
9.200000000000000000e+01, 3.999259646707444826e-01
9.300000000000000000e+01, 3.959678519105601091e-01
9.400000000000000000e+01, 3.982634017125647463e-01
9.500000000000000000e+01, 3.973271875364527972e-01
9.600000000000000000e+01, 3.987008371347287028e-01
9.700000000000000000e+01, 3.951681308574624407e-01
9.800000000000000000e+01, 4.003265598472559028e-01
9.900000000000000000e+01, 3.977863587615435570e-01
1.000000000000000000e+02, 3.959047577014278563e-01
1.010000000000000000e+02, 3.947025372315446923e-01
1.020000000000000000e+02, 3.942969257992423038e-01
1.030000000000000000e+02, 3.971066580065570895e-01
1.040000000000000000e+02, 3.977518734127721833e-01
1.050000000000000000e+02, 3.973654265679136266e-01
1.060000000000000000e+02, 3.974763460620597266e-01
1.070000000000000000e+02, 3.986024726788781058e-01
1.080000000000000000e+02, 3.985533662641811414e-01
1.090000000000000000e+02, 3.984045867594606660e-01
1.100000000000000000e+02, 3.986559536385947400e-01
1.110000000000000000e+02, 4.000864365572681658e-01
1.120000000000000000e+02, 3.993565541584935263e-01
1.130000000000000000e+02, 3.997732272365478456e-01
1.140000000000000000e+02, 3.997432026262262017e-01
1.150000000000000000e+02, 4.003061110347835294e-01
1.160000000000000000e+02, 3.994742947412037171e-01
1.170000000000000000e+02, 4.014434972480520614e-01
1.180000000000000000e+02, 4.003816627795107053e-01
1.190000000000000000e+02, 4.001366680332457682e-01
1.200000000000000000e+02, 3.982325805010628050e-01
1.210000000000000000e+02, 4.005157063934314254e-01
1.220000000000000000e+02, 3.993228738271464295e-01
1.230000000000000000e+02, 4.007041550190499901e-01
1.240000000000000000e+02, 3.986472999906456871e-01
1.250000000000000000e+02, 4.002542009363873610e-01
1.260000000000000000e+02, 3.976077450079139597e-01
1.270000000000000000e+02, 4.003501059788551752e-01
1.280000000000000000e+02, 3.980625195965307728e-01
1.290000000000000000e+02, 3.989014175253595140e-01
1.300000000000000000e+02, 3.969730168984790808e-01
1.310000000000000000e+02, 3.954894934141743312e-01
1.320000000000000000e+02, 3.943337808534905786e-01
1.330000000000000000e+02, 3.907408469671245221e-01
1.340000000000000000e+02, 3.915882742009562101e-01
1.350000000000000000e+02, 3.909207302698076703e-01
1.360000000000000000e+02, 3.924257589170630500e-01
1.370000000000000000e+02, 3.951854592274822719e-01
1.380000000000000000e+02, 3.946930219599086298e-01
1.390000000000000000e+02, 3.984810559922999929e-01
1.400000000000000000e+02, 3.953641682415292014e-01
1.410000000000000000e+02, 3.959372076608254076e-01
1.420000000000000000e+02, 3.965342574888238159e-01
1.430000000000000000e+02, 3.971297148018904655e-01
1.440000000000000000e+02, 3.975367387989190426e-01
1.450000000000000000e+02, 3.982799344974303768e-01
1.460000000000000000e+02, 3.986101130631850564e-01
1.470000000000000000e+02, 4.011442897181340950e-01
1.480000000000000000e+02, 3.996085238767488890e-01
1.490000000000000000e+02, 4.003244432157155863e-01
1.500000000000000000e+02, 3.992217174494859244e-01
1.510000000000000000e+02, 4.010237954044582054e-01
1.520000000000000000e+02, 3.993110201533502934e-01
1.530000000000000000e+02, 4.005830391386416833e-01
1.540000000000000000e+02, 3.990022223406176627e-01
1.550000000000000000e+02, 4.000009826207722163e-01
1.560000000000000000e+02, 3.979434313540596846e-01
1.570000000000000000e+02, 3.987763213264861051e-01
1.580000000000000000e+02, 3.986416809782186155e-01
1.590000000000000000e+02, 3.983802845868487097e-01
1.600000000000000000e+02, 3.972770618337702064e-01
1.610000000000000000e+02, 3.980283646940136477e-01
1.620000000000000000e+02, 3.959533625099369569e-01
1.630000000000000000e+02, 3.979611296844093316e-01
1.640000000000000000e+02, 3.959014463478420787e-01
1.650000000000000000e+02, 3.973129932007302134e-01
1.660000000000000000e+02, 3.961176143378475345e-01
1.670000000000000000e+02, 3.955661025941382691e-01
1.680000000000000000e+02, 3.949721680508401223e-01
1.690000000000000000e+02, 3.960349529672996249e-01
1.700000000000000000e+02, 3.982117109758824824e-01
1.710000000000000000e+02, 3.987038759556973400e-01
1.720000000000000000e+02, 3.975486913367006769e-01
1.730000000000000000e+02, 3.996908959772457193e-01
1.740000000000000000e+02, 3.990171673287044030e-01
1.750000000000000000e+02, 3.994823359419970576e-01
1.760000000000000000e+02, 3.989256656600319584e-01
1.770000000000000000e+02, 3.982948003782462720e-01
1.780000000000000000e+02, 3.984816499043425386e-01
1.790000000000000000e+02, 4.004883383636754779e-01
1.800000000000000000e+02, 4.000564325087163087e-01
1.810000000000000000e+02, 3.983794979336668929e-01
1.820000000000000000e+02, 3.979951899673641602e-01
1.830000000000000000e+02, 3.990033862654837060e-01
1.840000000000000000e+02, 3.970430053086724809e-01
1.850000000000000000e+02, 3.982171979949124530e-01
1.860000000000000000e+02, 3.979319897617040191e-01
1.870000000000000000e+02, 3.987186445234067733e-01
1.880000000000000000e+02, 3.978204184697240464e-01
1.890000000000000000e+02, 3.980770696183124624e-01
1.900000000000000000e+02, 3.943916460126373202e-01
1.910000000000000000e+02, 3.990823449044296756e-01
1.920000000000000000e+02, 3.934700890940152629e-01
1.930000000000000000e+02, 3.926780758238915814e-01
1.940000000000000000e+02, 3.932029761368681653e-01
1.950000000000000000e+02, 3.950521445529077136e-01
1.960000000000000000e+02, 3.956781715085300188e-01
1.970000000000000000e+02, 3.972793906308488276e-01
1.980000000000000000e+02, 3.959082489662101301e-01
1.990000000000000000e+02, 3.969965897371304231e-01
2.000000000000000000e+02, 3.981579407721721475e-01
2.010000000000000000e+02, 3.981804484196045379e-01
2.020000000000000000e+02, 3.987200293731761880e-01
2.030000000000000000e+02, 3.986443159844996753e-01
2.040000000000000000e+02, 3.993705509233928530e-01
2.050000000000000000e+02, 3.994315407838696652e-01
2.060000000000000000e+02, 3.994872802521691746e-01
2.070000000000000000e+02, 4.002447679930151159e-01
2.080000000000000000e+02, 4.000477739290774215e-01
2.090000000000000000e+02, 4.016518638105499583e-01
2.100000000000000000e+02, 3.998581861015561012e-01
2.110000000000000000e+02, 4.022664739093047559e-01
2.120000000000000000e+02, 4.012238159518158875e-01
2.130000000000000000e+02, 4.019215101546278479e-01
2.140000000000000000e+02, 3.998831597278949546e-01
2.150000000000000000e+02, 4.011565809320519205e-01
2.160000000000000000e+02, 4.002006025318464166e-01
2.170000000000000000e+02, 4.014238232423026354e-01
2.180000000000000000e+02, 4.000276703216293361e-01
2.190000000000000000e+02, 4.003675007830818089e-01
2.200000000000000000e+02, 3.982526715610692492e-01
2.210000000000000000e+02, 3.994601619005399007e-01
2.220000000000000000e+02, 3.943922240043891692e-01
2.230000000000000000e+02, 3.975283948338269591e-01
2.240000000000000000e+02, 3.939948630965679488e-01
2.250000000000000000e+02, 3.939443293001813062e-01
2.260000000000000000e+02, 3.926278356460851104e-01
2.270000000000000000e+02, 3.937893394162370608e-01
2.280000000000000000e+02, 3.926667703954482280e-01
2.290000000000000000e+02, 3.973187749704917282e-01
2.300000000000000000e+02, 3.939056046492775964e-01
2.310000000000000000e+02, 3.988940017777894975e-01
2.320000000000000000e+02, 3.940012538548720578e-01
2.330000000000000000e+02, 3.994147668879944879e-01
2.340000000000000000e+02, 3.958886312612919789e-01
2.350000000000000000e+02, 4.024218751810614836e-01
2.360000000000000000e+02, 3.980708686579728095e-01
2.370000000000000000e+02, 4.014274645364572791e-01
2.380000000000000000e+02, 3.983776202929860677e-01
2.390000000000000000e+02, 4.033365390980242493e-01
2.400000000000000000e+02, 3.982575798236759335e-01
2.410000000000000000e+02, 4.033580157815578326e-01
2.420000000000000000e+02, 3.986984123539153990e-01
2.430000000000000000e+02, 4.027561507234790339e-01
2.440000000000000000e+02, 3.978623264427820772e-01
2.450000000000000000e+02, 4.029169614292498758e-01
2.460000000000000000e+02, 3.983698210355650082e-01
2.470000000000000000e+02, 4.042376514342526650e-01
2.480000000000000000e+02, 3.977628683190008729e-01
2.490000000000000000e+02, 4.034691245844588270e-01
2.500000000000000000e+02, 3.983287025780748447e-01
2.510000000000000000e+02, 3.986384320872613518e-01
2.520000000000000000e+02, 3.932230631041705449e-01
2.530000000000000000e+02, 3.961245339248879449e-01
2.540000000000000000e+02, 3.916272846839650712e-01
2.550000000000000000e+02, 3.941934651956003899e-01
2.560000000000000000e+02, 3.938327881886584114e-01
2.570000000000000000e+02, 3.949816518099907858e-01
2.580000000000000000e+02, 3.961354592303680811e-01
2.590000000000000000e+02, 3.993515447593463108e-01
2.600000000000000000e+02, 3.996464681080035830e-01
2.610000000000000000e+02, 3.987577445652119579e-01
2.620000000000000000e+02, 3.994488244022339485e-01
2.630000000000000000e+02, 3.983393149288291801e-01
2.640000000000000000e+02, 4.001433780999119616e-01
2.650000000000000000e+02, 3.994891833611929899e-01
2.660000000000000000e+02, 3.996272431817653459e-01
2.670000000000000000e+02, 3.984068995076165409e-01
2.680000000000000000e+02, 4.000382340002227033e-01
2.690000000000000000e+02, 3.983021174583913915e-01
2.700000000000000000e+02, 3.996762382096369914e-01
2.710000000000000000e+02, 3.991404466249782734e-01
2.720000000000000000e+02, 4.018311555563837123e-01
2.730000000000000000e+02, 3.984284791714375884e-01
2.740000000000000000e+02, 3.993639715815081592e-01
2.750000000000000000e+02, 3.978434089964877352e-01
2.760000000000000000e+02, 3.992944407492851622e-01
2.770000000000000000e+02, 3.974595269973206779e-01
2.780000000000000000e+02, 3.987306216736434261e-01
2.790000000000000000e+02, 3.994750942172726749e-01
2.800000000000000000e+02, 3.987777738049944065e-01
2.810000000000000000e+02, 3.980874046707095770e-01
2.820000000000000000e+02, 3.935278848317149691e-01
2.830000000000000000e+02, 3.945944853036255640e-01
2.840000000000000000e+02, 3.870227387061095925e-01
2.850000000000000000e+02, 3.929653759133259205e-01
2.860000000000000000e+02, 3.910735055732162402e-01
2.870000000000000000e+02, 3.920704665315265514e-01
2.880000000000000000e+02, 3.947082632705562477e-01
2.890000000000000000e+02, 3.958506992567545346e-01
2.900000000000000000e+02, 3.986593992487993399e-01
2.910000000000000000e+02, 4.008266942036148306e-01
2.920000000000000000e+02, 3.985276929131185142e-01
2.930000000000000000e+02, 4.002259238524099039e-01
2.940000000000000000e+02, 3.993518485362251846e-01
2.950000000000000000e+02, 4.015239347733228215e-01
2.960000000000000000e+02, 3.996892727833131764e-01
2.970000000000000000e+02, 3.998931492794032261e-01
2.980000000000000000e+02, 4.005578806688437910e-01
2.990000000000000000e+02, 4.001125690118298994e-01
3.000000000000000000e+02, 4.016855555676470679e-01
3.010000000000000000e+02, 4.016035895252627608e-01
3.020000000000000000e+02, 4.004102184425195055e-01
3.030000000000000000e+02, 4.015808385504089917e-01
3.040000000000000000e+02, 3.999868625039187386e-01
3.050000000000000000e+02, 3.995907584291950587e-01
3.060000000000000000e+02, 3.977881053980913406e-01
3.070000000000000000e+02, 3.967815755770406350e-01
3.080000000000000000e+02, 3.989973870507502185e-01
3.090000000000000000e+02, 3.977524673795469479e-01
3.100000000000000000e+02, 3.996105737544325964e-01
3.110000000000000000e+02, 3.971811960051268575e-01
3.120000000000000000e+02, 3.964934757518691621e-01
3.130000000000000000e+02, 3.963053244987767010e-01
3.140000000000000000e+02, 3.965192895259038730e-01
3.150000000000000000e+02, 3.962697900587137112e-01
3.160000000000000000e+02, 3.953706739071437548e-01
3.170000000000000000e+02, 3.965024148734555554e-01
3.180000000000000000e+02, 3.953450121549854090e-01
3.190000000000000000e+02, 3.956823184129552029e-01
3.200000000000000000e+02, 3.959067321377638393e-01
3.210000000000000000e+02, 3.965427300567586077e-01
3.220000000000000000e+02, 3.978006848930770722e-01
3.230000000000000000e+02, 3.964063421773770246e-01
3.240000000000000000e+02, 3.969978698174109200e-01
3.250000000000000000e+02, 3.957817704445129592e-01
3.260000000000000000e+02, 3.987177335666057809e-01
3.270000000000000000e+02, 3.963093615500382638e-01
3.280000000000000000e+02, 3.977894043925797041e-01
3.290000000000000000e+02, 3.989124908379590995e-01
3.300000000000000000e+02, 4.025023870528870451e-01
3.310000000000000000e+02, 4.000634836576781872e-01
3.320000000000000000e+02, 3.998293043269513514e-01
3.330000000000000000e+02, 3.986492503350865801e-01
3.340000000000000000e+02, 3.992000530229991573e-01
3.350000000000000000e+02, 3.988631280225379272e-01
3.360000000000000000e+02, 3.983572384141567668e-01
3.370000000000000000e+02, 3.975837031342375205e-01
3.380000000000000000e+02, 3.979603128990112371e-01
3.390000000000000000e+02, 3.974217174242056227e-01
3.400000000000000000e+02, 3.970295679700336366e-01
3.410000000000000000e+02, 3.949848431042535246e-01
3.420000000000000000e+02, 3.958450587118824693e-01
3.430000000000000000e+02, 3.941749834636246730e-01
3.440000000000000000e+02, 3.908538304796355112e-01
3.450000000000000000e+02, 3.907099115747556528e-01
3.460000000000000000e+02, 3.902526620183024431e-01
3.470000000000000000e+02, 3.921173826715039779e-01
3.480000000000000000e+02, 3.960240116057911486e-01
3.490000000000000000e+02, 3.962225746655136938e-01
3.500000000000000000e+02, 3.972335952822931282e-01
3.510000000000000000e+02, 3.981250953687753835e-01
3.520000000000000000e+02, 4.011308673885466414e-01
3.530000000000000000e+02, 4.030827208886672564e-01
3.540000000000000000e+02, 4.032079142768478786e-01
3.550000000000000000e+02, 4.025282510138423753e-01
3.560000000000000000e+02, 4.026806610792296182e-01
3.570000000000000000e+02, 4.007308695183593450e-01
3.580000000000000000e+02, 4.003168748761092854e-01
3.590000000000000000e+02, 3.989699943663475024e-01
3.600000000000000000e+02, 4.006406796177855445e-01
3.610000000000000000e+02, 3.990380019310242887e-01
3.620000000000000000e+02, 4.006185378335168634e-01
3.630000000000000000e+02, 3.997850579587051700e-01
3.640000000000000000e+02, 3.998700399918465598e-01
3.650000000000000000e+02, 3.996635523658707001e-01
3.660000000000000000e+02, 3.996695011738914394e-01
3.670000000000000000e+02, 3.983809609466700818e-01
3.680000000000000000e+02, 4.006624089301330516e-01
3.690000000000000000e+02, 3.981179467384167170e-01
3.700000000000000000e+02, 3.998856271782800231e-01
3.710000000000000000e+02, 3.979720192772084331e-01
3.720000000000000000e+02, 3.968623691448872615e-01
3.730000000000000000e+02, 3.945770097740902149e-01
3.740000000000000000e+02, 3.937816784355246402e-01
3.750000000000000000e+02, 3.915657598290547270e-01
3.760000000000000000e+02, 3.930519050721307250e-01
3.770000000000000000e+02, 3.926279382663450668e-01
3.780000000000000000e+02, 3.917031655022831238e-01
3.790000000000000000e+02, 3.931981758715565878e-01
3.800000000000000000e+02, 3.959051673089702961e-01
3.810000000000000000e+02, 3.955687580519050561e-01
3.820000000000000000e+02, 3.968334215876017090e-01
3.830000000000000000e+02, 3.958675518116699932e-01
3.840000000000000000e+02, 3.984669773041434881e-01
3.850000000000000000e+02, 3.961742832571156780e-01
3.860000000000000000e+02, 3.990356494707883450e-01
3.870000000000000000e+02, 3.987537727172214552e-01
3.880000000000000000e+02, 4.000193376335425266e-01
3.890000000000000000e+02, 3.980089963922359142e-01
3.900000000000000000e+02, 3.996633484507550182e-01
3.910000000000000000e+02, 3.989645032766909738e-01
3.920000000000000000e+02, 4.022481507875076412e-01
3.930000000000000000e+02, 3.994935819070777328e-01
3.940000000000000000e+02, 4.009084137752545463e-01
};

\addlegendentry{target-velocity-corrected}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_high_rotation.tex <==
\addplot [name path=sensor-rotation-0, color=sensor-rotation-0Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 1.801984159943017388e-02
1.000000000000000000e+00, 3.484002925193364908e-02
2.000000000000000000e+00, 5.034865938582330780e-02
3.000000000000000000e+00, 1.398651931816349836e-01
4.000000000000000000e+00, 1.820507283309026614e-01
5.000000000000000000e+00, 2.374945458459068182e-01
6.000000000000000000e+00, 2.808804271464074853e-01
7.000000000000000000e+00, 3.156551543341772348e-01
8.000000000000000000e+00, 2.600363461256194331e-01
9.000000000000000000e+00, 2.314364276224344652e-01
1.000000000000000000e+01, 1.724168966393027913e-01
1.100000000000000000e+01, 7.625464616709286270e-02
1.200000000000000000e+01, 1.035837224422519465e-01
1.300000000000000000e+01, 5.848197012905840403e-02
1.400000000000000000e+01, 5.041845280993853540e-02
1.500000000000000000e+01, 4.629566160765998667e-02
1.600000000000000000e+01, 4.536554655559930926e-02
1.700000000000000000e+01, 6.944250683819909453e-02
1.800000000000000000e+01, 9.312061635509814861e-02
1.900000000000000000e+01, 1.024586764134284705e-01
2.000000000000000000e+01, 1.810835112440792039e-01
2.100000000000000000e+01, 3.646356694841197954e-01
2.200000000000000000e+01, 7.542603185510015074e-01
2.300000000000000000e+01, 5.913314488712326789e-01
2.400000000000000000e+01, 2.924605624127061820e-01
2.500000000000000000e+01, 1.013046910147015339e-01
2.600000000000000000e+01, 8.474396278507716207e-02
2.700000000000000000e+01, 3.018078877686291780e-02
2.800000000000000000e+01, 5.880917209942005536e-02
2.900000000000000000e+01, 3.667680481820300570e-02
3.000000000000000000e+01, 3.808789736255961678e-02
3.100000000000000000e+01, 5.559846771958557032e-02
3.200000000000000000e+01, 8.951813047004805735e-02
3.300000000000000000e+01, 1.234738989803717546e-01
3.400000000000000000e+01, 1.498189428369220977e-01
3.500000000000000000e+01, 1.623708938991884898e-01
3.600000000000000000e+01, 2.042174673633696258e-01
3.700000000000000000e+01, 2.551879081014014061e-01
3.800000000000000000e+01, 2.704585760012651052e-01
3.900000000000000000e+01, 2.030980999125722442e-01
4.000000000000000000e+01, 1.248857898549631529e-01
4.100000000000000000e+01, 1.471617588611255911e-01
4.200000000000000000e+01, 9.258990711234406368e-02
4.300000000000000000e+01, 4.806472060214837805e-02
4.400000000000000000e+01, 4.165855015898006775e-02
4.500000000000000000e+01, 3.381936216829665998e-02
4.600000000000000000e+01, 4.000153382857983553e-02
4.700000000000000000e+01, 5.113590614024655923e-02
4.800000000000000000e+01, 5.672779511870629232e-02
4.900000000000000000e+01, 1.101365320873675668e-01
5.000000000000000000e+01, 1.785680362604861182e-01
5.100000000000000000e+01, 4.615464073824243063e-01
5.200000000000000000e+01, 7.905651521068762788e-01
5.300000000000000000e+01, 5.337408661307018187e-01
5.400000000000000000e+01, 2.287410247272393671e-01
5.500000000000000000e+01, 1.149962583723097287e-01
5.600000000000000000e+01, 5.430802630089892613e-02
5.700000000000000000e+01, 7.575978018497984967e-02
5.800000000000000000e+01, 7.689624142450932065e-02
5.900000000000000000e+01, 6.786418220680270896e-02
6.000000000000000000e+01, 4.912831861897252322e-02
6.100000000000000000e+01, 7.150548398793300786e-02
6.200000000000000000e+01, 7.274601305059737177e-02
6.300000000000000000e+01, 9.877348221153529895e-02
6.400000000000000000e+01, 1.734118714774701697e-01
6.500000000000000000e+01, 1.613993616912183515e-01
6.600000000000000000e+01, 2.264424970096882428e-01
6.700000000000000000e+01, 2.963903705779372677e-01
6.800000000000000000e+01, 3.341423826001519992e-01
6.900000000000000000e+01, 2.655444052091607277e-01
7.000000000000000000e+01, 1.923346474672569806e-01
7.100000000000000000e+01, 1.300486720247589489e-01
7.200000000000000000e+01, 1.250247820151282330e-01
7.300000000000000000e+01, 3.895363108382608047e-02
7.400000000000000000e+01, 3.109222792638957622e-02
7.500000000000000000e+01, 4.498748999041650432e-02
7.600000000000000000e+01, 4.898790520350588401e-02
7.700000000000000000e+01, 6.443923861160552602e-02
7.800000000000000000e+01, 1.194838462962458381e-01
7.900000000000000000e+01, 1.390898510912297603e-01
8.000000000000000000e+01, 2.299909109839618493e-01
8.100000000000000000e+01, 2.649970178945490473e-01
8.200000000000000000e+01, 3.134850834657788021e-01
8.300000000000000000e+01, 2.803133452953889271e-01
8.400000000000000000e+01, 2.185100873670997590e-01
8.500000000000000000e+01, 1.603059191520304627e-01
8.600000000000000000e+01, 1.377492271380013900e-01
8.700000000000000000e+01, 7.151646910332538909e-02
8.800000000000000000e+01, 6.523173138286811334e-02
8.900000000000000000e+01, 4.031701687878712359e-02
9.000000000000000000e+01, 7.243009987687991369e-02
9.100000000000000000e+01, 5.229612728811565414e-02
9.200000000000000000e+01, 5.443538543568136184e-02
9.300000000000000000e+01, 3.501267225360893409e-02
9.400000000000000000e+01, 9.700508489964780601e-02
9.500000000000000000e+01, 1.470869595000620089e-01
9.600000000000000000e+01, 2.892173628276477060e-01
9.700000000000000000e+01, 6.580327331659033829e-01
9.800000000000000000e+01, 7.454162802084355333e-01
9.900000000000000000e+01, 4.023561762227453875e-01
1.000000000000000000e+02, 1.559728252613459820e-01
1.010000000000000000e+02, 6.512074291118243041e-02
1.020000000000000000e+02, 6.598798413119184858e-02
1.030000000000000000e+02, 2.717825814651332259e-02
1.040000000000000000e+02, 2.264393399896565129e-02
1.050000000000000000e+02, 1.704523641641848830e-02
1.060000000000000000e+02, 2.256599018204808599e-02
1.070000000000000000e+02, 4.755085964554309208e-02
1.080000000000000000e+02, 8.017560323806001421e-02
1.090000000000000000e+02, 1.468110325752635670e-01
1.100000000000000000e+02, 1.778103080944624381e-01
1.110000000000000000e+02, 2.270112176589429431e-01
1.120000000000000000e+02, 2.705332651658332033e-01
1.130000000000000000e+02, 2.324539318656621834e-01
1.140000000000000000e+02, 1.970719154615294400e-01
1.150000000000000000e+02, 1.778552289787736218e-01
1.160000000000000000e+02, 1.568773316640547089e-01
1.170000000000000000e+02, 9.105774329070907835e-02
1.180000000000000000e+02, 7.992199035450786582e-02
1.190000000000000000e+02, 4.328467084423219535e-02
1.200000000000000000e+02, 1.149482509263426676e-02
1.210000000000000000e+02, 2.065042355439981187e-02
1.220000000000000000e+02, 1.616688511229257691e-02
1.230000000000000000e+02, 6.070806917295166333e-02
1.240000000000000000e+02, 5.733595745204967536e-02
1.250000000000000000e+02, 1.581326188000192479e-01
1.260000000000000000e+02, 3.292738209710122654e-01
1.270000000000000000e+02, 7.348112726944169282e-01
1.280000000000000000e+02, 6.936690229058666279e-01
1.290000000000000000e+02, 3.174385639328458630e-01
1.300000000000000000e+02, 1.514783787974912366e-01
1.310000000000000000e+02, 1.130300530205829712e-01
1.320000000000000000e+02, 6.821725636177233820e-02
1.330000000000000000e+02, 5.022687317932881396e-02
1.340000000000000000e+02, 6.750148704675702771e-02
1.350000000000000000e+02, 8.413803383323484320e-02
1.360000000000000000e+02, 7.274074826930895799e-02
1.370000000000000000e+02, 5.596836712859799834e-02
1.380000000000000000e+02, 7.279556489258176555e-02
1.390000000000000000e+02, 1.105014482891280153e-01
1.400000000000000000e+02, 1.431851199608173975e-01
1.410000000000000000e+02, 2.295046530956600939e-01
1.420000000000000000e+02, 2.627111727630835336e-01
1.430000000000000000e+02, 3.291737657386439864e-01
1.440000000000000000e+02, 3.231264925418596001e-01
1.450000000000000000e+02, 1.808475303643686805e-01
1.460000000000000000e+02, 1.369874058312886000e-01
1.470000000000000000e+02, 1.141468823159665635e-01
1.480000000000000000e+02, 5.878729880564158294e-02
1.490000000000000000e+02, 4.649700560050213510e-02
1.500000000000000000e+02, 3.305529841005477865e-02
1.510000000000000000e+02, 2.676156899485750140e-02
1.520000000000000000e+02, 4.616382583635345732e-02
1.530000000000000000e+02, 6.205990137083620961e-02
1.540000000000000000e+02, 1.216997323466233738e-01
1.550000000000000000e+02, 1.804244930350140108e-01
1.560000000000000000e+02, 2.651555907287748148e-01
1.570000000000000000e+02, 3.233510901723137265e-01
1.580000000000000000e+02, 2.997241032991726506e-01
1.590000000000000000e+02, 2.608876980868285456e-01
1.600000000000000000e+02, 1.981181527202556802e-01
1.610000000000000000e+02, 1.774235777956852389e-01
1.620000000000000000e+02, 1.254256105372610897e-01
1.630000000000000000e+02, 7.702802073758732715e-02
1.640000000000000000e+02, 9.601634366668013176e-02
1.650000000000000000e+02, 7.792075918536119084e-02
1.660000000000000000e+02, 3.476959559231868058e-02
1.670000000000000000e+02, 5.029943404577374988e-02
1.680000000000000000e+02, 3.947959791530614854e-02
1.690000000000000000e+02, 6.346059157974058562e-02
1.700000000000000000e+02, 1.359433023950173680e-01
1.710000000000000000e+02, 2.101949897834420877e-01
1.720000000000000000e+02, 4.942416454176814522e-01
1.730000000000000000e+02, 7.822964502805225262e-01
1.740000000000000000e+02, 5.110428936388405896e-01
1.750000000000000000e+02, 2.369980497538173025e-01
1.760000000000000000e+02, 1.001788939039031934e-01
1.770000000000000000e+02, 7.017249729343220943e-02
1.780000000000000000e+02, 2.246064739504250937e-02
1.790000000000000000e+02, 2.369950343437743009e-02
1.800000000000000000e+02, 4.038983069494420791e-02
1.810000000000000000e+02, 2.920601444409164776e-02
1.820000000000000000e+02, 8.188341597357656765e-02
1.830000000000000000e+02, 1.119170429918101700e-01
1.840000000000000000e+02, 9.146829891453997496e-02
1.850000000000000000e+02, 1.500352867982480409e-01
1.860000000000000000e+02, 1.925507784632883856e-01
1.870000000000000000e+02, 2.736922873451968496e-01
1.880000000000000000e+02, 2.474088133245607446e-01
1.890000000000000000e+02, 2.329139977906895254e-01
1.900000000000000000e+02, 1.584016435841948678e-01
1.910000000000000000e+02, 1.538243866946975569e-01
1.920000000000000000e+02, 1.259262578759650919e-01
1.930000000000000000e+02, 1.021112238709493414e-01
1.940000000000000000e+02, 6.833310513647485041e-02
};

\addlegendentry{sensor-rotation-0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=sensor-rotation-1, color=sensor-rotation-1Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 4.016279478182699370e-02
1.000000000000000000e+00, 2.961434379032307565e-02
2.000000000000000000e+00, 7.783247635146199606e-02
3.000000000000000000e+00, 9.085059940676526447e-02
4.000000000000000000e+00, 1.746605267658171423e-01
5.000000000000000000e+00, 2.538355424264026050e-01
6.000000000000000000e+00, 3.050553878840000510e-01
7.000000000000000000e+00, 3.160829074926807536e-01
8.000000000000000000e+00, 2.846930879181086005e-01
9.000000000000000000e+00, 2.132049416792590746e-01
1.000000000000000000e+01, 1.338569845828895544e-01
1.100000000000000000e+01, 1.039071747831661202e-01
1.200000000000000000e+01, 1.075343358643176955e-01
1.300000000000000000e+01, 6.207407702100441182e-02
1.400000000000000000e+01, 6.740076955437630801e-02
1.500000000000000000e+01, 4.421273824777140898e-02
1.600000000000000000e+01, 3.819758881859160876e-02
1.700000000000000000e+01, 9.234739261239040264e-02
1.800000000000000000e+01, 9.390294212257895012e-02
1.900000000000000000e+01, 7.930109877813379393e-02
2.000000000000000000e+01, 2.195175650346772867e-01
2.100000000000000000e+01, 4.059207240437426867e-01
2.200000000000000000e+01, 7.609482952554981194e-01
2.300000000000000000e+01, 6.002307379628301076e-01
2.400000000000000000e+01, 2.659629173231903843e-01
2.500000000000000000e+01, 9.450310480226035981e-02
2.600000000000000000e+01, 6.593465439596490896e-02
2.700000000000000000e+01, 4.080594704399206907e-02
2.800000000000000000e+01, 1.161578468573690182e-02
2.900000000000000000e+01, 1.374354756686291257e-02
3.000000000000000000e+01, 2.638346216092808671e-02
3.100000000000000000e+01, 2.460321552870523704e-02
3.200000000000000000e+01, 7.716591827699213757e-02
3.300000000000000000e+01, 1.100438036261774249e-01
3.400000000000000000e+01, 1.569659159901387047e-01
3.500000000000000000e+01, 1.725918447659401112e-01
3.600000000000000000e+01, 2.608281960285039891e-01
3.700000000000000000e+01, 2.326836911446535650e-01
3.800000000000000000e+01, 2.499773326283434294e-01
3.900000000000000000e+01, 2.032714314661265009e-01
4.000000000000000000e+01, 1.541025727694248226e-01
4.100000000000000000e+01, 1.010270818879040883e-01
4.200000000000000000e+01, 8.930720502790603921e-02
4.300000000000000000e+01, 8.880700123924496758e-02
4.400000000000000000e+01, 3.393673313344570952e-02
4.500000000000000000e+01, 3.633048378745621504e-02
4.600000000000000000e+01, 1.265782937537670086e-02
4.700000000000000000e+01, 2.721730661920160679e-02
4.800000000000000000e+01, 6.687811904251569906e-02
4.900000000000000000e+01, 1.006626187025186220e-01
5.000000000000000000e+01, 2.993188008445527015e-01
5.100000000000000000e+01, 5.750203912238733839e-01
5.200000000000000000e+01, 7.707237695763753393e-01
5.300000000000000000e+01, 4.261342419386172087e-01
5.400000000000000000e+01, 1.279917537450067089e-01
5.500000000000000000e+01, 1.235598996423529911e-01
5.600000000000000000e+01, 5.047772747842631247e-02
5.700000000000000000e+01, 7.637479982618972096e-02
5.800000000000000000e+01, 5.469630651685154082e-02
5.900000000000000000e+01, 4.011579793134086719e-02
6.000000000000000000e+01, 4.756730493858020437e-02
6.100000000000000000e+01, 5.767134325026247732e-02
6.200000000000000000e+01, 1.188195280411151883e-01
6.300000000000000000e+01, 1.203950498332199137e-01
6.400000000000000000e+01, 1.293781924621712487e-01
6.500000000000000000e+01, 2.215656815191842932e-01
6.600000000000000000e+01, 2.593379701782571045e-01
6.700000000000000000e+01, 3.204631821453098328e-01
6.800000000000000000e+01, 3.104442042153439663e-01
6.900000000000000000e+01, 2.523431008464659397e-01
7.000000000000000000e+01, 1.552700331510897258e-01
7.100000000000000000e+01, 1.090542917055543903e-01
7.200000000000000000e+01, 6.875608811676714449e-02
7.300000000000000000e+01, 6.587268130821755108e-02
7.400000000000000000e+01, 5.084094229551227445e-02
7.500000000000000000e+01, 6.449522729898277129e-02
7.600000000000000000e+01, 4.067317675489837830e-02
7.700000000000000000e+01, 8.094069019439975587e-02
7.800000000000000000e+01, 1.356747817395476396e-01
7.900000000000000000e+01, 2.002799456239969522e-01
8.000000000000000000e+01, 2.626487872597772499e-01
8.100000000000000000e+01, 2.997941548448292415e-01
8.200000000000000000e+01, 3.290095648809620577e-01
8.300000000000000000e+01, 2.411240149598209981e-01
8.400000000000000000e+01, 1.656282136008811745e-01
8.500000000000000000e+01, 1.724791592737742463e-01
8.600000000000000000e+01, 7.006001026514413477e-02
8.700000000000000000e+01, 7.192889187860349032e-02
8.800000000000000000e+01, 5.130275796380837083e-02
8.900000000000000000e+01, 7.995093418995879997e-02
9.000000000000000000e+01, 4.113859194030398958e-02
9.100000000000000000e+01, 6.744624715701923179e-02
9.200000000000000000e+01, 9.835936145082829762e-02
9.300000000000000000e+01, 7.429393692397529003e-02
9.400000000000000000e+01, 1.637190509875570965e-01
9.500000000000000000e+01, 2.332942899476761756e-01
9.600000000000000000e+01, 5.580446233547279311e-01
9.700000000000000000e+01, 7.713696040302649992e-01
9.800000000000000000e+01, 4.452464843426015007e-01
9.900000000000000000e+01, 2.108719655386919745e-01
1.000000000000000000e+02, 9.694696845024750043e-02
1.010000000000000000e+02, 2.625694500945175563e-02
1.020000000000000000e+02, 2.644157801035960931e-02
1.030000000000000000e+02, 2.461125817352721040e-02
1.040000000000000000e+02, 2.448147010922746211e-02
1.050000000000000000e+02, 3.851717433502097748e-02
1.060000000000000000e+02, 8.367743410712225050e-02
1.070000000000000000e+02, 7.165548548204825341e-02
1.080000000000000000e+02, 1.487721187815658208e-01
1.090000000000000000e+02, 1.884843833696535909e-01
1.100000000000000000e+02, 1.787192853771300827e-01
1.110000000000000000e+02, 2.371944993400931512e-01
1.120000000000000000e+02, 2.500423508104560599e-01
1.130000000000000000e+02, 2.232375709489652638e-01
1.140000000000000000e+02, 1.706887295418394457e-01
1.150000000000000000e+02, 1.303998618068512028e-01
1.160000000000000000e+02, 1.467481650680411420e-01
1.170000000000000000e+02, 3.232184835460181344e-02
1.180000000000000000e+02, 5.634532165163754630e-02
1.190000000000000000e+02, 2.809150171423503706e-02
1.200000000000000000e+02, 8.646990559394308884e-03
1.210000000000000000e+02, 2.943758338339748371e-02
1.220000000000000000e+02, 2.864660552816985714e-02
1.230000000000000000e+02, 7.682829063706309025e-02
1.240000000000000000e+02, 1.595217503870064168e-01
1.250000000000000000e+02, 3.712929705062177899e-01
1.260000000000000000e+02, 7.413990918461048629e-01
1.270000000000000000e+02, 6.626442550236535389e-01
1.280000000000000000e+02, 2.876765268955767674e-01
1.290000000000000000e+02, 1.733583702839056051e-01
1.300000000000000000e+02, 6.341519100679526844e-02
1.310000000000000000e+02, 7.071408765395208185e-02
1.320000000000000000e+02, 7.161484060689168873e-02
1.330000000000000000e+02, 6.297583126024426659e-02
1.340000000000000000e+02, 3.968317550400912025e-02
1.350000000000000000e+02, 7.098064955930909192e-02
1.360000000000000000e+02, 7.985075947634263926e-02
1.370000000000000000e+02, 1.200339308716208142e-01
1.380000000000000000e+02, 1.443859742501127363e-01
1.390000000000000000e+02, 1.601664655037497165e-01
1.400000000000000000e+02, 2.333348837582931157e-01
1.410000000000000000e+02, 2.647953265482675400e-01
1.420000000000000000e+02, 2.952629235146800868e-01
1.430000000000000000e+02, 2.470374619839956210e-01
1.440000000000000000e+02, 1.771869219461767175e-01
1.450000000000000000e+02, 1.401735971203149078e-01
1.460000000000000000e+02, 1.116423414687108956e-01
1.470000000000000000e+02, 2.430555549855912059e-02
1.480000000000000000e+02, 1.656354493358741520e-02
1.490000000000000000e+02, 2.232723517872350905e-02
1.500000000000000000e+02, 3.332783807888071298e-02
1.510000000000000000e+02, 4.004575301791461067e-02
1.520000000000000000e+02, 1.206742430847562997e-01
1.530000000000000000e+02, 1.395371538157617053e-01
1.540000000000000000e+02, 1.733747046779357259e-01
1.550000000000000000e+02, 2.655763655447535010e-01
1.560000000000000000e+02, 3.090196487020354099e-01
1.570000000000000000e+02, 2.963010303494290065e-01
1.580000000000000000e+02, 2.390540008852602705e-01
1.590000000000000000e+02, 2.070441176896586355e-01
1.600000000000000000e+02, 1.288091196188157206e-01
1.610000000000000000e+02, 1.055575603100813026e-01
1.620000000000000000e+02, 1.139515177782688543e-01
1.630000000000000000e+02, 1.023017903551456526e-01
1.640000000000000000e+02, 4.550698181606167153e-02
1.650000000000000000e+02, 4.959331925711853856e-02
1.660000000000000000e+02, 3.088709813417488473e-02
1.670000000000000000e+02, 3.808941954785149270e-02
1.680000000000000000e+02, 9.570595873504002260e-02
1.690000000000000000e+02, 1.380262801829995334e-01
1.700000000000000000e+02, 3.487222816988035379e-01
1.710000000000000000e+02, 6.842952972536999745e-01
1.720000000000000000e+02, 7.092642459565597912e-01
1.730000000000000000e+02, 3.293106544080057208e-01
1.740000000000000000e+02, 1.469016674940455125e-01
1.750000000000000000e+02, 4.932746615938712192e-02
1.760000000000000000e+02, 5.917464212874612439e-02
1.770000000000000000e+02, 3.041801222307315145e-02
1.780000000000000000e+02, 1.811507787192702390e-02
1.790000000000000000e+02, 4.675788099707668677e-02
1.800000000000000000e+02, 3.816882414116934408e-02
1.810000000000000000e+02, 7.762236311461548355e-02
1.820000000000000000e+02, 9.852938659165103030e-02
1.830000000000000000e+02, 1.296978828838792619e-01
1.840000000000000000e+02, 1.909421965898852602e-01
1.850000000000000000e+02, 2.341332025234545422e-01
1.860000000000000000e+02, 2.269856911375072173e-01
1.870000000000000000e+02, 2.562691937199643166e-01
1.880000000000000000e+02, 1.691038926886295202e-01
1.890000000000000000e+02, 1.462462898547713386e-01
1.900000000000000000e+02, 1.189183463789403733e-01
1.910000000000000000e+02, 6.078472057462393913e-02
1.920000000000000000e+02, 5.778875148652268950e-02
1.930000000000000000e+02, 3.531593656790701224e-02
1.940000000000000000e+02, 4.086476046673424151e-02
};

\addlegendentry{sensor-rotation-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_high_uncertainty.tex <==
\addplot [name path=uncertainty, color=uncertaintyColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 8.086520070001906646e+00
1.100000000000000000e+01, 1.005510753643758548e+01
1.200000000000000000e+01, 1.333380098349204701e+01
1.300000000000000000e+01, 1.713629034269482787e+01
1.400000000000000000e+01, 2.116309726448623252e+01
1.500000000000000000e+01, 2.560886272197279112e+01
1.600000000000000000e+01, 2.581226557625914353e+01
1.700000000000000000e+01, 2.483414184010363357e+01
1.800000000000000000e+01, 2.249796239485261395e+01
1.900000000000000000e+01, 1.511100999891209540e+01
2.000000000000000000e+01, 7.142677203053965584e+00
2.100000000000000000e+01, 2.748154617728676641e+00
2.200000000000000000e+01, 1.514691002178706558e+00
2.300000000000000000e+01, 2.196306181462674978e+00
2.400000000000000000e+01, 1.582653659716496852e+00
2.500000000000000000e+01, 2.242186023031160325e+00
2.600000000000000000e+01, 4.392330542149661454e+00
2.700000000000000000e+01, 9.548414720751075890e+00
2.800000000000000000e+01, 1.834712919663457242e+01
2.900000000000000000e+01, 2.798152267084649836e+01
3.000000000000000000e+01, 2.827162381835115923e+01
3.100000000000000000e+01, 2.331482220435439245e+01
3.200000000000000000e+01, 2.048760552738565366e+01
3.300000000000000000e+01, 1.596136940111239255e+01
3.400000000000000000e+01, 1.246713917719161202e+01
3.500000000000000000e+01, 1.058381269844941386e+01
3.600000000000000000e+01, 1.113701909433762793e+01
3.700000000000000000e+01, 1.471875521502602169e+01
3.800000000000000000e+01, 1.994910956912454125e+01
3.900000000000000000e+01, 1.322825197426422505e+01
4.000000000000000000e+01, 1.032909281056172723e+01
4.100000000000000000e+01, 1.104109370439219617e+01
4.200000000000000000e+01, 1.291057272143264711e+01
4.300000000000000000e+01, 1.546927027803347698e+01
4.400000000000000000e+01, 1.892330388566630717e+01
4.500000000000000000e+01, 2.469405415357174149e+01
4.600000000000000000e+01, 2.844915425230404793e+01
4.700000000000000000e+01, 3.275007399159802901e+01
4.800000000000000000e+01, 1.968606269567679945e+01
4.900000000000000000e+01, 1.025870221566685814e+01
5.000000000000000000e+01, 4.605016790682682881e+00
5.100000000000000000e+01, 1.920745925226168493e+00
5.200000000000000000e+01, 1.797089519932279833e+00
5.300000000000000000e+01, 1.554203612966858383e+00
5.400000000000000000e+01, 1.685310911719967164e+00
5.500000000000000000e+01, 2.940005251686992338e+00
5.600000000000000000e+01, 6.278749254191324347e+00
5.700000000000000000e+01, 1.381756397130952863e+01
5.800000000000000000e+01, 2.062305033217931083e+01
5.900000000000000000e+01, 2.282888804698774621e+01
6.000000000000000000e+01, 2.563226877446244600e+01
6.100000000000000000e+01, 2.441452059190881840e+01
6.200000000000000000e+01, 2.107786036619002346e+01
6.300000000000000000e+01, 1.705773665073518686e+01
6.400000000000000000e+01, 1.339309124457031075e+01
6.500000000000000000e+01, 9.550586970800916120e+00
6.600000000000000000e+01, 7.723405862346892192e+00
6.700000000000000000e+01, 8.681116118873674736e+00
6.800000000000000000e+01, 1.390030177453352422e+01
6.900000000000000000e+01, 9.727436544300669397e+00
7.000000000000000000e+01, 7.275658129011777220e+00
7.100000000000000000e+01, 7.759083137344802594e+00
7.200000000000000000e+01, 9.386659217271624556e+00
7.300000000000000000e+01, 1.230891759580943301e+01
7.400000000000000000e+01, 1.838997142084675929e+01
7.500000000000000000e+01, 2.622973209143850681e+01
7.600000000000000000e+01, 2.555688802369764900e+01
7.700000000000000000e+01, 1.805242978484282901e+01
7.800000000000000000e+01, 1.305539942078237559e+01
7.900000000000000000e+01, 9.458880479595755730e+00
8.000000000000000000e+01, 7.559194829029094009e+00
8.100000000000000000e+01, 7.340167504266390530e+00
8.200000000000000000e+01, 1.141779788871959234e+01
8.300000000000000000e+01, 1.243595360198577637e+01
8.400000000000000000e+01, 8.493548935461143756e+00
8.500000000000000000e+01, 7.808376968219517877e+00
8.600000000000000000e+01, 1.000556506381009569e+01
8.700000000000000000e+01, 1.320638165375662609e+01
8.800000000000000000e+01, 1.759331900829549156e+01
8.900000000000000000e+01, 2.170650262648040041e+01
9.000000000000000000e+01, 2.111799093555177365e+01
9.100000000000000000e+01, 2.508461573429464408e+01
9.200000000000000000e+01, 2.337546597663809678e+01
9.300000000000000000e+01, 1.991933782431570066e+01
9.400000000000000000e+01, 1.460756305517264408e+01
9.500000000000000000e+01, 6.688744014128195303e+00
9.600000000000000000e+01, 2.610627965075507539e+00
9.700000000000000000e+01, 1.747901213205268034e+00
9.800000000000000000e+01, 1.870198647808616110e+00
9.900000000000000000e+01, 1.569788033864446319e+00
1.000000000000000000e+02, 2.212388729548195876e+00
1.010000000000000000e+02, 4.321297643127987698e+00
1.020000000000000000e+02, 9.078333870294533980e+00
1.030000000000000000e+02, 1.877385204453020862e+01
1.040000000000000000e+02, 2.580974733108097041e+01
1.050000000000000000e+02, 2.829857660574911904e+01
1.060000000000000000e+02, 2.203346353036213046e+01
1.070000000000000000e+02, 2.082781204128540153e+01
1.080000000000000000e+02, 1.619211627985345103e+01
1.090000000000000000e+02, 1.239138084042108190e+01
1.100000000000000000e+02, 1.089790952600064777e+01
1.110000000000000000e+02, 1.106084204113673763e+01
1.120000000000000000e+02, 1.439038513495768967e+01
1.130000000000000000e+02, 1.796022056316780180e+01
1.140000000000000000e+02, 1.362466559610968631e+01
1.150000000000000000e+02, 1.045965955113508983e+01
1.160000000000000000e+02, 1.074792841822902822e+01
1.170000000000000000e+02, 1.248856041502762437e+01
1.180000000000000000e+02, 1.588913659508649801e+01
1.190000000000000000e+02, 1.920935978285684342e+01
1.200000000000000000e+02, 2.244617127894970565e+01
1.210000000000000000e+02, 2.873181612687963593e+01
1.220000000000000000e+02, 2.774533724699605131e+01
1.230000000000000000e+02, 1.802565938184100247e+01
1.240000000000000000e+02, 9.534376706502818877e+00
1.250000000000000000e+02, 4.073647665987239819e+00
1.260000000000000000e+02, 1.996574496449894376e+00
1.270000000000000000e+02, 1.930876726669958021e+00
1.280000000000000000e+02, 2.184065924801089853e+00
1.290000000000000000e+02, 1.928502179848870401e+00
1.300000000000000000e+02, 2.948542935207004501e+00
1.310000000000000000e+02, 5.902183238077108207e+00
1.320000000000000000e+02, 1.231630567752170080e+01
1.330000000000000000e+02, 1.983961618907191138e+01
1.340000000000000000e+02, 2.513542062619034567e+01
1.350000000000000000e+02, 2.219253638091559822e+01
1.360000000000000000e+02, 2.186313602373606102e+01
1.370000000000000000e+02, 2.034720849252536112e+01
1.380000000000000000e+02, 1.664844588965511463e+01
1.390000000000000000e+02, 1.214817158264943942e+01
1.400000000000000000e+02, 9.617397549505483312e+00
1.410000000000000000e+02, 8.060037811825424114e+00
1.420000000000000000e+02, 9.428516266905393906e+00
1.430000000000000000e+02, 1.139594808259447767e+01
1.440000000000000000e+02, 9.775883993338506883e+00
1.450000000000000000e+02, 7.800218487103371956e+00
1.460000000000000000e+02, 8.050532744765476423e+00
1.470000000000000000e+02, 9.135686872953453275e+00
1.480000000000000000e+02, 1.266967455971106205e+01
1.490000000000000000e+02, 1.900435769371949846e+01
1.500000000000000000e+02, 2.574563977688653083e+01
1.510000000000000000e+02, 2.449249368822513162e+01
1.520000000000000000e+02, 1.710071075691669051e+01
1.530000000000000000e+02, 1.330619251992984786e+01
1.540000000000000000e+02, 9.900479581647356753e+00
1.550000000000000000e+02, 7.681265065716085694e+00
1.560000000000000000e+02, 8.166844756243150982e+00
1.570000000000000000e+02, 1.003363237646632555e+01
1.580000000000000000e+02, 1.118833808321157264e+01
1.590000000000000000e+02, 8.842672157322168047e+00
1.600000000000000000e+02, 8.537934099932204646e+00
1.610000000000000000e+02, 9.815940185436208054e+00
1.620000000000000000e+02, 1.185256289326928147e+01
1.630000000000000000e+02, 1.674015383248514155e+01
1.640000000000000000e+02, 2.183260217967160699e+01
1.650000000000000000e+02, 2.138346727741308939e+01
1.660000000000000000e+02, 2.282273364500722579e+01
1.670000000000000000e+02, 2.228298208167742089e+01
1.680000000000000000e+02, 1.951195803037056464e+01
1.690000000000000000e+02, 1.265151884591961817e+01
1.700000000000000000e+02, 5.497245275536224440e+00
1.710000000000000000e+02, 2.470929325871624727e+00
1.720000000000000000e+02, 2.764823654068520487e+00
1.730000000000000000e+02, 1.640960968454014957e+00
1.740000000000000000e+02, 1.775425364780138349e+00
1.750000000000000000e+02, 2.225798170216450877e+00
1.760000000000000000e+02, 3.875559568605999594e+00
1.770000000000000000e+02, 8.136234545426731302e+00
1.780000000000000000e+02, 1.572554339668574386e+01
1.790000000000000000e+02, 2.421897631315285793e+01
1.800000000000000000e+02, 2.602482788470110719e+01
1.810000000000000000e+02, 2.088114399968743840e+01
1.820000000000000000e+02, 1.872189845102505501e+01
1.830000000000000000e+02, 1.454006028707888731e+01
1.840000000000000000e+02, 1.338618093988949731e+01
1.850000000000000000e+02, 1.084317238474476142e+01
1.860000000000000000e+02, 1.174061370389754089e+01
1.870000000000000000e+02, 1.448631111915188718e+01
1.880000000000000000e+02, 1.488826934066772978e+01
1.890000000000000000e+02, 1.329994393520001772e+01
1.900000000000000000e+02, 1.147099467740729395e+01
1.910000000000000000e+02, 1.143877422866934523e+01
1.920000000000000000e+02, 1.278075669735216913e+01
1.930000000000000000e+02, 1.528945669392377127e+01
1.940000000000000000e+02, 1.814783975517758918e+01
};

\addlegendentry{uncertainty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_low_error.tex <==
\addplot [name path=error, color=errorColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 1.000000000000010429e-02
1.100000000000000000e+01, 1.000000000000010429e-02
1.200000000000000000e+01, 1.000000000000010429e-02
1.300000000000000000e+01, 1.000000000000010429e-02
1.400000000000000000e+01, 1.000000000000010429e-02
1.500000000000000000e+01, 1.000000000000010429e-02
1.600000000000000000e+01, 1.000000000000010429e-02
1.700000000000000000e+01, 1.000000000000010429e-02
1.800000000000000000e+01, 1.000000000000010429e-02
1.900000000000000000e+01, 1.000000000000010429e-02
2.000000000000000000e+01, 1.000000000000010429e-02
2.100000000000000000e+01, 1.000000000000010429e-02
2.200000000000000000e+01, 1.040834085586084257e-16
2.300000000000000000e+01, 9.999999999999894390e-03
2.400000000000000000e+01, 9.999999999999897859e-03
2.500000000000000000e+01, 1.999999999999989980e-02
2.600000000000000000e+01, 2.999999999999989481e-02
2.700000000000000000e+01, 3.999999999999990369e-02
2.800000000000000000e+01, 3.999999999999989675e-02
2.900000000000000000e+01, 4.999999999999989175e-02
3.000000000000000000e+01, 5.999999999999990064e-02
3.100000000000000000e+01, 6.999999999999989564e-02
3.200000000000000000e+01, 6.999999999999989564e-02
3.300000000000000000e+01, 7.999999999999990452e-02
3.400000000000000000e+01, 6.999999999999990952e-02
3.500000000000000000e+01, 2.999999999999988787e-02
3.600000000000000000e+01, 1.999999999999990674e-02
3.700000000000000000e+01, 1.999999999999990674e-02
3.800000000000000000e+01, 2.999999999999988787e-02
3.900000000000000000e+01, 2.999999999999988787e-02
4.000000000000000000e+01, 2.999999999999991562e-02
4.100000000000000000e+01, 2.999999999999988787e-02
4.200000000000000000e+01, 2.999999999999988787e-02
4.300000000000000000e+01, 3.999999999999989675e-02
4.400000000000000000e+01, 3.999999999999986899e-02
4.500000000000000000e+01, 4.999999999999987788e-02
4.600000000000000000e+01, 4.999999999999990563e-02
4.700000000000000000e+01, 5.999999999999991451e-02
4.800000000000000000e+01, 5.999999999999991451e-02
4.900000000000000000e+01, 3.999999999999986899e-02
5.000000000000000000e+01, 1.999999999999985123e-02
5.100000000000000000e+01, 1.999999999999990674e-02
5.200000000000000000e+01, 1.000000000000011990e-02
5.300000000000000000e+01, 3.999999999999992450e-02
5.400000000000000000e+01, 1.999999999999990674e-02
5.500000000000000000e+01, 2.999999999999986011e-02
5.600000000000000000e+01, 2.999999999999986011e-02
5.700000000000000000e+01, 3.999999999999986899e-02
5.800000000000000000e+01, 4.999999999999987788e-02
5.900000000000000000e+01, 5.999999999999988676e-02
6.000000000000000000e+01, 6.999999999999989564e-02
6.100000000000000000e+01, 6.999999999999984013e-02
6.200000000000000000e+01, 7.999999999999984901e-02
6.300000000000000000e+01, 5.999999999999988676e-02
6.400000000000000000e+01, 4.999999999999987788e-02
6.500000000000000000e+01, 1.999999999999990674e-02
6.600000000000000000e+01, 9.999999999999897859e-03
6.700000000000000000e+01, 9.999999999999842348e-03
6.800000000000000000e+01, 1.999999999999985123e-02
6.900000000000000000e+01, 2.999999999999986011e-02
7.000000000000000000e+01, 2.999999999999986011e-02
7.100000000000000000e+01, 1.999999999999990674e-02
7.200000000000000000e+01, 2.999999999999991562e-02
7.300000000000000000e+01, 2.999999999999991562e-02
7.400000000000000000e+01, 3.999999999999992450e-02
7.500000000000000000e+01, 3.999999999999992450e-02
7.600000000000000000e+01, 3.999999999999992450e-02
7.700000000000000000e+01, 4.999999999999982236e-02
7.800000000000000000e+01, 4.999999999999982236e-02
7.900000000000000000e+01, 3.999999999999981348e-02
8.000000000000000000e+01, 1.999999999999990674e-02
8.100000000000000000e+01, 9.999999999999897859e-03
8.200000000000000000e+01, 1.999999999999990674e-02
8.300000000000000000e+01, 1.999999999999990674e-02
8.400000000000000000e+01, 1.999999999999990674e-02
8.500000000000000000e+01, 2.999999999999991562e-02
8.600000000000000000e+01, 2.999999999999991562e-02
8.700000000000000000e+01, 3.999999999999992450e-02
8.800000000000000000e+01, 3.999999999999992450e-02
8.900000000000000000e+01, 4.999999999999982236e-02
9.000000000000000000e+01, 4.999999999999982236e-02
9.100000000000000000e+01, 4.999999999999982236e-02
9.200000000000000000e+01, 5.999999999999983125e-02
9.300000000000000000e+01, 6.999999999999984013e-02
9.400000000000000000e+01, 5.999999999999983125e-02
9.500000000000000000e+01, 1.999999999999990674e-02
9.600000000000000000e+01, 1.110223024625156540e-16
9.700000000000000000e+01, 1.000000000000011990e-02
9.800000000000000000e+01, 1.999999999999990674e-02
9.900000000000000000e+01, 1.110223024625156540e-16
1.000000000000000000e+02, 9.999999999999897859e-03
1.010000000000000000e+02, 9.999999999999897859e-03
1.020000000000000000e+02, 1.999999999999979572e-02
1.030000000000000000e+02, 2.999999999999980460e-02
1.040000000000000000e+02, 3.999999999999981348e-02
1.050000000000000000e+02, 4.999999999999982236e-02
1.060000000000000000e+02, 4.999999999999982236e-02
1.070000000000000000e+02, 3.999999999999992450e-02
1.080000000000000000e+02, 6.999999999999984013e-02
1.090000000000000000e+02, 5.999999999999994227e-02
1.100000000000000000e+02, 3.999999999999992450e-02
1.110000000000000000e+02, 1.999999999999990674e-02
1.120000000000000000e+02, 1.999999999999990674e-02
1.130000000000000000e+02, 2.999999999999991562e-02
1.140000000000000000e+02, 2.999999999999980460e-02
1.150000000000000000e+02, 2.999999999999980460e-02
1.160000000000000000e+02, 2.999999999999980460e-02
1.170000000000000000e+02, 2.999999999999980460e-02
1.180000000000000000e+02, 2.999999999999980460e-02
1.190000000000000000e+02, 2.999999999999991562e-02
1.200000000000000000e+02, 3.999999999999992450e-02
1.210000000000000000e+02, 3.999999999999992450e-02
1.220000000000000000e+02, 4.999999999999993339e-02
1.230000000000000000e+02, 4.999999999999993339e-02
1.240000000000000000e+02, 3.999999999999981348e-02
1.250000000000000000e+02, 2.000000000000001776e-02
1.260000000000000000e+02, 1.000000000000000888e-02
1.270000000000000000e+02, 1.000000000000000888e-02
1.280000000000000000e+02, 2.000000000000001776e-02
1.290000000000000000e+02, 3.000000000000002665e-02
1.300000000000000000e+02, 3.000000000000002665e-02
1.310000000000000000e+02, 4.000000000000003553e-02
1.320000000000000000e+02, 5.000000000000004441e-02
1.330000000000000000e+02, 4.999999999999982236e-02
1.340000000000000000e+02, 5.999999999999983125e-02
1.350000000000000000e+02, 6.999999999999984013e-02
1.360000000000000000e+02, 7.999999999999984901e-02
1.370000000000000000e+02, 7.999999999999984901e-02
1.380000000000000000e+02, 8.999999999999985789e-02
1.390000000000000000e+02, 7.999999999999984901e-02
1.400000000000000000e+02, 3.999999999999981348e-02
1.410000000000000000e+02, 9.999999999999786837e-03
1.420000000000000000e+02, 1.999999999999979572e-02
1.430000000000000000e+02, 1.999999999999979572e-02
1.440000000000000000e+02, 2.999999999999980460e-02
1.450000000000000000e+02, 2.999999999999980460e-02
1.460000000000000000e+02, 3.999999999999981348e-02
1.470000000000000000e+02, 3.999999999999981348e-02
1.480000000000000000e+02, 3.999999999999981348e-02
1.490000000000000000e+02, 4.999999999999982236e-02
1.500000000000000000e+02, 4.999999999999982236e-02
1.510000000000000000e+02, 5.999999999999983125e-02
1.520000000000000000e+02, 5.999999999999983125e-02
1.530000000000000000e+02, 5.999999999999983125e-02
1.540000000000000000e+02, 6.000000000000005329e-02
1.550000000000000000e+02, 4.000000000000003553e-02
1.560000000000000000e+02, 3.000000000000002665e-02
1.570000000000000000e+02, 3.000000000000002665e-02
1.580000000000000000e+02, 2.999999999999980460e-02
1.590000000000000000e+02, 3.999999999999981348e-02
1.600000000000000000e+02, 3.999999999999981348e-02
1.610000000000000000e+02, 3.999999999999981348e-02
1.620000000000000000e+02, 4.999999999999982236e-02
1.630000000000000000e+02, 4.999999999999982236e-02
1.640000000000000000e+02, 4.999999999999982236e-02
1.650000000000000000e+02, 5.999999999999983125e-02
1.660000000000000000e+02, 5.999999999999983125e-02
1.670000000000000000e+02, 6.999999999999984013e-02
1.680000000000000000e+02, 6.999999999999984013e-02
1.690000000000000000e+02, 6.999999999999984013e-02
1.700000000000000000e+02, 4.999999999999982236e-02
1.710000000000000000e+02, 2.220446049250313081e-16
1.720000000000000000e+02, 1.000000000000000888e-02
1.730000000000000000e+02, 9.999999999999786837e-03
1.740000000000000000e+02, 1.000000000000000888e-02
1.750000000000000000e+02, 3.999999999999981348e-02
1.760000000000000000e+02, 3.000000000000002665e-02
1.770000000000000000e+02, 3.000000000000002665e-02
1.780000000000000000e+02, 4.000000000000003553e-02
1.790000000000000000e+02, 5.000000000000004441e-02
1.800000000000000000e+02, 5.000000000000004441e-02
1.810000000000000000e+02, 6.000000000000005329e-02
1.820000000000000000e+02, 8.000000000000007105e-02
1.830000000000000000e+02, 7.999999999999984901e-02
1.840000000000000000e+02, 7.999999999999984901e-02
1.850000000000000000e+02, 4.999999999999982236e-02
1.860000000000000000e+02, 2.999999999999980460e-02
1.870000000000000000e+02, 2.999999999999980460e-02
1.880000000000000000e+02, 2.999999999999980460e-02
1.890000000000000000e+02, 3.999999999999981348e-02
1.900000000000000000e+02, 3.999999999999981348e-02
1.910000000000000000e+02, 3.999999999999981348e-02
1.920000000000000000e+02, 3.999999999999981348e-02
1.930000000000000000e+02, 3.999999999999981348e-02
1.940000000000000000e+02, 3.999999999999981348e-02
};

\addlegendentry{error}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_low_estimation.tex <==
\addplot [name path=estimationlower, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, -1.999999999999989633e-02
1.100000000000000000e+01, -1.999999999999989633e-02
1.200000000000000000e+01, -1.999999999999989633e-02
1.300000000000000000e+01, -1.999999999999989633e-02
1.400000000000000000e+01, -1.999999999999989633e-02
1.500000000000000000e+01, -2.999999999999989481e-02
1.600000000000000000e+01, -2.999999999999989481e-02
1.700000000000000000e+01, -2.999999999999989481e-02
1.800000000000000000e+01, -3.999999999999989675e-02
1.900000000000000000e+01, -4.999999999999989869e-02
2.000000000000000000e+01, -2.999999999999989481e-02
2.100000000000000000e+01, 1.040834085586084257e-16
2.200000000000000000e+01, 1.000000000000010429e-02
2.300000000000000000e+01, 1.000000000000010429e-02
2.400000000000000000e+01, 2.000000000000010450e-02
2.500000000000000000e+01, 3.000000000000010297e-02
2.600000000000000000e+01, 3.000000000000010297e-02
2.700000000000000000e+01, 3.000000000000010297e-02
2.800000000000000000e+01, 3.000000000000010297e-02
2.900000000000000000e+01, 3.000000000000010297e-02
3.000000000000000000e+01, 3.000000000000010297e-02
3.100000000000000000e+01, 3.000000000000010297e-02
3.200000000000000000e+01, 4.000000000000010492e-02
3.300000000000000000e+01, 4.000000000000010492e-02
3.400000000000000000e+01, 5.000000000000010686e-02
3.500000000000000000e+01, 8.000000000000009881e-02
3.600000000000000000e+01, 1.000000000000001027e-01
3.700000000000000000e+01, 1.000000000000001027e-01
3.800000000000000000e+01, 1.000000000000001027e-01
3.900000000000000000e+01, 1.100000000000001116e-01
4.000000000000000000e+01, 1.300000000000001155e-01
4.100000000000000000e+01, 1.400000000000000966e-01
4.200000000000000000e+01, 1.500000000000001055e-01
4.300000000000000000e+01, 1.500000000000001055e-01
4.400000000000000000e+01, 1.500000000000001055e-01
4.500000000000000000e+01, 1.600000000000001144e-01
4.600000000000000000e+01, 1.600000000000001144e-01
4.700000000000000000e+01, 1.600000000000001144e-01
4.800000000000000000e+01, 1.700000000000000955e-01
4.900000000000000000e+01, 2.100000000000001033e-01
5.000000000000000000e+01, 2.500000000000001110e-01
5.100000000000000000e+01, 2.800000000000001377e-01
5.200000000000000000e+01, 3.100000000000001088e-01
5.300000000000000000e+01, 2.700000000000001288e-01
5.400000000000000000e+01, 3.100000000000001088e-01
5.500000000000000000e+01, 3.200000000000001177e-01
5.600000000000000000e+01, 3.200000000000001177e-01
5.700000000000000000e+01, 3.200000000000001177e-01
5.800000000000000000e+01, 3.200000000000001177e-01
5.900000000000000000e+01, 3.200000000000001177e-01
6.000000000000000000e+01, 3.200000000000001177e-01
6.100000000000000000e+01, 3.200000000000001177e-01
6.200000000000000000e+01, 3.300000000000001266e-01
6.300000000000000000e+01, 3.500000000000000888e-01
6.400000000000000000e+01, 3.500000000000000888e-01
6.500000000000000000e+01, 3.700000000000001066e-01
6.600000000000000000e+01, 4.000000000000001332e-01
6.700000000000000000e+01, 4.200000000000000955e-01
6.800000000000000000e+01, 4.200000000000000955e-01
6.900000000000000000e+01, 4.200000000000000955e-01
7.000000000000000000e+01, 4.400000000000001132e-01
7.100000000000000000e+01, 4.600000000000001310e-01
7.200000000000000000e+01, 4.600000000000001310e-01
7.300000000000000000e+01, 4.700000000000001399e-01
7.400000000000000000e+01, 4.700000000000001399e-01
7.500000000000000000e+01, 4.800000000000000933e-01
7.600000000000000000e+01, 4.800000000000000933e-01
7.700000000000000000e+01, 4.900000000000001021e-01
7.800000000000000000e+01, 4.900000000000001021e-01
7.900000000000000000e+01, 5.100000000000001199e-01
8.000000000000000000e+01, 5.400000000000001465e-01
8.100000000000000000e+01, 5.600000000000001643e-01
8.200000000000000000e+01, 5.700000000000000622e-01
8.300000000000000000e+01, 5.700000000000000622e-01
8.400000000000000000e+01, 5.800000000000000711e-01
8.500000000000000000e+01, 5.900000000000000799e-01
8.600000000000000000e+01, 6.000000000000000888e-01
8.700000000000000000e+01, 6.000000000000000888e-01
8.800000000000000000e+01, 6.100000000000000977e-01
8.900000000000000000e+01, 6.100000000000000977e-01
9.000000000000000000e+01, 6.100000000000000977e-01
9.100000000000000000e+01, 6.200000000000001066e-01
9.200000000000000000e+01, 6.100000000000000977e-01
9.300000000000000000e+01, 6.100000000000000977e-01
9.400000000000000000e+01, 6.200000000000001066e-01
9.500000000000000000e+01, 6.700000000000001510e-01
9.600000000000000000e+01, 7.300000000000000933e-01
9.700000000000000000e+01, 7.700000000000001288e-01
9.800000000000000000e+01, 7.500000000000001110e-01
9.900000000000000000e+01, 7.800000000000001377e-01
1.000000000000000000e+02, 7.800000000000001377e-01
1.010000000000000000e+02, 7.900000000000001465e-01
1.020000000000000000e+02, 7.900000000000001465e-01
1.030000000000000000e+02, 7.900000000000001465e-01
1.040000000000000000e+02, 7.900000000000001465e-01
1.050000000000000000e+02, 7.900000000000001465e-01
1.060000000000000000e+02, 8.000000000000001554e-01
1.070000000000000000e+02, 8.100000000000001643e-01
1.080000000000000000e+02, 8.000000000000001554e-01
1.090000000000000000e+02, 8.000000000000001554e-01
1.100000000000000000e+02, 8.200000000000001732e-01
1.110000000000000000e+02, 8.400000000000000799e-01
1.120000000000000000e+02, 8.500000000000000888e-01
1.130000000000000000e+02, 8.500000000000000888e-01
1.140000000000000000e+02, 8.600000000000000977e-01
1.150000000000000000e+02, 8.700000000000001066e-01
1.160000000000000000e+02, 8.800000000000001155e-01
1.170000000000000000e+02, 8.975000000000001865e-01
1.180000000000000000e+02, 9.000000000000001332e-01
1.190000000000000000e+02, 9.100000000000001421e-01
1.200000000000000000e+02, 9.100000000000001421e-01
1.210000000000000000e+02, 9.200000000000001510e-01
1.220000000000000000e+02, 9.200000000000001510e-01
1.230000000000000000e+02, 9.200000000000001510e-01
1.240000000000000000e+02, 9.400000000000001688e-01
1.250000000000000000e+02, 9.800000000000000933e-01
1.260000000000000000e+02, 1.020000000000000018e+00
1.270000000000000000e+02, 1.050000000000000044e+00
1.280000000000000000e+02, 1.050000000000000044e+00
1.290000000000000000e+02, 1.060000000000000053e+00
1.300000000000000000e+02, 1.060000000000000053e+00
1.310000000000000000e+02, 1.070000000000000062e+00
1.320000000000000000e+02, 1.070000000000000062e+00
1.330000000000000000e+02, 1.070000000000000062e+00
1.340000000000000000e+02, 1.070000000000000062e+00
1.350000000000000000e+02, 1.070000000000000062e+00
1.360000000000000000e+02, 1.070000000000000062e+00
1.370000000000000000e+02, 1.080000000000000071e+00
1.380000000000000000e+02, 1.080000000000000071e+00
1.390000000000000000e+02, 1.080000000000000071e+00
1.400000000000000000e+02, 1.100000000000000089e+00
1.410000000000000000e+02, 1.140000000000000124e+00
1.420000000000000000e+02, 1.160000000000000142e+00
1.430000000000000000e+02, 1.170000000000000151e+00
1.440000000000000000e+02, 1.160000000000000142e+00
1.450000000000000000e+02, 1.170000000000000151e+00
1.460000000000000000e+02, 1.190000000000000169e+00
1.470000000000000000e+02, 1.210000000000000187e+00
1.480000000000000000e+02, 1.210000000000000187e+00
1.490000000000000000e+02, 1.210000000000000187e+00
1.500000000000000000e+02, 1.220000000000000195e+00
1.510000000000000000e+02, 1.220000000000000195e+00
1.520000000000000000e+02, 1.220000000000000195e+00
1.530000000000000000e+02, 1.230000000000000204e+00
1.540000000000000000e+02, 1.240000000000000213e+00
1.550000000000000000e+02, 1.260000000000000231e+00
1.560000000000000000e+02, 1.290000000000000036e+00
1.570000000000000000e+02, 1.310000000000000053e+00
1.580000000000000000e+02, 1.310000000000000053e+00
1.590000000000000000e+02, 1.320000000000000062e+00
1.600000000000000000e+02, 1.330000000000000071e+00
1.610000000000000000e+02, 1.340000000000000080e+00
1.620000000000000000e+02, 1.350000000000000089e+00
1.630000000000000000e+02, 1.350000000000000089e+00
1.640000000000000000e+02, 1.350000000000000089e+00
1.650000000000000000e+02, 1.360000000000000098e+00
1.660000000000000000e+02, 1.360000000000000098e+00
1.670000000000000000e+02, 1.360000000000000098e+00
1.680000000000000000e+02, 1.360000000000000098e+00
1.690000000000000000e+02, 1.360000000000000098e+00
1.700000000000000000e+02, 1.380000000000000115e+00
1.710000000000000000e+02, 1.450000000000000178e+00
1.720000000000000000e+02, 1.500000000000000222e+00
1.730000000000000000e+02, 1.500000000000000222e+00
1.740000000000000000e+02, 1.540000000000000036e+00
1.750000000000000000e+02, 1.500000000000000222e+00
1.760000000000000000e+02, 1.520000000000000240e+00
1.770000000000000000e+02, 1.530000000000000027e+00
1.780000000000000000e+02, 1.530000000000000027e+00
1.790000000000000000e+02, 1.530000000000000027e+00
1.800000000000000000e+02, 1.530000000000000027e+00
1.810000000000000000e+02, 1.540000000000000036e+00
1.820000000000000000e+02, 1.520000000000000240e+00
1.830000000000000000e+02, 1.540000000000000036e+00
1.840000000000000000e+02, 1.540000000000000036e+00
1.850000000000000000e+02, 1.550000000000000044e+00
1.860000000000000000e+02, 1.570000000000000062e+00
1.870000000000000000e+02, 1.590000000000000080e+00
1.880000000000000000e+02, 1.600000000000000089e+00
1.890000000000000000e+02, 1.600000000000000089e+00
1.900000000000000000e+02, 1.610000000000000098e+00
1.910000000000000000e+02, 1.620000000000000107e+00
1.920000000000000000e+02, 1.640000000000000124e+00
1.930000000000000000e+02, 1.650000000000000133e+00
1.940000000000000000e+02, 1.650000000000000133e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationupper, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 4.000000000000010492e-02
1.100000000000000000e+01, 4.000000000000010492e-02
1.200000000000000000e+01, 4.000000000000010492e-02
1.300000000000000000e+01, 4.000000000000010492e-02
1.400000000000000000e+01, 4.000000000000010492e-02
1.500000000000000000e+01, 5.000000000000010686e-02
1.600000000000000000e+01, 5.250000000000010908e-02
1.700000000000000000e+01, 6.000000000000010880e-02
1.800000000000000000e+01, 6.000000000000010880e-02
1.900000000000000000e+01, 7.000000000000010381e-02
2.000000000000000000e+01, 5.000000000000010686e-02
2.100000000000000000e+01, 3.000000000000010297e-02
2.200000000000000000e+01, 3.000000000000010297e-02
2.300000000000000000e+01, 3.000000000000010297e-02
2.400000000000000000e+01, 3.000000000000010297e-02
2.500000000000000000e+01, 4.000000000000010492e-02
2.600000000000000000e+01, 4.000000000000010492e-02
2.700000000000000000e+01, 4.000000000000010492e-02
2.800000000000000000e+01, 4.000000000000010492e-02
2.900000000000000000e+01, 4.000000000000010492e-02
3.000000000000000000e+01, 5.000000000000010686e-02
3.100000000000000000e+01, 5.000000000000010686e-02
3.200000000000000000e+01, 6.000000000000010880e-02
3.300000000000000000e+01, 6.000000000000010880e-02
3.400000000000000000e+01, 1.000000000000001027e-01
3.500000000000000000e+01, 1.700000000000000955e-01
3.600000000000000000e+01, 1.900000000000001132e-01
3.700000000000000000e+01, 2.000000000000001221e-01
3.800000000000000000e+01, 2.000000000000001221e-01
3.900000000000000000e+01, 2.000000000000001221e-01
4.000000000000000000e+01, 2.100000000000001033e-01
4.100000000000000000e+01, 2.200000000000001121e-01
4.200000000000000000e+01, 2.300000000000001210e-01
4.300000000000000000e+01, 2.300000000000001210e-01
4.400000000000000000e+01, 2.400000000000001021e-01
4.500000000000000000e+01, 2.500000000000001110e-01
4.600000000000000000e+01, 2.600000000000001199e-01
4.700000000000000000e+01, 2.600000000000001199e-01
4.800000000000000000e+01, 2.700000000000001288e-01
4.900000000000000000e+01, 3.000000000000000999e-01
5.000000000000000000e+01, 3.100000000000001088e-01
5.100000000000000000e+01, 3.100000000000001088e-01
5.200000000000000000e+01, 3.400000000000001354e-01
5.300000000000000000e+01, 3.000000000000000999e-01
5.400000000000000000e+01, 3.300000000000001266e-01
5.500000000000000000e+01, 3.300000000000001266e-01
5.600000000000000000e+01, 3.300000000000001266e-01
5.700000000000000000e+01, 3.400000000000001354e-01
5.800000000000000000e+01, 3.400000000000001354e-01
5.900000000000000000e+01, 3.400000000000001354e-01
6.000000000000000000e+01, 3.400000000000001354e-01
6.100000000000000000e+01, 3.500000000000000888e-01
6.200000000000000000e+01, 3.600000000000000977e-01
6.300000000000000000e+01, 3.900000000000001243e-01
6.400000000000000000e+01, 4.300000000000001044e-01
6.500000000000000000e+01, 4.900000000000001021e-01
6.600000000000000000e+01, 5.000000000000001110e-01
6.700000000000000000e+01, 5.000000000000001110e-01
6.800000000000000000e+01, 5.000000000000001110e-01
6.900000000000000000e+01, 5.000000000000001110e-01
7.000000000000000000e+01, 5.000000000000001110e-01
7.100000000000000000e+01, 5.100000000000001199e-01
7.200000000000000000e+01, 5.200000000000001288e-01
7.300000000000000000e+01, 5.300000000000001377e-01
7.400000000000000000e+01, 5.300000000000001377e-01
7.500000000000000000e+01, 5.400000000000001465e-01
7.600000000000000000e+01, 5.500000000000001554e-01
7.700000000000000000e+01, 5.600000000000001643e-01
7.800000000000000000e+01, 5.700000000000000622e-01
7.900000000000000000e+01, 5.900000000000000799e-01
8.000000000000000000e+01, 6.200000000000001066e-01
8.100000000000000000e+01, 6.300000000000001155e-01
8.200000000000000000e+01, 6.400000000000001243e-01
8.300000000000000000e+01, 6.400000000000001243e-01
8.400000000000000000e+01, 6.500000000000001332e-01
8.500000000000000000e+01, 6.500000000000001332e-01
8.600000000000000000e+01, 6.600000000000001421e-01
8.700000000000000000e+01, 6.700000000000001510e-01
8.800000000000000000e+01, 6.700000000000001510e-01
8.900000000000000000e+01, 6.800000000000001599e-01
9.000000000000000000e+01, 6.900000000000001688e-01
9.100000000000000000e+01, 7.000000000000000666e-01
9.200000000000000000e+01, 7.000000000000000666e-01
9.300000000000000000e+01, 7.100000000000000755e-01
9.400000000000000000e+01, 7.300000000000000933e-01
9.500000000000000000e+01, 7.900000000000001465e-01
9.600000000000000000e+01, 7.900000000000001465e-01
9.700000000000000000e+01, 8.000000000000001554e-01
9.800000000000000000e+01, 7.800000000000001377e-01
9.900000000000000000e+01, 8.100000000000001643e-01
1.000000000000000000e+02, 8.000000000000001554e-01
1.010000000000000000e+02, 8.100000000000001643e-01
1.020000000000000000e+02, 8.100000000000001643e-01
1.030000000000000000e+02, 8.100000000000001643e-01
1.040000000000000000e+02, 8.100000000000001643e-01
1.050000000000000000e+02, 8.100000000000001643e-01
1.060000000000000000e+02, 8.200000000000001732e-01
1.070000000000000000e+02, 8.400000000000000799e-01
1.080000000000000000e+02, 8.300000000000000711e-01
1.090000000000000000e+02, 8.500000000000000888e-01
1.100000000000000000e+02, 9.100000000000001421e-01
1.110000000000000000e+02, 9.500000000000001776e-01
1.120000000000000000e+02, 9.500000000000001776e-01
1.130000000000000000e+02, 9.600000000000000755e-01
1.140000000000000000e+02, 9.600000000000000755e-01
1.150000000000000000e+02, 9.600000000000000755e-01
1.160000000000000000e+02, 9.700000000000000844e-01
1.170000000000000000e+02, 9.800000000000000933e-01
1.180000000000000000e+02, 9.900000000000001021e-01
1.190000000000000000e+02, 1.000000000000000222e+00
1.200000000000000000e+02, 1.010000000000000231e+00
1.210000000000000000e+02, 1.020000000000000018e+00
1.220000000000000000e+02, 1.020000000000000018e+00
1.230000000000000000e+02, 1.030000000000000027e+00
1.240000000000000000e+02, 1.050000000000000044e+00
1.250000000000000000e+02, 1.070000000000000062e+00
1.260000000000000000e+02, 1.070000000000000062e+00
1.270000000000000000e+02, 1.070000000000000062e+00
1.280000000000000000e+02, 1.070000000000000062e+00
1.290000000000000000e+02, 1.070000000000000062e+00
1.300000000000000000e+02, 1.080000000000000071e+00
1.310000000000000000e+02, 1.080000000000000071e+00
1.320000000000000000e+02, 1.080000000000000071e+00
1.330000000000000000e+02, 1.080000000000000071e+00
1.340000000000000000e+02, 1.080000000000000071e+00
1.350000000000000000e+02, 1.090000000000000080e+00
1.360000000000000000e+02, 1.090000000000000080e+00
1.370000000000000000e+02, 1.100000000000000089e+00
1.380000000000000000e+02, 1.100000000000000089e+00
1.390000000000000000e+02, 1.140000000000000124e+00
1.400000000000000000e+02, 1.240000000000000213e+00
1.410000000000000000e+02, 1.260000000000000231e+00
1.420000000000000000e+02, 1.250000000000000222e+00
1.430000000000000000e+02, 1.250000000000000222e+00
1.440000000000000000e+02, 1.250000000000000222e+00
1.450000000000000000e+02, 1.250000000000000222e+00
1.460000000000000000e+02, 1.250000000000000222e+00
1.470000000000000000e+02, 1.260000000000000231e+00
1.480000000000000000e+02, 1.270000000000000240e+00
1.490000000000000000e+02, 1.280000000000000027e+00
1.500000000000000000e+02, 1.280000000000000027e+00
1.510000000000000000e+02, 1.290000000000000036e+00
1.520000000000000000e+02, 1.290000000000000036e+00
1.530000000000000000e+02, 1.300000000000000044e+00
1.540000000000000000e+02, 1.320000000000000062e+00
1.550000000000000000e+02, 1.350000000000000089e+00
1.560000000000000000e+02, 1.370000000000000107e+00
1.570000000000000000e+02, 1.380000000000000115e+00
1.580000000000000000e+02, 1.380000000000000115e+00
1.590000000000000000e+02, 1.390000000000000124e+00
1.600000000000000000e+02, 1.390000000000000124e+00
1.610000000000000000e+02, 1.400000000000000133e+00
1.620000000000000000e+02, 1.400000000000000133e+00
1.630000000000000000e+02, 1.410000000000000142e+00
1.640000000000000000e+02, 1.420000000000000151e+00
1.650000000000000000e+02, 1.430000000000000160e+00
1.660000000000000000e+02, 1.440000000000000169e+00
1.670000000000000000e+02, 1.440000000000000169e+00
1.680000000000000000e+02, 1.450000000000000178e+00
1.690000000000000000e+02, 1.470000000000000195e+00
1.700000000000000000e+02, 1.530000000000000027e+00
1.710000000000000000e+02, 1.570000000000000062e+00
1.720000000000000000e+02, 1.560000000000000053e+00
1.730000000000000000e+02, 1.530000000000000027e+00
1.740000000000000000e+02, 1.560000000000000053e+00
1.750000000000000000e+02, 1.520000000000000240e+00
1.760000000000000000e+02, 1.540000000000000036e+00
1.770000000000000000e+02, 1.550000000000000044e+00
1.780000000000000000e+02, 1.550000000000000044e+00
1.790000000000000000e+02, 1.550000000000000044e+00
1.800000000000000000e+02, 1.560000000000000053e+00
1.810000000000000000e+02, 1.570000000000000062e+00
1.820000000000000000e+02, 1.550000000000000044e+00
1.830000000000000000e+02, 1.570000000000000062e+00
1.840000000000000000e+02, 1.590000000000000080e+00
1.850000000000000000e+02, 1.650000000000000133e+00
1.860000000000000000e+02, 1.690000000000000169e+00
1.870000000000000000e+02, 1.700000000000000178e+00
1.880000000000000000e+02, 1.700000000000000178e+00
1.890000000000000000e+02, 1.700000000000000178e+00
1.900000000000000000e+02, 1.710000000000000187e+00
1.910000000000000000e+02, 1.720000000000000195e+00
1.920000000000000000e+02, 1.720000000000000195e+00
1.930000000000000000e+02, 1.730000000000000204e+00
1.940000000000000000e+02, 1.750000000000000222e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationmedian, color=estimationColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 1.000000000000010429e-02
1.100000000000000000e+01, 1.000000000000010429e-02
1.200000000000000000e+01, 1.000000000000010429e-02
1.300000000000000000e+01, 1.000000000000010429e-02
1.400000000000000000e+01, 1.000000000000010429e-02
1.500000000000000000e+01, 1.000000000000010429e-02
1.600000000000000000e+01, 1.000000000000010429e-02
1.700000000000000000e+01, 1.000000000000010429e-02
1.800000000000000000e+01, 1.000000000000010429e-02
1.900000000000000000e+01, 1.000000000000010429e-02
2.000000000000000000e+01, 1.000000000000010429e-02
2.100000000000000000e+01, 2.000000000000010450e-02
2.200000000000000000e+01, 2.000000000000010450e-02
2.300000000000000000e+01, 2.000000000000010450e-02
2.400000000000000000e+01, 3.000000000000010297e-02
2.500000000000000000e+01, 3.000000000000010297e-02
2.600000000000000000e+01, 3.000000000000010297e-02
2.700000000000000000e+01, 3.000000000000010297e-02
2.800000000000000000e+01, 4.000000000000010492e-02
2.900000000000000000e+01, 4.000000000000010492e-02
3.000000000000000000e+01, 4.000000000000010492e-02
3.100000000000000000e+01, 4.000000000000010492e-02
3.200000000000000000e+01, 5.000000000000010686e-02
3.300000000000000000e+01, 5.000000000000010686e-02
3.400000000000000000e+01, 7.000000000000010381e-02
3.500000000000000000e+01, 1.200000000000001066e-01
3.600000000000000000e+01, 1.400000000000000966e-01
3.700000000000000000e+01, 1.500000000000001055e-01
3.800000000000000000e+01, 1.500000000000001055e-01
3.900000000000000000e+01, 1.600000000000001144e-01
4.000000000000000000e+01, 1.700000000000000955e-01
4.100000000000000000e+01, 1.800000000000001044e-01
4.200000000000000000e+01, 1.900000000000001132e-01
4.300000000000000000e+01, 1.900000000000001132e-01
4.400000000000000000e+01, 2.000000000000001221e-01
4.500000000000000000e+01, 2.000000000000001221e-01
4.600000000000000000e+01, 2.100000000000001033e-01
4.700000000000000000e+01, 2.100000000000001033e-01
4.800000000000000000e+01, 2.200000000000001121e-01
4.900000000000000000e+01, 2.500000000000001110e-01
5.000000000000000000e+01, 2.800000000000001377e-01
5.100000000000000000e+01, 2.900000000000000910e-01
5.200000000000000000e+01, 3.300000000000001266e-01
5.300000000000000000e+01, 2.900000000000000910e-01
5.400000000000000000e+01, 3.200000000000001177e-01
5.500000000000000000e+01, 3.200000000000001177e-01
5.600000000000000000e+01, 3.300000000000001266e-01
5.700000000000000000e+01, 3.300000000000001266e-01
5.800000000000000000e+01, 3.300000000000001266e-01
5.900000000000000000e+01, 3.300000000000001266e-01
6.000000000000000000e+01, 3.300000000000001266e-01
6.100000000000000000e+01, 3.400000000000001354e-01
6.200000000000000000e+01, 3.400000000000001354e-01
6.300000000000000000e+01, 3.700000000000001066e-01
6.400000000000000000e+01, 3.900000000000001243e-01
6.500000000000000000e+01, 4.300000000000001044e-01
6.600000000000000000e+01, 4.500000000000001221e-01
6.700000000000000000e+01, 4.600000000000001310e-01
6.800000000000000000e+01, 4.600000000000001310e-01
6.900000000000000000e+01, 4.600000000000001310e-01
7.000000000000000000e+01, 4.700000000000001399e-01
7.100000000000000000e+01, 4.900000000000001021e-01
7.200000000000000000e+01, 4.900000000000001021e-01
7.300000000000000000e+01, 5.000000000000001110e-01
7.400000000000000000e+01, 5.000000000000001110e-01
7.500000000000000000e+01, 5.100000000000001199e-01
7.600000000000000000e+01, 5.200000000000001288e-01
7.700000000000000000e+01, 5.200000000000001288e-01
7.800000000000000000e+01, 5.300000000000001377e-01
7.900000000000000000e+01, 5.500000000000001554e-01
8.000000000000000000e+01, 5.800000000000000711e-01
8.100000000000000000e+01, 6.000000000000000888e-01
8.200000000000000000e+01, 6.000000000000000888e-01
8.300000000000000000e+01, 6.100000000000000977e-01
8.400000000000000000e+01, 6.200000000000001066e-01
8.500000000000000000e+01, 6.200000000000001066e-01
8.600000000000000000e+01, 6.300000000000001155e-01
8.700000000000000000e+01, 6.300000000000001155e-01
8.800000000000000000e+01, 6.400000000000001243e-01
8.900000000000000000e+01, 6.400000000000001243e-01
9.000000000000000000e+01, 6.500000000000001332e-01
9.100000000000000000e+01, 6.600000000000001421e-01
9.200000000000000000e+01, 6.600000000000001421e-01
9.300000000000000000e+01, 6.600000000000001421e-01
9.400000000000000000e+01, 6.800000000000001599e-01
9.500000000000000000e+01, 7.300000000000000933e-01
9.600000000000000000e+01, 7.600000000000001199e-01
9.700000000000000000e+01, 7.800000000000001377e-01
9.800000000000000000e+01, 7.600000000000001199e-01
9.900000000000000000e+01, 7.900000000000001465e-01
1.000000000000000000e+02, 7.900000000000001465e-01
1.010000000000000000e+02, 8.000000000000001554e-01
1.020000000000000000e+02, 8.000000000000001554e-01
1.030000000000000000e+02, 8.000000000000001554e-01
1.040000000000000000e+02, 8.000000000000001554e-01
1.050000000000000000e+02, 8.000000000000001554e-01
1.060000000000000000e+02, 8.100000000000001643e-01
1.070000000000000000e+02, 8.300000000000000711e-01
1.080000000000000000e+02, 8.100000000000001643e-01
1.090000000000000000e+02, 8.300000000000000711e-01
1.100000000000000000e+02, 8.600000000000000977e-01
1.110000000000000000e+02, 8.900000000000001243e-01
1.120000000000000000e+02, 9.000000000000001332e-01
1.130000000000000000e+02, 9.000000000000001332e-01
1.140000000000000000e+02, 9.100000000000001421e-01
1.150000000000000000e+02, 9.200000000000001510e-01
1.160000000000000000e+02, 9.300000000000001599e-01
1.170000000000000000e+02, 9.400000000000001688e-01
1.180000000000000000e+02, 9.500000000000001776e-01
1.190000000000000000e+02, 9.600000000000000755e-01
1.200000000000000000e+02, 9.600000000000000755e-01
1.210000000000000000e+02, 9.700000000000000844e-01
1.220000000000000000e+02, 9.700000000000000844e-01
1.230000000000000000e+02, 9.800000000000000933e-01
1.240000000000000000e+02, 1.000000000000000222e+00
1.250000000000000000e+02, 1.030000000000000027e+00
1.260000000000000000e+02, 1.050000000000000044e+00
1.270000000000000000e+02, 1.060000000000000053e+00
1.280000000000000000e+02, 1.060000000000000053e+00
1.290000000000000000e+02, 1.060000000000000053e+00
1.300000000000000000e+02, 1.070000000000000062e+00
1.310000000000000000e+02, 1.070000000000000062e+00
1.320000000000000000e+02, 1.070000000000000062e+00
1.330000000000000000e+02, 1.080000000000000071e+00
1.340000000000000000e+02, 1.080000000000000071e+00
1.350000000000000000e+02, 1.080000000000000071e+00
1.360000000000000000e+02, 1.080000000000000071e+00
1.370000000000000000e+02, 1.090000000000000080e+00
1.380000000000000000e+02, 1.090000000000000080e+00
1.390000000000000000e+02, 1.110000000000000098e+00
1.400000000000000000e+02, 1.160000000000000142e+00
1.410000000000000000e+02, 1.200000000000000178e+00
1.420000000000000000e+02, 1.200000000000000178e+00
1.430000000000000000e+02, 1.210000000000000187e+00
1.440000000000000000e+02, 1.210000000000000187e+00
1.450000000000000000e+02, 1.220000000000000195e+00
1.460000000000000000e+02, 1.220000000000000195e+00
1.470000000000000000e+02, 1.230000000000000204e+00
1.480000000000000000e+02, 1.240000000000000213e+00
1.490000000000000000e+02, 1.240000000000000213e+00
1.500000000000000000e+02, 1.250000000000000222e+00
1.510000000000000000e+02, 1.250000000000000222e+00
1.520000000000000000e+02, 1.260000000000000231e+00
1.530000000000000000e+02, 1.270000000000000240e+00
1.540000000000000000e+02, 1.280000000000000027e+00
1.550000000000000000e+02, 1.310000000000000053e+00
1.560000000000000000e+02, 1.330000000000000071e+00
1.570000000000000000e+02, 1.340000000000000080e+00
1.580000000000000000e+02, 1.350000000000000089e+00
1.590000000000000000e+02, 1.350000000000000089e+00
1.600000000000000000e+02, 1.360000000000000098e+00
1.610000000000000000e+02, 1.370000000000000107e+00
1.620000000000000000e+02, 1.370000000000000107e+00
1.630000000000000000e+02, 1.380000000000000115e+00
1.640000000000000000e+02, 1.390000000000000124e+00
1.650000000000000000e+02, 1.390000000000000124e+00
1.660000000000000000e+02, 1.400000000000000133e+00
1.670000000000000000e+02, 1.400000000000000133e+00
1.680000000000000000e+02, 1.410000000000000142e+00
1.690000000000000000e+02, 1.420000000000000151e+00
1.700000000000000000e+02, 1.450000000000000178e+00
1.710000000000000000e+02, 1.510000000000000231e+00
1.720000000000000000e+02, 1.530000000000000027e+00
1.730000000000000000e+02, 1.520000000000000240e+00
1.740000000000000000e+02, 1.550000000000000044e+00
1.750000000000000000e+02, 1.510000000000000231e+00
1.760000000000000000e+02, 1.530000000000000027e+00
1.770000000000000000e+02, 1.540000000000000036e+00
1.780000000000000000e+02, 1.540000000000000036e+00
1.790000000000000000e+02, 1.540000000000000036e+00
1.800000000000000000e+02, 1.550000000000000044e+00
1.810000000000000000e+02, 1.550000000000000044e+00
1.820000000000000000e+02, 1.540000000000000036e+00
1.830000000000000000e+02, 1.550000000000000044e+00
1.840000000000000000e+02, 1.560000000000000053e+00
1.850000000000000000e+02, 1.600000000000000089e+00
1.860000000000000000e+02, 1.630000000000000115e+00
1.870000000000000000e+02, 1.640000000000000124e+00
1.880000000000000000e+02, 1.650000000000000133e+00
1.890000000000000000e+02, 1.650000000000000133e+00
1.900000000000000000e+02, 1.660000000000000142e+00
1.910000000000000000e+02, 1.670000000000000151e+00
1.920000000000000000e+02, 1.680000000000000160e+00
1.930000000000000000e+02, 1.690000000000000169e+00
1.940000000000000000e+02, 1.700000000000000178e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addlegendentry{estimation}

\addplot [backGray, fill opacity=0.9, forget plot] fill between[of=estimationlower and estimationupper];

\addplot [name path=ground-truth, color=ground-truthColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 0.000000000000000000e+00
1.100000000000000000e+01, 0.000000000000000000e+00
1.200000000000000000e+01, 0.000000000000000000e+00
1.300000000000000000e+01, 0.000000000000000000e+00
1.400000000000000000e+01, 0.000000000000000000e+00
1.500000000000000000e+01, 0.000000000000000000e+00
1.600000000000000000e+01, 0.000000000000000000e+00
1.700000000000000000e+01, 0.000000000000000000e+00
1.800000000000000000e+01, 0.000000000000000000e+00
1.900000000000000000e+01, 0.000000000000000000e+00
2.000000000000000000e+01, 0.000000000000000000e+00
2.100000000000000000e+01, 1.000000000000000021e-02
2.200000000000000000e+01, 2.000000000000000042e-02
2.300000000000000000e+01, 2.999999999999999889e-02
2.400000000000000000e+01, 4.000000000000000083e-02
2.500000000000000000e+01, 5.000000000000000278e-02
2.600000000000000000e+01, 5.999999999999999778e-02
2.700000000000000000e+01, 7.000000000000000666e-02
2.800000000000000000e+01, 8.000000000000000167e-02
2.900000000000000000e+01, 8.999999999999999667e-02
3.000000000000000000e+01, 1.000000000000000056e-01
3.100000000000000000e+01, 1.100000000000000006e-01
3.200000000000000000e+01, 1.199999999999999956e-01
3.300000000000000000e+01, 1.300000000000000044e-01
3.400000000000000000e+01, 1.400000000000000133e-01
3.500000000000000000e+01, 1.499999999999999944e-01
3.600000000000000000e+01, 1.600000000000000033e-01
3.700000000000000000e+01, 1.700000000000000122e-01
3.800000000000000000e+01, 1.799999999999999933e-01
3.900000000000000000e+01, 1.900000000000000022e-01
4.000000000000000000e+01, 2.000000000000000111e-01
4.100000000000000000e+01, 2.099999999999999922e-01
4.200000000000000000e+01, 2.200000000000000011e-01
4.300000000000000000e+01, 2.300000000000000100e-01
4.400000000000000000e+01, 2.399999999999999911e-01
4.500000000000000000e+01, 2.500000000000000000e-01
4.600000000000000000e+01, 2.600000000000000089e-01
4.700000000000000000e+01, 2.700000000000000178e-01
4.800000000000000000e+01, 2.800000000000000266e-01
4.900000000000000000e+01, 2.899999999999999800e-01
5.000000000000000000e+01, 2.999999999999999889e-01
5.100000000000000000e+01, 3.099999999999999978e-01
5.200000000000000000e+01, 3.200000000000000067e-01
5.300000000000000000e+01, 3.300000000000000155e-01
5.400000000000000000e+01, 3.400000000000000244e-01
5.500000000000000000e+01, 3.499999999999999778e-01
5.600000000000000000e+01, 3.599999999999999867e-01
5.700000000000000000e+01, 3.699999999999999956e-01
5.800000000000000000e+01, 3.800000000000000044e-01
5.900000000000000000e+01, 3.900000000000000133e-01
6.000000000000000000e+01, 4.000000000000000222e-01
6.100000000000000000e+01, 4.099999999999999756e-01
6.200000000000000000e+01, 4.199999999999999845e-01
6.300000000000000000e+01, 4.299999999999999933e-01
6.400000000000000000e+01, 4.400000000000000022e-01
6.500000000000000000e+01, 4.500000000000000111e-01
6.600000000000000000e+01, 4.600000000000000200e-01
6.700000000000000000e+01, 4.699999999999999734e-01
6.800000000000000000e+01, 4.799999999999999822e-01
6.900000000000000000e+01, 4.899999999999999911e-01
7.000000000000000000e+01, 5.000000000000000000e-01
7.100000000000000000e+01, 5.100000000000000089e-01
7.200000000000000000e+01, 5.200000000000000178e-01
7.300000000000000000e+01, 5.300000000000000266e-01
7.400000000000000000e+01, 5.400000000000000355e-01
7.500000000000000000e+01, 5.500000000000000444e-01
7.600000000000000000e+01, 5.600000000000000533e-01
7.700000000000000000e+01, 5.699999999999999512e-01
7.800000000000000000e+01, 5.799999999999999600e-01
7.900000000000000000e+01, 5.899999999999999689e-01
8.000000000000000000e+01, 5.999999999999999778e-01
8.100000000000000000e+01, 6.099999999999999867e-01
8.200000000000000000e+01, 6.199999999999999956e-01
8.300000000000000000e+01, 6.300000000000000044e-01
8.400000000000000000e+01, 6.400000000000000133e-01
8.500000000000000000e+01, 6.500000000000000222e-01
8.600000000000000000e+01, 6.600000000000000311e-01
8.700000000000000000e+01, 6.700000000000000400e-01
8.800000000000000000e+01, 6.800000000000000488e-01
8.900000000000000000e+01, 6.899999999999999467e-01
9.000000000000000000e+01, 6.999999999999999556e-01
9.100000000000000000e+01, 7.099999999999999645e-01
9.200000000000000000e+01, 7.199999999999999734e-01
9.300000000000000000e+01, 7.299999999999999822e-01
9.400000000000000000e+01, 7.399999999999999911e-01
9.500000000000000000e+01, 7.500000000000000000e-01
9.600000000000000000e+01, 7.600000000000000089e-01
9.700000000000000000e+01, 7.700000000000000178e-01
9.800000000000000000e+01, 7.800000000000000266e-01
9.900000000000000000e+01, 7.900000000000000355e-01
1.000000000000000000e+02, 8.000000000000000444e-01
1.010000000000000000e+02, 8.100000000000000533e-01
1.020000000000000000e+02, 8.199999999999999512e-01
1.030000000000000000e+02, 8.299999999999999600e-01
1.040000000000000000e+02, 8.399999999999999689e-01
1.050000000000000000e+02, 8.499999999999999778e-01
1.060000000000000000e+02, 8.599999999999999867e-01
1.070000000000000000e+02, 8.699999999999999956e-01
1.080000000000000000e+02, 8.800000000000000044e-01
1.090000000000000000e+02, 8.900000000000000133e-01
1.100000000000000000e+02, 9.000000000000000222e-01
1.110000000000000000e+02, 9.100000000000000311e-01
1.120000000000000000e+02, 9.200000000000000400e-01
1.130000000000000000e+02, 9.300000000000000488e-01
1.140000000000000000e+02, 9.399999999999999467e-01
1.150000000000000000e+02, 9.499999999999999556e-01
1.160000000000000000e+02, 9.599999999999999645e-01
1.170000000000000000e+02, 9.699999999999999734e-01
1.180000000000000000e+02, 9.799999999999999822e-01
1.190000000000000000e+02, 9.899999999999999911e-01
1.200000000000000000e+02, 1.000000000000000000e+00
1.210000000000000000e+02, 1.010000000000000009e+00
1.220000000000000000e+02, 1.020000000000000018e+00
1.230000000000000000e+02, 1.030000000000000027e+00
1.240000000000000000e+02, 1.040000000000000036e+00
1.250000000000000000e+02, 1.050000000000000044e+00
1.260000000000000000e+02, 1.060000000000000053e+00
1.270000000000000000e+02, 1.070000000000000062e+00
1.280000000000000000e+02, 1.080000000000000071e+00
1.290000000000000000e+02, 1.090000000000000080e+00
1.300000000000000000e+02, 1.100000000000000089e+00
1.310000000000000000e+02, 1.110000000000000098e+00
1.320000000000000000e+02, 1.120000000000000107e+00
1.330000000000000000e+02, 1.129999999999999893e+00
1.340000000000000000e+02, 1.139999999999999902e+00
1.350000000000000000e+02, 1.149999999999999911e+00
1.360000000000000000e+02, 1.159999999999999920e+00
1.370000000000000000e+02, 1.169999999999999929e+00
1.380000000000000000e+02, 1.179999999999999938e+00
1.390000000000000000e+02, 1.189999999999999947e+00
1.400000000000000000e+02, 1.199999999999999956e+00
1.410000000000000000e+02, 1.209999999999999964e+00
1.420000000000000000e+02, 1.219999999999999973e+00
1.430000000000000000e+02, 1.229999999999999982e+00
1.440000000000000000e+02, 1.239999999999999991e+00
1.450000000000000000e+02, 1.250000000000000000e+00
1.460000000000000000e+02, 1.260000000000000009e+00
1.470000000000000000e+02, 1.270000000000000018e+00
1.480000000000000000e+02, 1.280000000000000027e+00
1.490000000000000000e+02, 1.290000000000000036e+00
1.500000000000000000e+02, 1.300000000000000044e+00
1.510000000000000000e+02, 1.310000000000000053e+00
1.520000000000000000e+02, 1.320000000000000062e+00
1.530000000000000000e+02, 1.330000000000000071e+00
1.540000000000000000e+02, 1.340000000000000080e+00
1.550000000000000000e+02, 1.350000000000000089e+00
1.560000000000000000e+02, 1.360000000000000098e+00
1.570000000000000000e+02, 1.370000000000000107e+00
1.580000000000000000e+02, 1.379999999999999893e+00
1.590000000000000000e+02, 1.389999999999999902e+00
1.600000000000000000e+02, 1.399999999999999911e+00
1.610000000000000000e+02, 1.409999999999999920e+00
1.620000000000000000e+02, 1.419999999999999929e+00
1.630000000000000000e+02, 1.429999999999999938e+00
1.640000000000000000e+02, 1.439999999999999947e+00
1.650000000000000000e+02, 1.449999999999999956e+00
1.660000000000000000e+02, 1.459999999999999964e+00
1.670000000000000000e+02, 1.469999999999999973e+00
1.680000000000000000e+02, 1.479999999999999982e+00
1.690000000000000000e+02, 1.489999999999999991e+00
1.700000000000000000e+02, 1.500000000000000000e+00
1.710000000000000000e+02, 1.510000000000000009e+00
1.720000000000000000e+02, 1.520000000000000018e+00
1.730000000000000000e+02, 1.530000000000000027e+00
1.740000000000000000e+02, 1.540000000000000036e+00
1.750000000000000000e+02, 1.550000000000000044e+00
1.760000000000000000e+02, 1.560000000000000053e+00
1.770000000000000000e+02, 1.570000000000000062e+00
1.780000000000000000e+02, 1.580000000000000071e+00
1.790000000000000000e+02, 1.590000000000000080e+00
1.800000000000000000e+02, 1.600000000000000089e+00
1.810000000000000000e+02, 1.610000000000000098e+00
1.820000000000000000e+02, 1.620000000000000107e+00
1.830000000000000000e+02, 1.629999999999999893e+00
1.840000000000000000e+02, 1.639999999999999902e+00
1.850000000000000000e+02, 1.649999999999999911e+00
1.860000000000000000e+02, 1.659999999999999920e+00
1.870000000000000000e+02, 1.669999999999999929e+00
1.880000000000000000e+02, 1.679999999999999938e+00
1.890000000000000000e+02, 1.689999999999999947e+00
1.900000000000000000e+02, 1.699999999999999956e+00
1.910000000000000000e+02, 1.709999999999999964e+00
1.920000000000000000e+02, 1.719999999999999973e+00
1.930000000000000000e+02, 1.729999999999999982e+00
1.940000000000000000e+02, 1.739999999999999991e+00
};

\addlegendentry{ground-truth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_low_rotation.tex <==
\addplot [name path=sensor-rotation-0, color=sensor-rotation-0Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 1.504317427411509464e-02
1.000000000000000000e+00, 4.575509588452019577e-02
2.000000000000000000e+00, 6.271103784338810661e-02
3.000000000000000000e+00, 1.080719779599757652e-01
4.000000000000000000e+00, 1.637832238275296337e-01
5.000000000000000000e+00, 2.241362826544165132e-01
6.000000000000000000e+00, 2.864382052762356468e-01
7.000000000000000000e+00, 3.091088926580931040e-01
8.000000000000000000e+00, 2.611030324628255128e-01
9.000000000000000000e+00, 2.084508805212584304e-01
1.000000000000000000e+01, 1.465402374123086493e-01
1.100000000000000000e+01, 1.120441055978677325e-01
1.200000000000000000e+01, 8.491640522278386116e-02
1.300000000000000000e+01, 7.093851554628131939e-02
1.400000000000000000e+01, 6.007480941865404878e-02
1.500000000000000000e+01, 5.071482872241332707e-02
1.600000000000000000e+01, 5.081087785539651486e-02
1.700000000000000000e+01, 5.254010884029070710e-02
1.800000000000000000e+01, 6.820638301614079246e-02
1.900000000000000000e+01, 1.067431792602134139e-01
2.000000000000000000e+01, 1.854685154807175773e-01
2.100000000000000000e+01, 3.883918193110258432e-01
2.200000000000000000e+01, 7.492794318818047916e-01
2.300000000000000000e+01, 6.195653899912234586e-01
2.400000000000000000e+01, 2.737938860484634973e-01
2.500000000000000000e+01, 1.207125926247708397e-01
2.600000000000000000e+01, 6.086534780220838325e-02
2.700000000000000000e+01, 3.146118003556638842e-02
2.800000000000000000e+01, 1.936758190334121957e-02
2.900000000000000000e+01, 5.754202461648265550e-03
3.000000000000000000e+01, 3.188395091280722682e-02
3.100000000000000000e+01, 4.612738004608239739e-02
3.200000000000000000e+01, 8.019714449939162326e-02
3.300000000000000000e+01, 1.009246098333651115e-01
3.400000000000000000e+01, 1.395766826731715815e-01
3.500000000000000000e+01, 1.775002341811846296e-01
3.600000000000000000e+01, 2.264400213203367762e-01
3.700000000000000000e+01, 2.411096616577397267e-01
3.800000000000000000e+01, 2.376814508450932617e-01
3.900000000000000000e+01, 1.975029760289813141e-01
4.000000000000000000e+01, 1.489711811301356881e-01
4.100000000000000000e+01, 1.224165912740059897e-01
4.200000000000000000e+01, 7.330883994507896018e-02
4.300000000000000000e+01, 6.630496220521585327e-02
4.400000000000000000e+01, 4.109503406678410853e-02
4.500000000000000000e+01, 1.311275519855172739e-02
4.600000000000000000e+01, 5.340495697036372856e-03
4.700000000000000000e+01, 1.159109657945989538e-02
4.800000000000000000e+01, 4.522339298002415325e-02
4.900000000000000000e+01, 9.306748630172667625e-02
5.000000000000000000e+01, 2.062782148480675204e-01
5.100000000000000000e+01, 4.621476622111252430e-01
5.200000000000000000e+01, 7.873179364389019108e-01
5.300000000000000000e+01, 5.216306610308288905e-01
5.400000000000000000e+01, 2.447196563679659709e-01
5.500000000000000000e+01, 1.233179031660212310e-01
5.600000000000000000e+01, 7.830705262969273051e-02
5.700000000000000000e+01, 5.515475224629697026e-02
5.800000000000000000e+01, 4.341348157404238683e-02
5.900000000000000000e+01, 5.518120771970228683e-02
6.000000000000000000e+01, 5.480642826886336638e-02
6.100000000000000000e+01, 5.521201864099083839e-02
6.200000000000000000e+01, 7.150500664305411980e-02
6.300000000000000000e+01, 9.837189334384009720e-02
6.400000000000000000e+01, 1.259725624163430813e-01
6.500000000000000000e+01, 1.792255593515745260e-01
6.600000000000000000e+01, 2.413868289688662072e-01
6.700000000000000000e+01, 3.006272114393934158e-01
6.800000000000000000e+01, 3.147115146624101523e-01
6.900000000000000000e+01, 2.473838178158717649e-01
7.000000000000000000e+01, 1.798530063950034008e-01
7.100000000000000000e+01, 1.332586765406447438e-01
7.200000000000000000e+01, 8.509613770667828758e-02
7.300000000000000000e+01, 4.820994999925336255e-02
7.400000000000000000e+01, 2.522170927628380674e-02
7.500000000000000000e+01, 5.043422693307758088e-03
7.600000000000000000e+01, 2.461119692518420887e-02
7.700000000000000000e+01, 4.847573620133845823e-02
7.800000000000000000e+01, 9.613415388863411071e-02
7.900000000000000000e+01, 1.452279984458992312e-01
8.000000000000000000e+01, 1.993998606214534841e-01
8.100000000000000000e+01, 2.721263804773249584e-01
8.200000000000000000e+01, 3.033008029799768579e-01
8.300000000000000000e+01, 2.840596243384849728e-01
8.400000000000000000e+01, 2.228466333800400712e-01
8.500000000000000000e+01, 1.668275209567193218e-01
8.600000000000000000e+01, 1.188016043113481468e-01
8.700000000000000000e+01, 8.888749565008055575e-02
8.800000000000000000e+01, 6.482817444661449768e-02
8.900000000000000000e+01, 6.294689725821119020e-02
9.000000000000000000e+01, 4.722150269712315634e-02
9.100000000000000000e+01, 5.081706553844139024e-02
9.200000000000000000e+01, 4.849782932347132536e-02
9.300000000000000000e+01, 6.997372872799406673e-02
9.400000000000000000e+01, 8.818385730395858491e-02
9.500000000000000000e+01, 1.547020066623236156e-01
9.600000000000000000e+01, 2.972322345729204174e-01
9.700000000000000000e+01, 6.247792971979000409e-01
9.800000000000000000e+01, 7.299282998766137842e-01
9.900000000000000000e+01, 3.766444564404485273e-01
1.000000000000000000e+02, 1.641974296022216950e-01
1.010000000000000000e+02, 7.210145929763081551e-02
1.020000000000000000e+02, 3.803647490971475559e-02
1.030000000000000000e+02, 1.645837868267419762e-02
1.040000000000000000e+02, 1.404246581746009144e-02
1.050000000000000000e+02, 2.551959623710161468e-02
1.060000000000000000e+02, 3.750779121564028207e-02
1.070000000000000000e+02, 6.723059040332089731e-02
1.080000000000000000e+02, 8.836143340880131536e-02
1.090000000000000000e+02, 1.133580327505913921e-01
1.100000000000000000e+02, 1.722313060455712697e-01
1.110000000000000000e+02, 2.091450121726753653e-01
1.120000000000000000e+02, 2.396603945053549789e-01
1.130000000000000000e+02, 2.478632554347465489e-01
1.140000000000000000e+02, 2.111614599007267112e-01
1.150000000000000000e+02, 1.674075274317257112e-01
1.160000000000000000e+02, 1.217720071686698297e-01
1.170000000000000000e+02, 9.801539754638352586e-02
1.180000000000000000e+02, 6.652436853914214798e-02
1.190000000000000000e+02, 4.192053312241422053e-02
1.200000000000000000e+02, 2.410588804071740754e-02
1.210000000000000000e+02, 1.576576724206832023e-02
1.220000000000000000e+02, 3.371367851410130879e-03
1.230000000000000000e+02, 2.953068040038393446e-02
1.240000000000000000e+02, 7.415560640545024174e-02
1.250000000000000000e+02, 1.508517371364358206e-01
1.260000000000000000e+02, 3.438922846643047704e-01
1.270000000000000000e+02, 7.064814378242352255e-01
1.280000000000000000e+02, 6.667448194892177105e-01
1.290000000000000000e+02, 3.188768074709515399e-01
1.300000000000000000e+02, 1.550951993379908189e-01
1.310000000000000000e+02, 1.024495728835647240e-01
1.320000000000000000e+02, 5.637670275287257060e-02
1.330000000000000000e+02, 6.130443985484034658e-02
1.340000000000000000e+02, 4.957712476191685619e-02
1.350000000000000000e+02, 4.707302515726774494e-02
1.360000000000000000e+02, 5.351072894968311733e-02
1.370000000000000000e+02, 5.613261197599360430e-02
1.380000000000000000e+02, 9.007519798483162865e-02
1.390000000000000000e+02, 1.139533036802517080e-01
1.400000000000000000e+02, 1.654698041779369966e-01
1.410000000000000000e+02, 2.148617248215858033e-01
1.420000000000000000e+02, 2.782654786452584683e-01
1.430000000000000000e+02, 3.143138862178264104e-01
1.440000000000000000e+02, 2.781654525680217205e-01
1.450000000000000000e+02, 2.081464007327533394e-01
1.460000000000000000e+02, 1.495527574708039598e-01
1.470000000000000000e+02, 9.411583983765531292e-02
1.480000000000000000e+02, 6.235976529499664273e-02
1.490000000000000000e+02, 2.747694732804248710e-02
1.500000000000000000e+02, 7.817288195676822329e-03
1.510000000000000000e+02, 1.880902077868890424e-02
1.520000000000000000e+02, 4.310860488010473390e-02
1.530000000000000000e+02, 8.222514333044046719e-02
1.540000000000000000e+02, 1.212723698889711932e-01
1.550000000000000000e+02, 1.776282873217468750e-01
1.560000000000000000e+02, 2.396364254303504082e-01
1.570000000000000000e+02, 2.953293381701050935e-01
1.580000000000000000e+02, 3.010888637596316197e-01
1.590000000000000000e+02, 2.522555655848316980e-01
1.600000000000000000e+02, 1.872797853990828543e-01
1.610000000000000000e+02, 1.321755411412221526e-01
1.620000000000000000e+02, 1.009821748768593291e-01
1.630000000000000000e+02, 6.562223323921057005e-02
1.640000000000000000e+02, 5.954099819415586275e-02
1.650000000000000000e+02, 5.702578657067845086e-02
1.660000000000000000e+02, 4.707723743384010368e-02
1.670000000000000000e+02, 4.848874256289099210e-02
1.680000000000000000e+02, 5.532927975747695126e-02
1.690000000000000000e+02, 8.285563153034047890e-02
1.700000000000000000e+02, 1.209727972979649790e-01
1.710000000000000000e+02, 2.227891772117407410e-01
1.720000000000000000e+02, 4.836369649697695450e-01
1.730000000000000000e+02, 7.790113199703830871e-01
1.740000000000000000e+02, 5.094512410201851305e-01
1.750000000000000000e+02, 2.271860849008781325e-01
1.760000000000000000e+02, 1.034546050551042734e-01
1.770000000000000000e+02, 5.633446732303403620e-02
1.780000000000000000e+02, 1.595655415876519670e-02
1.790000000000000000e+02, 6.926899637992782986e-03
1.800000000000000000e+02, 1.712716748685760154e-02
1.810000000000000000e+02, 3.402507326668605808e-02
1.820000000000000000e+02, 6.536846260622194982e-02
1.830000000000000000e+02, 7.839788411689027625e-02
1.840000000000000000e+02, 1.056497823103887124e-01
1.850000000000000000e+02, 1.484571854622266096e-01
1.860000000000000000e+02, 1.970897137176183533e-01
1.870000000000000000e+02, 2.306467969570552834e-01
1.880000000000000000e+02, 2.435444996964788167e-01
1.890000000000000000e+02, 2.291009110754743117e-01
1.900000000000000000e+02, 1.796562314754968914e-01
1.910000000000000000e+02, 1.374695879548576694e-01
1.920000000000000000e+02, 1.063210147590255283e-01
1.930000000000000000e+02, 6.861665799952897105e-02
1.940000000000000000e+02, 5.011058877715052901e-02
};

\addlegendentry{sensor-rotation-0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=sensor-rotation-1, color=sensor-rotation-1Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 1.508690107919590830e-02
1.000000000000000000e+00, 3.906415292805334033e-02
2.000000000000000000e+00, 6.320208050572552472e-02
3.000000000000000000e+00, 1.076548433186787224e-01
4.000000000000000000e+00, 1.614549132751362526e-01
5.000000000000000000e+00, 2.218614634518624174e-01
6.000000000000000000e+00, 2.910093118693751757e-01
7.000000000000000000e+00, 3.153271895612165254e-01
8.000000000000000000e+00, 2.581950137926996569e-01
9.000000000000000000e+00, 2.049764049451025250e-01
1.000000000000000000e+01, 1.543930841891563155e-01
1.100000000000000000e+01, 1.086235962410083272e-01
1.200000000000000000e+01, 8.632637459740702401e-02
1.300000000000000000e+01, 6.384332902088718509e-02
1.400000000000000000e+01, 5.170143157026375197e-02
1.500000000000000000e+01, 4.279448559779664568e-02
1.600000000000000000e+01, 3.925276108002916792e-02
1.700000000000000000e+01, 5.117228358572085273e-02
1.800000000000000000e+01, 8.072532234104837223e-02
1.900000000000000000e+01, 1.041193974549520784e-01
2.000000000000000000e+01, 1.857877414174728126e-01
2.100000000000000000e+01, 3.915842662749566827e-01
2.200000000000000000e+01, 7.545520523899972298e-01
2.300000000000000000e+01, 5.924022600440649322e-01
2.400000000000000000e+01, 2.627049457849806036e-01
2.500000000000000000e+01, 1.182746100214845386e-01
2.600000000000000000e+01, 6.109888261135106025e-02
2.700000000000000000e+01, 2.341701759862575144e-02
2.800000000000000000e+01, 1.206108434143590702e-02
2.900000000000000000e+01, 1.730604921468452059e-02
3.000000000000000000e+01, 3.217153186461648579e-02
3.100000000000000000e+01, 4.600324281401051846e-02
3.200000000000000000e+01, 6.834499558249898521e-02
3.300000000000000000e+01, 9.414324836429818766e-02
3.400000000000000000e+01, 1.466591494807059082e-01
3.500000000000000000e+01, 1.903209641076589465e-01
3.600000000000000000e+01, 2.324386263498944283e-01
3.700000000000000000e+01, 2.479910996992718275e-01
3.800000000000000000e+01, 2.353074417509080918e-01
3.900000000000000000e+01, 1.901301662602915832e-01
4.000000000000000000e+01, 1.439458721325251600e-01
4.100000000000000000e+01, 1.025987837467278868e-01
4.200000000000000000e+01, 6.809902025209077503e-02
4.300000000000000000e+01, 4.962920121557463926e-02
4.400000000000000000e+01, 3.391861243503112300e-02
4.500000000000000000e+01, 1.594196015215471399e-02
4.600000000000000000e+01, 9.248167626360210072e-03
4.700000000000000000e+01, 1.907973733979359890e-02
4.800000000000000000e+01, 6.019562051702329053e-02
4.900000000000000000e+01, 1.169694500630860390e-01
5.000000000000000000e+01, 2.602171370134991890e-01
5.100000000000000000e+01, 5.857901381080041769e-01
5.200000000000000000e+01, 7.667301574721766544e-01
5.300000000000000000e+01, 4.090034939594826557e-01
5.400000000000000000e+01, 1.918608215461221622e-01
5.500000000000000000e+01, 1.062800741947536320e-01
5.600000000000000000e+01, 7.376504519886853406e-02
5.700000000000000000e+01, 5.150055920406441945e-02
5.800000000000000000e+01, 4.532956978290388073e-02
5.900000000000000000e+01, 5.092749530518189682e-02
6.000000000000000000e+01, 5.298979012463381905e-02
6.100000000000000000e+01, 6.347253803488919766e-02
6.200000000000000000e+01, 8.490058972387483360e-02
6.300000000000000000e+01, 1.081210784655399909e-01
6.400000000000000000e+01, 1.516073558732136950e-01
6.500000000000000000e+01, 2.150011684769297660e-01
6.600000000000000000e+01, 2.707681494607517836e-01
6.700000000000000000e+01, 3.179949515077654665e-01
6.800000000000000000e+01, 2.890844730962867648e-01
6.900000000000000000e+01, 2.146473605188231604e-01
7.000000000000000000e+01, 1.492547604571685116e-01
7.100000000000000000e+01, 9.760771559673230013e-02
7.200000000000000000e+01, 5.909826036522421860e-02
7.300000000000000000e+01, 3.365056648960918634e-02
7.400000000000000000e+01, 4.530379372687274447e-03
7.500000000000000000e+01, 1.371184154549260487e-02
7.600000000000000000e+01, 4.295176621604211709e-02
7.700000000000000000e+01, 7.416760481147056938e-02
7.800000000000000000e+01, 1.149114584993886773e-01
7.900000000000000000e+01, 1.738633449209354975e-01
8.000000000000000000e+01, 2.427285902427659126e-01
8.100000000000000000e+01, 2.957154031168546804e-01
8.200000000000000000e+01, 3.005627210728751830e-01
8.300000000000000000e+01, 2.579694902872509688e-01
8.400000000000000000e+01, 1.795121136021679276e-01
8.500000000000000000e+01, 1.391319844415111195e-01
8.600000000000000000e+01, 1.031181243868110886e-01
8.700000000000000000e+01, 8.038553212182923680e-02
8.800000000000000000e+01, 5.804269976094320743e-02
8.900000000000000000e+01, 5.667694860174512378e-02
9.000000000000000000e+01, 5.502349050301071770e-02
9.100000000000000000e+01, 5.891551709020444866e-02
9.200000000000000000e+01, 6.729578795478931286e-02
9.300000000000000000e+01, 8.466172882056152704e-02
9.400000000000000000e+01, 1.253938025318009353e-01
9.500000000000000000e+01, 2.488715854767583613e-01
9.600000000000000000e+01, 5.349704817934578527e-01
9.700000000000000000e+01, 7.763474334989719505e-01
9.800000000000000000e+01, 4.507299230796870670e-01
9.900000000000000000e+01, 1.851080520683390240e-01
1.000000000000000000e+02, 9.549195149902497959e-02
1.010000000000000000e+02, 4.656699704245052113e-02
1.020000000000000000e+02, 2.987574375183514250e-02
1.030000000000000000e+02, 1.010154465895072608e-02
1.040000000000000000e+02, 2.077592628430863578e-02
1.050000000000000000e+02, 5.072205529079075459e-02
1.060000000000000000e+02, 6.356336828996832222e-02
1.070000000000000000e+02, 7.663354155650804744e-02
1.080000000000000000e+02, 1.123661116146753708e-01
1.090000000000000000e+02, 1.576076959570890113e-01
1.100000000000000000e+02, 2.028024687805620174e-01
1.110000000000000000e+02, 2.382776540076694538e-01
1.120000000000000000e+02, 2.453415252011469649e-01
1.130000000000000000e+02, 2.164063301467232525e-01
1.140000000000000000e+02, 1.750805432094329483e-01
1.150000000000000000e+02, 1.359623158031855183e-01
1.160000000000000000e+02, 9.565907439067505846e-02
1.170000000000000000e+02, 6.663952157022635936e-02
1.180000000000000000e+02, 4.388044317141515105e-02
1.190000000000000000e+02, 2.708759608653884404e-02
1.200000000000000000e+02, 1.007489374128207882e-02
1.210000000000000000e+02, 9.039314689624419752e-03
1.220000000000000000e+02, 2.980980020322251609e-02
1.230000000000000000e+02, 7.451347989677932493e-02
1.240000000000000000e+02, 1.568096617705133644e-01
1.250000000000000000e+02, 3.581155784875736381e-01
1.260000000000000000e+02, 7.168301216617586347e-01
1.270000000000000000e+02, 6.427381384658035213e-01
1.280000000000000000e+02, 3.006432760032608509e-01
1.290000000000000000e+02, 1.506554173265242103e-01
1.300000000000000000e+02, 9.123578139255217323e-02
1.310000000000000000e+02, 6.196041492505677262e-02
1.320000000000000000e+02, 5.368444724423522552e-02
1.330000000000000000e+02, 4.516704941150954944e-02
1.340000000000000000e+02, 5.508368737968809964e-02
1.350000000000000000e+02, 5.399284536640839433e-02
1.360000000000000000e+02, 6.597804197095177847e-02
1.370000000000000000e+02, 8.709991091611740677e-02
1.380000000000000000e+02, 1.240137126780668786e-01
1.390000000000000000e+02, 1.723817586992461015e-01
1.400000000000000000e+02, 2.282902989377576797e-01
1.410000000000000000e+02, 2.861196543192716657e-01
1.420000000000000000e+02, 3.014943526539495822e-01
1.430000000000000000e+02, 2.635945471749464586e-01
1.440000000000000000e+02, 1.908504585860120173e-01
1.450000000000000000e+02, 1.368694047979933104e-01
1.460000000000000000e+02, 8.551017076575183340e-02
1.470000000000000000e+02, 4.164207219583807018e-02
1.480000000000000000e+02, 2.728410697396630585e-02
1.490000000000000000e+02, 7.182148498815901089e-03
1.500000000000000000e+02, 2.855171436904332255e-02
1.510000000000000000e+02, 5.271682732707620722e-02
1.520000000000000000e+02, 8.463080177252264857e-02
1.530000000000000000e+02, 1.361114175699542073e-01
1.540000000000000000e+02, 1.961422232605656013e-01
1.550000000000000000e+02, 2.678495602228466166e-01
1.560000000000000000e+02, 3.098097871487597299e-01
1.570000000000000000e+02, 2.913176959007913180e-01
1.580000000000000000e+02, 2.187575718955243331e-01
1.590000000000000000e+02, 1.676666647027190427e-01
1.600000000000000000e+02, 1.159372429467301902e-01
1.610000000000000000e+02, 9.177331706658198307e-02
1.620000000000000000e+02, 7.094662570222950992e-02
1.630000000000000000e+02, 5.945067058043630726e-02
1.640000000000000000e+02, 4.965471495686345216e-02
1.650000000000000000e+02, 4.741500914408788847e-02
1.660000000000000000e+02, 5.526445081999725034e-02
1.670000000000000000e+02, 6.238860562918151220e-02
1.680000000000000000e+02, 8.983528188940445580e-02
1.690000000000000000e+02, 1.547783350269129887e-01
1.700000000000000000e+02, 3.258007665926438978e-01
1.710000000000000000e+02, 6.849684240686149117e-01
1.720000000000000000e+02, 6.997518343261597273e-01
1.730000000000000000e+02, 3.349545208873762614e-01
1.740000000000000000e+02, 1.492178114176435921e-01
1.750000000000000000e+02, 6.587131941687227044e-02
1.760000000000000000e+02, 3.010943273339793114e-02
1.770000000000000000e+02, 1.263479534478861507e-02
1.780000000000000000e+02, 9.753253633085504082e-03
1.790000000000000000e+02, 3.089279674686708915e-02
1.800000000000000000e+02, 4.839109543777671968e-02
1.810000000000000000e+02, 7.041095450121695465e-02
1.820000000000000000e+02, 9.651019894876253225e-02
1.830000000000000000e+02, 1.391073410679360134e-01
1.840000000000000000e+02, 1.744850851336825492e-01
1.850000000000000000e+02, 2.219446731286351671e-01
1.860000000000000000e+02, 2.481561785940282761e-01
1.870000000000000000e+02, 2.353275667293053541e-01
1.880000000000000000e+02, 2.011436452721866719e-01
1.890000000000000000e+02, 1.516450684621967471e-01
1.900000000000000000e+02, 1.188040102885787319e-01
1.910000000000000000e+02, 8.426966881655989505e-02
1.920000000000000000e+02, 5.699670732747300073e-02
1.930000000000000000e+02, 3.854694007368408837e-02
1.940000000000000000e+02, 1.690414911883655891e-02
};

\addlegendentry{sensor-rotation-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/ramp_low_uncertainty.tex <==
\addplot [name path=uncertainty, color=uncertaintyColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 7.959463664519113024e+00
1.100000000000000000e+01, 9.866460019643547241e+00
1.200000000000000000e+01, 1.411880459024650492e+01
1.300000000000000000e+01, 2.121012664460637964e+01
1.400000000000000000e+01, 3.388983609764329685e+01
1.500000000000000000e+01, 5.430392683869818882e+01
1.600000000000000000e+01, 7.992438030316219510e+01
1.700000000000000000e+01, 7.333594024320339599e+01
1.800000000000000000e+01, 3.678899185793707716e+01
1.900000000000000000e+01, 1.666204792575915761e+01
2.000000000000000000e+01, 7.053955985938115347e+00
2.100000000000000000e+01, 2.749678897798997212e+00
2.200000000000000000e+01, 1.503818071028947934e+00
2.300000000000000000e+01, 2.188494790989945926e+00
2.400000000000000000e+01, 1.573324337495142888e+00
2.500000000000000000e+01, 2.249941000262642099e+00
2.600000000000000000e+01, 4.348843529739950142e+00
2.700000000000000000e+01, 8.861519261654388302e+00
2.800000000000000000e+01, 1.682172002343967065e+01
2.900000000000000000e+01, 3.529395543023528603e+01
3.000000000000000000e+01, 3.091140194752825465e+01
3.100000000000000000e+01, 2.554946542147692412e+01
3.200000000000000000e+01, 2.090352781876764254e+01
3.300000000000000000e+01, 1.647193832448203210e+01
3.400000000000000000e+01, 1.288475000521677671e+01
3.500000000000000000e+01, 1.079572950285608179e+01
3.600000000000000000e+01, 1.060415303322866798e+01
3.700000000000000000e+01, 1.627915022774920573e+01
3.800000000000000000e+01, 2.573436832649119310e+01
3.900000000000000000e+01, 1.443663408296411177e+01
4.000000000000000000e+01, 1.083816953950814010e+01
4.100000000000000000e+01, 1.095176411391312499e+01
4.200000000000000000e+01, 1.310677852303901147e+01
4.300000000000000000e+01, 1.652047735631696668e+01
4.400000000000000000e+01, 2.053957703834332449e+01
4.500000000000000000e+01, 2.486438418151825758e+01
4.600000000000000000e+01, 3.341175793094789981e+01
4.700000000000000000e+01, 3.159706660081602791e+01
4.800000000000000000e+01, 1.798302723806072834e+01
4.900000000000000000e+01, 9.822686895712177346e+00
5.000000000000000000e+01, 4.524663591441766108e+00
5.100000000000000000e+01, 1.922264061684807901e+00
5.200000000000000000e+01, 1.797624733536715924e+00
5.300000000000000000e+01, 1.565963469511437500e+00
5.400000000000000000e+01, 1.686040958738173279e+00
5.500000000000000000e+01, 2.923058467933455251e+00
5.600000000000000000e+01, 6.322630776314841938e+00
5.700000000000000000e+01, 1.461028848280011339e+01
5.800000000000000000e+01, 3.369192043623045407e+01
5.900000000000000000e+01, 6.698240999380598737e+01
6.000000000000000000e+01, 7.602164615838444206e+01
6.100000000000000000e+01, 5.329325020144361247e+01
6.200000000000000000e+01, 3.330063159933512651e+01
6.300000000000000000e+01, 2.087697517633267807e+01
6.400000000000000000e+01, 1.373519719595342536e+01
6.500000000000000000e+01, 9.519216794188995578e+00
6.600000000000000000e+01, 7.617088614191729334e+00
6.700000000000000000e+01, 8.968748731873926516e+00
6.800000000000000000e+01, 1.711089243683886707e+01
6.900000000000000000e+01, 9.978863905920775323e+00
7.000000000000000000e+01, 7.283872880989616050e+00
7.100000000000000000e+01, 7.639000544625781153e+00
7.200000000000000000e+01, 9.507758255750271559e+00
7.300000000000000000e+01, 1.253376383362902047e+01
7.400000000000000000e+01, 1.608571453388218941e+01
7.500000000000000000e+01, 2.782587066869012205e+01
7.600000000000000000e+01, 2.232124529421944459e+01
7.700000000000000000e+01, 1.663500806804114518e+01
7.800000000000000000e+01, 1.260808544781255947e+01
7.900000000000000000e+01, 9.401988997024032457e+00
8.000000000000000000e+01, 7.415731851033361188e+00
8.100000000000000000e+01, 7.252810424106730380e+00
8.200000000000000000e+01, 1.282849116537145484e+01
8.300000000000000000e+01, 1.337239042908503350e+01
8.400000000000000000e+01, 8.580219075274845508e+00
8.500000000000000000e+01, 7.997855247068681450e+00
8.600000000000000000e+01, 9.776601573141332935e+00
8.700000000000000000e+01, 1.362541042569779748e+01
8.800000000000000000e+01, 2.064278755867387360e+01
8.900000000000000000e+01, 3.293622009923622329e+01
9.000000000000000000e+01, 5.318842425606206348e+01
9.100000000000000000e+01, 7.697888337157405658e+01
9.200000000000000000e+01, 6.881184435528425070e+01
9.300000000000000000e+01, 3.516777473910815388e+01
9.400000000000000000e+01, 1.569101269269315679e+01
9.500000000000000000e+01, 6.585726616366414987e+00
9.600000000000000000e+01, 2.627247265744888871e+00
9.700000000000000000e+01, 1.739671222623750069e+00
9.800000000000000000e+01, 1.883021381548835693e+00
9.900000000000000000e+01, 1.578534190850979790e+00
1.000000000000000000e+02, 2.212111792666793697e+00
1.010000000000000000e+02, 4.192140645782457042e+00
1.020000000000000000e+02, 8.515955900237191400e+00
1.030000000000000000e+02, 1.727999231566393945e+01
1.040000000000000000e+02, 3.277808550725401915e+01
1.050000000000000000e+02, 3.010954460389894294e+01
1.060000000000000000e+02, 2.499526150104072286e+01
1.070000000000000000e+02, 2.054414032317507122e+01
1.080000000000000000e+02, 1.632079571218808667e+01
1.090000000000000000e+02, 1.290831120244366836e+01
1.100000000000000000e+02, 1.086189735943872137e+01
1.110000000000000000e+02, 1.106469847943158058e+01
1.120000000000000000e+02, 1.697487621622607534e+01
1.130000000000000000e+02, 2.368813618621385331e+01
1.140000000000000000e+02, 1.484876000373946781e+01
1.150000000000000000e+02, 1.115072203811077145e+01
1.160000000000000000e+02, 1.116854684907319495e+01
1.170000000000000000e+02, 1.307287227226115434e+01
1.180000000000000000e+02, 1.628586824809044487e+01
1.190000000000000000e+02, 2.026988901989437508e+01
1.200000000000000000e+02, 2.442443253994800756e+01
1.210000000000000000e+02, 3.567250527575385632e+01
1.220000000000000000e+02, 3.386569991003226932e+01
1.230000000000000000e+02, 1.768628157481393970e+01
1.240000000000000000e+02, 9.074006333316962269e+00
1.250000000000000000e+02, 4.062539029280385350e+00
1.260000000000000000e+02, 1.979065866550232977e+00
1.270000000000000000e+02, 1.934258049916436351e+00
1.280000000000000000e+02, 2.196284720130664336e+00
1.290000000000000000e+02, 1.919276429292605002e+00
1.300000000000000000e+02, 2.903875626320260750e+00
1.310000000000000000e+02, 5.889672635206244955e+00
1.320000000000000000e+02, 1.340866508503711430e+01
1.330000000000000000e+02, 3.037564504330730131e+01
1.340000000000000000e+02, 6.108654682064825181e+01
1.350000000000000000e+02, 7.197941754883386523e+01
1.360000000000000000e+02, 5.042734187332585805e+01
1.370000000000000000e+02, 3.178301608638844300e+01
1.380000000000000000e+02, 2.059425002440517005e+01
1.390000000000000000e+02, 1.343145179271402156e+01
1.400000000000000000e+02, 9.538405812314071142e+00
1.410000000000000000e+02, 8.071656775336739642e+00
1.420000000000000000e+02, 1.008893101130907510e+01
1.430000000000000000e+02, 1.192530843073596714e+01
1.440000000000000000e+02, 9.872423338287827477e+00
1.450000000000000000e+02, 7.670952996147332392e+00
1.460000000000000000e+02, 7.831817828042446195e+00
1.470000000000000000e+02, 9.522817187229950520e+00
1.480000000000000000e+02, 1.232752375240761467e+01
1.490000000000000000e+02, 1.675229626433310770e+01
1.500000000000000000e+02, 2.029671026041587467e+01
1.510000000000000000e+02, 2.275680381568573551e+01
1.520000000000000000e+02, 1.674266814894028954e+01
1.530000000000000000e+02, 1.243463004007832140e+01
1.540000000000000000e+02, 9.320822201825397002e+00
1.550000000000000000e+02, 7.633990776548652768e+00
1.560000000000000000e+02, 7.992244955718676991e+00
1.570000000000000000e+02, 1.030580986740481464e+01
1.580000000000000000e+02, 1.278391494931388195e+01
1.590000000000000000e+02, 9.330106389991275506e+00
1.600000000000000000e+02, 8.401320180970447637e+00
1.610000000000000000e+02, 9.851708391612874038e+00
1.620000000000000000e+02, 1.351582446341371835e+01
1.630000000000000000e+02, 2.006723478011807771e+01
1.640000000000000000e+02, 3.170503184375695227e+01
1.650000000000000000e+02, 5.012827432749305956e+01
1.660000000000000000e+02, 7.175703295176876395e+01
1.670000000000000000e+02, 5.929841978253161727e+01
1.680000000000000000e+02, 3.091177656644195082e+01
1.690000000000000000e+02, 1.366195720514522449e+01
1.700000000000000000e+02, 5.495823604545122976e+00
1.710000000000000000e+02, 2.453338242342122388e+00
1.720000000000000000e+02, 2.794248401147239935e+00
1.730000000000000000e+02, 1.639119843968405377e+00
1.740000000000000000e+02, 1.781150877183687253e+00
1.750000000000000000e+02, 2.209515654944135044e+00
1.760000000000000000e+02, 3.840693943870440386e+00
1.770000000000000000e+02, 7.618420294610355192e+00
1.780000000000000000e+02, 1.620732244170149627e+01
1.790000000000000000e+02, 2.524628745458365486e+01
1.800000000000000000e+02, 2.909775415885411931e+01
1.810000000000000000e+02, 2.483614980706535746e+01
1.820000000000000000e+02, 2.039516690841107760e+01
1.830000000000000000e+02, 1.611714506357191823e+01
1.840000000000000000e+02, 1.294859747945513462e+01
1.850000000000000000e+02, 1.133334830932770032e+01
1.860000000000000000e+02, 1.211209798311671904e+01
1.870000000000000000e+02, 1.595217368332947139e+01
1.880000000000000000e+02, 1.724270115339777121e+01
1.890000000000000000e+02, 1.489123107450116557e+01
1.900000000000000000e+02, 1.188125147632795020e+01
1.910000000000000000e+02, 1.160126497405506996e+01
1.920000000000000000e+02, 1.313597852321434978e+01
1.930000000000000000e+02, 1.608714225102222173e+01
1.940000000000000000e+02, 2.013577948664548600e+01
};

\addlegendentry{uncertainty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_high_error.tex <==
\addplot [name path=error, color=errorColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 2.000000000000010450e-02
1.100000000000000000e+01, 2.000000000000010450e-02
1.200000000000000000e+01, 2.000000000000010450e-02
1.300000000000000000e+01, 3.000000000000010297e-02
1.400000000000000000e+01, 3.000000000000010297e-02
1.500000000000000000e+01, 3.000000000000010297e-02
1.600000000000000000e+01, 3.000000000000010297e-02
1.700000000000000000e+01, 3.000000000000010297e-02
1.800000000000000000e+01, 3.500000000000010048e-02
1.900000000000000000e+01, 2.000000000000010450e-02
2.000000000000000000e+01, 2.000000000000010450e-02
2.100000000000000000e+01, 1.000000000000010429e-02
2.200000000000000000e+01, 1.000000000000010429e-02
2.300000000000000000e+01, 1.000000000000010429e-02
2.400000000000000000e+01, 1.000000000000010429e-02
2.500000000000000000e+01, 1.000000000000010429e-02
2.600000000000000000e+01, 1.000000000000010429e-02
2.700000000000000000e+01, 1.000000000000010429e-02
2.800000000000000000e+01, 1.000000000000010429e-02
2.900000000000000000e+01, 1.000000000000010429e-02
3.000000000000000000e+01, 1.000000000000010429e-02
3.100000000000000000e+01, 1.000000000000010429e-02
3.200000000000000000e+01, 1.000000000000010429e-02
3.300000000000000000e+01, 1.000000000000010429e-02
3.400000000000000000e+01, 1.040834085586084257e-16
3.500000000000000000e+01, 1.040834085586084257e-16
3.600000000000000000e+01, 1.040834085586084257e-16
3.700000000000000000e+01, 9.999999999999896125e-03
3.800000000000000000e+01, 9.999999999999896125e-03
3.900000000000000000e+01, 2.000000000000010450e-02
4.000000000000000000e+01, 1.079999999999999849e+00
4.100000000000000000e+01, 9.399999999999998357e-01
4.200000000000000000e+01, 8.599999999999998757e-01
4.300000000000000000e+01, 7.799999999999998046e-01
4.400000000000000000e+01, 6.899999999999998357e-01
4.500000000000000000e+01, 5.699999999999998401e-01
4.600000000000000000e+01, 4.699999999999998623e-01
4.700000000000000000e+01, 4.299999999999998268e-01
4.800000000000000000e+01, 2.699999999999997957e-01
4.900000000000000000e+01, 5.999999999999983125e-02
5.000000000000000000e+01, 2.220446049250313081e-16
5.100000000000000000e+01, 2.220446049250313081e-16
5.200000000000000000e+01, 2.000000000000023981e-02
5.300000000000000000e+01, 9.999999999999786837e-03
5.400000000000000000e+01, 2.220446049250313081e-16
5.500000000000000000e+01, 2.220446049250313081e-16
5.600000000000000000e+01, 2.220446049250313081e-16
5.700000000000000000e+01, 2.220446049250313081e-16
5.800000000000000000e+01, 2.220446049250313081e-16
5.900000000000000000e+01, 2.220446049250313081e-16
6.000000000000000000e+01, 2.220446049250313081e-16
6.100000000000000000e+01, 2.220446049250313081e-16
6.200000000000000000e+01, 2.000000000000023981e-02
6.300000000000000000e+01, 3.000000000000024869e-02
6.400000000000000000e+01, 7.500000000000017764e-02
6.500000000000000000e+01, 6.000000000000027534e-02
6.600000000000000000e+01, 3.500000000000036415e-02
6.700000000000000000e+01, 3.000000000000024869e-02
6.800000000000000000e+01, 3.000000000000024869e-02
6.900000000000000000e+01, 3.000000000000024869e-02
7.000000000000000000e+01, 2.000000000000023981e-02
7.100000000000000000e+01, 2.000000000000023981e-02
7.200000000000000000e+01, 2.000000000000023981e-02
7.300000000000000000e+01, 2.000000000000023981e-02
7.400000000000000000e+01, 1.000000000000023093e-02
7.500000000000000000e+01, 2.000000000000023981e-02
7.600000000000000000e+01, 1.000000000000023093e-02
7.700000000000000000e+01, 1.000000000000023093e-02
7.800000000000000000e+01, 1.500000000000034639e-02
7.900000000000000000e+01, 3.500000000000036415e-02
8.000000000000000000e+01, 3.000000000000024869e-02
8.100000000000000000e+01, 4.000000000000025757e-02
8.200000000000000000e+01, 3.500000000000036415e-02
8.300000000000000000e+01, 3.000000000000024869e-02
8.400000000000000000e+01, 3.000000000000024869e-02
8.500000000000000000e+01, 3.000000000000024869e-02
8.600000000000000000e+01, 2.000000000000023981e-02
8.700000000000000000e+01, 2.000000000000023981e-02
8.800000000000000000e+01, 2.000000000000023981e-02
8.900000000000000000e+01, 2.000000000000023981e-02
9.000000000000000000e+01, 2.000000000000023981e-02
9.100000000000000000e+01, 2.000000000000023981e-02
9.200000000000000000e+01, 2.000000000000023981e-02
9.300000000000000000e+01, 1.059999999999999609e+00
9.400000000000000000e+01, 9.599999999999997424e-01
9.500000000000000000e+01, 4.299999999999997158e-01
9.600000000000000000e+01, 6.999999999999984013e-02
9.700000000000000000e+01, 9.999999999999786837e-03
9.800000000000000000e+01, 9.999999999999786837e-03
9.900000000000000000e+01, 4.440892098500626162e-16
1.000000000000000000e+02, 4.440892098500626162e-16
1.010000000000000000e+02, 4.440892098500626162e-16
1.020000000000000000e+02, 4.440892098500626162e-16
1.030000000000000000e+02, 4.440892098500626162e-16
1.040000000000000000e+02, 4.440892098500626162e-16
1.050000000000000000e+02, 4.440892098500626162e-16
1.060000000000000000e+02, 4.440892098500626162e-16
1.070000000000000000e+02, 2.000000000000046185e-02
1.080000000000000000e+02, 2.000000000000046185e-02
1.090000000000000000e+02, 7.500000000000017764e-02
1.100000000000000000e+02, 8.000000000000051514e-02
1.110000000000000000e+02, 3.500000000000014211e-02
1.120000000000000000e+02, 3.000000000000024869e-02
1.130000000000000000e+02, 3.500000000000014211e-02
1.140000000000000000e+02, 3.500000000000014211e-02
1.150000000000000000e+02, 4.000000000000047962e-02
1.160000000000000000e+02, 4.000000000000047962e-02
1.170000000000000000e+02, 4.000000000000047962e-02
1.180000000000000000e+02, 3.000000000000024869e-02
1.190000000000000000e+02, 4.500000000000037303e-02
1.200000000000000000e+02, 5.000000000000026645e-02
1.210000000000000000e+02, 4.000000000000047962e-02
1.220000000000000000e+02, 5.000000000000026645e-02
1.230000000000000000e+02, 4.000000000000047962e-02
1.240000000000000000e+02, 1.000000000000005329e-01
1.250000000000000000e+02, 6.000000000000049738e-02
1.260000000000000000e+02, 2.000000000000046185e-02
1.270000000000000000e+02, 3.000000000000024869e-02
1.280000000000000000e+02, 4.440892098500626162e-16
1.290000000000000000e+02, 1.000000000000023093e-02
1.300000000000000000e+02, 4.440892098500626162e-16
1.310000000000000000e+02, 4.440892098500626162e-16
1.320000000000000000e+02, 4.440892098500626162e-16
1.330000000000000000e+02, 4.440892098500626162e-16
1.340000000000000000e+02, 1.000000000000023093e-02
1.350000000000000000e+02, 1.000000000000023093e-02
1.360000000000000000e+02, 2.000000000000046185e-02
1.370000000000000000e+02, 5.000000000000337508e-03
1.380000000000000000e+02, 3.000000000000024869e-02
1.390000000000000000e+02, 1.000000000000005329e-01
1.400000000000000000e+02, 7.000000000000028422e-02
1.410000000000000000e+02, 5.000000000000026645e-02
1.420000000000000000e+02, 3.000000000000024869e-02
1.430000000000000000e+02, 3.000000000000024869e-02
1.440000000000000000e+02, 3.000000000000024869e-02
1.450000000000000000e+02, 3.000000000000024869e-02
1.460000000000000000e+02, 2.000000000000046185e-02
1.470000000000000000e+02, 2.000000000000046185e-02
1.480000000000000000e+02, 2.000000000000046185e-02
1.490000000000000000e+02, 3.000000000000024869e-02
1.500000000000000000e+02, 3.000000000000024869e-02
1.510000000000000000e+02, 4.000000000000047962e-02
1.520000000000000000e+02, 5.000000000000026645e-02
1.530000000000000000e+02, 5.000000000000026645e-02
1.540000000000000000e+02, 5.000000000000026645e-02
1.550000000000000000e+02, 2.350000000000000089e+00
1.560000000000000000e+02, 2.340000000000000302e+00
1.570000000000000000e+02, 2.330000000000000071e+00
1.580000000000000000e+02, 2.459999999999999964e+00
1.590000000000000000e+02, 2.360000000000000320e+00
1.600000000000000000e+02, 2.360000000000000320e+00
1.610000000000000000e+02, 4.000000000000001332e-01
1.620000000000000000e+02, 9.000000000000010769e-02
1.630000000000000000e+02, 7.000000000000010381e-02
1.640000000000000000e+02, 5.000000000000010686e-02
1.650000000000000000e+02, 9.999999999999896125e-03
1.660000000000000000e+02, 2.000000000000010450e-02
1.670000000000000000e+02, 2.000000000000010450e-02
1.680000000000000000e+02, 3.000000000000010297e-02
1.690000000000000000e+02, 4.000000000000010492e-02
1.700000000000000000e+02, 4.500000000000010936e-02
1.710000000000000000e+02, 5.000000000000010686e-02
1.720000000000000000e+02, 1.040834085586084257e-16
1.730000000000000000e+02, 1.000000000000010429e-02
1.740000000000000000e+02, 1.000000000000010429e-02
1.750000000000000000e+02, 1.000000000000010429e-02
1.760000000000000000e+02, 1.000000000000010429e-02
1.770000000000000000e+02, 1.000000000000010429e-02
1.780000000000000000e+02, 1.000000000000010429e-02
1.790000000000000000e+02, 1.000000000000010429e-02
1.800000000000000000e+02, 1.000000000000010429e-02
1.810000000000000000e+02, 1.000000000000010429e-02
1.820000000000000000e+02, 1.000000000000010429e-02
1.830000000000000000e+02, 1.000000000000010429e-02
1.840000000000000000e+02, 1.000000000000010429e-02
1.850000000000000000e+02, 1.000000000000010429e-02
1.860000000000000000e+02, 2.000000000000010450e-02
1.870000000000000000e+02, 1.000000000000010429e-02
1.880000000000000000e+02, 3.000000000000010297e-02
1.890000000000000000e+02, 3.000000000000010297e-02
1.900000000000000000e+02, 4.000000000000010492e-02
1.910000000000000000e+02, 3.500000000000010048e-02
1.920000000000000000e+02, 2.500000000000010547e-02
1.930000000000000000e+02, 1.000000000000010429e-02
1.940000000000000000e+02, 2.000000000000010450e-02
};

\addlegendentry{error}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_high_estimation.tex <==
\addplot [name path=estimationlower, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, -1.099999999999999034e-01
1.100000000000000000e+01, -1.099999999999999034e-01
1.200000000000000000e+01, -1.099999999999999034e-01
1.300000000000000000e+01, -1.199999999999998984e-01
1.400000000000000000e+01, -1.199999999999998984e-01
1.500000000000000000e+01, -1.499999999999999112e-01
1.600000000000000000e+01, -1.799999999999999101e-01
1.700000000000000000e+01, -1.899999999999998912e-01
1.800000000000000000e+01, -1.999999999999999001e-01
1.900000000000000000e+01, -2.599999999999998979e-01
2.000000000000000000e+01, -1.599999999999998923e-01
2.100000000000000000e+01, -4.999999999999989869e-02
2.200000000000000000e+01, -2.999999999999989481e-02
2.300000000000000000e+01, -2.999999999999989481e-02
2.400000000000000000e+01, -1.999999999999989633e-02
2.500000000000000000e+01, -1.999999999999989633e-02
2.600000000000000000e+01, -1.999999999999989633e-02
2.700000000000000000e+01, -1.999999999999989633e-02
2.800000000000000000e+01, -1.999999999999989633e-02
2.900000000000000000e+01, -1.999999999999989633e-02
3.000000000000000000e+01, -1.999999999999989633e-02
3.100000000000000000e+01, -1.999999999999989633e-02
3.200000000000000000e+01, -2.999999999999989481e-02
3.300000000000000000e+01, -2.999999999999989481e-02
3.400000000000000000e+01, -9.999999999999989453e-02
3.500000000000000000e+01, -2.299999999999998990e-01
3.600000000000000000e+01, -2.499999999999998890e-01
3.700000000000000000e+01, -2.399999999999999079e-01
3.800000000000000000e+01, -2.399999999999999079e-01
3.900000000000000000e+01, -2.199999999999998901e-01
4.000000000000000000e+01, -1.199999999999998984e-01
4.100000000000000000e+01, 1.000000000000001027e-01
4.200000000000000000e+01, 1.800000000000001044e-01
4.300000000000000000e+01, 2.500000000000001110e-01
4.400000000000000000e+01, 3.300000000000001266e-01
4.500000000000000000e+01, 3.900000000000001243e-01
4.600000000000000000e+01, 4.600000000000001310e-01
4.700000000000000000e+01, 5.200000000000001288e-01
4.800000000000000000e+01, 6.800000000000001599e-01
4.900000000000000000e+01, 9.600000000000000755e-01
5.000000000000000000e+01, 1.100000000000000089e+00
5.100000000000000000e+01, 1.150000000000000133e+00
5.200000000000000000e+01, 1.170000000000000151e+00
5.300000000000000000e+01, 1.150000000000000133e+00
5.400000000000000000e+01, 1.170000000000000151e+00
5.500000000000000000e+01, 1.170000000000000151e+00
5.600000000000000000e+01, 1.170000000000000151e+00
5.700000000000000000e+01, 1.170000000000000151e+00
5.800000000000000000e+01, 1.170000000000000151e+00
5.900000000000000000e+01, 1.170000000000000151e+00
6.000000000000000000e+01, 1.160000000000000142e+00
6.100000000000000000e+01, 1.160000000000000142e+00
6.200000000000000000e+01, 1.170000000000000151e+00
6.300000000000000000e+01, 1.120000000000000107e+00
6.400000000000000000e+01, 1.030000000000000027e+00
6.500000000000000000e+01, 1.020000000000000018e+00
6.600000000000000000e+01, 1.040000000000000036e+00
6.700000000000000000e+01, 1.060000000000000053e+00
6.800000000000000000e+01, 1.070000000000000062e+00
6.900000000000000000e+01, 1.080000000000000071e+00
7.000000000000000000e+01, 1.090000000000000080e+00
7.100000000000000000e+01, 1.100000000000000089e+00
7.200000000000000000e+01, 1.100000000000000089e+00
7.300000000000000000e+01, 1.100000000000000089e+00
7.400000000000000000e+01, 1.100000000000000089e+00
7.500000000000000000e+01, 1.080000000000000071e+00
7.600000000000000000e+01, 1.060000000000000053e+00
7.700000000000000000e+01, 1.070000000000000062e+00
7.800000000000000000e+01, 1.067500000000000115e+00
7.900000000000000000e+01, 1.060000000000000053e+00
8.000000000000000000e+01, 1.080000000000000071e+00
8.100000000000000000e+01, 1.070000000000000062e+00
8.200000000000000000e+01, 1.090000000000000080e+00
8.300000000000000000e+01, 1.080000000000000071e+00
8.400000000000000000e+01, 1.090000000000000080e+00
8.500000000000000000e+01, 1.100000000000000089e+00
8.600000000000000000e+01, 1.100000000000000089e+00
8.700000000000000000e+01, 1.090000000000000080e+00
8.800000000000000000e+01, 1.090000000000000080e+00
8.900000000000000000e+01, 1.080000000000000071e+00
9.000000000000000000e+01, 1.060000000000000053e+00
9.100000000000000000e+01, 1.050000000000000044e+00
9.200000000000000000e+01, 1.047500000000000098e+00
9.300000000000000000e+01, 1.050000000000000044e+00
9.400000000000000000e+01, 1.150000000000000133e+00
9.500000000000000000e+01, 1.680000000000000160e+00
9.600000000000000000e+01, 2.120000000000000107e+00
9.700000000000000000e+01, 2.240000000000000213e+00
9.800000000000000000e+01, 2.250000000000000000e+00
9.900000000000000000e+01, 2.260000000000000231e+00
1.000000000000000000e+02, 2.270000000000000018e+00
1.010000000000000000e+02, 2.270000000000000018e+00
1.020000000000000000e+02, 2.270000000000000018e+00
1.030000000000000000e+02, 2.270000000000000018e+00
1.040000000000000000e+02, 2.270000000000000018e+00
1.050000000000000000e+02, 2.270000000000000018e+00
1.060000000000000000e+02, 2.260000000000000231e+00
1.070000000000000000e+02, 2.260000000000000231e+00
1.080000000000000000e+02, 2.200000000000000178e+00
1.090000000000000000e+02, 2.110000000000000320e+00
1.100000000000000000e+02, 2.060000000000000053e+00
1.110000000000000000e+02, 2.100000000000000089e+00
1.120000000000000000e+02, 2.120000000000000107e+00
1.130000000000000000e+02, 2.120000000000000107e+00
1.140000000000000000e+02, 2.130000000000000338e+00
1.150000000000000000e+02, 2.140000000000000124e+00
1.160000000000000000e+02, 2.160000000000000142e+00
1.170000000000000000e+02, 2.169999999999999929e+00
1.180000000000000000e+02, 2.169999999999999929e+00
1.190000000000000000e+02, 2.160000000000000142e+00
1.200000000000000000e+02, 2.137500000000000178e+00
1.210000000000000000e+02, 2.140000000000000124e+00
1.220000000000000000e+02, 2.140000000000000124e+00
1.230000000000000000e+02, 2.110000000000000320e+00
1.240000000000000000e+02, 2.100000000000000089e+00
1.250000000000000000e+02, 2.130000000000000338e+00
1.260000000000000000e+02, 2.220000000000000195e+00
1.270000000000000000e+02, 2.290000000000000036e+00
1.280000000000000000e+02, 2.260000000000000231e+00
1.290000000000000000e+02, 2.270000000000000018e+00
1.300000000000000000e+02, 2.270000000000000018e+00
1.310000000000000000e+02, 2.280000000000000249e+00
1.320000000000000000e+02, 2.270000000000000018e+00
1.330000000000000000e+02, 2.270000000000000018e+00
1.340000000000000000e+02, 2.270000000000000018e+00
1.350000000000000000e+02, 2.260000000000000231e+00
1.360000000000000000e+02, 2.280000000000000249e+00
1.370000000000000000e+02, 2.250000000000000000e+00
1.380000000000000000e+02, 2.189999999999999947e+00
1.390000000000000000e+02, 2.070000000000000284e+00
1.400000000000000000e+02, 1.987500000000000266e+00
1.410000000000000000e+02, 2.080000000000000071e+00
1.420000000000000000e+02, 2.140000000000000124e+00
1.430000000000000000e+02, 2.140000000000000124e+00
1.440000000000000000e+02, 2.147500000000000409e+00
1.450000000000000000e+02, 2.160000000000000142e+00
1.460000000000000000e+02, 2.180000000000000160e+00
1.470000000000000000e+02, 2.189999999999999947e+00
1.480000000000000000e+02, 2.200000000000000178e+00
1.490000000000000000e+02, 2.200000000000000178e+00
1.500000000000000000e+02, 2.180000000000000160e+00
1.510000000000000000e+02, 2.180000000000000160e+00
1.520000000000000000e+02, 2.189999999999999947e+00
1.530000000000000000e+02, 2.189999999999999947e+00
1.540000000000000000e+02, 2.160000000000000142e+00
1.550000000000000000e+02, 2.140000000000000124e+00
1.560000000000000000e+02, 2.160000000000000142e+00
1.570000000000000000e+02, 2.169999999999999929e+00
1.580000000000000000e+02, 2.310000000000000053e+00
1.590000000000000000e+02, 2.160000000000000142e+00
1.600000000000000000e+02, 2.169999999999999929e+00
1.610000000000000000e+02, 6.000000000000010880e-02
1.620000000000000000e+02, -4.999999999999989869e-02
1.630000000000000000e+02, -8.999999999999989952e-02
1.640000000000000000e+02, -1.399999999999999023e-01
1.650000000000000000e+02, -1.599999999999998923e-01
1.660000000000000000e+02, -1.299999999999998934e-01
1.670000000000000000e+02, -1.499999999999999112e-01
1.680000000000000000e+02, -1.699999999999999012e-01
1.690000000000000000e+02, -1.899999999999998912e-01
1.700000000000000000e+02, -2.499999999999998890e-01
1.710000000000000000e+02, -2.499999999999998890e-01
1.720000000000000000e+02, -1.099999999999999034e-01
1.730000000000000000e+02, -3.999999999999989675e-02
1.740000000000000000e+02, -2.999999999999989481e-02
1.750000000000000000e+02, -1.999999999999989633e-02
1.760000000000000000e+02, -1.999999999999989633e-02
1.770000000000000000e+02, -1.999999999999989633e-02
1.780000000000000000e+02, -1.999999999999989633e-02
1.790000000000000000e+02, -1.999999999999989633e-02
1.800000000000000000e+02, -1.999999999999989633e-02
1.810000000000000000e+02, -1.999999999999989633e-02
1.820000000000000000e+02, -1.999999999999989633e-02
1.830000000000000000e+02, -2.999999999999989481e-02
1.840000000000000000e+02, -3.999999999999989675e-02
1.850000000000000000e+02, -4.999999999999989869e-02
1.860000000000000000e+02, -1.599999999999998923e-01
1.870000000000000000e+02, -2.199999999999998901e-01
1.880000000000000000e+02, -2.199999999999998901e-01
1.890000000000000000e+02, -2.099999999999999090e-01
1.900000000000000000e+02, -2.099999999999999090e-01
1.910000000000000000e+02, -1.899999999999998912e-01
1.920000000000000000e+02, -1.899999999999998912e-01
1.930000000000000000e+02, -1.799999999999999101e-01
1.940000000000000000e+02, -1.724999999999999034e-01
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationupper, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 1.325000000000001177e-01
1.100000000000000000e+01, 1.400000000000000966e-01
1.200000000000000000e+01, 1.425000000000000988e-01
1.300000000000000000e+01, 1.500000000000001055e-01
1.400000000000000000e+01, 1.700000000000000955e-01
1.500000000000000000e+01, 1.900000000000001132e-01
1.600000000000000000e+01, 2.100000000000001033e-01
1.700000000000000000e+01, 2.300000000000001210e-01
1.800000000000000000e+01, 2.600000000000001199e-01
1.900000000000000000e+01, 3.300000000000001266e-01
2.000000000000000000e+01, 2.100000000000001033e-01
2.100000000000000000e+01, 7.250000000000010603e-02
2.200000000000000000e+01, 5.000000000000010686e-02
2.300000000000000000e+01, 5.000000000000010686e-02
2.400000000000000000e+01, 4.000000000000010492e-02
2.500000000000000000e+01, 4.000000000000010492e-02
2.600000000000000000e+01, 4.000000000000010492e-02
2.700000000000000000e+01, 4.000000000000010492e-02
2.800000000000000000e+01, 4.000000000000010492e-02
2.900000000000000000e+01, 4.000000000000010492e-02
3.000000000000000000e+01, 4.000000000000010492e-02
3.100000000000000000e+01, 4.000000000000010492e-02
3.200000000000000000e+01, 5.000000000000010686e-02
3.300000000000000000e+01, 5.000000000000010686e-02
3.400000000000000000e+01, 1.200000000000001066e-01
3.500000000000000000e+01, 2.300000000000001210e-01
3.600000000000000000e+01, 2.600000000000001199e-01
3.700000000000000000e+01, 2.400000000000001021e-01
3.800000000000000000e+01, 2.400000000000001021e-01
3.900000000000000000e+01, 2.300000000000001210e-01
4.000000000000000000e+01, 2.600000000000001199e-01
4.100000000000000000e+01, 4.300000000000001044e-01
4.200000000000000000e+01, 5.300000000000001377e-01
4.300000000000000000e+01, 6.400000000000001243e-01
4.400000000000000000e+01, 7.600000000000001199e-01
4.500000000000000000e+01, 8.700000000000001066e-01
4.600000000000000000e+01, 9.800000000000000933e-01
4.700000000000000000e+01, 1.010000000000000231e+00
4.800000000000000000e+01, 1.150000000000000133e+00
4.900000000000000000e+01, 1.380000000000000115e+00
5.000000000000000000e+01, 1.350000000000000089e+00
5.100000000000000000e+01, 1.250000000000000222e+00
5.200000000000000000e+01, 1.260000000000000231e+00
5.300000000000000000e+01, 1.220000000000000195e+00
5.400000000000000000e+01, 1.230000000000000204e+00
5.500000000000000000e+01, 1.230000000000000204e+00
5.600000000000000000e+01, 1.230000000000000204e+00
5.700000000000000000e+01, 1.230000000000000204e+00
5.800000000000000000e+01, 1.230000000000000204e+00
5.900000000000000000e+01, 1.230000000000000204e+00
6.000000000000000000e+01, 1.240000000000000213e+00
6.100000000000000000e+01, 1.250000000000000222e+00
6.200000000000000000e+01, 1.270000000000000240e+00
6.300000000000000000e+01, 1.380000000000000115e+00
6.400000000000000000e+01, 1.680000000000000160e+00
6.500000000000000000e+01, 1.610000000000000098e+00
6.600000000000000000e+01, 1.490000000000000213e+00
6.700000000000000000e+01, 1.440000000000000169e+00
6.800000000000000000e+01, 1.440000000000000169e+00
6.900000000000000000e+01, 1.420000000000000151e+00
7.000000000000000000e+01, 1.380000000000000115e+00
7.100000000000000000e+01, 1.360000000000000098e+00
7.200000000000000000e+01, 1.340000000000000080e+00
7.300000000000000000e+01, 1.350000000000000089e+00
7.400000000000000000e+01, 1.340000000000000080e+00
7.500000000000000000e+01, 1.360000000000000098e+00
7.600000000000000000e+01, 1.380000000000000115e+00
7.700000000000000000e+01, 1.370000000000000107e+00
7.800000000000000000e+01, 1.380000000000000115e+00
7.900000000000000000e+01, 1.440000000000000169e+00
8.000000000000000000e+01, 1.440000000000000169e+00
8.100000000000000000e+01, 1.400000000000000133e+00
8.200000000000000000e+01, 1.370000000000000107e+00
8.300000000000000000e+01, 1.360000000000000098e+00
8.400000000000000000e+01, 1.370000000000000107e+00
8.500000000000000000e+01, 1.350000000000000089e+00
8.600000000000000000e+01, 1.350000000000000089e+00
8.700000000000000000e+01, 1.350000000000000089e+00
8.800000000000000000e+01, 1.360000000000000098e+00
8.900000000000000000e+01, 1.380000000000000115e+00
9.000000000000000000e+01, 1.390000000000000124e+00
9.100000000000000000e+01, 1.420000000000000151e+00
9.200000000000000000e+01, 1.430000000000000160e+00
9.300000000000000000e+01, 1.510000000000000231e+00
9.400000000000000000e+01, 1.670000000000000151e+00
9.500000000000000000e+01, 2.050000000000000266e+00
9.600000000000000000e+01, 2.330000000000000071e+00
9.700000000000000000e+01, 2.350000000000000089e+00
9.800000000000000000e+01, 2.330000000000000071e+00
9.900000000000000000e+01, 2.330000000000000071e+00
1.000000000000000000e+02, 2.330000000000000071e+00
1.010000000000000000e+02, 2.330000000000000071e+00
1.020000000000000000e+02, 2.330000000000000071e+00
1.030000000000000000e+02, 2.330000000000000071e+00
1.040000000000000000e+02, 2.330000000000000071e+00
1.050000000000000000e+02, 2.350000000000000089e+00
1.060000000000000000e+02, 2.350000000000000089e+00
1.070000000000000000e+02, 2.380000000000000338e+00
1.080000000000000000e+02, 2.479999999999999982e+00
1.090000000000000000e+02, 2.500000000000000000e+00
1.100000000000000000e+02, 2.500000000000000000e+00
1.110000000000000000e+02, 2.500000000000000000e+00
1.120000000000000000e+02, 2.500000000000000000e+00
1.130000000000000000e+02, 2.500000000000000000e+00
1.140000000000000000e+02, 2.500000000000000000e+00
1.150000000000000000e+02, 2.500000000000000000e+00
1.160000000000000000e+02, 2.500000000000000000e+00
1.170000000000000000e+02, 2.500000000000000000e+00
1.180000000000000000e+02, 2.500000000000000000e+00
1.190000000000000000e+02, 2.500000000000000000e+00
1.200000000000000000e+02, 2.500000000000000000e+00
1.210000000000000000e+02, 2.500000000000000000e+00
1.220000000000000000e+02, 2.500000000000000000e+00
1.230000000000000000e+02, 2.500000000000000000e+00
1.240000000000000000e+02, 2.500000000000000000e+00
1.250000000000000000e+02, 2.500000000000000000e+00
1.260000000000000000e+02, 2.470000000000000195e+00
1.270000000000000000e+02, 2.390000000000000124e+00
1.280000000000000000e+02, 2.340000000000000302e+00
1.290000000000000000e+02, 2.340000000000000302e+00
1.300000000000000000e+02, 2.330000000000000071e+00
1.310000000000000000e+02, 2.340000000000000302e+00
1.320000000000000000e+02, 2.340000000000000302e+00
1.330000000000000000e+02, 2.340000000000000302e+00
1.340000000000000000e+02, 2.340000000000000302e+00
1.350000000000000000e+02, 2.350000000000000089e+00
1.360000000000000000e+02, 2.370000000000000107e+00
1.370000000000000000e+02, 2.380000000000000338e+00
1.380000000000000000e+02, 2.500000000000000000e+00
1.390000000000000000e+02, 2.500000000000000000e+00
1.400000000000000000e+02, 2.500000000000000000e+00
1.410000000000000000e+02, 2.500000000000000000e+00
1.420000000000000000e+02, 2.500000000000000000e+00
1.430000000000000000e+02, 2.500000000000000000e+00
1.440000000000000000e+02, 2.500000000000000000e+00
1.450000000000000000e+02, 2.500000000000000000e+00
1.460000000000000000e+02, 2.470000000000000195e+00
1.470000000000000000e+02, 2.459999999999999964e+00
1.480000000000000000e+02, 2.470000000000000195e+00
1.490000000000000000e+02, 2.472500000000000142e+00
1.500000000000000000e+02, 2.479999999999999982e+00
1.510000000000000000e+02, 2.490000000000000213e+00
1.520000000000000000e+02, 2.500000000000000000e+00
1.530000000000000000e+02, 2.500000000000000000e+00
1.540000000000000000e+02, 2.500000000000000000e+00
1.550000000000000000e+02, 2.500000000000000000e+00
1.560000000000000000e+02, 2.500000000000000000e+00
1.570000000000000000e+02, 2.500000000000000000e+00
1.580000000000000000e+02, 2.500000000000000000e+00
1.590000000000000000e+02, 2.500000000000000000e+00
1.600000000000000000e+02, 2.500000000000000000e+00
1.610000000000000000e+02, 2.479999999999999982e+00
1.620000000000000000e+02, 2.400000000000001021e-01
1.630000000000000000e+02, 2.200000000000001121e-01
1.640000000000000000e+02, 2.000000000000001221e-01
1.650000000000000000e+02, 1.800000000000001044e-01
1.660000000000000000e+02, 1.700000000000000955e-01
1.670000000000000000e+02, 1.900000000000001132e-01
1.680000000000000000e+02, 2.200000000000001121e-01
1.690000000000000000e+02, 2.400000000000001021e-01
1.700000000000000000e+02, 2.900000000000000910e-01
1.710000000000000000e+02, 3.400000000000001354e-01
1.720000000000000000e+02, 1.300000000000001155e-01
1.730000000000000000e+02, 6.000000000000010880e-02
1.740000000000000000e+02, 5.000000000000010686e-02
1.750000000000000000e+02, 4.000000000000010492e-02
1.760000000000000000e+02, 4.000000000000010492e-02
1.770000000000000000e+02, 4.000000000000010492e-02
1.780000000000000000e+02, 4.000000000000010492e-02
1.790000000000000000e+02, 4.000000000000010492e-02
1.800000000000000000e+02, 4.000000000000010492e-02
1.810000000000000000e+02, 4.000000000000010492e-02
1.820000000000000000e+02, 4.000000000000010492e-02
1.830000000000000000e+02, 5.000000000000010686e-02
1.840000000000000000e+02, 5.000000000000010686e-02
1.850000000000000000e+02, 7.000000000000010381e-02
1.860000000000000000e+02, 1.900000000000001132e-01
1.870000000000000000e+02, 2.400000000000001021e-01
1.880000000000000000e+02, 2.400000000000001021e-01
1.890000000000000000e+02, 2.500000000000001110e-01
1.900000000000000000e+02, 2.400000000000001021e-01
1.910000000000000000e+02, 2.400000000000001021e-01
1.920000000000000000e+02, 2.100000000000001033e-01
1.930000000000000000e+02, 2.000000000000001221e-01
1.940000000000000000e+02, 1.900000000000001132e-01
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationmedian, color=estimationColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 2.000000000000010450e-02
1.100000000000000000e+01, 2.000000000000010450e-02
1.200000000000000000e+01, 2.000000000000010450e-02
1.300000000000000000e+01, 3.000000000000010297e-02
1.400000000000000000e+01, 3.000000000000010297e-02
1.500000000000000000e+01, 3.000000000000010297e-02
1.600000000000000000e+01, 3.000000000000010297e-02
1.700000000000000000e+01, 3.000000000000010297e-02
1.800000000000000000e+01, 3.500000000000010048e-02
1.900000000000000000e+01, 2.000000000000010450e-02
2.000000000000000000e+01, 2.000000000000010450e-02
2.100000000000000000e+01, 1.000000000000010429e-02
2.200000000000000000e+01, 1.000000000000010429e-02
2.300000000000000000e+01, 1.000000000000010429e-02
2.400000000000000000e+01, 1.000000000000010429e-02
2.500000000000000000e+01, 1.000000000000010429e-02
2.600000000000000000e+01, 1.000000000000010429e-02
2.700000000000000000e+01, 1.000000000000010429e-02
2.800000000000000000e+01, 1.000000000000010429e-02
2.900000000000000000e+01, 1.000000000000010429e-02
3.000000000000000000e+01, 1.000000000000010429e-02
3.100000000000000000e+01, 1.000000000000010429e-02
3.200000000000000000e+01, 1.000000000000010429e-02
3.300000000000000000e+01, 1.000000000000010429e-02
3.400000000000000000e+01, 1.040834085586084257e-16
3.500000000000000000e+01, 1.040834085586084257e-16
3.600000000000000000e+01, 1.040834085586084257e-16
3.700000000000000000e+01, -9.999999999999896125e-03
3.800000000000000000e+01, -9.999999999999896125e-03
3.900000000000000000e+01, 2.000000000000010450e-02
4.000000000000000000e+01, 1.200000000000001066e-01
4.100000000000000000e+01, 2.600000000000001199e-01
4.200000000000000000e+01, 3.400000000000001354e-01
4.300000000000000000e+01, 4.200000000000000955e-01
4.400000000000000000e+01, 5.100000000000001199e-01
4.500000000000000000e+01, 6.300000000000001155e-01
4.600000000000000000e+01, 7.300000000000000933e-01
4.700000000000000000e+01, 7.700000000000001288e-01
4.800000000000000000e+01, 9.300000000000001599e-01
4.900000000000000000e+01, 1.140000000000000124e+00
5.000000000000000000e+01, 1.200000000000000178e+00
5.100000000000000000e+01, 1.200000000000000178e+00
5.200000000000000000e+01, 1.220000000000000195e+00
5.300000000000000000e+01, 1.190000000000000169e+00
5.400000000000000000e+01, 1.200000000000000178e+00
5.500000000000000000e+01, 1.200000000000000178e+00
5.600000000000000000e+01, 1.200000000000000178e+00
5.700000000000000000e+01, 1.200000000000000178e+00
5.800000000000000000e+01, 1.200000000000000178e+00
5.900000000000000000e+01, 1.200000000000000178e+00
6.000000000000000000e+01, 1.200000000000000178e+00
6.100000000000000000e+01, 1.200000000000000178e+00
6.200000000000000000e+01, 1.220000000000000195e+00
6.300000000000000000e+01, 1.230000000000000204e+00
6.400000000000000000e+01, 1.275000000000000133e+00
6.500000000000000000e+01, 1.260000000000000231e+00
6.600000000000000000e+01, 1.235000000000000320e+00
6.700000000000000000e+01, 1.230000000000000204e+00
6.800000000000000000e+01, 1.230000000000000204e+00
6.900000000000000000e+01, 1.230000000000000204e+00
7.000000000000000000e+01, 1.220000000000000195e+00
7.100000000000000000e+01, 1.220000000000000195e+00
7.200000000000000000e+01, 1.220000000000000195e+00
7.300000000000000000e+01, 1.220000000000000195e+00
7.400000000000000000e+01, 1.210000000000000187e+00
7.500000000000000000e+01, 1.220000000000000195e+00
7.600000000000000000e+01, 1.210000000000000187e+00
7.700000000000000000e+01, 1.210000000000000187e+00
7.800000000000000000e+01, 1.215000000000000302e+00
7.900000000000000000e+01, 1.235000000000000320e+00
8.000000000000000000e+01, 1.230000000000000204e+00
8.100000000000000000e+01, 1.240000000000000213e+00
8.200000000000000000e+01, 1.235000000000000320e+00
8.300000000000000000e+01, 1.230000000000000204e+00
8.400000000000000000e+01, 1.230000000000000204e+00
8.500000000000000000e+01, 1.230000000000000204e+00
8.600000000000000000e+01, 1.220000000000000195e+00
8.700000000000000000e+01, 1.220000000000000195e+00
8.800000000000000000e+01, 1.220000000000000195e+00
8.900000000000000000e+01, 1.220000000000000195e+00
9.000000000000000000e+01, 1.220000000000000195e+00
9.100000000000000000e+01, 1.220000000000000195e+00
9.200000000000000000e+01, 1.220000000000000195e+00
9.300000000000000000e+01, 1.240000000000000213e+00
9.400000000000000000e+01, 1.340000000000000080e+00
9.500000000000000000e+01, 1.870000000000000107e+00
9.600000000000000000e+01, 2.229999999999999982e+00
9.700000000000000000e+01, 2.290000000000000036e+00
9.800000000000000000e+01, 2.290000000000000036e+00
9.900000000000000000e+01, 2.300000000000000266e+00
1.000000000000000000e+02, 2.300000000000000266e+00
1.010000000000000000e+02, 2.300000000000000266e+00
1.020000000000000000e+02, 2.300000000000000266e+00
1.030000000000000000e+02, 2.300000000000000266e+00
1.040000000000000000e+02, 2.300000000000000266e+00
1.050000000000000000e+02, 2.300000000000000266e+00
1.060000000000000000e+02, 2.300000000000000266e+00
1.070000000000000000e+02, 2.320000000000000284e+00
1.080000000000000000e+02, 2.320000000000000284e+00
1.090000000000000000e+02, 2.375000000000000000e+00
1.100000000000000000e+02, 2.380000000000000338e+00
1.110000000000000000e+02, 2.334999999999999964e+00
1.120000000000000000e+02, 2.330000000000000071e+00
1.130000000000000000e+02, 2.334999999999999964e+00
1.140000000000000000e+02, 2.334999999999999964e+00
1.150000000000000000e+02, 2.340000000000000302e+00
1.160000000000000000e+02, 2.340000000000000302e+00
1.170000000000000000e+02, 2.340000000000000302e+00
1.180000000000000000e+02, 2.330000000000000071e+00
1.190000000000000000e+02, 2.345000000000000195e+00
1.200000000000000000e+02, 2.350000000000000089e+00
1.210000000000000000e+02, 2.340000000000000302e+00
1.220000000000000000e+02, 2.350000000000000089e+00
1.230000000000000000e+02, 2.340000000000000302e+00
1.240000000000000000e+02, 2.400000000000000355e+00
1.250000000000000000e+02, 2.360000000000000320e+00
1.260000000000000000e+02, 2.320000000000000284e+00
1.270000000000000000e+02, 2.330000000000000071e+00
1.280000000000000000e+02, 2.300000000000000266e+00
1.290000000000000000e+02, 2.310000000000000053e+00
1.300000000000000000e+02, 2.300000000000000266e+00
1.310000000000000000e+02, 2.300000000000000266e+00
1.320000000000000000e+02, 2.300000000000000266e+00
1.330000000000000000e+02, 2.300000000000000266e+00
1.340000000000000000e+02, 2.310000000000000053e+00
1.350000000000000000e+02, 2.310000000000000053e+00
1.360000000000000000e+02, 2.320000000000000284e+00
1.370000000000000000e+02, 2.305000000000000160e+00
1.380000000000000000e+02, 2.330000000000000071e+00
1.390000000000000000e+02, 2.400000000000000355e+00
1.400000000000000000e+02, 2.370000000000000107e+00
1.410000000000000000e+02, 2.350000000000000089e+00
1.420000000000000000e+02, 2.330000000000000071e+00
1.430000000000000000e+02, 2.330000000000000071e+00
1.440000000000000000e+02, 2.330000000000000071e+00
1.450000000000000000e+02, 2.330000000000000071e+00
1.460000000000000000e+02, 2.320000000000000284e+00
1.470000000000000000e+02, 2.320000000000000284e+00
1.480000000000000000e+02, 2.320000000000000284e+00
1.490000000000000000e+02, 2.330000000000000071e+00
1.500000000000000000e+02, 2.330000000000000071e+00
1.510000000000000000e+02, 2.340000000000000302e+00
1.520000000000000000e+02, 2.350000000000000089e+00
1.530000000000000000e+02, 2.350000000000000089e+00
1.540000000000000000e+02, 2.350000000000000089e+00
1.550000000000000000e+02, 2.350000000000000089e+00
1.560000000000000000e+02, 2.340000000000000302e+00
1.570000000000000000e+02, 2.330000000000000071e+00
1.580000000000000000e+02, 2.459999999999999964e+00
1.590000000000000000e+02, 2.360000000000000320e+00
1.600000000000000000e+02, 2.360000000000000320e+00
1.610000000000000000e+02, 4.000000000000001332e-01
1.620000000000000000e+02, 9.000000000000010769e-02
1.630000000000000000e+02, 7.000000000000010381e-02
1.640000000000000000e+02, 5.000000000000010686e-02
1.650000000000000000e+02, -9.999999999999896125e-03
1.660000000000000000e+02, 2.000000000000010450e-02
1.670000000000000000e+02, 2.000000000000010450e-02
1.680000000000000000e+02, 3.000000000000010297e-02
1.690000000000000000e+02, 4.000000000000010492e-02
1.700000000000000000e+02, 4.500000000000010936e-02
1.710000000000000000e+02, 5.000000000000010686e-02
1.720000000000000000e+02, 1.040834085586084257e-16
1.730000000000000000e+02, 1.000000000000010429e-02
1.740000000000000000e+02, 1.000000000000010429e-02
1.750000000000000000e+02, 1.000000000000010429e-02
1.760000000000000000e+02, 1.000000000000010429e-02
1.770000000000000000e+02, 1.000000000000010429e-02
1.780000000000000000e+02, 1.000000000000010429e-02
1.790000000000000000e+02, 1.000000000000010429e-02
1.800000000000000000e+02, 1.000000000000010429e-02
1.810000000000000000e+02, 1.000000000000010429e-02
1.820000000000000000e+02, 1.000000000000010429e-02
1.830000000000000000e+02, 1.000000000000010429e-02
1.840000000000000000e+02, 1.000000000000010429e-02
1.850000000000000000e+02, 1.000000000000010429e-02
1.860000000000000000e+02, 2.000000000000010450e-02
1.870000000000000000e+02, 1.000000000000010429e-02
1.880000000000000000e+02, 3.000000000000010297e-02
1.890000000000000000e+02, 3.000000000000010297e-02
1.900000000000000000e+02, 4.000000000000010492e-02
1.910000000000000000e+02, 3.500000000000010048e-02
1.920000000000000000e+02, 2.500000000000010547e-02
1.930000000000000000e+02, 1.000000000000010429e-02
1.940000000000000000e+02, 2.000000000000010450e-02
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addlegendentry{estimation}

\addplot [backGray, fill opacity=0.9, forget plot] fill between[of=estimationlower and estimationupper];

\addplot [name path=ground-truth, color=ground-truthColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 0.000000000000000000e+00
1.100000000000000000e+01, 0.000000000000000000e+00
1.200000000000000000e+01, 0.000000000000000000e+00
1.300000000000000000e+01, 0.000000000000000000e+00
1.400000000000000000e+01, 0.000000000000000000e+00
1.500000000000000000e+01, 0.000000000000000000e+00
1.600000000000000000e+01, 0.000000000000000000e+00
1.700000000000000000e+01, 0.000000000000000000e+00
1.800000000000000000e+01, 0.000000000000000000e+00
1.900000000000000000e+01, 0.000000000000000000e+00
2.000000000000000000e+01, 0.000000000000000000e+00
2.100000000000000000e+01, 0.000000000000000000e+00
2.200000000000000000e+01, 0.000000000000000000e+00
2.300000000000000000e+01, 0.000000000000000000e+00
2.400000000000000000e+01, 0.000000000000000000e+00
2.500000000000000000e+01, 0.000000000000000000e+00
2.600000000000000000e+01, 0.000000000000000000e+00
2.700000000000000000e+01, 0.000000000000000000e+00
2.800000000000000000e+01, 0.000000000000000000e+00
2.900000000000000000e+01, 0.000000000000000000e+00
3.000000000000000000e+01, 0.000000000000000000e+00
3.100000000000000000e+01, 0.000000000000000000e+00
3.200000000000000000e+01, 0.000000000000000000e+00
3.300000000000000000e+01, 0.000000000000000000e+00
3.400000000000000000e+01, 0.000000000000000000e+00
3.500000000000000000e+01, 0.000000000000000000e+00
3.600000000000000000e+01, 0.000000000000000000e+00
3.700000000000000000e+01, 0.000000000000000000e+00
3.800000000000000000e+01, 0.000000000000000000e+00
3.900000000000000000e+01, 0.000000000000000000e+00
4.000000000000000000e+01, 1.199999999999999956e+00
4.100000000000000000e+01, 1.199999999999999956e+00
4.200000000000000000e+01, 1.199999999999999956e+00
4.300000000000000000e+01, 1.199999999999999956e+00
4.400000000000000000e+01, 1.199999999999999956e+00
4.500000000000000000e+01, 1.199999999999999956e+00
4.600000000000000000e+01, 1.199999999999999956e+00
4.700000000000000000e+01, 1.199999999999999956e+00
4.800000000000000000e+01, 1.199999999999999956e+00
4.900000000000000000e+01, 1.199999999999999956e+00
5.000000000000000000e+01, 1.199999999999999956e+00
5.100000000000000000e+01, 1.199999999999999956e+00
5.200000000000000000e+01, 1.199999999999999956e+00
5.300000000000000000e+01, 1.199999999999999956e+00
5.400000000000000000e+01, 1.199999999999999956e+00
5.500000000000000000e+01, 1.199999999999999956e+00
5.600000000000000000e+01, 1.199999999999999956e+00
5.700000000000000000e+01, 1.199999999999999956e+00
5.800000000000000000e+01, 1.199999999999999956e+00
5.900000000000000000e+01, 1.199999999999999956e+00
6.000000000000000000e+01, 1.199999999999999956e+00
6.100000000000000000e+01, 1.199999999999999956e+00
6.200000000000000000e+01, 1.199999999999999956e+00
6.300000000000000000e+01, 1.199999999999999956e+00
6.400000000000000000e+01, 1.199999999999999956e+00
6.500000000000000000e+01, 1.199999999999999956e+00
6.600000000000000000e+01, 1.199999999999999956e+00
6.700000000000000000e+01, 1.199999999999999956e+00
6.800000000000000000e+01, 1.199999999999999956e+00
6.900000000000000000e+01, 1.199999999999999956e+00
7.000000000000000000e+01, 1.199999999999999956e+00
7.100000000000000000e+01, 1.199999999999999956e+00
7.200000000000000000e+01, 1.199999999999999956e+00
7.300000000000000000e+01, 1.199999999999999956e+00
7.400000000000000000e+01, 1.199999999999999956e+00
7.500000000000000000e+01, 1.199999999999999956e+00
7.600000000000000000e+01, 1.199999999999999956e+00
7.700000000000000000e+01, 1.199999999999999956e+00
7.800000000000000000e+01, 1.199999999999999956e+00
7.900000000000000000e+01, 1.199999999999999956e+00
8.000000000000000000e+01, 1.199999999999999956e+00
8.100000000000000000e+01, 1.199999999999999956e+00
8.200000000000000000e+01, 1.199999999999999956e+00
8.300000000000000000e+01, 1.199999999999999956e+00
8.400000000000000000e+01, 1.199999999999999956e+00
8.500000000000000000e+01, 1.199999999999999956e+00
8.600000000000000000e+01, 1.199999999999999956e+00
8.700000000000000000e+01, 1.199999999999999956e+00
8.800000000000000000e+01, 1.199999999999999956e+00
8.900000000000000000e+01, 1.199999999999999956e+00
9.000000000000000000e+01, 1.199999999999999956e+00
9.100000000000000000e+01, 1.199999999999999956e+00
9.200000000000000000e+01, 1.199999999999999956e+00
9.300000000000000000e+01, 2.299999999999999822e+00
9.400000000000000000e+01, 2.299999999999999822e+00
9.500000000000000000e+01, 2.299999999999999822e+00
9.600000000000000000e+01, 2.299999999999999822e+00
9.700000000000000000e+01, 2.299999999999999822e+00
9.800000000000000000e+01, 2.299999999999999822e+00
9.900000000000000000e+01, 2.299999999999999822e+00
1.000000000000000000e+02, 2.299999999999999822e+00
1.010000000000000000e+02, 2.299999999999999822e+00
1.020000000000000000e+02, 2.299999999999999822e+00
1.030000000000000000e+02, 2.299999999999999822e+00
1.040000000000000000e+02, 2.299999999999999822e+00
1.050000000000000000e+02, 2.299999999999999822e+00
1.060000000000000000e+02, 2.299999999999999822e+00
1.070000000000000000e+02, 2.299999999999999822e+00
1.080000000000000000e+02, 2.299999999999999822e+00
1.090000000000000000e+02, 2.299999999999999822e+00
1.100000000000000000e+02, 2.299999999999999822e+00
1.110000000000000000e+02, 2.299999999999999822e+00
1.120000000000000000e+02, 2.299999999999999822e+00
1.130000000000000000e+02, 2.299999999999999822e+00
1.140000000000000000e+02, 2.299999999999999822e+00
1.150000000000000000e+02, 2.299999999999999822e+00
1.160000000000000000e+02, 2.299999999999999822e+00
1.170000000000000000e+02, 2.299999999999999822e+00
1.180000000000000000e+02, 2.299999999999999822e+00
1.190000000000000000e+02, 2.299999999999999822e+00
1.200000000000000000e+02, 2.299999999999999822e+00
1.210000000000000000e+02, 2.299999999999999822e+00
1.220000000000000000e+02, 2.299999999999999822e+00
1.230000000000000000e+02, 2.299999999999999822e+00
1.240000000000000000e+02, 2.299999999999999822e+00
1.250000000000000000e+02, 2.299999999999999822e+00
1.260000000000000000e+02, 2.299999999999999822e+00
1.270000000000000000e+02, 2.299999999999999822e+00
1.280000000000000000e+02, 2.299999999999999822e+00
1.290000000000000000e+02, 2.299999999999999822e+00
1.300000000000000000e+02, 2.299999999999999822e+00
1.310000000000000000e+02, 2.299999999999999822e+00
1.320000000000000000e+02, 2.299999999999999822e+00
1.330000000000000000e+02, 2.299999999999999822e+00
1.340000000000000000e+02, 2.299999999999999822e+00
1.350000000000000000e+02, 2.299999999999999822e+00
1.360000000000000000e+02, 2.299999999999999822e+00
1.370000000000000000e+02, 2.299999999999999822e+00
1.380000000000000000e+02, 2.299999999999999822e+00
1.390000000000000000e+02, 2.299999999999999822e+00
1.400000000000000000e+02, 2.299999999999999822e+00
1.410000000000000000e+02, 2.299999999999999822e+00
1.420000000000000000e+02, 2.299999999999999822e+00
1.430000000000000000e+02, 2.299999999999999822e+00
1.440000000000000000e+02, 2.299999999999999822e+00
1.450000000000000000e+02, 2.299999999999999822e+00
1.460000000000000000e+02, 2.299999999999999822e+00
1.470000000000000000e+02, 2.299999999999999822e+00
1.480000000000000000e+02, 2.299999999999999822e+00
1.490000000000000000e+02, 2.299999999999999822e+00
1.500000000000000000e+02, 2.299999999999999822e+00
1.510000000000000000e+02, 2.299999999999999822e+00
1.520000000000000000e+02, 2.299999999999999822e+00
1.530000000000000000e+02, 2.299999999999999822e+00
1.540000000000000000e+02, 2.299999999999999822e+00
1.550000000000000000e+02, 0.000000000000000000e+00
1.560000000000000000e+02, 0.000000000000000000e+00
1.570000000000000000e+02, 0.000000000000000000e+00
1.580000000000000000e+02, 0.000000000000000000e+00
1.590000000000000000e+02, 0.000000000000000000e+00
1.600000000000000000e+02, 0.000000000000000000e+00
1.610000000000000000e+02, 0.000000000000000000e+00
1.620000000000000000e+02, 0.000000000000000000e+00
1.630000000000000000e+02, 0.000000000000000000e+00
1.640000000000000000e+02, 0.000000000000000000e+00
1.650000000000000000e+02, 0.000000000000000000e+00
1.660000000000000000e+02, 0.000000000000000000e+00
1.670000000000000000e+02, 0.000000000000000000e+00
1.680000000000000000e+02, 0.000000000000000000e+00
1.690000000000000000e+02, 0.000000000000000000e+00
1.700000000000000000e+02, 0.000000000000000000e+00
1.710000000000000000e+02, 0.000000000000000000e+00
1.720000000000000000e+02, 0.000000000000000000e+00
1.730000000000000000e+02, 0.000000000000000000e+00
1.740000000000000000e+02, 0.000000000000000000e+00
1.750000000000000000e+02, 0.000000000000000000e+00
1.760000000000000000e+02, 0.000000000000000000e+00
1.770000000000000000e+02, 0.000000000000000000e+00
1.780000000000000000e+02, 0.000000000000000000e+00
1.790000000000000000e+02, 0.000000000000000000e+00
1.800000000000000000e+02, 0.000000000000000000e+00
1.810000000000000000e+02, 0.000000000000000000e+00
1.820000000000000000e+02, 0.000000000000000000e+00
1.830000000000000000e+02, 0.000000000000000000e+00
1.840000000000000000e+02, 0.000000000000000000e+00
1.850000000000000000e+02, 0.000000000000000000e+00
1.860000000000000000e+02, 0.000000000000000000e+00
1.870000000000000000e+02, 0.000000000000000000e+00
1.880000000000000000e+02, 0.000000000000000000e+00
1.890000000000000000e+02, 0.000000000000000000e+00
1.900000000000000000e+02, 0.000000000000000000e+00
1.910000000000000000e+02, 0.000000000000000000e+00
1.920000000000000000e+02, 0.000000000000000000e+00
1.930000000000000000e+02, 0.000000000000000000e+00
1.940000000000000000e+02, 0.000000000000000000e+00
};

\addlegendentry{ground-truth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_high_filter.tex <==
\addplot [name path=target-velocity, color=target-velocityColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 4.000000000000000222e-01
1.000000000000000000e+00, 4.000000000000000222e-01
2.000000000000000000e+00, 3.956907456501841391e-01
3.000000000000000000e+00, 3.963103168612088223e-01
4.000000000000000000e+00, 3.972149334979231394e-01
5.000000000000000000e+00, 3.961365223630156640e-01
6.000000000000000000e+00, 3.973033029129279248e-01
7.000000000000000000e+00, 3.972455606836805542e-01
8.000000000000000000e+00, 3.979176934032611079e-01
9.000000000000000000e+00, 3.980115327061656272e-01
1.000000000000000000e+01, 3.983260310444375341e-01
1.100000000000000000e+01, 3.982025575521566108e-01
1.200000000000000000e+01, 3.982459019288128177e-01
1.300000000000000000e+01, 3.981645665399833889e-01
1.400000000000000000e+01, 3.978974858491948763e-01
1.500000000000000000e+01, 3.978486971696576502e-01
1.600000000000000000e+01, 3.979136723658311392e-01
1.700000000000000000e+01, 3.976974797959594854e-01
1.800000000000000000e+01, 3.977239995052112564e-01
1.900000000000000000e+01, 3.979216439701138697e-01
2.000000000000000000e+01, 3.982720838964842192e-01
2.100000000000000000e+01, 3.980660176222874380e-01
2.200000000000000000e+01, 3.980130980774795324e-01
2.300000000000000000e+01, 3.979705918118819907e-01
2.400000000000000000e+01, 3.981472703073188901e-01
2.500000000000000000e+01, 3.984145760338247411e-01
2.600000000000000000e+01, 3.981763333288155238e-01
2.700000000000000000e+01, 3.983097025921228385e-01
2.800000000000000000e+01, 3.983076896319152072e-01
2.900000000000000000e+01, 3.983949388476373810e-01
3.000000000000000000e+01, 3.978574873293854175e-01
3.100000000000000000e+01, 3.978301884867203042e-01
3.200000000000000000e+01, 3.981307564519579456e-01
3.300000000000000000e+01, 3.980152688138747230e-01
3.400000000000000000e+01, 3.979105743845625653e-01
3.500000000000000000e+01, 3.981375492822534223e-01
3.600000000000000000e+01, 3.981458987666484095e-01
3.700000000000000000e+01, 3.980520785919101634e-01
3.800000000000000000e+01, 3.980994133944449898e-01
3.900000000000000000e+01, 3.980952550385349342e-01
4.000000000000000000e+01, 3.979832826541665480e-01
4.100000000000000000e+01, 3.978996954565955368e-01
4.200000000000000000e+01, 3.979894055319254109e-01
4.300000000000000000e+01, 3.980802593149682655e-01
4.400000000000000000e+01, 3.982976056662058673e-01
4.500000000000000000e+01, 3.980884721702923068e-01
4.600000000000000000e+01, 3.981459267198707019e-01
4.700000000000000000e+01, 3.981131096669354164e-01
4.800000000000000000e+01, 3.979642662818358989e-01
4.900000000000000000e+01, 3.981418413070422213e-01
5.000000000000000000e+01, 3.977621233589634375e-01
5.100000000000000000e+01, 3.981348339709925854e-01
5.200000000000000000e+01, 3.981832099346249154e-01
5.300000000000000000e+01, 3.979942428518526421e-01
5.400000000000000000e+01, 3.980872574129369346e-01
5.500000000000000000e+01, 3.978089763808118073e-01
5.600000000000000000e+01, 3.978101502222743946e-01
5.700000000000000000e+01, 3.978688133441469210e-01
5.800000000000000000e+01, 3.978557999459845229e-01
5.900000000000000000e+01, 3.980640141944556953e-01
6.000000000000000000e+01, 3.980535794542116035e-01
6.100000000000000000e+01, 3.978105205075290751e-01
6.200000000000000000e+01, 3.980194543393004714e-01
6.300000000000000000e+01, 3.979510527965659517e-01
6.400000000000000000e+01, 3.979562707160287927e-01
6.500000000000000000e+01, 3.981040273663444262e-01
6.600000000000000000e+01, 3.981245001898922053e-01
6.700000000000000000e+01, 3.981143071482057261e-01
6.800000000000000000e+01, 3.981154650688318308e-01
6.900000000000000000e+01, 3.983318373203511564e-01
7.000000000000000000e+01, 3.986157745054372814e-01
7.100000000000000000e+01, 3.982421049025203774e-01
7.200000000000000000e+01, 3.982820882718840494e-01
7.300000000000000000e+01, 3.982128834358930058e-01
7.400000000000000000e+01, 3.980881955880770651e-01
7.500000000000000000e+01, 3.981722474445729132e-01
7.600000000000000000e+01, 3.979132830424832457e-01
7.700000000000000000e+01, 3.977095670852079934e-01
7.800000000000000000e+01, 3.981434674254770156e-01
7.900000000000000000e+01, 3.980256477108521929e-01
8.000000000000000000e+01, 3.981755874389071304e-01
8.100000000000000000e+01, 4.323061881948257468e-01
8.200000000000000000e+01, 4.180594787180589300e-01
8.300000000000000000e+01, 4.451080555119486526e-01
8.400000000000000000e+01, 4.222286819775569189e-01
8.500000000000000000e+01, 4.446631224493376444e-01
8.600000000000000000e+01, 4.179982698808791253e-01
8.700000000000000000e+01, 4.382345354474204147e-01
8.800000000000000000e+01, 4.089791903542615015e-01
8.900000000000000000e+01, 4.286754516953102390e-01
9.000000000000000000e+01, 4.002124511694385434e-01
9.100000000000000000e+01, 4.194244721739643356e-01
9.200000000000000000e+01, 3.918059197685134221e-01
9.300000000000000000e+01, 4.118983113282075337e-01
9.400000000000000000e+01, 3.857978291971623230e-01
9.500000000000000000e+01, 4.062862248418283029e-01
9.600000000000000000e+01, 3.807021424351307859e-01
9.700000000000000000e+01, 4.015843654244594108e-01
9.800000000000000000e+01, 3.773079412638115082e-01
9.900000000000000000e+01, 3.988865220220304542e-01
1.000000000000000000e+02, 3.753083254693900805e-01
1.010000000000000000e+02, 3.975302014266047235e-01
1.020000000000000000e+02, 3.740082035898676383e-01
1.030000000000000000e+02, 3.965668867031311162e-01
1.040000000000000000e+02, 3.738789451390854834e-01
1.050000000000000000e+02, 3.966874745942144953e-01
1.060000000000000000e+02, 3.743744617601449942e-01
1.070000000000000000e+02, 3.967328108942947962e-01
1.080000000000000000e+02, 3.742566664766800999e-01
1.090000000000000000e+02, 3.971178004357542868e-01
1.100000000000000000e+02, 3.745975540341848209e-01
1.110000000000000000e+02, 3.971993218342417808e-01
1.120000000000000000e+02, 3.749600724110509486e-01
1.130000000000000000e+02, 3.975899546856013766e-01
1.140000000000000000e+02, 3.748909425932429595e-01
1.150000000000000000e+02, 3.975259512999743672e-01
1.160000000000000000e+02, 3.752776288569771301e-01
1.170000000000000000e+02, 3.977297368484229989e-01
1.180000000000000000e+02, 3.752792014108731200e-01
1.190000000000000000e+02, 3.977110375438691614e-01
1.200000000000000000e+02, 3.751002349404676250e-01
1.210000000000000000e+02, 3.975504269687005765e-01
1.220000000000000000e+02, 3.753893291911326591e-01
1.230000000000000000e+02, 3.981284370713361054e-01
1.240000000000000000e+02, 3.754827638921354183e-01
1.250000000000000000e+02, 3.980968725858196056e-01
1.260000000000000000e+02, 3.750996887139048663e-01
1.270000000000000000e+02, 3.980947093976098250e-01
1.280000000000000000e+02, 3.757140750203099011e-01
1.290000000000000000e+02, 3.979575617489686801e-01
1.300000000000000000e+02, 3.753184955404850198e-01
1.310000000000000000e+02, 3.976042557642111563e-01
1.320000000000000000e+02, 3.752304828814423399e-01
1.330000000000000000e+02, 3.977756771254663537e-01
1.340000000000000000e+02, 3.751720340644529306e-01
1.350000000000000000e+02, 3.978128994122449025e-01
1.360000000000000000e+02, 3.750881494599823118e-01
1.370000000000000000e+02, 3.981234924734318170e-01
1.380000000000000000e+02, 3.756266018202515378e-01
1.390000000000000000e+02, 3.982500114788872780e-01
1.400000000000000000e+02, 3.755643105792147995e-01
1.410000000000000000e+02, 3.986473968372438170e-01
1.420000000000000000e+02, 3.757959705139173323e-01
1.430000000000000000e+02, 3.987329431271298685e-01
1.440000000000000000e+02, 3.759006179333923559e-01
1.450000000000000000e+02, 3.982372424540536748e-01
1.460000000000000000e+02, 3.755154823800636033e-01
1.470000000000000000e+02, 3.979000647339945296e-01
1.480000000000000000e+02, 3.751033022821375074e-01
1.490000000000000000e+02, 3.976452734977437009e-01
1.500000000000000000e+02, 3.750938931276488475e-01
1.510000000000000000e+02, 3.979545480752084696e-01
1.520000000000000000e+02, 3.751038245634262802e-01
1.530000000000000000e+02, 3.978082776051752312e-01
1.540000000000000000e+02, 3.752107507037226175e-01
1.550000000000000000e+02, 3.981671225910622391e-01
1.560000000000000000e+02, 3.752900396451592790e-01
1.570000000000000000e+02, 3.976840281240871522e-01
1.580000000000000000e+02, 3.753599809746880345e-01
1.590000000000000000e+02, 3.980257495906575071e-01
1.600000000000000000e+02, 3.754542499827385194e-01
1.610000000000000000e+02, 3.980501323446187234e-01
1.620000000000000000e+02, 3.755275899424935782e-01
1.630000000000000000e+02, 3.980510011450192343e-01
1.640000000000000000e+02, 3.755031873965334333e-01
1.650000000000000000e+02, 3.980551225781429059e-01
1.660000000000000000e+02, 3.753569175866639518e-01
1.670000000000000000e+02, 3.978847972040928660e-01
1.680000000000000000e+02, 3.757938820051789919e-01
1.690000000000000000e+02, 3.983187246985154251e-01
1.700000000000000000e+02, 3.757827538515994825e-01
1.710000000000000000e+02, 3.982945841838744228e-01
1.720000000000000000e+02, 3.757493079095012289e-01
1.730000000000000000e+02, 3.980890744457014074e-01
1.740000000000000000e+02, 3.753792989870223806e-01
1.750000000000000000e+02, 3.981235429569572881e-01
1.760000000000000000e+02, 3.756698507529148690e-01
1.770000000000000000e+02, 3.981717622488061270e-01
1.780000000000000000e+02, 3.753966312474721345e-01
1.790000000000000000e+02, 3.980645630926232803e-01
1.800000000000000000e+02, 3.751222549396050487e-01
1.810000000000000000e+02, 3.976969548949407240e-01
1.820000000000000000e+02, 3.753541516659705257e-01
1.830000000000000000e+02, 3.983466013842217324e-01
1.840000000000000000e+02, 3.756565889007484893e-01
1.850000000000000000e+02, 3.982408173770984883e-01
1.860000000000000000e+02, 3.752334677614226899e-01
1.870000000000000000e+02, 4.292863059896093181e-01
1.880000000000000000e+02, 3.936529943426067546e-01
1.890000000000000000e+02, 4.411089923570306603e-01
1.900000000000000000e+02, 3.978349304755937066e-01
1.910000000000000000e+02, 4.412878237009874582e-01
1.920000000000000000e+02, 3.939484924062643945e-01
1.930000000000000000e+02, 4.352650947609492116e-01
1.940000000000000000e+02, 3.856809556442098996e-01
1.950000000000000000e+02, 4.264029418780646563e-01
1.960000000000000000e+02, 3.777911672322982195e-01
1.970000000000000000e+02, 4.180831137551682675e-01
1.980000000000000000e+02, 3.695726551006028315e-01
1.990000000000000000e+02, 4.105552254754233354e-01
2.000000000000000000e+02, 3.632709565117512862e-01
2.010000000000000000e+02, 4.048933646886483939e-01
2.020000000000000000e+02, 3.589601736324595782e-01
2.030000000000000000e+02, 4.014632270554642224e-01
2.040000000000000000e+02, 3.563532648852908435e-01
2.050000000000000000e+02, 3.986789018785844574e-01
2.060000000000000000e+02, 3.547520744899281819e-01
2.070000000000000000e+02, 3.973337023316280137e-01
2.080000000000000000e+02, 3.533443159468556694e-01
2.090000000000000000e+02, 3.966565816926734267e-01
2.100000000000000000e+02, 3.533861042903159166e-01
2.110000000000000000e+02, 3.967983269050671113e-01
2.120000000000000000e+02, 3.537126958340520155e-01
2.130000000000000000e+02, 3.971646304202691713e-01
2.140000000000000000e+02, 3.538973024348729401e-01
2.150000000000000000e+02, 3.974139402111184771e-01
2.160000000000000000e+02, 3.540158655283601186e-01
2.170000000000000000e+02, 3.974346408974258615e-01
2.180000000000000000e+02, 3.543314073627212846e-01
2.190000000000000000e+02, 3.974100248033626270e-01
2.200000000000000000e+02, 3.542259815644046572e-01
2.210000000000000000e+02, 3.973159351330217692e-01
2.220000000000000000e+02, 3.541660800850910951e-01
2.230000000000000000e+02, 3.977390389257263736e-01
2.240000000000000000e+02, 3.548569702904599277e-01
2.250000000000000000e+02, 3.983126757235723181e-01
2.260000000000000000e+02, 3.544822309158192630e-01
2.270000000000000000e+02, 3.978992870019767425e-01
2.280000000000000000e+02, 3.544708551491784210e-01
2.290000000000000000e+02, 3.979068155310181432e-01
2.300000000000000000e+02, 3.553375102768007165e-01
2.310000000000000000e+02, 3.986999376302636233e-01
2.320000000000000000e+02, 3.549896563418065698e-01
2.330000000000000000e+02, 3.980902006488653000e-01
2.340000000000000000e+02, 3.547946564409265036e-01
2.350000000000000000e+02, 3.980489128723443959e-01
2.360000000000000000e+02, 3.545981590335439138e-01
2.370000000000000000e+02, 3.979883770139387433e-01
2.380000000000000000e+02, 3.546204987219539473e-01
2.390000000000000000e+02, 3.981009179223599093e-01
2.400000000000000000e+02, 3.550371631771893077e-01
2.410000000000000000e+02, 3.979730054103872705e-01
2.420000000000000000e+02, 3.549130909833424496e-01
2.430000000000000000e+02, 3.981861875570937293e-01
2.440000000000000000e+02, 3.546804882881311460e-01
2.450000000000000000e+02, 3.983258738127961607e-01
2.460000000000000000e+02, 3.548513657362355467e-01
2.470000000000000000e+02, 3.980338756989509896e-01
2.480000000000000000e+02, 3.549656022767727626e-01
2.490000000000000000e+02, 3.982719343456911365e-01
2.500000000000000000e+02, 3.548512339820616424e-01
2.510000000000000000e+02, 3.981089314190445760e-01
2.520000000000000000e+02, 3.549061785021483395e-01
2.530000000000000000e+02, 3.983495344736468491e-01
2.540000000000000000e+02, 3.547285668315953711e-01
2.550000000000000000e+02, 3.978125997680265202e-01
2.560000000000000000e+02, 3.547034309867743707e-01
2.570000000000000000e+02, 3.979815753840192372e-01
2.580000000000000000e+02, 3.544909551498072742e-01
2.590000000000000000e+02, 3.977117289564620073e-01
2.600000000000000000e+02, 3.546976614123530380e-01
2.610000000000000000e+02, 3.978998499234570607e-01
2.620000000000000000e+02, 3.545862912490365670e-01
2.630000000000000000e+02, 3.980442493946979576e-01
2.640000000000000000e+02, 3.547231448755752692e-01
2.650000000000000000e+02, 3.979608874103168770e-01
2.660000000000000000e+02, 3.547926938652213869e-01
2.670000000000000000e+02, 3.983636670692699555e-01
2.680000000000000000e+02, 3.549358043452723876e-01
2.690000000000000000e+02, 3.979482047989062465e-01
2.700000000000000000e+02, 3.547363928330286020e-01
2.710000000000000000e+02, 3.980922716813707352e-01
2.720000000000000000e+02, 3.546496434648475082e-01
2.730000000000000000e+02, 3.978011216933995398e-01
2.740000000000000000e+02, 3.543690778300516153e-01
2.750000000000000000e+02, 3.976813910037427791e-01
2.760000000000000000e+02, 3.547598022523022476e-01
2.770000000000000000e+02, 3.985537702040786723e-01
2.780000000000000000e+02, 3.550193653113470349e-01
2.790000000000000000e+02, 3.984137614349035905e-01
2.800000000000000000e+02, 3.548857640088075582e-01
2.810000000000000000e+02, 3.981033364132361418e-01
2.820000000000000000e+02, 3.547525978120217305e-01
2.830000000000000000e+02, 3.981846848849839304e-01
2.840000000000000000e+02, 3.553304562243900233e-01
2.850000000000000000e+02, 3.983243252781400456e-01
2.860000000000000000e+02, 3.547331819088655469e-01
2.870000000000000000e+02, 3.981521235050440310e-01
2.880000000000000000e+02, 3.551126953471740455e-01
2.890000000000000000e+02, 3.984726602396033712e-01
2.900000000000000000e+02, 3.548420408729869857e-01
2.910000000000000000e+02, 3.983348542156869287e-01
2.920000000000000000e+02, 3.547987980974893207e-01
2.930000000000000000e+02, 3.980035344641858486e-01
2.940000000000000000e+02, 3.544902023251520484e-01
2.950000000000000000e+02, 3.977053627122545398e-01
2.960000000000000000e+02, 3.541131744168856121e-01
2.970000000000000000e+02, 3.975509072126026111e-01
2.980000000000000000e+02, 3.544934419204758824e-01
2.990000000000000000e+02, 3.981157744293858936e-01
3.000000000000000000e+02, 3.545829610682643684e-01
3.010000000000000000e+02, 3.978523013219950055e-01
3.020000000000000000e+02, 3.546603674790670402e-01
3.030000000000000000e+02, 3.979272515243171271e-01
3.040000000000000000e+02, 3.545041928333620973e-01
3.050000000000000000e+02, 3.980311302201529067e-01
3.060000000000000000e+02, 3.544288223888998335e-01
3.070000000000000000e+02, 3.976703485591689402e-01
3.080000000000000000e+02, 3.544446087391657230e-01
3.090000000000000000e+02, 3.979542620346845361e-01
3.100000000000000000e+02, 3.549512483099031002e-01
3.110000000000000000e+02, 3.325843944715832778e-01
3.120000000000000000e+02, 3.162007525064740587e-01
3.130000000000000000e+02, 3.086092100785525760e-01
3.140000000000000000e+02, 3.089600187432596790e-01
3.150000000000000000e+02, 3.087095387265844648e-01
3.160000000000000000e+02, 3.176033258906614254e-01
3.170000000000000000e+02, 3.219502175236358399e-01
3.180000000000000000e+02, 3.334519448131820218e-01
3.190000000000000000e+02, 3.394300707619517521e-01
3.200000000000000000e+02, 3.507643506919814191e-01
3.210000000000000000e+02, 3.564760279938543608e-01
3.220000000000000000e+02, 3.665104773384665893e-01
3.230000000000000000e+02, 3.715561828088834728e-01
3.240000000000000000e+02, 3.790112105590560665e-01
3.250000000000000000e+02, 3.831223478465922705e-01
3.260000000000000000e+02, 3.882031124909697262e-01
3.270000000000000000e+02, 3.908356915467396941e-01
3.280000000000000000e+02, 3.945266508307722630e-01
3.290000000000000000e+02, 3.957942096030279688e-01
3.300000000000000000e+02, 3.979732166830470819e-01
3.310000000000000000e+02, 3.990647942983249763e-01
3.320000000000000000e+02, 3.999137610569778456e-01
3.330000000000000000e+02, 4.003401740096508288e-01
3.340000000000000000e+02, 4.006956407722874758e-01
3.350000000000000000e+02, 4.004593910286821656e-01
3.360000000000000000e+02, 4.002441686896655026e-01
3.370000000000000000e+02, 4.007600565107338753e-01
3.380000000000000000e+02, 4.005161723750316205e-01
3.390000000000000000e+02, 4.003763713801898882e-01
3.400000000000000000e+02, 3.997026215216237244e-01
3.410000000000000000e+02, 3.998173037558747644e-01
3.420000000000000000e+02, 3.990718341298868932e-01
3.430000000000000000e+02, 3.991139913441881237e-01
3.440000000000000000e+02, 3.992568912113939605e-01
3.450000000000000000e+02, 3.994054245491262534e-01
3.460000000000000000e+02, 3.988981510354245863e-01
3.470000000000000000e+02, 3.984398519701009556e-01
3.480000000000000000e+02, 3.981130855018176207e-01
3.490000000000000000e+02, 3.981916172735870951e-01
3.500000000000000000e+02, 3.974941417807362765e-01
3.510000000000000000e+02, 3.974847532522963744e-01
3.520000000000000000e+02, 3.977409366676619706e-01
3.530000000000000000e+02, 3.975767688010982126e-01
3.540000000000000000e+02, 3.978040352127828472e-01
3.550000000000000000e+02, 3.977607267474954078e-01
3.560000000000000000e+02, 3.973982933747349788e-01
3.570000000000000000e+02, 3.974450896905538655e-01
3.580000000000000000e+02, 3.975754069896760279e-01
3.590000000000000000e+02, 3.979052757402754548e-01
3.600000000000000000e+02, 3.980923193569843033e-01
3.610000000000000000e+02, 3.984640644035552515e-01
3.620000000000000000e+02, 3.977859065179556453e-01
3.630000000000000000e+02, 3.981501862845460704e-01
3.640000000000000000e+02, 3.981773347374877314e-01
3.650000000000000000e+02, 3.981117191164814662e-01
3.660000000000000000e+02, 3.980779390484345259e-01
3.670000000000000000e+02, 3.981262032602668754e-01
3.680000000000000000e+02, 3.982064986430594034e-01
3.690000000000000000e+02, 3.982648442933161004e-01
3.700000000000000000e+02, 3.984293263157170362e-01
3.710000000000000000e+02, 3.985431223655078181e-01
3.720000000000000000e+02, 3.986205123053766508e-01
3.730000000000000000e+02, 3.985030769771171766e-01
3.740000000000000000e+02, 3.978242656625099460e-01
3.750000000000000000e+02, 3.977725498644453239e-01
3.760000000000000000e+02, 3.973287180449697198e-01
3.770000000000000000e+02, 3.974586951781787780e-01
3.780000000000000000e+02, 3.977426228456711343e-01
3.790000000000000000e+02, 3.976531511152946452e-01
3.800000000000000000e+02, 3.975822079810921172e-01
3.810000000000000000e+02, 3.979891294388356315e-01
3.820000000000000000e+02, 3.980172635516558977e-01
3.830000000000000000e+02, 3.978476823777225002e-01
3.840000000000000000e+02, 3.981269133243553471e-01
3.850000000000000000e+02, 3.980164928905493005e-01
3.860000000000000000e+02, 3.982604696425967594e-01
3.870000000000000000e+02, 3.981152412849979783e-01
3.880000000000000000e+02, 3.981069962709149479e-01
3.890000000000000000e+02, 3.980594835424178246e-01
3.900000000000000000e+02, 3.984636617048606944e-01
3.910000000000000000e+02, 3.981618059985049252e-01
3.920000000000000000e+02, 3.981171340653837931e-01
3.930000000000000000e+02, 3.982600283673960462e-01
3.940000000000000000e+02, 3.982498037945745306e-01
};

\addlegendentry{target-velocity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=target-velocity-corrected, color=target-velocity-correctedColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 4.000000000000000222e-01
1.000000000000000000e+00, 4.000000000000000222e-01
2.000000000000000000e+00, 3.938060159103708435e-01
3.000000000000000000e+00, 3.970610343253380137e-01
4.000000000000000000e+00, 3.975267328892231333e-01
5.000000000000000000e+00, 3.985228133611647960e-01
6.000000000000000000e+00, 3.979632500008183360e-01
7.000000000000000000e+00, 3.984659473764665116e-01
8.000000000000000000e+00, 3.979239484553557249e-01
9.000000000000000000e+00, 3.978792883413592718e-01
1.000000000000000000e+01, 3.986272084971007046e-01
1.100000000000000000e+01, 3.980826625087686699e-01
1.200000000000000000e+01, 3.981394538677639483e-01
1.300000000000000000e+01, 3.983010985845094609e-01
1.400000000000000000e+01, 3.981416690900636546e-01
1.500000000000000000e+01, 3.979126210234121275e-01
1.600000000000000000e+01, 3.983184110298965130e-01
1.700000000000000000e+01, 3.981248241559719458e-01
1.800000000000000000e+01, 3.978328151691814529e-01
1.900000000000000000e+01, 3.979322969593738213e-01
2.000000000000000000e+01, 4.001115964347072285e-01
2.100000000000000000e+01, 3.972694712726209110e-01
2.200000000000000000e+01, 3.996142149129442989e-01
2.300000000000000000e+01, 3.977100485647281358e-01
2.400000000000000000e+01, 3.995155492819010279e-01
2.500000000000000000e+01, 3.971950956149745138e-01
2.600000000000000000e+01, 3.991896184338764586e-01
2.700000000000000000e+01, 3.970402124491594353e-01
2.800000000000000000e+01, 3.991040296213634875e-01
2.900000000000000000e+01, 3.967337832092427963e-01
3.000000000000000000e+01, 3.994964931327710245e-01
3.100000000000000000e+01, 3.964811145066953202e-01
3.200000000000000000e+01, 4.000965892038444438e-01
3.300000000000000000e+01, 3.966400186120646598e-01
3.400000000000000000e+01, 4.000161566380240341e-01
3.500000000000000000e+01, 3.962132091520049748e-01
3.600000000000000000e+01, 4.001479729613192093e-01
3.700000000000000000e+01, 3.964182317248769460e-01
3.800000000000000000e+01, 4.006869795857256333e-01
3.900000000000000000e+01, 3.963481917480939920e-01
4.000000000000000000e+01, 3.985432200111577172e-01
4.100000000000000000e+01, 3.952143909194825167e-01
4.200000000000000000e+01, 3.966894468191118905e-01
4.300000000000000000e+01, 3.955273591933718969e-01
4.400000000000000000e+01, 3.970820022891488055e-01
4.500000000000000000e+01, 3.969451162544774814e-01
4.600000000000000000e+01, 3.987277357134457190e-01
4.700000000000000000e+01, 3.986766051684734191e-01
4.800000000000000000e+01, 3.991534616424248227e-01
4.900000000000000000e+01, 3.987453501155050484e-01
5.000000000000000000e+01, 3.997241561840185753e-01
5.100000000000000000e+01, 3.986134256594533465e-01
5.200000000000000000e+01, 3.995074028727506610e-01
5.300000000000000000e+01, 3.987454507281923410e-01
5.400000000000000000e+01, 3.994576232695294382e-01
5.500000000000000000e+01, 3.987432398102889186e-01
5.600000000000000000e+01, 3.993563310882705109e-01
5.700000000000000000e+01, 3.989167847464341610e-01
5.800000000000000000e+01, 3.992607650598993252e-01
5.900000000000000000e+01, 3.986135076889971152e-01
6.000000000000000000e+01, 3.989251388209646976e-01
6.100000000000000000e+01, 3.982470309786007023e-01
6.200000000000000000e+01, 3.988609598501204889e-01
6.300000000000000000e+01, 3.984718264722492131e-01
6.400000000000000000e+01, 3.988288824792861065e-01
6.500000000000000000e+01, 3.979633815982122069e-01
6.600000000000000000e+01, 3.992063415026806950e-01
6.700000000000000000e+01, 3.978991353898753136e-01
6.800000000000000000e+01, 4.000451731753853490e-01
6.900000000000000000e+01, 3.975704216144964054e-01
7.000000000000000000e+01, 4.008758593045094187e-01
7.100000000000000000e+01, 3.975559431344695693e-01
7.200000000000000000e+01, 4.008981173077682536e-01
7.300000000000000000e+01, 3.970102984357908316e-01
7.400000000000000000e+01, 3.995035674582551599e-01
7.500000000000000000e+01, 3.966576646800511474e-01
7.600000000000000000e+01, 3.998844556811889106e-01
7.700000000000000000e+01, 3.975808966504759123e-01
7.800000000000000000e+01, 4.001958117836631468e-01
7.900000000000000000e+01, 3.969696405550091067e-01
8.000000000000000000e+01, 4.015993172772173159e-01
8.100000000000000000e+01, 4.292093122340490674e-01
8.200000000000000000e+01, 4.204796682399367658e-01
8.300000000000000000e+01, 4.385932132890335566e-01
8.400000000000000000e+01, 4.230732425486660730e-01
8.500000000000000000e+01, 4.354495159941841886e-01
8.600000000000000000e+01, 4.169611081643679329e-01
8.700000000000000000e+01, 4.271934092742449285e-01
8.800000000000000000e+01, 4.080293047948937435e-01
8.900000000000000000e+01, 4.164891622684473438e-01
9.000000000000000000e+01, 4.000005980413205986e-01
9.100000000000000000e+01, 4.066564425631843394e-01
9.200000000000000000e+01, 3.918093479530395662e-01
9.300000000000000000e+01, 3.990221867500604036e-01
9.400000000000000000e+01, 3.868853332971790571e-01
9.500000000000000000e+01, 3.946108260446266058e-01
9.600000000000000000e+01, 3.841301353132839935e-01
9.700000000000000000e+01, 3.886512218083235659e-01
9.800000000000000000e+01, 3.813333557550565578e-01
9.900000000000000000e+01, 3.797317483234806668e-01
1.000000000000000000e+02, 3.754350699025527094e-01
1.010000000000000000e+02, 3.752526061416432412e-01
1.020000000000000000e+02, 3.737505252086093521e-01
1.030000000000000000e+02, 3.750984450608623177e-01
1.040000000000000000e+02, 3.770305143142501092e-01
1.050000000000000000e+02, 3.805630327254679868e-01
1.060000000000000000e+02, 3.822969276325671739e-01
1.070000000000000000e+02, 3.852739244789844530e-01
1.080000000000000000e+02, 3.876583777969953015e-01
1.090000000000000000e+02, 3.904261613209158988e-01
1.100000000000000000e+02, 3.920144044099901359e-01
1.110000000000000000e+02, 3.934233462711479445e-01
1.120000000000000000e+02, 3.943881073041507479e-01
1.130000000000000000e+02, 3.955488573015918941e-01
1.140000000000000000e+02, 3.964351343049111187e-01
1.150000000000000000e+02, 3.976407392184160283e-01
1.160000000000000000e+02, 3.980032716666572767e-01
1.170000000000000000e+02, 3.985238773660928491e-01
1.180000000000000000e+02, 3.988086664296539574e-01
1.190000000000000000e+02, 3.986450742805589531e-01
1.200000000000000000e+02, 3.990629550662139202e-01
1.210000000000000000e+02, 3.995187595932547797e-01
1.220000000000000000e+02, 3.991239341574101540e-01
1.230000000000000000e+02, 3.989963013590284158e-01
1.240000000000000000e+02, 3.987452523937831117e-01
1.250000000000000000e+02, 3.987807408889785799e-01
1.260000000000000000e+02, 3.980175273459909957e-01
1.270000000000000000e+02, 3.984452981322691434e-01
1.280000000000000000e+02, 3.970524295859916286e-01
1.290000000000000000e+02, 3.986246086840534719e-01
1.300000000000000000e+02, 3.968148756223736084e-01
1.310000000000000000e+02, 3.968952650886040656e-01
1.320000000000000000e+02, 3.931637877906642431e-01
1.330000000000000000e+02, 3.950848149326737779e-01
1.340000000000000000e+02, 3.924030273510022981e-01
1.350000000000000000e+02, 3.949752774163726166e-01
1.360000000000000000e+02, 3.946454822082883229e-01
1.370000000000000000e+02, 3.978124062804987426e-01
1.380000000000000000e+02, 3.974333072860454230e-01
1.390000000000000000e+02, 3.994719329724313317e-01
1.400000000000000000e+02, 3.982712110883840362e-01
1.410000000000000000e+02, 3.998614801696783738e-01
1.420000000000000000e+02, 3.986630569566249616e-01
1.430000000000000000e+02, 4.005721569374152136e-01
1.440000000000000000e+02, 3.996712491120678057e-01
1.450000000000000000e+02, 4.014304960196606320e-01
1.460000000000000000e+02, 3.996151945488277679e-01
1.470000000000000000e+02, 4.013596066178559685e-01
1.480000000000000000e+02, 3.990290036800425155e-01
1.490000000000000000e+02, 4.006074087756071322e-01
1.500000000000000000e+02, 3.985826046825161617e-01
1.510000000000000000e+02, 4.004024444420146711e-01
1.520000000000000000e+02, 3.981275726577638840e-01
1.530000000000000000e+02, 3.997725920587092419e-01
1.540000000000000000e+02, 3.981116631020458763e-01
1.550000000000000000e+02, 3.993816840656221334e-01
1.560000000000000000e+02, 3.973840888952074879e-01
1.570000000000000000e+02, 3.991411175633038932e-01
1.580000000000000000e+02, 3.971097774378581358e-01
1.590000000000000000e+02, 3.986868470182468593e-01
1.600000000000000000e+02, 3.964985675407426968e-01
1.610000000000000000e+02, 3.978340651189222754e-01
1.620000000000000000e+02, 3.958878494729438646e-01
1.630000000000000000e+02, 3.969738789857619743e-01
1.640000000000000000e+02, 3.956038877104895435e-01
1.650000000000000000e+02, 3.974645670124982155e-01
1.660000000000000000e+02, 3.958561891702954139e-01
1.670000000000000000e+02, 3.982110422620892543e-01
1.680000000000000000e+02, 3.971749819046442864e-01
1.690000000000000000e+02, 3.991477994801784224e-01
1.700000000000000000e+02, 3.974164835934406170e-01
1.710000000000000000e+02, 3.993853921480824409e-01
1.720000000000000000e+02, 3.980081341034831244e-01
1.730000000000000000e+02, 3.996728558992949099e-01
1.740000000000000000e+02, 3.981584393188664084e-01
1.750000000000000000e+02, 3.998786801217181219e-01
1.760000000000000000e+02, 3.980437287319281148e-01
1.770000000000000000e+02, 3.999107298313627767e-01
1.780000000000000000e+02, 3.982291633488531657e-01
1.790000000000000000e+02, 4.000380533184230147e-01
1.800000000000000000e+02, 3.981326420915471953e-01
1.810000000000000000e+02, 3.994141703615303740e-01
1.820000000000000000e+02, 3.973854451905828866e-01
1.830000000000000000e+02, 3.994431551229579158e-01
1.840000000000000000e+02, 3.971556023210482955e-01
1.850000000000000000e+02, 3.988225606018224179e-01
1.860000000000000000e+02, 3.966253814393326804e-01
1.870000000000000000e+02, 3.996210194693151641e-01
1.880000000000000000e+02, 4.294605046717675512e-01
1.890000000000000000e+02, 4.186317854160276353e-01
1.900000000000000000e+02, 4.393400732073989845e-01
1.910000000000000000e+02, 4.210586013554163953e-01
1.920000000000000000e+02, 4.213567465279102198e-01
1.930000000000000000e+02, 4.094717214301180075e-01
1.940000000000000000e+02, 3.979688191026137245e-01
1.950000000000000000e+02, 3.927072988174998280e-01
1.960000000000000000e+02, 3.859598991930631717e-01
1.970000000000000000e+02, 3.827568662594578175e-01
1.980000000000000000e+02, 3.814592040898068248e-01
1.990000000000000000e+02, 3.814006907013482994e-01
2.000000000000000000e+02, 3.821336028310098332e-01
2.010000000000000000e+02, 3.828049183472858052e-01
2.020000000000000000e+02, 3.840749899404304335e-01
2.030000000000000000e+02, 3.853957045453302310e-01
2.040000000000000000e+02, 3.871998024411829609e-01
2.050000000000000000e+02, 3.883518458822469155e-01
2.060000000000000000e+02, 3.901899490570576168e-01
2.070000000000000000e+02, 3.914066609023739707e-01
2.080000000000000000e+02, 3.930608491916392500e-01
2.090000000000000000e+02, 3.942576237175970388e-01
2.100000000000000000e+02, 3.949580841775470197e-01
2.110000000000000000e+02, 3.956997692569043101e-01
2.120000000000000000e+02, 3.965819829362870474e-01
2.130000000000000000e+02, 3.969842189129180743e-01
2.140000000000000000e+02, 3.974759591450315321e-01
2.150000000000000000e+02, 3.981286596700996938e-01
2.160000000000000000e+02, 3.985455749043006479e-01
2.170000000000000000e+02, 3.981791046259786082e-01
2.180000000000000000e+02, 3.984485563815655662e-01
2.190000000000000000e+02, 3.978592025077366534e-01
2.200000000000000000e+02, 3.988856019952736753e-01
2.210000000000000000e+02, 3.968825031105555623e-01
2.220000000000000000e+02, 3.984955002224510046e-01
2.230000000000000000e+02, 3.969698469894025195e-01
2.240000000000000000e+02, 3.987653680702899495e-01
2.250000000000000000e+02, 3.975487115763135515e-01
2.260000000000000000e+02, 3.985179840959170439e-01
2.270000000000000000e+02, 3.972385999674091783e-01
2.280000000000000000e+02, 3.983599982209412582e-01
2.290000000000000000e+02, 3.971220693140081748e-01
2.300000000000000000e+02, 3.984889624307077494e-01
2.310000000000000000e+02, 3.970944898244660459e-01
2.320000000000000000e+02, 3.981991601577505313e-01
2.330000000000000000e+02, 3.963853207580917415e-01
2.340000000000000000e+02, 3.977871354531740122e-01
2.350000000000000000e+02, 3.970209289660519003e-01
2.360000000000000000e+02, 3.980082131341378116e-01
2.370000000000000000e+02, 3.968974871920424308e-01
2.380000000000000000e+02, 3.982838522579413842e-01
2.390000000000000000e+02, 3.971611710180602550e-01
2.400000000000000000e+02, 3.984571232123025331e-01
2.410000000000000000e+02, 3.963213569284048665e-01
2.420000000000000000e+02, 3.980157060215377962e-01
2.430000000000000000e+02, 3.965633926540861331e-01
2.440000000000000000e+02, 3.985760570706253780e-01
2.450000000000000000e+02, 3.963607747480708543e-01
2.460000000000000000e+02, 3.988144849797150004e-01
2.470000000000000000e+02, 3.968018723085589006e-01
2.480000000000000000e+02, 3.989772659415191658e-01
2.490000000000000000e+02, 3.972636714702213467e-01
2.500000000000000000e+02, 3.991446509964751144e-01
2.510000000000000000e+02, 3.966952019910382488e-01
2.520000000000000000e+02, 3.981271828931455814e-01
2.530000000000000000e+02, 3.963858059581323312e-01
2.540000000000000000e+02, 3.971019751363968897e-01
2.550000000000000000e+02, 3.962782809640454373e-01
2.560000000000000000e+02, 3.970521934036177480e-01
2.570000000000000000e+02, 3.959646256347991722e-01
2.580000000000000000e+02, 3.968622189583838056e-01
2.590000000000000000e+02, 3.973785167390659900e-01
2.600000000000000000e+02, 3.980728984119221159e-01
2.610000000000000000e+02, 3.983682922507386093e-01
2.620000000000000000e+02, 3.981111432240239667e-01
2.630000000000000000e+02, 3.981550335850412847e-01
2.640000000000000000e+02, 3.980171426375472832e-01
2.650000000000000000e+02, 3.979800779010234657e-01
2.660000000000000000e+02, 3.985566689521560235e-01
2.670000000000000000e+02, 3.986426878506318938e-01
2.680000000000000000e+02, 3.982702106752463722e-01
2.690000000000000000e+02, 3.982401702978788371e-01
2.700000000000000000e+02, 3.983488616358943357e-01
2.710000000000000000e+02, 3.984631737620216718e-01
2.720000000000000000e+02, 3.984171148931491269e-01
2.730000000000000000e+02, 3.982868055938106888e-01
2.740000000000000000e+02, 3.985218067894559790e-01
2.750000000000000000e+02, 3.975958137711812501e-01
2.760000000000000000e+02, 3.981255358475619399e-01
2.770000000000000000e+02, 3.976044705471512009e-01
2.780000000000000000e+02, 3.984059523918075940e-01
2.790000000000000000e+02, 3.973636034583671317e-01
2.800000000000000000e+02, 3.995686089156452736e-01
2.810000000000000000e+02, 3.973452597983634926e-01
2.820000000000000000e+02, 4.001520178935229488e-01
2.830000000000000000e+02, 3.975019628693658991e-01
2.840000000000000000e+02, 3.994740001445200583e-01
2.850000000000000000e+02, 3.967098464926395174e-01
2.860000000000000000e+02, 3.978016614326283507e-01
2.870000000000000000e+02, 3.965430682253042183e-01
2.880000000000000000e+02, 3.973182940651204254e-01
2.890000000000000000e+02, 3.963162522742305072e-01
2.900000000000000000e+02, 3.968362156748831415e-01
2.910000000000000000e+02, 3.963265152673174918e-01
2.920000000000000000e+02, 3.964588565968221179e-01
2.930000000000000000e+02, 3.957426726364286496e-01
2.940000000000000000e+02, 3.975870818479879665e-01
2.950000000000000000e+02, 3.963433667377376235e-01
2.960000000000000000e+02, 3.971023778722666542e-01
2.970000000000000000e+02, 3.967968490582181595e-01
2.980000000000000000e+02, 3.972028198963713508e-01
2.990000000000000000e+02, 3.964252473254450404e-01
3.000000000000000000e+02, 3.978011883387814196e-01
3.010000000000000000e+02, 3.960337785918702780e-01
3.020000000000000000e+02, 3.976583711608854821e-01
3.030000000000000000e+02, 3.969286347729511499e-01
3.040000000000000000e+02, 3.983640106784009927e-01
3.050000000000000000e+02, 3.971470765596110120e-01
3.060000000000000000e+02, 3.985780287893975760e-01
3.070000000000000000e+02, 3.971471198886845633e-01
3.080000000000000000e+02, 3.982855111786404723e-01
3.090000000000000000e+02, 3.971735540677436838e-01
3.100000000000000000e+02, 3.980172286689522831e-01
3.110000000000000000e+02, 3.965358075081938938e-01
3.120000000000000000e+02, 3.960366487852167161e-01
3.130000000000000000e+02, 3.223038629672716482e-01
3.140000000000000000e+02, 3.469930199771746882e-01
3.150000000000000000e+02, 2.934430061775969434e-01
3.160000000000000000e+02, 3.334716894500698303e-01
3.170000000000000000e+02, 2.907725924531229245e-01
3.180000000000000000e+02, 3.414777633844857663e-01
3.190000000000000000e+02, 2.978020859572561019e-01
3.200000000000000000e+02, 3.512417870410666776e-01
3.210000000000000000e+02, 3.361954831424419643e-01
3.220000000000000000e+02, 3.613956786974099611e-01
3.230000000000000000e+02, 3.922784150615722942e-01
3.240000000000000000e+02, 3.769031560554424454e-01
3.250000000000000000e+02, 3.923547407525075914e-01
3.260000000000000000e+02, 4.179782798120194598e-01
3.270000000000000000e+02, 4.183416264110091931e-01
3.280000000000000000e+02, 4.428330728611017397e-01
3.290000000000000000e+02, 4.519710690082122118e-01
3.300000000000000000e+02, 4.656304895646465880e-01
3.310000000000000000e+02, 4.698492312424777939e-01
3.320000000000000000e+02, 4.740997072274198976e-01
3.330000000000000000e+02, 4.699064393246467630e-01
3.340000000000000000e+02, 4.676674243357983318e-01
3.350000000000000000e+02, 4.587193220354629508e-01
3.360000000000000000e+02, 4.535867197989900124e-01
3.370000000000000000e+02, 4.430158039871881503e-01
3.380000000000000000e+02, 4.399651367529207047e-01
3.390000000000000000e+02, 4.292403412967372711e-01
3.400000000000000000e+02, 4.270957118270309882e-01
3.410000000000000000e+02, 4.176372799921850287e-01
3.420000000000000000e+02, 4.157314497228801198e-01
3.430000000000000000e+02, 4.067802845352491703e-01
3.440000000000000000e+02, 4.046776841260796287e-01
3.450000000000000000e+02, 4.002721645795386252e-01
3.460000000000000000e+02, 3.991148479649479497e-01
3.470000000000000000e+02, 3.974159368923330105e-01
3.480000000000000000e+02, 3.980032881964112867e-01
3.490000000000000000e+02, 3.971776660712490470e-01
3.500000000000000000e+02, 3.971856542845483284e-01
3.510000000000000000e+02, 3.963892277652475427e-01
3.520000000000000000e+02, 3.973302331448510527e-01
3.530000000000000000e+02, 3.965022132248468556e-01
3.540000000000000000e+02, 3.972985237879674836e-01
3.550000000000000000e+02, 3.964909887425354107e-01
3.560000000000000000e+02, 3.973296124256678885e-01
3.570000000000000000e+02, 3.968443677319289375e-01
3.580000000000000000e+02, 3.979357502678969039e-01
3.590000000000000000e+02, 3.974163350854068022e-01
3.600000000000000000e+02, 3.982611934946382326e-01
3.610000000000000000e+02, 3.979389589006231409e-01
3.620000000000000000e+02, 3.985245972312930762e-01
3.630000000000000000e+02, 3.981499825457773811e-01
3.640000000000000000e+02, 3.988397604848817890e-01
3.650000000000000000e+02, 3.978441246607633541e-01
3.660000000000000000e+02, 3.990391880097502453e-01
3.670000000000000000e+02, 3.983178119029351372e-01
3.680000000000000000e+02, 3.994615848450748796e-01
3.690000000000000000e+02, 3.982526414827057826e-01
3.700000000000000000e+02, 3.989436755398731438e-01
3.710000000000000000e+02, 3.979018501692809240e-01
3.720000000000000000e+02, 4.009188765656458986e-01
3.730000000000000000e+02, 3.968358958999435582e-01
3.740000000000000000e+02, 4.005662708479702516e-01
3.750000000000000000e+02, 3.969820045540006226e-01
3.760000000000000000e+02, 3.997466998951348938e-01
3.770000000000000000e+02, 3.958368090141974882e-01
3.780000000000000000e+02, 3.992598909344096114e-01
3.790000000000000000e+02, 3.964304756046690970e-01
3.800000000000000000e+02, 3.991939104171573494e-01
3.810000000000000000e+02, 3.963509370918688601e-01
3.820000000000000000e+02, 3.997035953910240691e-01
3.830000000000000000e+02, 3.964737312415337334e-01
3.840000000000000000e+02, 3.993355206282129810e-01
3.850000000000000000e+02, 3.962939291090247784e-01
3.860000000000000000e+02, 4.001195423212967617e-01
3.870000000000000000e+02, 3.966585183284214722e-01
3.880000000000000000e+02, 4.003478932952067026e-01
3.890000000000000000e+02, 3.960057292277557872e-01
3.900000000000000000e+02, 4.007022852629196219e-01
3.910000000000000000e+02, 3.968880526781625173e-01
3.920000000000000000e+02, 4.012552526910261874e-01
3.930000000000000000e+02, 3.966132612869056606e-01
3.940000000000000000e+02, 4.015836633058765259e-01
};

\addlegendentry{target-velocity-corrected}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_high_rotation.tex <==
\addplot [name path=sensor-rotation-0, color=sensor-rotation-0Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 1.734775087910714331e-02
1.000000000000000000e+00, 5.546405272775582762e-02
2.000000000000000000e+00, 5.881213914660684411e-02
3.000000000000000000e+00, 8.443240854236300219e-02
4.000000000000000000e+00, 1.367312596701014682e-01
5.000000000000000000e+00, 2.346494814108587568e-01
6.000000000000000000e+00, 2.889969340003982756e-01
7.000000000000000000e+00, 2.920167262264339869e-01
8.000000000000000000e+00, 2.848560573336696433e-01
9.000000000000000000e+00, 2.163056973040013986e-01
1.000000000000000000e+01, 1.421826996906337404e-01
1.100000000000000000e+01, 1.147239511364946812e-01
1.200000000000000000e+01, 9.539902161712413009e-02
1.300000000000000000e+01, 8.114910630465901886e-02
1.400000000000000000e+01, 7.398450044262643022e-02
1.500000000000000000e+01, 5.594756300126751264e-02
1.600000000000000000e+01, 5.921909304288176107e-02
1.700000000000000000e+01, 6.451509181264847292e-02
1.800000000000000000e+01, 5.845507532946053741e-02
1.900000000000000000e+01, 1.143950441837348758e-01
2.000000000000000000e+01, 1.960532411929149510e-01
2.100000000000000000e+01, 3.996440370534312114e-01
2.200000000000000000e+01, 7.528479147883564426e-01
2.300000000000000000e+01, 6.206476097660938995e-01
2.400000000000000000e+01, 2.909931675392078421e-01
2.500000000000000000e+01, 1.205133972208630444e-01
2.600000000000000000e+01, 6.759618386053362071e-02
2.700000000000000000e+01, 3.561660955775560605e-02
2.800000000000000000e+01, 5.443997760638721872e-02
2.900000000000000000e+01, 2.327646107590521096e-02
3.000000000000000000e+01, 7.481743007418356628e-02
3.100000000000000000e+01, 3.583405971415119795e-02
3.200000000000000000e+01, 8.288105990161327707e-02
3.300000000000000000e+01, 8.841568623015282069e-02
3.400000000000000000e+01, 1.717803524489905087e-01
3.500000000000000000e+01, 1.750674277187490857e-01
3.600000000000000000e+01, 2.006165409523946730e-01
3.700000000000000000e+01, 2.632633610145608261e-01
3.800000000000000000e+01, 2.429599822867604397e-01
3.900000000000000000e+01, 2.006776744851348493e-01
4.000000000000000000e+01, 1.567708235963497787e-01
4.100000000000000000e+01, 1.027509166509200239e-01
4.200000000000000000e+01, 1.074194226786397283e-01
4.300000000000000000e+01, 3.959711439766476493e-02
4.400000000000000000e+01, 4.084614222991012067e-02
4.500000000000000000e+01, 3.457409221527660281e-02
4.600000000000000000e+01, 5.312992942608930208e-02
4.700000000000000000e+01, 2.877625089297877400e-02
4.800000000000000000e+01, 3.120865400216556174e-02
4.900000000000000000e+01, 1.055926240595968790e-01
5.000000000000000000e+01, 2.006331130531610885e-01
5.100000000000000000e+01, 4.851179575614314454e-01
5.200000000000000000e+01, 7.799202174305555069e-01
5.300000000000000000e+01, 5.370430673639239316e-01
5.400000000000000000e+01, 2.449948893692222573e-01
5.500000000000000000e+01, 1.481727219992012845e-01
5.600000000000000000e+01, 8.526165285805863137e-02
5.700000000000000000e+01, 1.064078479091751378e-01
5.800000000000000000e+01, 5.446397332055569196e-02
5.900000000000000000e+01, 5.734147107723074066e-02
6.000000000000000000e+01, 4.045429556812137756e-02
6.100000000000000000e+01, 7.552197065811623589e-02
6.200000000000000000e+01, 9.484060046175800396e-02
6.300000000000000000e+01, 9.202612610809648985e-02
6.400000000000000000e+01, 1.391285452685106505e-01
6.500000000000000000e+01, 1.490263356339238399e-01
6.600000000000000000e+01, 2.504615754561312357e-01
6.700000000000000000e+01, 3.073452878597677240e-01
6.800000000000000000e+01, 3.219954399004568146e-01
6.900000000000000000e+01, 2.500792043484618699e-01
7.000000000000000000e+01, 1.989685665174043272e-01
7.100000000000000000e+01, 1.563226196894931253e-01
7.200000000000000000e+01, 7.371034597297206059e-02
7.300000000000000000e+01, 6.425523969200033769e-02
7.400000000000000000e+01, 4.814417158457996032e-02
7.500000000000000000e+01, 1.690551420553627199e-02
7.600000000000000000e+01, 5.933901745031085889e-02
7.700000000000000000e+01, 7.193394618026911769e-02
7.800000000000000000e+01, 1.076672980418671988e-01
7.900000000000000000e+01, 1.361099659581358756e-01
8.000000000000000000e+01, 2.001189436914138919e-01
8.100000000000000000e+01, 2.786640816553488387e-01
8.200000000000000000e+01, 2.928933781946066461e-01
8.300000000000000000e+01, 3.118650711077236570e-01
8.400000000000000000e+01, 2.109953708732148769e-01
8.500000000000000000e+01, 1.643077652060982718e-01
8.600000000000000000e+01, 1.327918665485224026e-01
8.700000000000000000e+01, 8.434476166283302878e-02
8.800000000000000000e+01, 1.094238164004988079e-01
8.900000000000000000e+01, 6.059932993132725876e-02
9.000000000000000000e+01, 5.238261422583962573e-02
9.100000000000000000e+01, 3.709562854403573862e-02
9.200000000000000000e+01, 6.368032733992884387e-02
9.300000000000000000e+01, 7.008555412839645449e-02
9.400000000000000000e+01, 1.020129550533494939e-01
9.500000000000000000e+01, 1.497842105369762422e-01
9.600000000000000000e+01, 3.012891440712595070e-01
9.700000000000000000e+01, 6.402357798284861179e-01
9.800000000000000000e+01, 7.656177076447825414e-01
9.900000000000000000e+01, 3.594225659902298697e-01
1.000000000000000000e+02, 1.755710934818164037e-01
1.010000000000000000e+02, 8.487189653447595183e-02
1.020000000000000000e+02, 4.336133703131014178e-02
1.030000000000000000e+02, 2.325540444929651007e-02
1.040000000000000000e+02, 1.321167201273031576e-02
1.050000000000000000e+02, 2.088290902862616552e-02
1.060000000000000000e+02, 5.520042502711561272e-02
1.070000000000000000e+02, 5.033994064902354987e-02
1.080000000000000000e+02, 1.026634767633636119e-01
1.090000000000000000e+02, 1.213458518023743105e-01
1.100000000000000000e+02, 1.685616351086460518e-01
1.110000000000000000e+02, 2.000005768874816570e-01
1.120000000000000000e+02, 2.218093317338289128e-01
1.130000000000000000e+02, 2.494955033806016687e-01
1.140000000000000000e+02, 2.196214290968077631e-01
1.150000000000000000e+02, 1.765310989006820264e-01
1.160000000000000000e+02, 1.424114577034028828e-01
1.170000000000000000e+02, 9.349005337559929130e-02
1.180000000000000000e+02, 7.597515194211648670e-02
1.190000000000000000e+02, 4.948166108181534240e-02
1.200000000000000000e+02, 5.754589839868853862e-02
1.210000000000000000e+02, 2.091724735698418866e-02
1.220000000000000000e+02, 1.129367867915010391e-02
1.230000000000000000e+02, 4.594569917942940840e-02
1.240000000000000000e+02, 5.630982177470387345e-02
1.250000000000000000e+02, 1.437850960944200007e-01
1.260000000000000000e+02, 3.173881269513177950e-01
1.270000000000000000e+02, 6.912471943800616581e-01
1.280000000000000000e+02, 6.621308355114260413e-01
1.290000000000000000e+02, 3.156494547581650822e-01
1.300000000000000000e+02, 1.541333177843166591e-01
1.310000000000000000e+02, 1.129116952646510991e-01
1.320000000000000000e+02, 6.931645044276707468e-02
1.330000000000000000e+02, 7.572573803905872925e-02
1.340000000000000000e+02, 5.856004680520889016e-02
1.350000000000000000e+02, 5.329483751564861871e-02
1.360000000000000000e+02, 8.559622462488776506e-02
1.370000000000000000e+02, 9.007920038632409587e-02
1.380000000000000000e+02, 9.204460636734715373e-02
1.390000000000000000e+02, 9.741809237772618146e-02
1.400000000000000000e+02, 1.549587265122485680e-01
1.410000000000000000e+02, 2.525529489975267827e-01
1.420000000000000000e+02, 2.941598017374888463e-01
1.430000000000000000e+02, 2.830882698576039358e-01
1.440000000000000000e+02, 2.897527163920316506e-01
1.450000000000000000e+02, 1.957526409218039443e-01
1.460000000000000000e+02, 1.488787565276724900e-01
1.470000000000000000e+02, 8.806575349710814293e-02
1.480000000000000000e+02, 6.242703095226870974e-02
1.490000000000000000e+02, 3.880389991407186961e-02
1.500000000000000000e+02, 3.124233638174619271e-02
1.510000000000000000e+02, 2.390625990895465028e-02
1.520000000000000000e+02, 5.759442220632708664e-02
1.530000000000000000e+02, 9.344564037662239642e-02
1.540000000000000000e+02, 1.309731668624760925e-01
1.550000000000000000e+02, 1.995994084345833475e-01
1.560000000000000000e+02, 2.545433155147087678e-01
1.570000000000000000e+02, 3.240496457696255828e-01
1.580000000000000000e+02, 3.016829553756562032e-01
1.590000000000000000e+02, 2.421559362030585860e-01
1.600000000000000000e+02, 2.071235556014867363e-01
1.610000000000000000e+02, 1.300956139781432042e-01
1.620000000000000000e+02, 9.322513929004697109e-02
1.630000000000000000e+02, 9.107068376064908488e-02
1.640000000000000000e+02, 6.748045654407450189e-02
1.650000000000000000e+02, 9.010393937739599735e-02
1.660000000000000000e+02, 4.964245953052938420e-02
1.670000000000000000e+02, 6.411656716021939262e-02
1.680000000000000000e+02, 7.163100651696607812e-02
1.690000000000000000e+02, 7.955385554830012029e-02
1.700000000000000000e+02, 1.420288987352954779e-01
1.710000000000000000e+02, 2.020845144028299567e-01
1.720000000000000000e+02, 4.715976024063248118e-01
1.730000000000000000e+02, 7.538578704380528572e-01
1.740000000000000000e+02, 5.288295009779004907e-01
1.750000000000000000e+02, 2.415866503114584840e-01
1.760000000000000000e+02, 9.612556844374270382e-02
1.770000000000000000e+02, 5.729128773372757499e-02
1.780000000000000000e+02, 2.245775874018638221e-02
1.790000000000000000e+02, 1.547309059625591801e-02
1.800000000000000000e+02, 5.170838931645881792e-02
1.810000000000000000e+02, 4.413160756944212865e-02
1.820000000000000000e+02, 4.124184023926162623e-02
1.830000000000000000e+02, 7.771951231522102044e-02
1.840000000000000000e+02, 9.652511312562664370e-02
1.850000000000000000e+02, 1.626069370833662653e-01
1.860000000000000000e+02, 1.984241963053561819e-01
1.870000000000000000e+02, 2.252176088135736387e-01
1.880000000000000000e+02, 2.079902079314871755e-01
1.890000000000000000e+02, 2.068814408847919895e-01
1.900000000000000000e+02, 2.150391583311072052e-01
1.910000000000000000e+02, 1.545570469767938993e-01
1.920000000000000000e+02, 1.026611856276965079e-01
1.930000000000000000e+02, 7.777510463112045913e-02
1.940000000000000000e+02, 5.376422026181961605e-02
};

\addlegendentry{sensor-rotation-0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=sensor-rotation-1, color=sensor-rotation-1Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 2.995118814211224570e-02
1.000000000000000000e+00, 4.321811702181677789e-02
2.000000000000000000e+00, 6.254454004329937367e-02
3.000000000000000000e+00, 1.163191624937365415e-01
4.000000000000000000e+00, 1.338022295162364372e-01
5.000000000000000000e+00, 2.557754605304469186e-01
6.000000000000000000e+00, 2.867536559854332867e-01
7.000000000000000000e+00, 3.301606064920022954e-01
8.000000000000000000e+00, 2.310145116383000019e-01
9.000000000000000000e+00, 2.023168180788561532e-01
1.000000000000000000e+01, 1.344054638448434758e-01
1.100000000000000000e+01, 1.117152697657100846e-01
1.200000000000000000e+01, 7.111966485181199504e-02
1.300000000000000000e+01, 6.462338483902459185e-02
1.400000000000000000e+01, 5.997977642152298172e-02
1.500000000000000000e+01, 4.657108235145108327e-02
1.600000000000000000e+01, 1.646700444502391392e-02
1.700000000000000000e+01, 7.673124736715902783e-02
1.800000000000000000e+01, 7.182824619535786714e-02
1.900000000000000000e+01, 1.118661394247073698e-01
2.000000000000000000e+01, 1.666134247903095500e-01
2.100000000000000000e+01, 3.636298183670902406e-01
2.200000000000000000e+01, 7.321359310990975811e-01
2.300000000000000000e+01, 6.153945888852166979e-01
2.400000000000000000e+01, 2.885187522495945012e-01
2.500000000000000000e+01, 1.439237464947866751e-01
2.600000000000000000e+01, 7.284186227800924784e-02
2.700000000000000000e+01, 3.702484894486690603e-02
2.800000000000000000e+01, 4.192348236224818087e-02
2.900000000000000000e+01, 3.086884150621318698e-02
3.000000000000000000e+01, 2.835645838490654172e-02
3.100000000000000000e+01, 6.041849757267015592e-02
3.200000000000000000e+01, 5.647531553590823261e-02
3.300000000000000000e+01, 1.007222407648006579e-01
3.400000000000000000e+01, 1.275856392168041031e-01
3.500000000000000000e+01, 1.626799152018244266e-01
3.600000000000000000e+01, 2.262852142997451854e-01
3.700000000000000000e+01, 2.445646185195562428e-01
3.800000000000000000e+01, 2.479198710792441251e-01
3.900000000000000000e+01, 2.148244112055696375e-01
4.000000000000000000e+01, 9.450393233016382566e-02
4.100000000000000000e+01, 8.956035729050795813e-02
4.200000000000000000e+01, 8.918668477925437155e-02
4.300000000000000000e+01, 4.001117261085133242e-02
4.400000000000000000e+01, 2.128399882787240793e-02
4.500000000000000000e+01, 3.536735109912425568e-02
4.600000000000000000e+01, 6.404502336647364957e-02
4.700000000000000000e+01, 6.378121320648104386e-02
4.800000000000000000e+01, 1.211846291554826149e-01
4.900000000000000000e+01, 2.188259949115219094e-01
5.000000000000000000e+01, 4.967099950949234732e-01
5.100000000000000000e+01, 7.829943624197711616e-01
5.200000000000000000e+01, 4.610651540396988879e-01
5.300000000000000000e+01, 1.976141747839870733e-01
5.400000000000000000e+01, 1.293067740821709777e-01
5.500000000000000000e+01, 1.167413820338815134e-01
5.600000000000000000e+01, 6.430158575602558380e-02
5.700000000000000000e+01, 6.938210708733168197e-02
5.800000000000000000e+01, 3.966906829065221241e-02
5.900000000000000000e+01, 6.861533525738733319e-02
6.000000000000000000e+01, 6.843284196244552031e-02
6.100000000000000000e+01, 7.820163441214857125e-02
6.200000000000000000e+01, 9.590982897041984423e-02
6.300000000000000000e+01, 1.405630927878129821e-01
6.400000000000000000e+01, 1.851290264198648672e-01
6.500000000000000000e+01, 2.414453825030654366e-01
6.600000000000000000e+01, 3.114004811861219579e-01
6.700000000000000000e+01, 2.865554525627649340e-01
6.800000000000000000e+01, 2.113854698251953768e-01
6.900000000000000000e+01, 1.871990196561603426e-01
7.000000000000000000e+01, 1.169109014116054279e-01
7.100000000000000000e+01, 5.036779461441281275e-02
7.200000000000000000e+01, 4.291533709338835739e-02
7.300000000000000000e+01, 1.911133455097853082e-02
7.400000000000000000e+01, 3.739853398820105340e-02
7.500000000000000000e+01, 3.186900547405355222e-02
7.600000000000000000e+01, 7.358903133654016993e-02
7.700000000000000000e+01, 9.752926243683689156e-02
7.800000000000000000e+01, 1.454001135386787102e-01
7.900000000000000000e+01, 2.205515272250424541e-01
8.000000000000000000e+01, 2.614942117124376408e-01
8.100000000000000000e+01, 3.100807065941099117e-01
8.200000000000000000e+01, 2.797940654155161022e-01
8.300000000000000000e+01, 2.078971886538743818e-01
8.400000000000000000e+01, 1.226023664589713374e-01
8.500000000000000000e+01, 8.174052706347836872e-02
8.600000000000000000e+01, 1.017169653176425298e-01
8.700000000000000000e+01, 6.607583533446118040e-02
8.800000000000000000e+01, 5.275523044176918391e-02
8.900000000000000000e+01, 5.460795173025774496e-02
9.000000000000000000e+01, 5.246086691662286278e-02
9.100000000000000000e+01, 5.899040501588281166e-02
9.200000000000000000e+01, 9.398808764429901486e-02
9.300000000000000000e+01, 1.614695792376694139e-01
9.400000000000000000e+01, 3.639190712237464487e-01
9.500000000000000000e+01, 7.499149221766484574e-01
9.600000000000000000e+01, 6.554804942148502178e-01
9.700000000000000000e+01, 2.921013971361517414e-01
9.800000000000000000e+01, 1.516376373617786544e-01
9.900000000000000000e+01, 7.788930009087656481e-02
1.000000000000000000e+02, 3.349992814284031423e-02
1.010000000000000000e+02, 2.274905381151953038e-02
1.020000000000000000e+02, 2.071750334372390520e-02
1.030000000000000000e+02, 4.729133777243296755e-02
1.040000000000000000e+02, 4.940478317564352129e-02
1.050000000000000000e+02, 1.068196640628727850e-01
1.060000000000000000e+02, 1.144891211647035695e-01
1.070000000000000000e+02, 1.347278209056618492e-01
1.080000000000000000e+02, 1.856671861888558595e-01
1.090000000000000000e+02, 2.160962872295118520e-01
1.100000000000000000e+02, 2.404175053179588295e-01
1.110000000000000000e+02, 2.299221088440471517e-01
1.120000000000000000e+02, 1.848476972987930789e-01
1.130000000000000000e+02, 1.658782375376857687e-01
1.140000000000000000e+02, 1.126192755440351551e-01
1.150000000000000000e+02, 7.118395883431384574e-02
1.160000000000000000e+02, 9.873567949441387770e-02
1.170000000000000000e+02, 3.143342600311530011e-02
1.180000000000000000e+02, 2.700296127893397208e-02
1.190000000000000000e+02, 2.497636838585694241e-02
1.200000000000000000e+02, 1.971513671284996078e-02
1.210000000000000000e+02, 7.518233129994318642e-02
1.220000000000000000e+02, 6.885329234371319329e-02
1.230000000000000000e+02, 1.770415596230962285e-01
1.240000000000000000e+02, 4.703346909755924954e-01
1.250000000000000000e+02, 7.498939380961182621e-01
1.260000000000000000e+02, 5.422377653878174275e-01
1.270000000000000000e+02, 2.436163872357248461e-01
1.280000000000000000e+02, 1.068403314466707388e-01
1.290000000000000000e+02, 9.074685685459411844e-02
1.300000000000000000e+02, 4.554758073233758364e-02
1.310000000000000000e+02, 7.618878786948381221e-02
1.320000000000000000e+02, 7.428859794737453781e-02
1.330000000000000000e+02, 5.800099289425961896e-02
1.340000000000000000e+02, 6.306260499585648882e-02
1.350000000000000000e+02, 6.841704627861942833e-02
1.360000000000000000e+02, 8.262045913318268042e-02
1.370000000000000000e+02, 1.229643630936643334e-01
1.380000000000000000e+02, 1.844391297486633885e-01
1.390000000000000000e+02, 2.492672505723723675e-01
1.400000000000000000e+02, 3.042510051985188868e-01
1.410000000000000000e+02, 3.103211767718688230e-01
1.420000000000000000e+02, 2.310417163026757537e-01
1.430000000000000000e+02, 2.088794768034756000e-01
1.440000000000000000e+02, 1.469548016135892865e-01
1.450000000000000000e+02, 8.126402048100350717e-02
1.460000000000000000e+02, 6.282899070997668978e-02
1.470000000000000000e+02, 7.631423513970497785e-02
1.480000000000000000e+02, 2.782676885669011640e-02
1.490000000000000000e+02, 3.316818815845644364e-02
1.500000000000000000e+02, 5.245994023933036460e-02
1.510000000000000000e+02, 9.912472962360498185e-02
1.520000000000000000e+02, 1.108544169491528508e-01
1.530000000000000000e+02, 2.105282479647239136e-01
1.540000000000000000e+02, 2.871152357680128997e-01
1.550000000000000000e+02, 1.592541952113935566e-01
1.560000000000000000e+02, 2.798046750416806616e-01
1.570000000000000000e+02, 3.071275787865556106e-01
1.580000000000000000e+02, 3.116030426431080635e-01
1.590000000000000000e+02, 2.372541331681979615e-01
1.600000000000000000e+02, 1.991216022345330960e-01
1.610000000000000000e+02, 1.314488107146256080e-01
1.620000000000000000e+02, 6.450254063630833645e-02
1.630000000000000000e+02, 8.368459164634813041e-02
1.640000000000000000e+02, 6.782463839267999228e-02
1.650000000000000000e+02, 6.498440003901592710e-02
1.660000000000000000e+02, 3.620448920480680982e-02
1.670000000000000000e+02, 5.420914324649507565e-02
1.680000000000000000e+02, 7.601473046171308701e-02
1.690000000000000000e+02, 5.339384204017526281e-02
1.700000000000000000e+02, 8.968352399575804657e-02
1.710000000000000000e+02, 2.237326273733995508e-01
1.720000000000000000e+02, 4.981450662206995394e-01
1.730000000000000000e+02, 7.858665035752706585e-01
1.740000000000000000e+02, 5.123845710856255176e-01
1.750000000000000000e+02, 2.334355383261791095e-01
1.760000000000000000e+02, 1.039806930788409883e-01
1.770000000000000000e+02, 7.266662603143686505e-02
1.780000000000000000e+02, 3.984819512350822046e-02
1.790000000000000000e+02, 4.026720001805412369e-02
1.800000000000000000e+02, 1.617413999911058650e-02
1.810000000000000000e+02, 4.973977753791820888e-02
1.820000000000000000e+02, 5.546044597376607876e-02
1.830000000000000000e+02, 8.591569123278876285e-02
1.840000000000000000e+02, 1.239344271858555530e-01
1.850000000000000000e+02, 1.483639302672285221e-01
1.860000000000000000e+02, 1.830043174929250893e-01
1.870000000000000000e+02, 2.338888355146620524e-01
1.880000000000000000e+02, 2.607963154482809687e-01
1.890000000000000000e+02, 2.285771621874087278e-01
1.900000000000000000e+02, 1.723695173904055133e-01
1.910000000000000000e+02, 1.633961551769182452e-01
1.920000000000000000e+02, 9.850372676573809771e-02
1.930000000000000000e+02, 7.267010517098787536e-02
1.940000000000000000e+02, 5.776028947793841045e-02
};

\addlegendentry{sensor-rotation-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_high_uncertainty.tex <==
\addplot [name path=uncertainty, color=uncertaintyColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 8.007911134485727445e+00
1.100000000000000000e+01, 1.010173275449337993e+01
1.200000000000000000e+01, 1.326420775031162691e+01
1.300000000000000000e+01, 1.759801819453416982e+01
1.400000000000000000e+01, 2.199010003130009849e+01
1.500000000000000000e+01, 2.430940854029924481e+01
1.600000000000000000e+01, 2.515497558682557155e+01
1.700000000000000000e+01, 2.526670076028266010e+01
1.800000000000000000e+01, 2.219657489244768556e+01
1.900000000000000000e+01, 1.513252655175988970e+01
2.000000000000000000e+01, 7.014374857932135221e+00
2.100000000000000000e+01, 2.771329199855987913e+00
2.200000000000000000e+01, 1.509962038265876938e+00
2.300000000000000000e+01, 2.245812868745104218e+00
2.400000000000000000e+01, 1.580148829056821969e+00
2.500000000000000000e+01, 2.242116559166758893e+00
2.600000000000000000e+01, 4.389840174928829164e+00
2.700000000000000000e+01, 9.335164752110447495e+00
2.800000000000000000e+01, 1.859436521834475187e+01
2.900000000000000000e+01, 2.927012476548905084e+01
3.000000000000000000e+01, 2.852571424732220606e+01
3.100000000000000000e+01, 2.262604425260963836e+01
3.200000000000000000e+01, 1.885731138198155321e+01
3.300000000000000000e+01, 1.591016004325375199e+01
3.400000000000000000e+01, 1.286791843782508238e+01
3.500000000000000000e+01, 1.095831044760979367e+01
3.600000000000000000e+01, 1.052298243731488014e+01
3.700000000000000000e+01, 1.376773746858741099e+01
3.800000000000000000e+01, 1.848185665992395599e+01
3.900000000000000000e+01, 1.385699180119371832e+01
4.000000000000000000e+01, 7.831054400506502589e+00
4.100000000000000000e+01, 9.959771369870107804e+00
4.200000000000000000e+01, 1.311318293927752343e+01
4.300000000000000000e+01, 1.678466144779847724e+01
4.400000000000000000e+01, 2.030373637986485136e+01
4.500000000000000000e+01, 2.500871514194867018e+01
4.600000000000000000e+01, 2.884023613654435536e+01
4.700000000000000000e+01, 2.360375102755952881e+01
4.800000000000000000e+01, 1.352785550331326547e+01
4.900000000000000000e+01, 6.460030208777062910e+00
5.000000000000000000e+01, 2.776141344705264302e+00
5.100000000000000000e+01, 1.991997779159343951e+00
5.200000000000000000e+01, 1.535816131633209292e+00
5.300000000000000000e+01, 1.673584834335799520e+00
5.400000000000000000e+01, 2.097296486189660136e+00
5.500000000000000000e+01, 3.800823548565830379e+00
5.600000000000000000e+01, 7.987436453520500024e+00
5.700000000000000000e+01, 1.514140682473833976e+01
5.800000000000000000e+01, 2.191904509553297231e+01
5.900000000000000000e+01, 2.430644084612232803e+01
6.000000000000000000e+01, 2.455833626576800555e+01
6.100000000000000000e+01, 2.264410521073992300e+01
6.200000000000000000e+01, 1.993294604162883843e+01
6.300000000000000000e+01, 1.511909258774868192e+01
6.400000000000000000e+01, 1.124837492960946861e+01
6.500000000000000000e+01, 8.772655892488559815e+00
6.600000000000000000e+01, 8.248437413368890248e+00
6.700000000000000000e+01, 1.067830420735654684e+01
6.800000000000000000e+01, 1.166889530861478264e+01
6.900000000000000000e+01, 8.805337596139811041e+00
7.000000000000000000e+01, 7.470543132635047101e+00
7.100000000000000000e+01, 8.490889249366592395e+00
7.200000000000000000e+01, 1.063606184237784191e+01
7.300000000000000000e+01, 1.400195517515770405e+01
7.400000000000000000e+01, 1.997260352306992104e+01
7.500000000000000000e+01, 2.542286078116854497e+01
7.600000000000000000e+01, 2.211934229757142134e+01
7.700000000000000000e+01, 1.567121765602189143e+01
7.800000000000000000e+01, 1.172778351525463947e+01
7.900000000000000000e+01, 8.888208544662463240e+00
8.000000000000000000e+01, 7.398996035135386506e+00
8.100000000000000000e+01, 8.485869958924736167e+00
8.200000000000000000e+01, 1.109797195138802550e+01
8.300000000000000000e+01, 1.073235315936681644e+01
8.400000000000000000e+01, 8.479813500959256345e+00
8.500000000000000000e+01, 8.611385989375033745e+00
8.600000000000000000e+01, 1.048357738604600797e+01
8.700000000000000000e+01, 1.403288066214068230e+01
8.800000000000000000e+01, 1.817464734253609748e+01
8.900000000000000000e+01, 2.179408690860795517e+01
9.000000000000000000e+01, 2.379434796003033270e+01
9.100000000000000000e+01, 2.432270343942132129e+01
9.200000000000000000e+01, 2.385385392862188780e+01
9.300000000000000000e+01, 9.237453813658984103e+00
9.400000000000000000e+01, 4.866444146539082638e+00
9.500000000000000000e+01, 2.622390056277970061e+00
9.600000000000000000e+01, 3.194450147226329584e+00
9.700000000000000000e+01, 1.649418986469459059e+00
9.800000000000000000e+01, 2.357660807007050607e+00
9.900000000000000000e+01, 2.238586852597552745e+00
1.000000000000000000e+02, 3.007039957202329639e+00
1.010000000000000000e+02, 5.611410599862496795e+00
1.020000000000000000e+02, 1.128252174884280912e+01
1.030000000000000000e+02, 1.890695992434724104e+01
1.040000000000000000e+02, 2.396179002870592356e+01
1.050000000000000000e+02, 2.365373335038652769e+01
1.060000000000000000e+02, 1.978048417186267471e+01
1.070000000000000000e+02, 1.585528062880087319e+01
1.080000000000000000e+02, 1.325305546650768207e+01
1.090000000000000000e+02, 1.181434948031233390e+01
1.100000000000000000e+02, 1.237389977811170994e+01
1.110000000000000000e+02, 1.312428140823197076e+01
1.120000000000000000e+02, 1.308507527964285799e+01
1.130000000000000000e+02, 1.385950123263300782e+01
1.140000000000000000e+02, 1.275410487671145177e+01
1.150000000000000000e+02, 1.178156969804837040e+01
1.160000000000000000e+02, 1.238948342657756285e+01
1.170000000000000000e+02, 1.418410893941581641e+01
1.180000000000000000e+02, 1.723591236924376702e+01
1.190000000000000000e+02, 2.092494746329887434e+01
1.200000000000000000e+02, 2.460641899919171749e+01
1.210000000000000000e+02, 2.370132598657919942e+01
1.220000000000000000e+02, 1.773611644468508075e+01
1.230000000000000000e+02, 9.240905675080474779e+00
1.240000000000000000e+02, 4.015636091408481434e+00
1.250000000000000000e+02, 2.514067720489420843e+00
1.260000000000000000e+02, 2.238817896265401508e+00
1.270000000000000000e+02, 1.551172108297139474e+00
1.280000000000000000e+02, 2.883553049288095416e+00
1.290000000000000000e+02, 2.565469167345762802e+00
1.300000000000000000e+02, 3.665406383598807327e+00
1.310000000000000000e+02, 6.905615430648566644e+00
1.320000000000000000e+02, 1.349506515928653627e+01
1.330000000000000000e+02, 2.008904717645333804e+01
1.340000000000000000e+02, 2.373429999819456881e+01
1.350000000000000000e+02, 2.326507496424129329e+01
1.360000000000000000e+02, 2.186455633540424870e+01
1.370000000000000000e+02, 1.806860824993597348e+01
1.380000000000000000e+02, 1.376718677308341654e+01
1.390000000000000000e+02, 1.037841942148684993e+01
1.400000000000000000e+02, 9.630855552743945225e+00
1.410000000000000000e+02, 1.034287318588186544e+01
1.420000000000000000e+02, 9.080958873649585428e+00
1.430000000000000000e+02, 9.016314854886132935e+00
1.440000000000000000e+02, 9.255487497575739297e+00
1.450000000000000000e+02, 8.553482277176829740e+00
1.460000000000000000e+02, 8.812533246422216138e+00
1.470000000000000000e+02, 1.077304881720149865e+01
1.480000000000000000e+02, 1.470257526770604173e+01
1.490000000000000000e+02, 1.866750894332605526e+01
1.500000000000000000e+02, 2.055961548125501537e+01
1.510000000000000000e+02, 1.899997688118042660e+01
1.520000000000000000e+02, 1.455218472098719218e+01
1.530000000000000000e+02, 1.054665333927447968e+01
1.540000000000000000e+02, 8.709186296887931888e+00
1.550000000000000000e+02, 6.834407126237893593e+00
1.560000000000000000e+02, 6.594174562764242964e+00
1.570000000000000000e+02, 7.709170498689043249e+00
1.580000000000000000e+02, 1.438994816903576002e+01
1.590000000000000000e+02, 1.084302286783777447e+01
1.600000000000000000e+02, 7.858816307899558318e+00
1.610000000000000000e+02, 8.228338528662010987e+00
1.620000000000000000e+02, 1.074586376659040710e+01
1.630000000000000000e+02, 1.445567573739981526e+01
1.640000000000000000e+02, 1.867994306646801306e+01
1.650000000000000000e+02, 2.232958752688821136e+01
1.660000000000000000e+02, 2.396628883477108118e+01
1.670000000000000000e+02, 2.468142495125597691e+01
1.680000000000000000e+02, 2.496292020589108418e+01
1.690000000000000000e+02, 2.089354137127993738e+01
1.700000000000000000e+02, 1.288252208468230720e+01
1.710000000000000000e+02, 5.632669710777129524e+00
1.720000000000000000e+02, 2.206459468602534280e+00
1.730000000000000000e+02, 1.622239294558789791e+00
1.740000000000000000e+02, 1.607780956434194941e+00
1.750000000000000000e+02, 1.578451175388482897e+00
1.760000000000000000e+02, 2.587143070416536794e+00
1.770000000000000000e+02, 5.298048523896477846e+00
1.780000000000000000e+02, 1.126182362686539307e+01
1.790000000000000000e+02, 2.204483970696866990e+01
1.800000000000000000e+02, 2.968853450569867647e+01
1.810000000000000000e+02, 2.605684708270674221e+01
1.820000000000000000e+02, 2.147805538039348505e+01
1.830000000000000000e+02, 1.836828010978455694e+01
1.840000000000000000e+02, 1.479121547128918124e+01
1.850000000000000000e+02, 1.223076776498097296e+01
1.860000000000000000e+02, 1.051938370394698019e+01
1.870000000000000000e+02, 1.079248083458984908e+01
1.880000000000000000e+02, 1.577975016167037126e+01
1.890000000000000000e+02, 1.815423806673035045e+01
1.900000000000000000e+02, 1.234962857159033867e+01
1.910000000000000000e+02, 1.064434448508170306e+01
1.920000000000000000e+02, 1.128795149824348343e+01
1.930000000000000000e+02, 1.316082164972944213e+01
1.940000000000000000e+02, 1.581317168290425812e+01
};

\addlegendentry{uncertainty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_low_error.tex <==
\addplot [name path=error, color=errorColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 1.000000000000010429e-02
1.100000000000000000e+01, 1.000000000000010429e-02
1.200000000000000000e+01, 1.000000000000010429e-02
1.300000000000000000e+01, 1.000000000000010429e-02
1.400000000000000000e+01, 1.000000000000010429e-02
1.500000000000000000e+01, 1.000000000000010429e-02
1.600000000000000000e+01, 1.000000000000010429e-02
1.700000000000000000e+01, 1.000000000000010429e-02
1.800000000000000000e+01, 1.000000000000010429e-02
1.900000000000000000e+01, 1.000000000000010429e-02
2.000000000000000000e+01, 1.000000000000010429e-02
2.100000000000000000e+01, 1.000000000000010429e-02
2.200000000000000000e+01, 1.000000000000010429e-02
2.300000000000000000e+01, 1.000000000000010429e-02
2.400000000000000000e+01, 1.000000000000010429e-02
2.500000000000000000e+01, 1.000000000000010429e-02
2.600000000000000000e+01, 1.000000000000010429e-02
2.700000000000000000e+01, 1.000000000000010429e-02
2.800000000000000000e+01, 1.000000000000010429e-02
2.900000000000000000e+01, 1.000000000000010429e-02
3.000000000000000000e+01, 1.000000000000010429e-02
3.100000000000000000e+01, 1.000000000000010429e-02
3.200000000000000000e+01, 1.000000000000010429e-02
3.300000000000000000e+01, 1.000000000000010429e-02
3.400000000000000000e+01, 1.000000000000010429e-02
3.500000000000000000e+01, 1.000000000000010429e-02
3.600000000000000000e+01, 1.000000000000010429e-02
3.700000000000000000e+01, 1.000000000000010429e-02
3.800000000000000000e+01, 1.000000000000010429e-02
3.900000000000000000e+01, 1.000000000000010429e-02
4.000000000000000000e+01, 1.129999999999999893e+00
4.100000000000000000e+01, 1.079999999999999849e+00
4.200000000000000000e+01, 1.019999999999999796e+00
4.300000000000000000e+01, 8.949999999999997957e-01
4.400000000000000000e+01, 6.599999999999998090e-01
4.500000000000000000e+01, 3.499999999999998668e-01
4.600000000000000000e+01, 2.299999999999998712e-01
4.700000000000000000e+01, 1.899999999999997247e-01
4.800000000000000000e+01, 9.999999999999986677e-02
4.900000000000000000e+01, 1.999999999999979572e-02
5.000000000000000000e+01, 1.000000000000023093e-02
5.100000000000000000e+01, 1.000000000000023093e-02
5.200000000000000000e+01, 2.000000000000023981e-02
5.300000000000000000e+01, 9.999999999999786837e-03
5.400000000000000000e+01, 1.000000000000023093e-02
5.500000000000000000e+01, 1.000000000000023093e-02
5.600000000000000000e+01, 1.000000000000023093e-02
5.700000000000000000e+01, 1.000000000000023093e-02
5.800000000000000000e+01, 1.000000000000023093e-02
5.900000000000000000e+01, 1.000000000000023093e-02
6.000000000000000000e+01, 1.000000000000023093e-02
6.100000000000000000e+01, 1.000000000000023093e-02
6.200000000000000000e+01, 3.000000000000024869e-02
6.300000000000000000e+01, 1.000000000000023093e-02
6.400000000000000000e+01, 1.000000000000023093e-02
6.500000000000000000e+01, 2.000000000000023981e-02
6.600000000000000000e+01, 2.000000000000023981e-02
6.700000000000000000e+01, 2.000000000000023981e-02
6.800000000000000000e+01, 1.000000000000023093e-02
6.900000000000000000e+01, 1.000000000000023093e-02
7.000000000000000000e+01, 1.000000000000023093e-02
7.100000000000000000e+01, 1.500000000000034639e-02
7.200000000000000000e+01, 2.000000000000023981e-02
7.300000000000000000e+01, 2.000000000000023981e-02
7.400000000000000000e+01, 1.000000000000023093e-02
7.500000000000000000e+01, 2.000000000000023981e-02
7.600000000000000000e+01, 1.000000000000023093e-02
7.700000000000000000e+01, 1.000000000000023093e-02
7.800000000000000000e+01, 1.000000000000023093e-02
7.900000000000000000e+01, 2.000000000000023981e-02
8.000000000000000000e+01, 2.000000000000023981e-02
8.100000000000000000e+01, 2.000000000000023981e-02
8.200000000000000000e+01, 2.000000000000023981e-02
8.300000000000000000e+01, 2.000000000000023981e-02
8.400000000000000000e+01, 1.000000000000023093e-02
8.500000000000000000e+01, 2.000000000000023981e-02
8.600000000000000000e+01, 2.000000000000023981e-02
8.700000000000000000e+01, 1.000000000000023093e-02
8.800000000000000000e+01, 1.000000000000023093e-02
8.900000000000000000e+01, 1.000000000000023093e-02
9.000000000000000000e+01, 1.000000000000023093e-02
9.100000000000000000e+01, 1.000000000000023093e-02
9.200000000000000000e+01, 1.000000000000023093e-02
9.300000000000000000e+01, 1.079999999999999627e+00
9.400000000000000000e+01, 1.029999999999999583e+00
9.500000000000000000e+01, 5.299999999999995826e-01
9.600000000000000000e+01, 7.999999999999962697e-02
9.700000000000000000e+01, 2.999999999999980460e-02
9.800000000000000000e+01, 9.999999999999786837e-03
9.900000000000000000e+01, 9.999999999999786837e-03
1.000000000000000000e+02, 9.999999999999786837e-03
1.010000000000000000e+02, 9.999999999999786837e-03
1.020000000000000000e+02, 9.999999999999786837e-03
1.030000000000000000e+02, 4.440892098500626162e-16
1.040000000000000000e+02, 4.440892098500626162e-16
1.050000000000000000e+02, 4.440892098500626162e-16
1.060000000000000000e+02, 4.440892098500626162e-16
1.070000000000000000e+02, 2.000000000000046185e-02
1.080000000000000000e+02, 1.000000000000023093e-02
1.090000000000000000e+02, 1.000000000000023093e-02
1.100000000000000000e+02, 2.000000000000046185e-02
1.110000000000000000e+02, 2.000000000000046185e-02
1.120000000000000000e+02, 2.000000000000046185e-02
1.130000000000000000e+02, 2.000000000000046185e-02
1.140000000000000000e+02, 2.000000000000046185e-02
1.150000000000000000e+02, 2.000000000000046185e-02
1.160000000000000000e+02, 2.000000000000046185e-02
1.170000000000000000e+02, 2.000000000000046185e-02
1.180000000000000000e+02, 2.000000000000046185e-02
1.190000000000000000e+02, 3.000000000000024869e-02
1.200000000000000000e+02, 3.000000000000024869e-02
1.210000000000000000e+02, 3.000000000000024869e-02
1.220000000000000000e+02, 3.000000000000024869e-02
1.230000000000000000e+02, 3.000000000000024869e-02
1.240000000000000000e+02, 3.000000000000024869e-02
1.250000000000000000e+02, 2.000000000000046185e-02
1.260000000000000000e+02, 2.000000000000046185e-02
1.270000000000000000e+02, 3.000000000000024869e-02
1.280000000000000000e+02, 9.999999999999786837e-03
1.290000000000000000e+02, 1.000000000000023093e-02
1.300000000000000000e+02, 4.440892098500626162e-16
1.310000000000000000e+02, 1.000000000000023093e-02
1.320000000000000000e+02, 1.000000000000023093e-02
1.330000000000000000e+02, 1.000000000000023093e-02
1.340000000000000000e+02, 1.000000000000023093e-02
1.350000000000000000e+02, 1.000000000000023093e-02
1.360000000000000000e+02, 3.000000000000024869e-02
1.370000000000000000e+02, 4.440892098500626162e-16
1.380000000000000000e+02, 1.000000000000023093e-02
1.390000000000000000e+02, 3.000000000000024869e-02
1.400000000000000000e+02, 3.000000000000024869e-02
1.410000000000000000e+02, 3.000000000000024869e-02
1.420000000000000000e+02, 2.000000000000046185e-02
1.430000000000000000e+02, 2.000000000000046185e-02
1.440000000000000000e+02, 2.000000000000046185e-02
1.450000000000000000e+02, 2.000000000000046185e-02
1.460000000000000000e+02, 2.000000000000046185e-02
1.470000000000000000e+02, 2.000000000000046185e-02
1.480000000000000000e+02, 2.000000000000046185e-02
1.490000000000000000e+02, 2.000000000000046185e-02
1.500000000000000000e+02, 2.000000000000046185e-02
1.510000000000000000e+02, 1.500000000000056843e-02
1.520000000000000000e+02, 2.000000000000046185e-02
1.530000000000000000e+02, 2.000000000000046185e-02
1.540000000000000000e+02, 2.000000000000046185e-02
1.550000000000000000e+02, 2.320000000000000284e+00
1.560000000000000000e+02, 2.320000000000000284e+00
1.570000000000000000e+02, 2.320000000000000284e+00
1.580000000000000000e+02, 2.360000000000000320e+00
1.590000000000000000e+02, 2.340000000000000302e+00
1.600000000000000000e+02, 2.340000000000000302e+00
1.610000000000000000e+02, 4.000000000000010492e-02
1.620000000000000000e+02, 3.000000000000010297e-02
1.630000000000000000e+02, 2.000000000000010450e-02
1.640000000000000000e+02, 2.000000000000010450e-02
1.650000000000000000e+02, 1.040834085586084257e-16
1.660000000000000000e+02, 1.000000000000010429e-02
1.670000000000000000e+02, 1.000000000000010429e-02
1.680000000000000000e+02, 1.000000000000010429e-02
1.690000000000000000e+02, 1.000000000000010429e-02
1.700000000000000000e+02, 1.040834085586084257e-16
1.710000000000000000e+02, 1.000000000000010429e-02
1.720000000000000000e+02, 1.000000000000010429e-02
1.730000000000000000e+02, 1.000000000000010429e-02
1.740000000000000000e+02, 1.000000000000010429e-02
1.750000000000000000e+02, 1.000000000000010429e-02
1.760000000000000000e+02, 1.000000000000010429e-02
1.770000000000000000e+02, 1.000000000000010429e-02
1.780000000000000000e+02, 1.000000000000010429e-02
1.790000000000000000e+02, 1.000000000000010429e-02
1.800000000000000000e+02, 1.000000000000010429e-02
1.810000000000000000e+02, 1.000000000000010429e-02
1.820000000000000000e+02, 1.000000000000010429e-02
1.830000000000000000e+02, 1.000000000000010429e-02
1.840000000000000000e+02, 1.000000000000010429e-02
1.850000000000000000e+02, 1.000000000000010429e-02
1.860000000000000000e+02, 1.000000000000010429e-02
1.870000000000000000e+02, 1.000000000000010429e-02
1.880000000000000000e+02, 1.000000000000010429e-02
1.890000000000000000e+02, 1.000000000000010429e-02
1.900000000000000000e+02, 1.000000000000010429e-02
1.910000000000000000e+02, 1.000000000000010429e-02
1.920000000000000000e+02, 1.000000000000010429e-02
1.930000000000000000e+02, 1.000000000000010429e-02
1.940000000000000000e+02, 1.000000000000010429e-02
};

\addlegendentry{error}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_low_estimation.tex <==
\addplot [name path=estimationlower, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, -1.999999999999989633e-02
1.100000000000000000e+01, -1.999999999999989633e-02
1.200000000000000000e+01, -1.999999999999989633e-02
1.300000000000000000e+01, -1.999999999999989633e-02
1.400000000000000000e+01, -1.999999999999989633e-02
1.500000000000000000e+01, -1.999999999999989633e-02
1.600000000000000000e+01, -2.999999999999989481e-02
1.700000000000000000e+01, -2.999999999999989481e-02
1.800000000000000000e+01, -3.999999999999989675e-02
1.900000000000000000e+01, -4.999999999999989869e-02
2.000000000000000000e+01, -2.999999999999989481e-02
2.100000000000000000e+01, -9.999999999999896125e-03
2.200000000000000000e+01, 1.040834085586084257e-16
2.300000000000000000e+01, 1.040834085586084257e-16
2.400000000000000000e+01, 1.040834085586084257e-16
2.500000000000000000e+01, 1.040834085586084257e-16
2.600000000000000000e+01, 1.040834085586084257e-16
2.700000000000000000e+01, 1.040834085586084257e-16
2.800000000000000000e+01, 1.040834085586084257e-16
2.900000000000000000e+01, 1.040834085586084257e-16
3.000000000000000000e+01, 1.040834085586084257e-16
3.100000000000000000e+01, 1.040834085586084257e-16
3.200000000000000000e+01, 1.040834085586084257e-16
3.300000000000000000e+01, 1.040834085586084257e-16
3.400000000000000000e+01, -9.999999999999896125e-03
3.500000000000000000e+01, -2.999999999999989481e-02
3.600000000000000000e+01, -2.999999999999989481e-02
3.700000000000000000e+01, -2.999999999999989481e-02
3.800000000000000000e+01, -2.999999999999989481e-02
3.900000000000000000e+01, -2.999999999999989481e-02
4.000000000000000000e+01, 7.500000000000103806e-03
4.100000000000000000e+01, 8.000000000000009881e-02
4.200000000000000000e+01, 1.300000000000001155e-01
4.300000000000000000e+01, 2.500000000000001110e-01
4.400000000000000000e+01, 4.700000000000001399e-01
4.500000000000000000e+01, 7.800000000000001377e-01
4.600000000000000000e+01, 8.800000000000001155e-01
4.700000000000000000e+01, 9.300000000000001599e-01
4.800000000000000000e+01, 1.030000000000000027e+00
4.900000000000000000e+01, 1.130000000000000115e+00
5.000000000000000000e+01, 1.180000000000000160e+00
5.100000000000000000e+01, 1.197500000000000231e+00
5.200000000000000000e+01, 1.210000000000000187e+00
5.300000000000000000e+01, 1.180000000000000160e+00
5.400000000000000000e+01, 1.200000000000000178e+00
5.500000000000000000e+01, 1.200000000000000178e+00
5.600000000000000000e+01, 1.200000000000000178e+00
5.700000000000000000e+01, 1.200000000000000178e+00
5.800000000000000000e+01, 1.200000000000000178e+00
5.900000000000000000e+01, 1.200000000000000178e+00
6.000000000000000000e+01, 1.190000000000000169e+00
6.100000000000000000e+01, 1.200000000000000178e+00
6.200000000000000000e+01, 1.210000000000000187e+00
6.300000000000000000e+01, 1.180000000000000160e+00
6.400000000000000000e+01, 1.150000000000000133e+00
6.500000000000000000e+01, 1.150000000000000133e+00
6.600000000000000000e+01, 1.170000000000000151e+00
6.700000000000000000e+01, 1.180000000000000160e+00
6.800000000000000000e+01, 1.170000000000000151e+00
6.900000000000000000e+01, 1.170000000000000151e+00
7.000000000000000000e+01, 1.180000000000000160e+00
7.100000000000000000e+01, 1.180000000000000160e+00
7.200000000000000000e+01, 1.190000000000000169e+00
7.300000000000000000e+01, 1.190000000000000169e+00
7.400000000000000000e+01, 1.190000000000000169e+00
7.500000000000000000e+01, 1.180000000000000160e+00
7.600000000000000000e+01, 1.180000000000000160e+00
7.700000000000000000e+01, 1.180000000000000160e+00
7.800000000000000000e+01, 1.180000000000000160e+00
7.900000000000000000e+01, 1.170000000000000151e+00
8.000000000000000000e+01, 1.180000000000000160e+00
8.100000000000000000e+01, 1.180000000000000160e+00
8.200000000000000000e+01, 1.180000000000000160e+00
8.300000000000000000e+01, 1.180000000000000160e+00
8.400000000000000000e+01, 1.180000000000000160e+00
8.500000000000000000e+01, 1.180000000000000160e+00
8.600000000000000000e+01, 1.190000000000000169e+00
8.700000000000000000e+01, 1.190000000000000169e+00
8.800000000000000000e+01, 1.180000000000000160e+00
8.900000000000000000e+01, 1.180000000000000160e+00
9.000000000000000000e+01, 1.180000000000000160e+00
9.100000000000000000e+01, 1.170000000000000151e+00
9.200000000000000000e+01, 1.170000000000000151e+00
9.300000000000000000e+01, 1.170000000000000151e+00
9.400000000000000000e+01, 1.220000000000000195e+00
9.500000000000000000e+01, 1.710000000000000187e+00
9.600000000000000000e+01, 2.189999999999999947e+00
9.700000000000000000e+01, 2.260000000000000231e+00
9.800000000000000000e+01, 2.280000000000000249e+00
9.900000000000000000e+01, 2.290000000000000036e+00
1.000000000000000000e+02, 2.280000000000000249e+00
1.010000000000000000e+02, 2.280000000000000249e+00
1.020000000000000000e+02, 2.290000000000000036e+00
1.030000000000000000e+02, 2.290000000000000036e+00
1.040000000000000000e+02, 2.290000000000000036e+00
1.050000000000000000e+02, 2.290000000000000036e+00
1.060000000000000000e+02, 2.290000000000000036e+00
1.070000000000000000e+02, 2.290000000000000036e+00
1.080000000000000000e+02, 2.280000000000000249e+00
1.090000000000000000e+02, 2.260000000000000231e+00
1.100000000000000000e+02, 2.250000000000000000e+00
1.110000000000000000e+02, 2.260000000000000231e+00
1.120000000000000000e+02, 2.270000000000000018e+00
1.130000000000000000e+02, 2.270000000000000018e+00
1.140000000000000000e+02, 2.270000000000000018e+00
1.150000000000000000e+02, 2.270000000000000018e+00
1.160000000000000000e+02, 2.280000000000000249e+00
1.170000000000000000e+02, 2.280000000000000249e+00
1.180000000000000000e+02, 2.280000000000000249e+00
1.190000000000000000e+02, 2.280000000000000249e+00
1.200000000000000000e+02, 2.270000000000000018e+00
1.210000000000000000e+02, 2.280000000000000249e+00
1.220000000000000000e+02, 2.270000000000000018e+00
1.230000000000000000e+02, 2.270000000000000018e+00
1.240000000000000000e+02, 2.260000000000000231e+00
1.250000000000000000e+02, 2.270000000000000018e+00
1.260000000000000000e+02, 2.280000000000000249e+00
1.270000000000000000e+02, 2.310000000000000053e+00
1.280000000000000000e+02, 2.280000000000000249e+00
1.290000000000000000e+02, 2.290000000000000036e+00
1.300000000000000000e+02, 2.290000000000000036e+00
1.310000000000000000e+02, 2.300000000000000266e+00
1.320000000000000000e+02, 2.300000000000000266e+00
1.330000000000000000e+02, 2.300000000000000266e+00
1.340000000000000000e+02, 2.300000000000000266e+00
1.350000000000000000e+02, 2.300000000000000266e+00
1.360000000000000000e+02, 2.310000000000000053e+00
1.370000000000000000e+02, 2.280000000000000249e+00
1.380000000000000000e+02, 2.280000000000000249e+00
1.390000000000000000e+02, 2.250000000000000000e+00
1.400000000000000000e+02, 2.240000000000000213e+00
1.410000000000000000e+02, 2.260000000000000231e+00
1.420000000000000000e+02, 2.280000000000000249e+00
1.430000000000000000e+02, 2.280000000000000249e+00
1.440000000000000000e+02, 2.280000000000000249e+00
1.450000000000000000e+02, 2.280000000000000249e+00
1.460000000000000000e+02, 2.280000000000000249e+00
1.470000000000000000e+02, 2.290000000000000036e+00
1.480000000000000000e+02, 2.290000000000000036e+00
1.490000000000000000e+02, 2.280000000000000249e+00
1.500000000000000000e+02, 2.280000000000000249e+00
1.510000000000000000e+02, 2.280000000000000249e+00
1.520000000000000000e+02, 2.280000000000000249e+00
1.530000000000000000e+02, 2.280000000000000249e+00
1.540000000000000000e+02, 2.270000000000000018e+00
1.550000000000000000e+02, 2.270000000000000018e+00
1.560000000000000000e+02, 2.280000000000000249e+00
1.570000000000000000e+02, 2.280000000000000249e+00
1.580000000000000000e+02, 2.320000000000000284e+00
1.590000000000000000e+02, 2.290000000000000036e+00
1.600000000000000000e+02, 2.290000000000000036e+00
1.610000000000000000e+02, 1.000000000000010429e-02
1.620000000000000000e+02, -9.999999999999896125e-03
1.630000000000000000e+02, -9.999999999999896125e-03
1.640000000000000000e+02, -2.999999999999989481e-02
1.650000000000000000e+02, -2.999999999999989481e-02
1.660000000000000000e+02, -2.999999999999989481e-02
1.670000000000000000e+02, -2.999999999999989481e-02
1.680000000000000000e+02, -2.999999999999989481e-02
1.690000000000000000e+02, -3.999999999999989675e-02
1.700000000000000000e+02, -3.999999999999989675e-02
1.710000000000000000e+02, -3.999999999999989675e-02
1.720000000000000000e+02, -9.999999999999896125e-03
1.730000000000000000e+02, 1.040834085586084257e-16
1.740000000000000000e+02, 1.040834085586084257e-16
1.750000000000000000e+02, 1.040834085586084257e-16
1.760000000000000000e+02, 1.040834085586084257e-16
1.770000000000000000e+02, 1.040834085586084257e-16
1.780000000000000000e+02, 1.040834085586084257e-16
1.790000000000000000e+02, 1.040834085586084257e-16
1.800000000000000000e+02, 1.040834085586084257e-16
1.810000000000000000e+02, 1.040834085586084257e-16
1.820000000000000000e+02, 1.040834085586084257e-16
1.830000000000000000e+02, 1.040834085586084257e-16
1.840000000000000000e+02, 1.040834085586084257e-16
1.850000000000000000e+02, 1.040834085586084257e-16
1.860000000000000000e+02, -1.999999999999989633e-02
1.870000000000000000e+02, -3.999999999999989675e-02
1.880000000000000000e+02, -3.999999999999989675e-02
1.890000000000000000e+02, -3.999999999999989675e-02
1.900000000000000000e+02, -3.999999999999989675e-02
1.910000000000000000e+02, -3.999999999999989675e-02
1.920000000000000000e+02, -2.999999999999989481e-02
1.930000000000000000e+02, -2.999999999999989481e-02
1.940000000000000000e+02, -2.999999999999989481e-02
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationupper, color=backGray, line width=1.5pt, draw opacity=0.9, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 4.000000000000010492e-02
1.100000000000000000e+01, 4.000000000000010492e-02
1.200000000000000000e+01, 4.000000000000010492e-02
1.300000000000000000e+01, 4.000000000000010492e-02
1.400000000000000000e+01, 4.000000000000010492e-02
1.500000000000000000e+01, 5.000000000000010686e-02
1.600000000000000000e+01, 5.000000000000010686e-02
1.700000000000000000e+01, 5.000000000000010686e-02
1.800000000000000000e+01, 6.000000000000010880e-02
1.900000000000000000e+01, 7.000000000000010381e-02
2.000000000000000000e+01, 5.000000000000010686e-02
2.100000000000000000e+01, 2.000000000000010450e-02
2.200000000000000000e+01, 2.000000000000010450e-02
2.300000000000000000e+01, 2.000000000000010450e-02
2.400000000000000000e+01, 2.000000000000010450e-02
2.500000000000000000e+01, 2.000000000000010450e-02
2.600000000000000000e+01, 2.000000000000010450e-02
2.700000000000000000e+01, 2.000000000000010450e-02
2.800000000000000000e+01, 2.000000000000010450e-02
2.900000000000000000e+01, 2.000000000000010450e-02
3.000000000000000000e+01, 2.000000000000010450e-02
3.100000000000000000e+01, 2.000000000000010450e-02
3.200000000000000000e+01, 2.000000000000010450e-02
3.300000000000000000e+01, 2.000000000000010450e-02
3.400000000000000000e+01, 3.000000000000010297e-02
3.500000000000000000e+01, 5.250000000000010908e-02
3.600000000000000000e+01, 6.000000000000010880e-02
3.700000000000000000e+01, 6.000000000000010880e-02
3.800000000000000000e+01, 6.000000000000010880e-02
3.900000000000000000e+01, 6.000000000000010880e-02
4.000000000000000000e+01, 1.000000000000001027e-01
4.100000000000000000e+01, 1.600000000000001144e-01
4.200000000000000000e+01, 2.200000000000001121e-01
4.300000000000000000e+01, 3.500000000000000888e-01
4.400000000000000000e+01, 6.100000000000000977e-01
4.500000000000000000e+01, 9.100000000000001421e-01
4.600000000000000000e+01, 1.060000000000000053e+00
4.700000000000000000e+01, 1.080000000000000071e+00
4.800000000000000000e+01, 1.180000000000000160e+00
4.900000000000000000e+01, 1.240000000000000213e+00
5.000000000000000000e+01, 1.240000000000000213e+00
5.100000000000000000e+01, 1.220000000000000195e+00
5.200000000000000000e+01, 1.230000000000000204e+00
5.300000000000000000e+01, 1.200000000000000178e+00
5.400000000000000000e+01, 1.220000000000000195e+00
5.500000000000000000e+01, 1.220000000000000195e+00
5.600000000000000000e+01, 1.220000000000000195e+00
5.700000000000000000e+01, 1.220000000000000195e+00
5.800000000000000000e+01, 1.220000000000000195e+00
5.900000000000000000e+01, 1.220000000000000195e+00
6.000000000000000000e+01, 1.220000000000000195e+00
6.100000000000000000e+01, 1.220000000000000195e+00
6.200000000000000000e+01, 1.240000000000000213e+00
6.300000000000000000e+01, 1.260000000000000231e+00
6.400000000000000000e+01, 1.290000000000000036e+00
6.500000000000000000e+01, 1.290000000000000036e+00
6.600000000000000000e+01, 1.260000000000000231e+00
6.700000000000000000e+01, 1.260000000000000231e+00
6.800000000000000000e+01, 1.250000000000000222e+00
6.900000000000000000e+01, 1.250000000000000222e+00
7.000000000000000000e+01, 1.250000000000000222e+00
7.100000000000000000e+01, 1.250000000000000222e+00
7.200000000000000000e+01, 1.250000000000000222e+00
7.300000000000000000e+01, 1.240000000000000213e+00
7.400000000000000000e+01, 1.250000000000000222e+00
7.500000000000000000e+01, 1.250000000000000222e+00
7.600000000000000000e+01, 1.250000000000000222e+00
7.700000000000000000e+01, 1.250000000000000222e+00
7.800000000000000000e+01, 1.250000000000000222e+00
7.900000000000000000e+01, 1.260000000000000231e+00
8.000000000000000000e+01, 1.252500000000000169e+00
8.100000000000000000e+01, 1.260000000000000231e+00
8.200000000000000000e+01, 1.250000000000000222e+00
8.300000000000000000e+01, 1.250000000000000222e+00
8.400000000000000000e+01, 1.250000000000000222e+00
8.500000000000000000e+01, 1.240000000000000213e+00
8.600000000000000000e+01, 1.240000000000000213e+00
8.700000000000000000e+01, 1.250000000000000222e+00
8.800000000000000000e+01, 1.240000000000000213e+00
8.900000000000000000e+01, 1.250000000000000222e+00
9.000000000000000000e+01, 1.250000000000000222e+00
9.100000000000000000e+01, 1.260000000000000231e+00
9.200000000000000000e+01, 1.260000000000000231e+00
9.300000000000000000e+01, 1.270000000000000240e+00
9.400000000000000000e+01, 1.320000000000000062e+00
9.500000000000000000e+01, 1.820000000000000062e+00
9.600000000000000000e+01, 2.250000000000000000e+00
9.700000000000000000e+01, 2.280000000000000249e+00
9.800000000000000000e+01, 2.300000000000000266e+00
9.900000000000000000e+01, 2.300000000000000266e+00
1.000000000000000000e+02, 2.300000000000000266e+00
1.010000000000000000e+02, 2.300000000000000266e+00
1.020000000000000000e+02, 2.300000000000000266e+00
1.030000000000000000e+02, 2.300000000000000266e+00
1.040000000000000000e+02, 2.300000000000000266e+00
1.050000000000000000e+02, 2.310000000000000053e+00
1.060000000000000000e+02, 2.310000000000000053e+00
1.070000000000000000e+02, 2.340000000000000302e+00
1.080000000000000000e+02, 2.350000000000000089e+00
1.090000000000000000e+02, 2.380000000000000338e+00
1.100000000000000000e+02, 2.380000000000000338e+00
1.110000000000000000e+02, 2.380000000000000338e+00
1.120000000000000000e+02, 2.370000000000000107e+00
1.130000000000000000e+02, 2.370000000000000107e+00
1.140000000000000000e+02, 2.370000000000000107e+00
1.150000000000000000e+02, 2.370000000000000107e+00
1.160000000000000000e+02, 2.370000000000000107e+00
1.170000000000000000e+02, 2.370000000000000107e+00
1.180000000000000000e+02, 2.370000000000000107e+00
1.190000000000000000e+02, 2.370000000000000107e+00
1.200000000000000000e+02, 2.370000000000000107e+00
1.210000000000000000e+02, 2.380000000000000338e+00
1.220000000000000000e+02, 2.380000000000000338e+00
1.230000000000000000e+02, 2.390000000000000124e+00
1.240000000000000000e+02, 2.400000000000000355e+00
1.250000000000000000e+02, 2.370000000000000107e+00
1.260000000000000000e+02, 2.360000000000000320e+00
1.270000000000000000e+02, 2.350000000000000089e+00
1.280000000000000000e+02, 2.310000000000000053e+00
1.290000000000000000e+02, 2.320000000000000284e+00
1.300000000000000000e+02, 2.310000000000000053e+00
1.310000000000000000e+02, 2.310000000000000053e+00
1.320000000000000000e+02, 2.310000000000000053e+00
1.330000000000000000e+02, 2.320000000000000284e+00
1.340000000000000000e+02, 2.320000000000000284e+00
1.350000000000000000e+02, 2.320000000000000284e+00
1.360000000000000000e+02, 2.340000000000000302e+00
1.370000000000000000e+02, 2.320000000000000284e+00
1.380000000000000000e+02, 2.350000000000000089e+00
1.390000000000000000e+02, 2.420000000000000373e+00
1.400000000000000000e+02, 2.430000000000000160e+00
1.410000000000000000e+02, 2.400000000000000355e+00
1.420000000000000000e+02, 2.370000000000000107e+00
1.430000000000000000e+02, 2.360000000000000320e+00
1.440000000000000000e+02, 2.360000000000000320e+00
1.450000000000000000e+02, 2.360000000000000320e+00
1.460000000000000000e+02, 2.350000000000000089e+00
1.470000000000000000e+02, 2.350000000000000089e+00
1.480000000000000000e+02, 2.350000000000000089e+00
1.490000000000000000e+02, 2.350000000000000089e+00
1.500000000000000000e+02, 2.350000000000000089e+00
1.510000000000000000e+02, 2.350000000000000089e+00
1.520000000000000000e+02, 2.350000000000000089e+00
1.530000000000000000e+02, 2.360000000000000320e+00
1.540000000000000000e+02, 2.360000000000000320e+00
1.550000000000000000e+02, 2.370000000000000107e+00
1.560000000000000000e+02, 2.370000000000000107e+00
1.570000000000000000e+02, 2.360000000000000320e+00
1.580000000000000000e+02, 2.400000000000000355e+00
1.590000000000000000e+02, 2.380000000000000338e+00
1.600000000000000000e+02, 2.380000000000000338e+00
1.610000000000000000e+02, 9.000000000000010769e-02
1.620000000000000000e+02, 6.000000000000010880e-02
1.630000000000000000e+02, 6.000000000000010880e-02
1.640000000000000000e+02, 5.000000000000010686e-02
1.650000000000000000e+02, 5.000000000000010686e-02
1.660000000000000000e+02, 4.000000000000010492e-02
1.670000000000000000e+02, 5.000000000000010686e-02
1.680000000000000000e+02, 5.000000000000010686e-02
1.690000000000000000e+02, 5.000000000000010686e-02
1.700000000000000000e+02, 5.000000000000010686e-02
1.710000000000000000e+02, 7.000000000000010381e-02
1.720000000000000000e+02, 4.000000000000010492e-02
1.730000000000000000e+02, 2.000000000000010450e-02
1.740000000000000000e+02, 2.000000000000010450e-02
1.750000000000000000e+02, 2.000000000000010450e-02
1.760000000000000000e+02, 2.000000000000010450e-02
1.770000000000000000e+02, 2.000000000000010450e-02
1.780000000000000000e+02, 2.000000000000010450e-02
1.790000000000000000e+02, 2.000000000000010450e-02
1.800000000000000000e+02, 2.000000000000010450e-02
1.810000000000000000e+02, 2.000000000000010450e-02
1.820000000000000000e+02, 2.000000000000010450e-02
1.830000000000000000e+02, 2.000000000000010450e-02
1.840000000000000000e+02, 2.000000000000010450e-02
1.850000000000000000e+02, 2.000000000000010450e-02
1.860000000000000000e+02, 4.000000000000010492e-02
1.870000000000000000e+02, 6.000000000000010880e-02
1.880000000000000000e+02, 6.000000000000010880e-02
1.890000000000000000e+02, 6.000000000000010880e-02
1.900000000000000000e+02, 6.000000000000010880e-02
1.910000000000000000e+02, 6.000000000000010880e-02
1.920000000000000000e+02, 5.000000000000010686e-02
1.930000000000000000e+02, 5.000000000000010686e-02
1.940000000000000000e+02, 6.000000000000010880e-02
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationmedian, color=estimationColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 1.000000000000010429e-02
1.100000000000000000e+01, 1.000000000000010429e-02
1.200000000000000000e+01, 1.000000000000010429e-02
1.300000000000000000e+01, 1.000000000000010429e-02
1.400000000000000000e+01, 1.000000000000010429e-02
1.500000000000000000e+01, 1.000000000000010429e-02
1.600000000000000000e+01, 1.000000000000010429e-02
1.700000000000000000e+01, 1.000000000000010429e-02
1.800000000000000000e+01, 1.000000000000010429e-02
1.900000000000000000e+01, 1.000000000000010429e-02
2.000000000000000000e+01, 1.000000000000010429e-02
2.100000000000000000e+01, 1.000000000000010429e-02
2.200000000000000000e+01, 1.000000000000010429e-02
2.300000000000000000e+01, 1.000000000000010429e-02
2.400000000000000000e+01, 1.000000000000010429e-02
2.500000000000000000e+01, 1.000000000000010429e-02
2.600000000000000000e+01, 1.000000000000010429e-02
2.700000000000000000e+01, 1.000000000000010429e-02
2.800000000000000000e+01, 1.000000000000010429e-02
2.900000000000000000e+01, 1.000000000000010429e-02
3.000000000000000000e+01, 1.000000000000010429e-02
3.100000000000000000e+01, 1.000000000000010429e-02
3.200000000000000000e+01, 1.000000000000010429e-02
3.300000000000000000e+01, 1.000000000000010429e-02
3.400000000000000000e+01, 1.000000000000010429e-02
3.500000000000000000e+01, 1.000000000000010429e-02
3.600000000000000000e+01, 1.000000000000010429e-02
3.700000000000000000e+01, 1.000000000000010429e-02
3.800000000000000000e+01, 1.000000000000010429e-02
3.900000000000000000e+01, 1.000000000000010429e-02
4.000000000000000000e+01, 7.000000000000010381e-02
4.100000000000000000e+01, 1.200000000000001066e-01
4.200000000000000000e+01, 1.800000000000001044e-01
4.300000000000000000e+01, 3.050000000000001044e-01
4.400000000000000000e+01, 5.400000000000001465e-01
4.500000000000000000e+01, 8.500000000000000888e-01
4.600000000000000000e+01, 9.700000000000000844e-01
4.700000000000000000e+01, 1.010000000000000231e+00
4.800000000000000000e+01, 1.100000000000000089e+00
4.900000000000000000e+01, 1.180000000000000160e+00
5.000000000000000000e+01, 1.210000000000000187e+00
5.100000000000000000e+01, 1.210000000000000187e+00
5.200000000000000000e+01, 1.220000000000000195e+00
5.300000000000000000e+01, 1.190000000000000169e+00
5.400000000000000000e+01, 1.210000000000000187e+00
5.500000000000000000e+01, 1.210000000000000187e+00
5.600000000000000000e+01, 1.210000000000000187e+00
5.700000000000000000e+01, 1.210000000000000187e+00
5.800000000000000000e+01, 1.210000000000000187e+00
5.900000000000000000e+01, 1.210000000000000187e+00
6.000000000000000000e+01, 1.210000000000000187e+00
6.100000000000000000e+01, 1.210000000000000187e+00
6.200000000000000000e+01, 1.230000000000000204e+00
6.300000000000000000e+01, 1.210000000000000187e+00
6.400000000000000000e+01, 1.210000000000000187e+00
6.500000000000000000e+01, 1.220000000000000195e+00
6.600000000000000000e+01, 1.220000000000000195e+00
6.700000000000000000e+01, 1.220000000000000195e+00
6.800000000000000000e+01, 1.210000000000000187e+00
6.900000000000000000e+01, 1.210000000000000187e+00
7.000000000000000000e+01, 1.210000000000000187e+00
7.100000000000000000e+01, 1.215000000000000302e+00
7.200000000000000000e+01, 1.220000000000000195e+00
7.300000000000000000e+01, 1.220000000000000195e+00
7.400000000000000000e+01, 1.210000000000000187e+00
7.500000000000000000e+01, 1.220000000000000195e+00
7.600000000000000000e+01, 1.210000000000000187e+00
7.700000000000000000e+01, 1.210000000000000187e+00
7.800000000000000000e+01, 1.210000000000000187e+00
7.900000000000000000e+01, 1.220000000000000195e+00
8.000000000000000000e+01, 1.220000000000000195e+00
8.100000000000000000e+01, 1.220000000000000195e+00
8.200000000000000000e+01, 1.220000000000000195e+00
8.300000000000000000e+01, 1.220000000000000195e+00
8.400000000000000000e+01, 1.210000000000000187e+00
8.500000000000000000e+01, 1.220000000000000195e+00
8.600000000000000000e+01, 1.220000000000000195e+00
8.700000000000000000e+01, 1.210000000000000187e+00
8.800000000000000000e+01, 1.210000000000000187e+00
8.900000000000000000e+01, 1.210000000000000187e+00
9.000000000000000000e+01, 1.210000000000000187e+00
9.100000000000000000e+01, 1.210000000000000187e+00
9.200000000000000000e+01, 1.210000000000000187e+00
9.300000000000000000e+01, 1.220000000000000195e+00
9.400000000000000000e+01, 1.270000000000000240e+00
9.500000000000000000e+01, 1.770000000000000240e+00
9.600000000000000000e+01, 2.220000000000000195e+00
9.700000000000000000e+01, 2.270000000000000018e+00
9.800000000000000000e+01, 2.290000000000000036e+00
9.900000000000000000e+01, 2.290000000000000036e+00
1.000000000000000000e+02, 2.290000000000000036e+00
1.010000000000000000e+02, 2.290000000000000036e+00
1.020000000000000000e+02, 2.290000000000000036e+00
1.030000000000000000e+02, 2.300000000000000266e+00
1.040000000000000000e+02, 2.300000000000000266e+00
1.050000000000000000e+02, 2.300000000000000266e+00
1.060000000000000000e+02, 2.300000000000000266e+00
1.070000000000000000e+02, 2.320000000000000284e+00
1.080000000000000000e+02, 2.310000000000000053e+00
1.090000000000000000e+02, 2.310000000000000053e+00
1.100000000000000000e+02, 2.320000000000000284e+00
1.110000000000000000e+02, 2.320000000000000284e+00
1.120000000000000000e+02, 2.320000000000000284e+00
1.130000000000000000e+02, 2.320000000000000284e+00
1.140000000000000000e+02, 2.320000000000000284e+00
1.150000000000000000e+02, 2.320000000000000284e+00
1.160000000000000000e+02, 2.320000000000000284e+00
1.170000000000000000e+02, 2.320000000000000284e+00
1.180000000000000000e+02, 2.320000000000000284e+00
1.190000000000000000e+02, 2.330000000000000071e+00
1.200000000000000000e+02, 2.330000000000000071e+00
1.210000000000000000e+02, 2.330000000000000071e+00
1.220000000000000000e+02, 2.330000000000000071e+00
1.230000000000000000e+02, 2.330000000000000071e+00
1.240000000000000000e+02, 2.330000000000000071e+00
1.250000000000000000e+02, 2.320000000000000284e+00
1.260000000000000000e+02, 2.320000000000000284e+00
1.270000000000000000e+02, 2.330000000000000071e+00
1.280000000000000000e+02, 2.290000000000000036e+00
1.290000000000000000e+02, 2.310000000000000053e+00
1.300000000000000000e+02, 2.300000000000000266e+00
1.310000000000000000e+02, 2.310000000000000053e+00
1.320000000000000000e+02, 2.310000000000000053e+00
1.330000000000000000e+02, 2.310000000000000053e+00
1.340000000000000000e+02, 2.310000000000000053e+00
1.350000000000000000e+02, 2.310000000000000053e+00
1.360000000000000000e+02, 2.330000000000000071e+00
1.370000000000000000e+02, 2.300000000000000266e+00
1.380000000000000000e+02, 2.310000000000000053e+00
1.390000000000000000e+02, 2.330000000000000071e+00
1.400000000000000000e+02, 2.330000000000000071e+00
1.410000000000000000e+02, 2.330000000000000071e+00
1.420000000000000000e+02, 2.320000000000000284e+00
1.430000000000000000e+02, 2.320000000000000284e+00
1.440000000000000000e+02, 2.320000000000000284e+00
1.450000000000000000e+02, 2.320000000000000284e+00
1.460000000000000000e+02, 2.320000000000000284e+00
1.470000000000000000e+02, 2.320000000000000284e+00
1.480000000000000000e+02, 2.320000000000000284e+00
1.490000000000000000e+02, 2.320000000000000284e+00
1.500000000000000000e+02, 2.320000000000000284e+00
1.510000000000000000e+02, 2.315000000000000391e+00
1.520000000000000000e+02, 2.320000000000000284e+00
1.530000000000000000e+02, 2.320000000000000284e+00
1.540000000000000000e+02, 2.320000000000000284e+00
1.550000000000000000e+02, 2.320000000000000284e+00
1.560000000000000000e+02, 2.320000000000000284e+00
1.570000000000000000e+02, 2.320000000000000284e+00
1.580000000000000000e+02, 2.360000000000000320e+00
1.590000000000000000e+02, 2.340000000000000302e+00
1.600000000000000000e+02, 2.340000000000000302e+00
1.610000000000000000e+02, 4.000000000000010492e-02
1.620000000000000000e+02, 3.000000000000010297e-02
1.630000000000000000e+02, 2.000000000000010450e-02
1.640000000000000000e+02, 2.000000000000010450e-02
1.650000000000000000e+02, 1.040834085586084257e-16
1.660000000000000000e+02, 1.000000000000010429e-02
1.670000000000000000e+02, 1.000000000000010429e-02
1.680000000000000000e+02, 1.000000000000010429e-02
1.690000000000000000e+02, 1.000000000000010429e-02
1.700000000000000000e+02, 1.040834085586084257e-16
1.710000000000000000e+02, 1.000000000000010429e-02
1.720000000000000000e+02, 1.000000000000010429e-02
1.730000000000000000e+02, 1.000000000000010429e-02
1.740000000000000000e+02, 1.000000000000010429e-02
1.750000000000000000e+02, 1.000000000000010429e-02
1.760000000000000000e+02, 1.000000000000010429e-02
1.770000000000000000e+02, 1.000000000000010429e-02
1.780000000000000000e+02, 1.000000000000010429e-02
1.790000000000000000e+02, 1.000000000000010429e-02
1.800000000000000000e+02, 1.000000000000010429e-02
1.810000000000000000e+02, 1.000000000000010429e-02
1.820000000000000000e+02, 1.000000000000010429e-02
1.830000000000000000e+02, 1.000000000000010429e-02
1.840000000000000000e+02, 1.000000000000010429e-02
1.850000000000000000e+02, 1.000000000000010429e-02
1.860000000000000000e+02, 1.000000000000010429e-02
1.870000000000000000e+02, 1.000000000000010429e-02
1.880000000000000000e+02, 1.000000000000010429e-02
1.890000000000000000e+02, 1.000000000000010429e-02
1.900000000000000000e+02, 1.000000000000010429e-02
1.910000000000000000e+02, 1.000000000000010429e-02
1.920000000000000000e+02, 1.000000000000010429e-02
1.930000000000000000e+02, 1.000000000000010429e-02
1.940000000000000000e+02, 1.000000000000010429e-02
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addlegendentry{estimation}

\addplot [backGray, fill opacity=0.9, forget plot] fill between[of=estimationlower and estimationupper];

\addplot [name path=ground-truth, color=ground-truthColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 0.000000000000000000e+00
1.100000000000000000e+01, 0.000000000000000000e+00
1.200000000000000000e+01, 0.000000000000000000e+00
1.300000000000000000e+01, 0.000000000000000000e+00
1.400000000000000000e+01, 0.000000000000000000e+00
1.500000000000000000e+01, 0.000000000000000000e+00
1.600000000000000000e+01, 0.000000000000000000e+00
1.700000000000000000e+01, 0.000000000000000000e+00
1.800000000000000000e+01, 0.000000000000000000e+00
1.900000000000000000e+01, 0.000000000000000000e+00
2.000000000000000000e+01, 0.000000000000000000e+00
2.100000000000000000e+01, 0.000000000000000000e+00
2.200000000000000000e+01, 0.000000000000000000e+00
2.300000000000000000e+01, 0.000000000000000000e+00
2.400000000000000000e+01, 0.000000000000000000e+00
2.500000000000000000e+01, 0.000000000000000000e+00
2.600000000000000000e+01, 0.000000000000000000e+00
2.700000000000000000e+01, 0.000000000000000000e+00
2.800000000000000000e+01, 0.000000000000000000e+00
2.900000000000000000e+01, 0.000000000000000000e+00
3.000000000000000000e+01, 0.000000000000000000e+00
3.100000000000000000e+01, 0.000000000000000000e+00
3.200000000000000000e+01, 0.000000000000000000e+00
3.300000000000000000e+01, 0.000000000000000000e+00
3.400000000000000000e+01, 0.000000000000000000e+00
3.500000000000000000e+01, 0.000000000000000000e+00
3.600000000000000000e+01, 0.000000000000000000e+00
3.700000000000000000e+01, 0.000000000000000000e+00
3.800000000000000000e+01, 0.000000000000000000e+00
3.900000000000000000e+01, 0.000000000000000000e+00
4.000000000000000000e+01, 1.199999999999999956e+00
4.100000000000000000e+01, 1.199999999999999956e+00
4.200000000000000000e+01, 1.199999999999999956e+00
4.300000000000000000e+01, 1.199999999999999956e+00
4.400000000000000000e+01, 1.199999999999999956e+00
4.500000000000000000e+01, 1.199999999999999956e+00
4.600000000000000000e+01, 1.199999999999999956e+00
4.700000000000000000e+01, 1.199999999999999956e+00
4.800000000000000000e+01, 1.199999999999999956e+00
4.900000000000000000e+01, 1.199999999999999956e+00
5.000000000000000000e+01, 1.199999999999999956e+00
5.100000000000000000e+01, 1.199999999999999956e+00
5.200000000000000000e+01, 1.199999999999999956e+00
5.300000000000000000e+01, 1.199999999999999956e+00
5.400000000000000000e+01, 1.199999999999999956e+00
5.500000000000000000e+01, 1.199999999999999956e+00
5.600000000000000000e+01, 1.199999999999999956e+00
5.700000000000000000e+01, 1.199999999999999956e+00
5.800000000000000000e+01, 1.199999999999999956e+00
5.900000000000000000e+01, 1.199999999999999956e+00
6.000000000000000000e+01, 1.199999999999999956e+00
6.100000000000000000e+01, 1.199999999999999956e+00
6.200000000000000000e+01, 1.199999999999999956e+00
6.300000000000000000e+01, 1.199999999999999956e+00
6.400000000000000000e+01, 1.199999999999999956e+00
6.500000000000000000e+01, 1.199999999999999956e+00
6.600000000000000000e+01, 1.199999999999999956e+00
6.700000000000000000e+01, 1.199999999999999956e+00
6.800000000000000000e+01, 1.199999999999999956e+00
6.900000000000000000e+01, 1.199999999999999956e+00
7.000000000000000000e+01, 1.199999999999999956e+00
7.100000000000000000e+01, 1.199999999999999956e+00
7.200000000000000000e+01, 1.199999999999999956e+00
7.300000000000000000e+01, 1.199999999999999956e+00
7.400000000000000000e+01, 1.199999999999999956e+00
7.500000000000000000e+01, 1.199999999999999956e+00
7.600000000000000000e+01, 1.199999999999999956e+00
7.700000000000000000e+01, 1.199999999999999956e+00
7.800000000000000000e+01, 1.199999999999999956e+00
7.900000000000000000e+01, 1.199999999999999956e+00
8.000000000000000000e+01, 1.199999999999999956e+00
8.100000000000000000e+01, 1.199999999999999956e+00
8.200000000000000000e+01, 1.199999999999999956e+00
8.300000000000000000e+01, 1.199999999999999956e+00
8.400000000000000000e+01, 1.199999999999999956e+00
8.500000000000000000e+01, 1.199999999999999956e+00
8.600000000000000000e+01, 1.199999999999999956e+00
8.700000000000000000e+01, 1.199999999999999956e+00
8.800000000000000000e+01, 1.199999999999999956e+00
8.900000000000000000e+01, 1.199999999999999956e+00
9.000000000000000000e+01, 1.199999999999999956e+00
9.100000000000000000e+01, 1.199999999999999956e+00
9.200000000000000000e+01, 1.199999999999999956e+00
9.300000000000000000e+01, 2.299999999999999822e+00
9.400000000000000000e+01, 2.299999999999999822e+00
9.500000000000000000e+01, 2.299999999999999822e+00
9.600000000000000000e+01, 2.299999999999999822e+00
9.700000000000000000e+01, 2.299999999999999822e+00
9.800000000000000000e+01, 2.299999999999999822e+00
9.900000000000000000e+01, 2.299999999999999822e+00
1.000000000000000000e+02, 2.299999999999999822e+00
1.010000000000000000e+02, 2.299999999999999822e+00
1.020000000000000000e+02, 2.299999999999999822e+00
1.030000000000000000e+02, 2.299999999999999822e+00
1.040000000000000000e+02, 2.299999999999999822e+00
1.050000000000000000e+02, 2.299999999999999822e+00
1.060000000000000000e+02, 2.299999999999999822e+00
1.070000000000000000e+02, 2.299999999999999822e+00
1.080000000000000000e+02, 2.299999999999999822e+00
1.090000000000000000e+02, 2.299999999999999822e+00
1.100000000000000000e+02, 2.299999999999999822e+00
1.110000000000000000e+02, 2.299999999999999822e+00
1.120000000000000000e+02, 2.299999999999999822e+00
1.130000000000000000e+02, 2.299999999999999822e+00
1.140000000000000000e+02, 2.299999999999999822e+00
1.150000000000000000e+02, 2.299999999999999822e+00
1.160000000000000000e+02, 2.299999999999999822e+00
1.170000000000000000e+02, 2.299999999999999822e+00
1.180000000000000000e+02, 2.299999999999999822e+00
1.190000000000000000e+02, 2.299999999999999822e+00
1.200000000000000000e+02, 2.299999999999999822e+00
1.210000000000000000e+02, 2.299999999999999822e+00
1.220000000000000000e+02, 2.299999999999999822e+00
1.230000000000000000e+02, 2.299999999999999822e+00
1.240000000000000000e+02, 2.299999999999999822e+00
1.250000000000000000e+02, 2.299999999999999822e+00
1.260000000000000000e+02, 2.299999999999999822e+00
1.270000000000000000e+02, 2.299999999999999822e+00
1.280000000000000000e+02, 2.299999999999999822e+00
1.290000000000000000e+02, 2.299999999999999822e+00
1.300000000000000000e+02, 2.299999999999999822e+00
1.310000000000000000e+02, 2.299999999999999822e+00
1.320000000000000000e+02, 2.299999999999999822e+00
1.330000000000000000e+02, 2.299999999999999822e+00
1.340000000000000000e+02, 2.299999999999999822e+00
1.350000000000000000e+02, 2.299999999999999822e+00
1.360000000000000000e+02, 2.299999999999999822e+00
1.370000000000000000e+02, 2.299999999999999822e+00
1.380000000000000000e+02, 2.299999999999999822e+00
1.390000000000000000e+02, 2.299999999999999822e+00
1.400000000000000000e+02, 2.299999999999999822e+00
1.410000000000000000e+02, 2.299999999999999822e+00
1.420000000000000000e+02, 2.299999999999999822e+00
1.430000000000000000e+02, 2.299999999999999822e+00
1.440000000000000000e+02, 2.299999999999999822e+00
1.450000000000000000e+02, 2.299999999999999822e+00
1.460000000000000000e+02, 2.299999999999999822e+00
1.470000000000000000e+02, 2.299999999999999822e+00
1.480000000000000000e+02, 2.299999999999999822e+00
1.490000000000000000e+02, 2.299999999999999822e+00
1.500000000000000000e+02, 2.299999999999999822e+00
1.510000000000000000e+02, 2.299999999999999822e+00
1.520000000000000000e+02, 2.299999999999999822e+00
1.530000000000000000e+02, 2.299999999999999822e+00
1.540000000000000000e+02, 2.299999999999999822e+00
1.550000000000000000e+02, 0.000000000000000000e+00
1.560000000000000000e+02, 0.000000000000000000e+00
1.570000000000000000e+02, 0.000000000000000000e+00
1.580000000000000000e+02, 0.000000000000000000e+00
1.590000000000000000e+02, 0.000000000000000000e+00
1.600000000000000000e+02, 0.000000000000000000e+00
1.610000000000000000e+02, 0.000000000000000000e+00
1.620000000000000000e+02, 0.000000000000000000e+00
1.630000000000000000e+02, 0.000000000000000000e+00
1.640000000000000000e+02, 0.000000000000000000e+00
1.650000000000000000e+02, 0.000000000000000000e+00
1.660000000000000000e+02, 0.000000000000000000e+00
1.670000000000000000e+02, 0.000000000000000000e+00
1.680000000000000000e+02, 0.000000000000000000e+00
1.690000000000000000e+02, 0.000000000000000000e+00
1.700000000000000000e+02, 0.000000000000000000e+00
1.710000000000000000e+02, 0.000000000000000000e+00
1.720000000000000000e+02, 0.000000000000000000e+00
1.730000000000000000e+02, 0.000000000000000000e+00
1.740000000000000000e+02, 0.000000000000000000e+00
1.750000000000000000e+02, 0.000000000000000000e+00
1.760000000000000000e+02, 0.000000000000000000e+00
1.770000000000000000e+02, 0.000000000000000000e+00
1.780000000000000000e+02, 0.000000000000000000e+00
1.790000000000000000e+02, 0.000000000000000000e+00
1.800000000000000000e+02, 0.000000000000000000e+00
1.810000000000000000e+02, 0.000000000000000000e+00
1.820000000000000000e+02, 0.000000000000000000e+00
1.830000000000000000e+02, 0.000000000000000000e+00
1.840000000000000000e+02, 0.000000000000000000e+00
1.850000000000000000e+02, 0.000000000000000000e+00
1.860000000000000000e+02, 0.000000000000000000e+00
1.870000000000000000e+02, 0.000000000000000000e+00
1.880000000000000000e+02, 0.000000000000000000e+00
1.890000000000000000e+02, 0.000000000000000000e+00
1.900000000000000000e+02, 0.000000000000000000e+00
1.910000000000000000e+02, 0.000000000000000000e+00
1.920000000000000000e+02, 0.000000000000000000e+00
1.930000000000000000e+02, 0.000000000000000000e+00
1.940000000000000000e+02, 0.000000000000000000e+00
};

\addlegendentry{ground-truth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_low_rotation.tex <==
\addplot [name path=sensor-rotation-0, color=sensor-rotation-0Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 7.921781896903791823e-03
1.000000000000000000e+00, 3.186092366112945606e-02
2.000000000000000000e+00, 7.143335131595604515e-02
3.000000000000000000e+00, 1.142063307279307938e-01
4.000000000000000000e+00, 1.626494882907606743e-01
5.000000000000000000e+00, 2.302236618693406789e-01
6.000000000000000000e+00, 2.911484207358538967e-01
7.000000000000000000e+00, 3.042935643793793221e-01
8.000000000000000000e+00, 2.693023288167049611e-01
9.000000000000000000e+00, 2.152550585605670919e-01
1.000000000000000000e+01, 1.474032740502742855e-01
1.100000000000000000e+01, 1.092340541187523384e-01
1.200000000000000000e+01, 8.591306340870095981e-02
1.300000000000000000e+01, 6.681805078697150568e-02
1.400000000000000000e+01, 4.917365986932955430e-02
1.500000000000000000e+01, 5.309507934515142469e-02
1.600000000000000000e+01, 5.502847090474311670e-02
1.700000000000000000e+01, 5.623359891686392081e-02
1.800000000000000000e+01, 7.249058076524411698e-02
1.900000000000000000e+01, 1.147879468799006680e-01
2.000000000000000000e+01, 1.822102099451347601e-01
2.100000000000000000e+01, 3.882082180285290618e-01
2.200000000000000000e+01, 7.431707274745100733e-01
2.300000000000000000e+01, 6.149929864327354778e-01
2.400000000000000000e+01, 2.731729853542221864e-01
2.500000000000000000e+01, 1.191302826339316057e-01
2.600000000000000000e+01, 5.845667648661970889e-02
2.700000000000000000e+01, 2.909722092915209210e-02
2.800000000000000000e+01, 9.940893118853506155e-03
2.900000000000000000e+01, 1.991813346856111458e-02
3.000000000000000000e+01, 3.058672387314415042e-02
3.100000000000000000e+01, 4.980421163073125296e-02
3.200000000000000000e+01, 7.226184969988456996e-02
3.300000000000000000e+01, 9.847482692418753347e-02
3.400000000000000000e+01, 1.457040932597257477e-01
3.500000000000000000e+01, 1.820440022247747924e-01
3.600000000000000000e+01, 2.221931713081404802e-01
3.700000000000000000e+01, 2.505534577825040410e-01
3.800000000000000000e+01, 2.440566699162301234e-01
3.900000000000000000e+01, 2.039620066067026893e-01
4.000000000000000000e+01, 1.477582496362303821e-01
4.100000000000000000e+01, 1.122778064242898471e-01
4.200000000000000000e+01, 8.538581808446782384e-02
4.300000000000000000e+01, 5.794818813570282862e-02
4.400000000000000000e+01, 3.606019618502152163e-02
4.500000000000000000e+01, 1.501879230812815623e-02
4.600000000000000000e+01, 8.772683143695496344e-03
4.700000000000000000e+01, 1.983425704815426627e-02
4.800000000000000000e+01, 4.601257360190306317e-02
4.900000000000000000e+01, 9.434455770588576207e-02
5.000000000000000000e+01, 1.992850039069044288e-01
5.100000000000000000e+01, 4.644118862929885183e-01
5.200000000000000000e+01, 7.805460281373054476e-01
5.300000000000000000e+01, 5.217103796324081832e-01
5.400000000000000000e+01, 2.473945683614324487e-01
5.500000000000000000e+01, 1.239018985035093834e-01
5.600000000000000000e+01, 8.793635029907539979e-02
5.700000000000000000e+01, 6.119919615104492394e-02
5.800000000000000000e+01, 4.670959381109483083e-02
5.900000000000000000e+01, 5.365064396020629428e-02
6.000000000000000000e+01, 4.946723954673487578e-02
6.100000000000000000e+01, 6.001607813903199473e-02
6.200000000000000000e+01, 7.318488487149707455e-02
6.300000000000000000e+01, 9.742326464907090366e-02
6.400000000000000000e+01, 1.351124986098662661e-01
6.500000000000000000e+01, 1.719886874462248083e-01
6.600000000000000000e+01, 2.359787303789509239e-01
6.700000000000000000e+01, 2.923638838551168573e-01
6.800000000000000000e+01, 3.066063836983982660e-01
6.900000000000000000e+01, 2.563199811293726538e-01
7.000000000000000000e+01, 1.791186161282351808e-01
7.100000000000000000e+01, 1.201401850791536940e-01
7.200000000000000000e+01, 7.647336683261532486e-02
7.300000000000000000e+01, 5.265828101185577453e-02
7.400000000000000000e+01, 2.050209000493558378e-02
7.500000000000000000e+01, 1.119623245702158938e-02
7.600000000000000000e+01, 3.017662067167132742e-02
7.700000000000000000e+01, 5.618417575125793373e-02
7.800000000000000000e+01, 8.731995396047563529e-02
7.900000000000000000e+01, 1.432537035022709848e-01
8.000000000000000000e+01, 2.092499475515799956e-01
8.100000000000000000e+01, 2.654539641909308134e-01
8.200000000000000000e+01, 3.189014783330381131e-01
8.300000000000000000e+01, 2.872725336128442719e-01
8.400000000000000000e+01, 2.236114341741304301e-01
8.500000000000000000e+01, 1.651755689742657462e-01
8.600000000000000000e+01, 1.199175693387900532e-01
8.700000000000000000e+01, 8.932508571418401599e-02
8.800000000000000000e+01, 7.232618892667187771e-02
8.900000000000000000e+01, 6.552219597022110320e-02
9.000000000000000000e+01, 5.404615300120040738e-02
9.100000000000000000e+01, 4.788036997305407383e-02
9.200000000000000000e+01, 5.853251824171665924e-02
9.300000000000000000e+01, 6.378512389100006452e-02
9.400000000000000000e+01, 8.999030961913902227e-02
9.500000000000000000e+01, 1.567498966890280010e-01
9.600000000000000000e+01, 2.950789795895412682e-01
9.700000000000000000e+01, 6.324264785689460711e-01
9.800000000000000000e+01, 7.433712604280516834e-01
9.900000000000000000e+01, 3.773914428673418309e-01
1.000000000000000000e+02, 1.694580779265496551e-01
1.010000000000000000e+02, 7.651344773225488005e-02
1.020000000000000000e+02, 3.673652366695282639e-02
1.030000000000000000e+02, 2.920125580383490377e-03
1.040000000000000000e+02, 1.105406094065655188e-02
1.050000000000000000e+02, 2.870687352674974532e-02
1.060000000000000000e+02, 4.101130620954267919e-02
1.070000000000000000e+02, 6.695631193109602419e-02
1.080000000000000000e+02, 8.756292071391220955e-02
1.090000000000000000e+02, 1.291116891030595626e-01
1.100000000000000000e+02, 1.555452377688928411e-01
1.110000000000000000e+02, 2.158697546818292845e-01
1.120000000000000000e+02, 2.404776287307147098e-01
1.130000000000000000e+02, 2.443796125744558123e-01
1.140000000000000000e+02, 2.123483023447827189e-01
1.150000000000000000e+02, 1.704498728702452670e-01
1.160000000000000000e+02, 1.284954286634326925e-01
1.170000000000000000e+02, 9.259084829730623856e-02
1.180000000000000000e+02, 7.182552639475187073e-02
1.190000000000000000e+02, 4.414034306902490934e-02
1.200000000000000000e+02, 3.069828034125416175e-02
1.210000000000000000e+02, 1.128495827702681240e-02
1.220000000000000000e+02, 1.054221787721524618e-02
1.230000000000000000e+02, 3.374147405708358138e-02
1.240000000000000000e+02, 7.048424131456779151e-02
1.250000000000000000e+02, 1.559031113492799214e-01
1.260000000000000000e+02, 3.365095800668225778e-01
1.270000000000000000e+02, 7.124634380164105441e-01
1.280000000000000000e+02, 6.711744397540351237e-01
1.290000000000000000e+02, 3.205971197407485040e-01
1.300000000000000000e+02, 1.574292384961643587e-01
1.310000000000000000e+02, 9.581081313017021650e-02
1.320000000000000000e+02, 6.201929445498707144e-02
1.330000000000000000e+02, 5.575422940451402881e-02
1.340000000000000000e+02, 4.274598054327816143e-02
1.350000000000000000e+02, 4.266197029498882548e-02
1.360000000000000000e+02, 5.234189334203311755e-02
1.370000000000000000e+02, 7.139170130099112277e-02
1.380000000000000000e+02, 8.940574643560846024e-02
1.390000000000000000e+02, 1.180966564916574174e-01
1.400000000000000000e+02, 1.646398231611663765e-01
1.410000000000000000e+02, 2.158494508251113386e-01
1.420000000000000000e+02, 2.790261362341873719e-01
1.430000000000000000e+02, 3.120672096604854007e-01
1.440000000000000000e+02, 2.735345575412723163e-01
1.450000000000000000e+02, 2.190081247988472646e-01
1.460000000000000000e+02, 1.421305568916919060e-01
1.470000000000000000e+02, 1.031206626542217203e-01
1.480000000000000000e+02, 5.716392655141969148e-02
1.490000000000000000e+02, 2.882527620739913990e-02
1.500000000000000000e+02, 7.217019711251627771e-03
1.510000000000000000e+02, 2.243157035298018118e-02
1.520000000000000000e+02, 5.088722554679249443e-02
1.530000000000000000e+02, 7.369322514523267420e-02
1.540000000000000000e+02, 1.106215351904411004e-01
1.550000000000000000e+02, 1.753700828365860609e-01
1.560000000000000000e+02, 2.410342608656772523e-01
1.570000000000000000e+02, 2.977827496130520668e-01
1.580000000000000000e+02, 2.983223292021458528e-01
1.590000000000000000e+02, 2.525527147260396288e-01
1.600000000000000000e+02, 1.843488428497114529e-01
1.610000000000000000e+02, 1.361574983428527064e-01
1.620000000000000000e+02, 9.473179274706174102e-02
1.630000000000000000e+02, 7.450450010499062858e-02
1.640000000000000000e+02, 6.617521638734971678e-02
1.650000000000000000e+02, 5.453696422303652008e-02
1.660000000000000000e+02, 3.991286981120814592e-02
1.670000000000000000e+02, 5.015253808464663343e-02
1.680000000000000000e+02, 5.335376004000747657e-02
1.690000000000000000e+02, 7.910924519322745652e-02
1.700000000000000000e+02, 1.203752405205339854e-01
1.710000000000000000e+02, 2.182987188302845105e-01
1.720000000000000000e+02, 4.750679610589274571e-01
1.730000000000000000e+02, 7.736861259814222791e-01
1.740000000000000000e+02, 5.196324761081434485e-01
1.750000000000000000e+02, 2.183053511500638588e-01
1.760000000000000000e+02, 1.055135816085028266e-01
1.770000000000000000e+02, 5.173084054675402416e-02
1.780000000000000000e+02, 2.153904328266275509e-02
1.790000000000000000e+02, 1.445024810597659269e-02
1.800000000000000000e+02, 2.016490671721753863e-02
1.810000000000000000e+02, 3.549704705444459152e-02
1.820000000000000000e+02, 5.666267901146163077e-02
1.830000000000000000e+02, 7.624331949784197981e-02
1.840000000000000000e+02, 1.127809629849536449e-01
1.850000000000000000e+02, 1.458788548307463351e-01
1.860000000000000000e+02, 1.972368140839298178e-01
1.870000000000000000e+02, 2.334862807907807369e-01
1.880000000000000000e+02, 2.543411055543927657e-01
1.890000000000000000e+02, 2.331049083796441768e-01
1.900000000000000000e+02, 1.896166749695232245e-01
1.910000000000000000e+02, 1.436306210107527181e-01
1.920000000000000000e+02, 1.051747109663189739e-01
1.930000000000000000e+02, 7.917783764854233186e-02
1.940000000000000000e+02, 5.112966621965055192e-02
};

\addlegendentry{sensor-rotation-0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=sensor-rotation-1, color=sensor-rotation-1Color, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 1.069565924133816445e-02
1.000000000000000000e+00, 4.141509787923210173e-02
2.000000000000000000e+00, 7.709672517343416076e-02
3.000000000000000000e+00, 1.069408070968098368e-01
4.000000000000000000e+00, 1.560978694050798310e-01
5.000000000000000000e+00, 2.291565604280594026e-01
6.000000000000000000e+00, 2.918612157416062836e-01
7.000000000000000000e+00, 3.051528392274366341e-01
8.000000000000000000e+00, 2.651999327434768072e-01
9.000000000000000000e+00, 2.014472175019098588e-01
1.000000000000000000e+01, 1.524822825763595124e-01
1.100000000000000000e+01, 1.166978263409684802e-01
1.200000000000000000e+01, 8.700657459200962507e-02
1.300000000000000000e+01, 6.845529681695310120e-02
1.400000000000000000e+01, 5.160757222307791464e-02
1.500000000000000000e+01, 4.577571630854163076e-02
1.600000000000000000e+01, 4.794233017367379585e-02
1.700000000000000000e+01, 5.035117162632434668e-02
1.800000000000000000e+01, 6.625780110793322297e-02
1.900000000000000000e+01, 1.057056924605600523e-01
2.000000000000000000e+01, 1.801985506841323192e-01
2.100000000000000000e+01, 3.915504372762602658e-01
2.200000000000000000e+01, 7.606155801660794413e-01
2.300000000000000000e+01, 6.144254185000640467e-01
2.400000000000000000e+01, 2.761188590849026347e-01
2.500000000000000000e+01, 1.344337802319913455e-01
2.600000000000000000e+01, 6.041570921596714494e-02
2.700000000000000000e+01, 2.578278663176760549e-02
2.800000000000000000e+01, 1.655186461390684496e-02
2.900000000000000000e+01, 1.829730502005454812e-02
3.000000000000000000e+01, 2.823849385203689236e-02
3.100000000000000000e+01, 4.963084950017598862e-02
3.200000000000000000e+01, 7.742188562265021889e-02
3.300000000000000000e+01, 9.994588290076834858e-02
3.400000000000000000e+01, 1.419619544271147338e-01
3.500000000000000000e+01, 1.854226900870536154e-01
3.600000000000000000e+01, 2.229739128427517814e-01
3.700000000000000000e+01, 2.527509573343086346e-01
3.800000000000000000e+01, 2.376264635541219805e-01
3.900000000000000000e+01, 1.878307703399835216e-01
4.000000000000000000e+01, 1.045236250523867844e-01
4.100000000000000000e+01, 7.799194471058031042e-02
4.200000000000000000e+01, 5.632850027332214626e-02
4.300000000000000000e+01, 3.034887653056273990e-02
4.400000000000000000e+01, 1.838635841157712156e-02
4.500000000000000000e+01, 4.712927596181274055e-03
4.600000000000000000e+01, 1.613118209832357236e-02
4.700000000000000000e+01, 5.218925236768361120e-02
4.800000000000000000e+01, 1.112449317445783209e-01
4.900000000000000000e+01, 2.353125274721442894e-01
5.000000000000000000e+01, 5.319104424229785799e-01
5.100000000000000000e+01, 7.741682345349104599e-01
5.200000000000000000e+01, 4.550277544863740586e-01
5.300000000000000000e+01, 2.153150946604173166e-01
5.400000000000000000e+01, 1.170309943828868882e-01
5.500000000000000000e+01, 6.865194104119397289e-02
5.600000000000000000e+01, 5.004587341068373468e-02
5.700000000000000000e+01, 4.242908553869111782e-02
5.800000000000000000e+01, 4.718367689315856178e-02
5.900000000000000000e+01, 4.816029045787690449e-02
6.000000000000000000e+01, 6.177017753705558306e-02
6.100000000000000000e+01, 8.035596337465217287e-02
6.200000000000000000e+01, 9.962627063448128983e-02
6.300000000000000000e+01, 1.391406672769990582e-01
6.400000000000000000e+01, 1.892466252091878909e-01
6.500000000000000000e+01, 2.662189530078031274e-01
6.600000000000000000e+01, 3.083611868684529300e-01
6.700000000000000000e+01, 2.919228791925737032e-01
6.800000000000000000e+01, 2.418573319244033959e-01
6.900000000000000000e+01, 1.730135645904697927e-01
7.000000000000000000e+01, 1.124319398238673440e-01
7.100000000000000000e+01, 7.279235509167168716e-02
7.200000000000000000e+01, 3.595939256838561610e-02
7.300000000000000000e+01, 1.695704675527041558e-02
7.400000000000000000e+01, 7.258407620376036706e-03
7.500000000000000000e+01, 4.314462884044002050e-02
7.600000000000000000e+01, 6.771649521284862916e-02
7.700000000000000000e+01, 1.025065121765750542e-01
7.800000000000000000e+01, 1.588782420199688072e-01
7.900000000000000000e+01, 2.152057337801988879e-01
8.000000000000000000e+01, 2.838660518906039321e-01
8.100000000000000000e+01, 3.082259709309660423e-01
8.200000000000000000e+01, 2.765111415321663269e-01
8.300000000000000000e+01, 2.185770586412904559e-01
8.400000000000000000e+01, 1.510686377123128254e-01
8.500000000000000000e+01, 1.175525904542315536e-01
8.600000000000000000e+01, 9.116366801891348515e-02
8.700000000000000000e+01, 6.280808869566534280e-02
8.800000000000000000e+01, 4.887383385819690090e-02
8.900000000000000000e+01, 4.942801231694637226e-02
9.000000000000000000e+01, 4.941851730984509611e-02
9.100000000000000000e+01, 4.968746132122602716e-02
9.200000000000000000e+01, 6.681877026857414859e-02
9.300000000000000000e+01, 1.779223694072027961e-01
9.400000000000000000e+01, 3.743171789675710515e-01
9.500000000000000000e+01, 7.373727654241771790e-01
9.600000000000000000e+01, 6.446485328698716710e-01
9.700000000000000000e+01, 2.990183663752302712e-01
9.800000000000000000e+01, 1.341163595139181208e-01
9.900000000000000000e+01, 6.230984536435422994e-02
1.000000000000000000e+02, 3.568048791545022635e-02
1.010000000000000000e+02, 5.082663380491890016e-03
1.020000000000000000e+02, 1.327996206100706331e-02
1.030000000000000000e+02, 3.571891096210830924e-02
1.040000000000000000e+02, 4.409935802907863356e-02
1.050000000000000000e+02, 6.492041508721783927e-02
1.060000000000000000e+02, 9.871950461339538963e-02
1.070000000000000000e+02, 1.349626222235298378e-01
1.080000000000000000e+02, 1.717103055335492956e-01
1.090000000000000000e+02, 2.304914881457453268e-01
1.100000000000000000e+02, 2.429806552894359373e-01
1.110000000000000000e+02, 2.396866831405754517e-01
1.120000000000000000e+02, 2.039751329656156464e-01
1.130000000000000000e+02, 1.611067431034202413e-01
1.140000000000000000e+02, 1.258130573624759718e-01
1.150000000000000000e+02, 8.330770855289501564e-02
1.160000000000000000e+02, 5.951688064484911278e-02
1.170000000000000000e+02, 3.922300527026183203e-02
1.180000000000000000e+02, 2.881529628524454392e-02
1.190000000000000000e+02, 5.874242836541134112e-03
1.200000000000000000e+02, 1.835674965753755772e-02
1.210000000000000000e+02, 3.734795385891787750e-02
1.220000000000000000e+02, 9.598509199463524377e-02
1.230000000000000000e+02, 1.987735727321438550e-01
1.240000000000000000e+02, 4.462917293809193775e-01
1.250000000000000000e+02, 7.723094950574681539e-01
1.260000000000000000e+02, 5.538476415162312261e-01
1.270000000000000000e+02, 2.518064895372266743e-01
1.280000000000000000e+02, 1.284197302499019977e-01
1.290000000000000000e+02, 8.554827076299170718e-02
1.300000000000000000e+02, 6.229141596721012725e-02
1.310000000000000000e+02, 4.609373975221352226e-02
1.320000000000000000e+02, 4.889308483865099919e-02
1.330000000000000000e+02, 5.223862013508904362e-02
1.340000000000000000e+02, 6.202866338371595262e-02
1.350000000000000000e+02, 7.320402325560111667e-02
1.360000000000000000e+02, 9.169957951849976030e-02
1.370000000000000000e+02, 1.264223136016482119e-01
1.380000000000000000e+02, 1.706291960986596745e-01
1.390000000000000000e+02, 2.430953216190798738e-01
1.400000000000000000e+02, 2.960202906491454233e-01
1.410000000000000000e+02, 2.977355032591466055e-01
1.420000000000000000e+02, 2.588465259930622930e-01
1.430000000000000000e+02, 1.879237374241243541e-01
1.440000000000000000e+02, 1.287056142588087204e-01
1.450000000000000000e+02, 7.273624317347075763e-02
1.460000000000000000e+02, 5.019253194011440850e-02
1.470000000000000000e+02, 2.238030095634607058e-02
1.480000000000000000e+02, 6.645399646734322097e-03
1.490000000000000000e+02, 2.941769636204141433e-02
1.500000000000000000e+02, 5.945688969144128505e-02
1.510000000000000000e+02, 8.257679379814052145e-02
1.520000000000000000e+02, 1.301321482723516165e-01
1.530000000000000000e+02, 1.987550596247293910e-01
1.540000000000000000e+02, 2.664458279265930485e-01
1.550000000000000000e+02, 1.758961902383421039e-01
1.560000000000000000e+02, 2.450733758890173697e-01
1.570000000000000000e+02, 3.038428728871090390e-01
1.580000000000000000e+02, 3.048992218192053127e-01
1.590000000000000000e+02, 2.489730345798722988e-01
1.600000000000000000e+02, 1.896946561666546793e-01
1.610000000000000000e+02, 1.435894455840279194e-01
1.620000000000000000e+02, 9.635419808376276263e-02
1.630000000000000000e+02, 7.767619002454603794e-02
1.640000000000000000e+02, 6.270812717773378842e-02
1.650000000000000000e+02, 5.129693565600886712e-02
1.660000000000000000e+02, 5.025859801089181678e-02
1.670000000000000000e+02, 5.255114037674577659e-02
1.680000000000000000e+02, 5.898156004848768147e-02
1.690000000000000000e+02, 8.201331133401275342e-02
1.700000000000000000e+02, 1.205926040284408252e-01
1.710000000000000000e+02, 2.158367812195446656e-01
1.720000000000000000e+02, 4.883853552040594570e-01
1.730000000000000000e+02, 7.838483154213043980e-01
1.740000000000000000e+02, 5.025807431106313894e-01
1.750000000000000000e+02, 2.206489748186739319e-01
1.760000000000000000e+02, 1.174109479208004791e-01
1.770000000000000000e+02, 4.769337532376168032e-02
1.780000000000000000e+02, 2.464906108840115781e-02
1.790000000000000000e+02, 2.165141580620393112e-03
1.800000000000000000e+02, 1.524784246427830954e-02
1.810000000000000000e+02, 3.476090832558028504e-02
1.820000000000000000e+02, 5.526119754202089840e-02
1.830000000000000000e+02, 8.741136734100733718e-02
1.840000000000000000e+02, 1.117855305102087304e-01
1.850000000000000000e+02, 1.498780680488841499e-01
1.860000000000000000e+02, 1.879932161817514935e-01
1.870000000000000000e+02, 2.330433751961460687e-01
1.880000000000000000e+02, 2.581100911436823853e-01
1.890000000000000000e+02, 2.281670637015071890e-01
1.900000000000000000e+02, 1.850192980233454909e-01
1.910000000000000000e+02, 1.424724090002287835e-01
1.920000000000000000e+02, 1.049762843093557663e-01
1.930000000000000000e+02, 6.873176238565696650e-02
1.940000000000000000e+02, 5.092533341734726410e-02
};

\addlegendentry{sensor-rotation-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/exp/steps_low_uncertainty.tex <==
\addplot [name path=uncertainty, color=uncertaintyColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 7.927141483025801350e+00
1.100000000000000000e+01, 9.905930867482966917e+00
1.200000000000000000e+01, 1.396852521599585017e+01
1.300000000000000000e+01, 2.129821330699839521e+01
1.400000000000000000e+01, 3.372890411159252722e+01
1.500000000000000000e+01, 5.531810565206373553e+01
1.600000000000000000e+01, 8.209298477401651439e+01
1.700000000000000000e+01, 7.075419694208801502e+01
1.800000000000000000e+01, 3.674852630675968612e+01
1.900000000000000000e+01, 1.666455410214301480e+01
2.000000000000000000e+01, 7.051188380217894291e+00
2.100000000000000000e+01, 2.766331082702177646e+00
2.200000000000000000e+01, 1.508622042810333186e+00
2.300000000000000000e+01, 2.254572036163319027e+00
2.400000000000000000e+01, 1.581525657077745173e+00
2.500000000000000000e+01, 2.233377384003141231e+00
2.600000000000000000e+01, 4.298567763382985518e+00
2.700000000000000000e+01, 8.751439705514071576e+00
2.800000000000000000e+01, 1.644322907950920865e+01
2.900000000000000000e+01, 3.565277304178147233e+01
3.000000000000000000e+01, 3.202058721427743393e+01
3.100000000000000000e+01, 2.588692472668504507e+01
3.200000000000000000e+01, 2.104677893694060131e+01
3.300000000000000000e+01, 1.670802952926915452e+01
3.400000000000000000e+01, 1.315809257759920570e+01
3.500000000000000000e+01, 1.089851958159291101e+01
3.600000000000000000e+01, 1.059483625355394665e+01
3.700000000000000000e+01, 1.521041281443307902e+01
3.800000000000000000e+01, 2.762948889342226977e+01
3.900000000000000000e+01, 1.529857769360310371e+01
4.000000000000000000e+01, 7.946920173830688938e+00
4.100000000000000000e+01, 1.013012277642328129e+01
4.200000000000000000e+01, 1.381891497194682294e+01
4.300000000000000000e+01, 1.826622180344422119e+01
4.400000000000000000e+01, 2.231539882532858599e+01
4.500000000000000000e+01, 2.890320035581296310e+01
4.600000000000000000e+01, 2.992610953273617724e+01
4.700000000000000000e+01, 2.341185831270843209e+01
4.800000000000000000e+01, 1.280658436168692127e+01
4.900000000000000000e+01, 6.253729732607689940e+00
5.000000000000000000e+01, 2.742971852377265929e+00
5.100000000000000000e+01, 1.986177981226569411e+00
5.200000000000000000e+01, 1.529027481717435855e+00
5.300000000000000000e+01, 1.669613962617661151e+00
5.400000000000000000e+01, 2.090836511239963613e+00
5.500000000000000000e+01, 3.759623129219367144e+00
5.600000000000000000e+01, 8.169237065149740573e+00
5.700000000000000000e+01, 1.861469834528963574e+01
5.800000000000000000e+01, 4.087206132871336450e+01
5.900000000000000000e+01, 6.794637321221949833e+01
6.000000000000000000e+01, 6.476932912386112662e+01
6.100000000000000000e+01, 4.372018737506171249e+01
6.200000000000000000e+01, 2.679772489288323456e+01
6.300000000000000000e+01, 1.753262497515959950e+01
6.400000000000000000e+01, 1.179481412345738889e+01
6.500000000000000000e+01, 8.756136730118857514e+00
6.600000000000000000e+01, 8.235905508691850230e+00
6.700000000000000000e+01, 1.161210898990728779e+01
6.800000000000000000e+01, 1.362886991680178284e+01
6.900000000000000000e+01, 9.018192391731659541e+00
7.000000000000000000e+01, 7.566760126801010955e+00
7.100000000000000000e+01, 8.267039530080047882e+00
7.200000000000000000e+01, 1.036138727539329807e+01
7.300000000000000000e+01, 1.349627229787067861e+01
7.400000000000000000e+01, 2.053928481600001277e+01
7.500000000000000000e+01, 2.338119808547016376e+01
7.600000000000000000e+01, 1.980617077247553937e+01
7.700000000000000000e+01, 1.513781564806312829e+01
7.800000000000000000e+01, 1.140366732258279647e+01
7.900000000000000000e+01, 8.693869424777195931e+00
8.000000000000000000e+01, 7.391678323702927322e+00
8.100000000000000000e+01, 8.624759746701933238e+00
8.200000000000000000e+01, 1.126533251050072160e+01
8.300000000000000000e+01, 1.117839466765918388e+01
8.400000000000000000e+01, 8.514512815371833909e+00
8.500000000000000000e+01, 8.502088314423435378e+00
8.600000000000000000e+01, 1.063421594752111154e+01
8.700000000000000000e+01, 1.506283816294708622e+01
8.800000000000000000e+01, 2.285009241877735775e+01
8.900000000000000000e+01, 3.600963950065871444e+01
9.000000000000000000e+01, 5.721353937352179742e+01
9.100000000000000000e+01, 7.611193236850303379e+01
9.200000000000000000e+01, 5.556254406414428360e+01
9.300000000000000000e+01, 1.043468545085620391e+01
9.400000000000000000e+01, 4.996324549264926418e+00
9.500000000000000000e+01, 2.608918402029567485e+00
9.600000000000000000e+01, 3.163185984629696357e+00
9.700000000000000000e+01, 1.646697920195161480e+00
9.800000000000000000e+01, 2.350338175680624531e+00
9.900000000000000000e+01, 2.224774722586880138e+00
1.000000000000000000e+02, 2.988610828400426023e+00
1.010000000000000000e+02, 5.432203728638071993e+00
1.020000000000000000e+02, 1.149451905215667225e+01
1.030000000000000000e+02, 1.854607375814629933e+01
1.040000000000000000e+02, 2.906681163856929118e+01
1.050000000000000000e+02, 2.596737271112686329e+01
1.060000000000000000e+02, 2.096459228759440307e+01
1.070000000000000000e+02, 1.692050173610735442e+01
1.080000000000000000e+02, 1.374733013463734999e+01
1.090000000000000000e+02, 1.213570594983023199e+01
1.100000000000000000e+02, 1.291121792809826729e+01
1.110000000000000000e+02, 1.526413853279752786e+01
1.120000000000000000e+02, 1.390481454931893879e+01
1.130000000000000000e+02, 1.621351738093468242e+01
1.140000000000000000e+02, 1.381929816664117894e+01
1.150000000000000000e+02, 1.226557414194196305e+01
1.160000000000000000e+02, 1.272522325500140283e+01
1.170000000000000000e+02, 1.481235236418050683e+01
1.180000000000000000e+02, 1.831461637134579945e+01
1.190000000000000000e+02, 2.277516286615794883e+01
1.200000000000000000e+02, 2.853971573535118722e+01
1.210000000000000000e+02, 2.353464494749836433e+01
1.220000000000000000e+02, 1.875177804091286404e+01
1.230000000000000000e+02, 9.071004407711766859e+00
1.240000000000000000e+02, 3.952517665419890136e+00
1.250000000000000000e+02, 2.489659026351736415e+00
1.260000000000000000e+02, 2.233026554815131348e+00
1.270000000000000000e+02, 1.545602914795347615e+00
1.280000000000000000e+02, 2.868705660631841958e+00
1.290000000000000000e+02, 2.554590278846044615e+00
1.300000000000000000e+02, 3.661121069248508775e+00
1.310000000000000000e+02, 7.265614773475277843e+00
1.320000000000000000e+02, 1.614781606500203992e+01
1.330000000000000000e+02, 3.436618878469774074e+01
1.340000000000000000e+02, 5.356884240769702643e+01
1.350000000000000000e+02, 5.231705653737598993e+01
1.360000000000000000e+02, 3.528340028284742402e+01
1.370000000000000000e+02, 2.291406999846341463e+01
1.380000000000000000e+02, 1.532533592257557586e+01
1.390000000000000000e+02, 1.098828737544117118e+01
1.400000000000000000e+02, 9.453245152710273658e+00
1.410000000000000000e+02, 1.144503603013398418e+01
1.420000000000000000e+02, 9.315105308555349239e+00
1.430000000000000000e+02, 9.248325982325289019e+00
1.440000000000000000e+02, 9.604086880913936142e+00
1.450000000000000000e+02, 8.508862934238422326e+00
1.460000000000000000e+02, 8.829715354319851883e+00
1.470000000000000000e+02, 1.056740741001944173e+01
1.480000000000000000e+02, 1.428827704831359213e+01
1.490000000000000000e+02, 1.747958890577855584e+01
1.500000000000000000e+02, 1.812680892467956895e+01
1.510000000000000000e+02, 1.922333615559687559e+01
1.520000000000000000e+02, 1.404638220028833118e+01
1.530000000000000000e+02, 1.050403962366541677e+01
1.540000000000000000e+02, 8.640450977336744387e+00
1.550000000000000000e+02, 6.764915080545342185e+00
1.560000000000000000e+02, 6.546017674454717827e+00
1.570000000000000000e+02, 7.618646880614422301e+00
1.580000000000000000e+02, 2.026338883091811738e+01
1.590000000000000000e+02, 1.179518297269674676e+01
1.600000000000000000e+02, 8.010509180356290670e+00
1.610000000000000000e+02, 8.269265486004261589e+00
1.620000000000000000e+02, 1.070050291722581193e+01
1.630000000000000000e+02, 1.552311947726029828e+01
1.640000000000000000e+02, 2.377559305873376871e+01
1.650000000000000000e+02, 3.814025300576007993e+01
1.660000000000000000e+02, 6.262076675072758292e+01
1.670000000000000000e+02, 8.364010654175211812e+01
1.680000000000000000e+02, 6.178654947011391840e+01
1.690000000000000000e+02, 2.950119512581250092e+01
1.700000000000000000e+02, 1.340661336007111615e+01
1.710000000000000000e+02, 5.584736696925016730e+00
1.720000000000000000e+02, 2.200302019564813971e+00
1.730000000000000000e+02, 1.619958301577733462e+00
1.740000000000000000e+02, 1.602472373617509049e+00
1.750000000000000000e+02, 1.578232610464451735e+00
1.760000000000000000e+02, 2.572154259958188582e+00
1.770000000000000000e+02, 5.178422347286907979e+00
1.780000000000000000e+02, 1.033800174578729170e+01
1.790000000000000000e+02, 2.067555914507882875e+01
1.800000000000000000e+02, 3.238251476403961249e+01
1.810000000000000000e+02, 2.912455423861102943e+01
1.820000000000000000e+02, 2.453344324227456141e+01
1.830000000000000000e+02, 1.993929968007768849e+01
1.840000000000000000e+02, 1.577520765217788323e+01
1.850000000000000000e+02, 1.248715265538494279e+01
1.860000000000000000e+02, 1.056266202931496245e+01
1.870000000000000000e+02, 1.103475341504612217e+01
1.880000000000000000e+02, 1.922786707883326329e+01
1.890000000000000000e+02, 2.315389778987920621e+01
1.900000000000000000e+02, 1.333953490351941618e+01
1.910000000000000000e+02, 1.072843640651845831e+01
1.920000000000000000e+02, 1.121739284036870643e+01
1.930000000000000000e+02, 1.359355082708471940e+01
1.940000000000000000e+02, 1.707276421034594804e+01
};

\addlegendentry{uncertainty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/ramp_high_estimation.tex <==
\addplot [name path=estimationlower, color=backGray, line width=1.5pt, draw opacity=0.1, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, -1.299999999999998934e-01
1.100000000000000000e+01, -1.424999999999999045e-01
1.200000000000000000e+01, -1.499999999999999112e-01
1.300000000000000000e+01, -1.624999999999998945e-01
1.400000000000000000e+01, -1.749999999999999056e-01
1.500000000000000000e+01, -2.124999999999999112e-01
1.600000000000000000e+01, -1.999999999999999001e-01
1.700000000000000000e+01, -2.124999999999999112e-01
1.800000000000000000e+01, -2.699999999999999067e-01
1.900000000000000000e+01, -2.524999999999998912e-01
2.000000000000000000e+01, -1.324999999999998956e-01
2.100000000000000000e+01, -4.999999999999989869e-02
2.200000000000000000e+01, -9.999999999999896125e-03
2.300000000000000000e+01, -2.499999999999895969e-03
2.400000000000000000e+01, 1.040834085586084257e-16
2.500000000000000000e+01, -9.999999999999896125e-03
2.600000000000000000e+01, -9.999999999999896125e-03
2.700000000000000000e+01, 1.040834085586084257e-16
2.800000000000000000e+01, 7.500000000000103806e-03
2.900000000000000000e+01, 1.000000000000010429e-02
3.000000000000000000e+01, 7.500000000000103806e-03
3.100000000000000000e+01, 1.000000000000010429e-02
3.200000000000000000e+01, 7.500000000000103806e-03
3.300000000000000000e+01, 7.500000000000103806e-03
3.400000000000000000e+01, -1.249999999999989661e-02
3.500000000000000000e+01, -1.224999999999999006e-01
3.600000000000000000e+01, -1.049999999999998990e-01
3.700000000000000000e+01, -1.224999999999999006e-01
3.800000000000000000e+01, -1.324999999999998956e-01
3.900000000000000000e+01, -5.499999999999989619e-02
4.000000000000000000e+01, 2.500000000000104569e-03
4.100000000000000000e+01, 5.000000000000010686e-02
4.200000000000000000e+01, 4.750000000000010464e-02
4.300000000000000000e+01, 7.750000000000009659e-02
4.400000000000000000e+01, 5.750000000000010658e-02
4.500000000000000000e+01, 1.750000000000010575e-02
4.600000000000000000e+01, 2.000000000000010450e-02
4.700000000000000000e+01, -4.999999999999896888e-03
4.800000000000000000e+01, 7.500000000000103806e-03
4.900000000000000000e+01, -2.499999999999989730e-02
5.000000000000000000e+01, 1.975000000000001199e-01
5.100000000000000000e+01, 2.500000000000001110e-01
5.200000000000000000e+01, 2.900000000000000910e-01
5.300000000000000000e+01, 2.575000000000001177e-01
5.400000000000000000e+01, 2.900000000000000910e-01
5.500000000000000000e+01, 2.900000000000000910e-01
5.600000000000000000e+01, 2.900000000000000910e-01
5.700000000000000000e+01, 2.900000000000000910e-01
5.800000000000000000e+01, 2.900000000000000910e-01
5.900000000000000000e+01, 2.900000000000000910e-01
6.000000000000000000e+01, 2.900000000000000910e-01
6.100000000000000000e+01, 2.800000000000001377e-01
6.200000000000000000e+01, 2.875000000000000888e-01
6.300000000000000000e+01, 2.775000000000001354e-01
6.400000000000000000e+01, 1.950000000000001177e-01
6.500000000000000000e+01, 2.400000000000001021e-01
6.600000000000000000e+01, 3.000000000000000999e-01
6.700000000000000000e+01, 2.700000000000001288e-01
6.800000000000000000e+01, 2.800000000000001377e-01
6.900000000000000000e+01, 2.775000000000001354e-01
7.000000000000000000e+01, 3.275000000000001243e-01
7.100000000000000000e+01, 3.375000000000001332e-01
7.200000000000000000e+01, 3.450000000000000844e-01
7.300000000000000000e+01, 3.675000000000001044e-01
7.400000000000000000e+01, 3.575000000000000955e-01
7.500000000000000000e+01, 3.700000000000001066e-01
7.600000000000000000e+01, 3.775000000000001132e-01
7.700000000000000000e+01, 3.700000000000001066e-01
7.800000000000000000e+01, 3.775000000000001132e-01
7.900000000000000000e+01, 3.700000000000001066e-01
8.000000000000000000e+01, 4.000000000000001332e-01
8.100000000000000000e+01, 4.200000000000000955e-01
8.200000000000000000e+01, 4.775000000000000910e-01
8.300000000000000000e+01, 4.575000000000001288e-01
8.400000000000000000e+01, 4.700000000000001399e-01
8.500000000000000000e+01, 5.300000000000001377e-01
8.600000000000000000e+01, 5.300000000000001377e-01
8.700000000000000000e+01, 5.475000000000000977e-01
8.800000000000000000e+01, 5.375000000000000888e-01
8.900000000000000000e+01, 5.375000000000000888e-01
9.000000000000000000e+01, 5.400000000000001465e-01
9.100000000000000000e+01, 5.300000000000001377e-01
9.200000000000000000e+01, 5.300000000000001377e-01
9.300000000000000000e+01, 5.100000000000001199e-01
9.400000000000000000e+01, 4.850000000000000977e-01
9.500000000000000000e+01, 5.400000000000001465e-01
9.600000000000000000e+01, 6.900000000000001688e-01
9.700000000000000000e+01, 7.500000000000001110e-01
9.800000000000000000e+01, 7.300000000000000933e-01
9.900000000000000000e+01, 7.675000000000000711e-01
1.000000000000000000e+02, 7.700000000000001288e-01
1.010000000000000000e+02, 7.700000000000001288e-01
1.020000000000000000e+02, 7.700000000000001288e-01
1.030000000000000000e+02, 7.700000000000001288e-01
1.040000000000000000e+02, 7.700000000000001288e-01
1.050000000000000000e+02, 7.700000000000001288e-01
1.060000000000000000e+02, 7.700000000000001288e-01
1.070000000000000000e+02, 7.800000000000001377e-01
1.080000000000000000e+02, 7.700000000000001288e-01
1.090000000000000000e+02, 7.475000000000000533e-01
1.100000000000000000e+02, 7.200000000000000844e-01
1.110000000000000000e+02, 6.700000000000001510e-01
1.120000000000000000e+02, 7.475000000000000533e-01
1.130000000000000000e+02, 7.100000000000000755e-01
1.140000000000000000e+02, 7.250000000000000888e-01
1.150000000000000000e+02, 7.650000000000001243e-01
1.160000000000000000e+02, 7.275000000000000355e-01
1.170000000000000000e+02, 7.175000000000000266e-01
1.180000000000000000e+02, 7.100000000000000755e-01
1.190000000000000000e+02, 7.300000000000000933e-01
1.200000000000000000e+02, 7.150000000000000799e-01
1.210000000000000000e+02, 7.000000000000000666e-01
1.220000000000000000e+02, 6.725000000000000977e-01
1.230000000000000000e+02, 6.675000000000002043e-01
1.240000000000000000e+02, 7.725000000000001865e-01
1.250000000000000000e+02, 8.775000000000001688e-01
1.260000000000000000e+02, 9.600000000000000755e-01
1.270000000000000000e+02, 1.017500000000000071e+00
1.280000000000000000e+02, 1.020000000000000018e+00
1.290000000000000000e+02, 1.030000000000000027e+00
1.300000000000000000e+02, 1.050000000000000044e+00
1.310000000000000000e+02, 1.050000000000000044e+00
1.320000000000000000e+02, 1.050000000000000044e+00
1.330000000000000000e+02, 1.050000000000000044e+00
1.340000000000000000e+02, 1.040000000000000036e+00
1.350000000000000000e+02, 1.050000000000000044e+00
1.360000000000000000e+02, 1.050000000000000044e+00
1.370000000000000000e+02, 1.050000000000000044e+00
1.380000000000000000e+02, 1.047500000000000098e+00
1.390000000000000000e+02, 9.900000000000001021e-01
1.400000000000000000e+02, 9.250000000000001554e-01
1.410000000000000000e+02, 1.035000000000000142e+00
1.420000000000000000e+02, 1.010000000000000231e+00
1.430000000000000000e+02, 1.027500000000000080e+00
1.440000000000000000e+02, 1.017500000000000071e+00
1.450000000000000000e+02, 1.027500000000000080e+00
1.460000000000000000e+02, 1.090000000000000080e+00
1.470000000000000000e+02, 1.087500000000000133e+00
1.480000000000000000e+02, 1.107500000000000151e+00
1.490000000000000000e+02, 1.100000000000000089e+00
1.500000000000000000e+02, 1.127500000000000169e+00
1.510000000000000000e+02, 1.090000000000000080e+00
1.520000000000000000e+02, 1.095000000000000195e+00
1.530000000000000000e+02, 1.100000000000000089e+00
1.540000000000000000e+02, 1.110000000000000098e+00
1.550000000000000000e+02, 1.150000000000000133e+00
1.560000000000000000e+02, 1.187500000000000222e+00
1.570000000000000000e+02, 1.207500000000000240e+00
1.580000000000000000e+02, 1.220000000000000195e+00
1.590000000000000000e+02, 1.220000000000000195e+00
1.600000000000000000e+02, 1.240000000000000213e+00
1.610000000000000000e+02, 1.250000000000000222e+00
1.620000000000000000e+02, 1.237500000000000266e+00
1.630000000000000000e+02, 1.240000000000000213e+00
1.640000000000000000e+02, 1.240000000000000213e+00
1.650000000000000000e+02, 1.230000000000000204e+00
1.660000000000000000e+02, 1.210000000000000187e+00
1.670000000000000000e+02, 1.210000000000000187e+00
1.680000000000000000e+02, 1.207500000000000240e+00
1.690000000000000000e+02, 1.237500000000000266e+00
1.700000000000000000e+02, 1.297500000000000098e+00
1.710000000000000000e+02, 1.400000000000000133e+00
1.720000000000000000e+02, 1.437500000000000222e+00
1.730000000000000000e+02, 1.477500000000000258e+00
1.740000000000000000e+02, 1.500000000000000222e+00
1.750000000000000000e+02, 1.480000000000000204e+00
1.760000000000000000e+02, 1.510000000000000231e+00
1.770000000000000000e+02, 1.510000000000000231e+00
1.780000000000000000e+02, 1.510000000000000231e+00
1.790000000000000000e+02, 1.510000000000000231e+00
1.800000000000000000e+02, 1.510000000000000231e+00
1.810000000000000000e+02, 1.520000000000000240e+00
1.820000000000000000e+02, 1.497500000000000275e+00
1.830000000000000000e+02, 1.510000000000000231e+00
1.840000000000000000e+02, 1.500000000000000222e+00
1.850000000000000000e+02, 1.457500000000000240e+00
1.860000000000000000e+02, 1.502500000000000169e+00
1.870000000000000000e+02, 1.502500000000000169e+00
1.880000000000000000e+02, 1.507500000000000284e+00
1.890000000000000000e+02, 1.527500000000000080e+00
1.900000000000000000e+02, 1.550000000000000044e+00
1.910000000000000000e+02, 1.540000000000000036e+00
1.920000000000000000e+02, 1.557500000000000107e+00
1.930000000000000000e+02, 1.590000000000000080e+00
1.940000000000000000e+02, 1.555000000000000160e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationupper, color=backGray, line width=1.5pt, draw opacity=0.1, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 1.700000000000000955e-01
1.100000000000000000e+01, 1.325000000000001177e-01
1.200000000000000000e+01, 1.325000000000001177e-01
1.300000000000000000e+01, 1.300000000000001155e-01
1.400000000000000000e+01, 1.500000000000001055e-01
1.500000000000000000e+01, 1.625000000000001166e-01
1.600000000000000000e+01, 2.125000000000001055e-01
1.700000000000000000e+01, 2.075000000000001288e-01
1.800000000000000000e+01, 2.125000000000001055e-01
1.900000000000000000e+01, 2.225000000000001144e-01
2.000000000000000000e+01, 2.125000000000001055e-01
2.100000000000000000e+01, 1.000000000000001027e-01
2.200000000000000000e+01, 6.000000000000010880e-02
2.300000000000000000e+01, 6.000000000000010880e-02
2.400000000000000000e+01, 7.000000000000010381e-02
2.500000000000000000e+01, 6.250000000000011102e-02
2.600000000000000000e+01, 6.250000000000011102e-02
2.700000000000000000e+01, 7.000000000000010381e-02
2.800000000000000000e+01, 7.000000000000010381e-02
2.900000000000000000e+01, 7.000000000000010381e-02
3.000000000000000000e+01, 7.000000000000010381e-02
3.100000000000000000e+01, 7.000000000000010381e-02
3.200000000000000000e+01, 8.000000000000009881e-02
3.300000000000000000e+01, 9.250000000000010991e-02
3.400000000000000000e+01, 1.975000000000001199e-01
3.500000000000000000e+01, 3.225000000000001199e-01
3.600000000000000000e+01, 4.000000000000001332e-01
3.700000000000000000e+01, 3.900000000000001243e-01
3.800000000000000000e+01, 4.025000000000001354e-01
3.900000000000000000e+01, 3.850000000000001199e-01
4.000000000000000000e+01, 4.200000000000000955e-01
4.100000000000000000e+01, 4.150000000000000910e-01
4.200000000000000000e+01, 4.300000000000001044e-01
4.300000000000000000e+01, 4.500000000000001221e-01
4.400000000000000000e+01, 4.625000000000001332e-01
4.500000000000000000e+01, 4.725000000000001421e-01
4.600000000000000000e+01, 4.625000000000001332e-01
4.700000000000000000e+01, 4.500000000000001221e-01
4.800000000000000000e+01, 4.525000000000001243e-01
4.900000000000000000e+01, 4.725000000000001421e-01
5.000000000000000000e+01, 4.500000000000001221e-01
5.100000000000000000e+01, 3.600000000000000977e-01
5.200000000000000000e+01, 3.800000000000001155e-01
5.300000000000000000e+01, 3.400000000000001354e-01
5.400000000000000000e+01, 3.500000000000000888e-01
5.500000000000000000e+01, 3.500000000000000888e-01
5.600000000000000000e+01, 3.500000000000000888e-01
5.700000000000000000e+01, 3.500000000000000888e-01
5.800000000000000000e+01, 3.500000000000000888e-01
5.900000000000000000e+01, 3.500000000000000888e-01
6.000000000000000000e+01, 3.500000000000000888e-01
6.100000000000000000e+01, 3.525000000000000910e-01
6.200000000000000000e+01, 3.725000000000001088e-01
6.300000000000000000e+01, 4.000000000000001332e-01
6.400000000000000000e+01, 5.800000000000000711e-01
6.500000000000000000e+01, 7.025000000000001243e-01
6.600000000000000000e+01, 7.625000000000001776e-01
6.700000000000000000e+01, 7.200000000000000844e-01
6.800000000000000000e+01, 6.925000000000001155e-01
6.900000000000000000e+01, 6.600000000000001421e-01
7.000000000000000000e+01, 6.625000000000000888e-01
7.100000000000000000e+01, 6.625000000000000888e-01
7.200000000000000000e+01, 6.325000000000000622e-01
7.300000000000000000e+01, 6.400000000000001243e-01
7.400000000000000000e+01, 6.500000000000001332e-01
7.500000000000000000e+01, 6.625000000000000888e-01
7.600000000000000000e+01, 7.000000000000000666e-01
7.700000000000000000e+01, 7.075000000000000178e-01
7.800000000000000000e+01, 7.400000000000001021e-01
7.900000000000000000e+01, 7.300000000000000933e-01
8.000000000000000000e+01, 7.475000000000000533e-01
8.100000000000000000e+01, 7.500000000000001110e-01
8.200000000000000000e+01, 7.425000000000001599e-01
8.300000000000000000e+01, 7.800000000000001377e-01
8.400000000000000000e+01, 7.525000000000001688e-01
8.500000000000000000e+01, 7.400000000000001021e-01
8.600000000000000000e+01, 7.400000000000001021e-01
8.700000000000000000e+01, 7.500000000000001110e-01
8.800000000000000000e+01, 7.625000000000001776e-01
8.900000000000000000e+01, 7.800000000000001377e-01
9.000000000000000000e+01, 8.500000000000000888e-01
9.100000000000000000e+01, 8.800000000000001155e-01
9.200000000000000000e+01, 8.925000000000000711e-01
9.300000000000000000e+01, 9.225000000000000977e-01
9.400000000000000000e+01, 1.002500000000000169e+00
9.500000000000000000e+01, 1.090000000000000080e+00
9.600000000000000000e+01, 9.325000000000001066e-01
9.700000000000000000e+01, 8.400000000000000799e-01
9.800000000000000000e+01, 8.100000000000001643e-01
9.900000000000000000e+01, 8.325000000000000178e-01
1.000000000000000000e+02, 8.300000000000000711e-01
1.010000000000000000e+02, 8.325000000000000178e-01
1.020000000000000000e+02, 8.300000000000000711e-01
1.030000000000000000e+02, 8.300000000000000711e-01
1.040000000000000000e+02, 8.300000000000000711e-01
1.050000000000000000e+02, 8.325000000000000178e-01
1.060000000000000000e+02, 8.400000000000000799e-01
1.070000000000000000e+02, 8.600000000000000977e-01
1.080000000000000000e+02, 8.425000000000000266e-01
1.090000000000000000e+02, 9.000000000000001332e-01
1.100000000000000000e+02, 1.282499999999999973e+00
1.110000000000000000e+02, 1.267500000000000071e+00
1.120000000000000000e+02, 1.180000000000000160e+00
1.130000000000000000e+02, 1.150000000000000133e+00
1.140000000000000000e+02, 1.160000000000000142e+00
1.150000000000000000e+02, 1.140000000000000124e+00
1.160000000000000000e+02, 1.142500000000000071e+00
1.170000000000000000e+02, 1.120000000000000107e+00
1.180000000000000000e+02, 1.092500000000000027e+00
1.190000000000000000e+02, 1.102500000000000036e+00
1.200000000000000000e+02, 1.130000000000000115e+00
1.210000000000000000e+02, 1.170000000000000151e+00
1.220000000000000000e+02, 1.170000000000000151e+00
1.230000000000000000e+02, 1.162500000000000089e+00
1.240000000000000000e+02, 1.220000000000000195e+00
1.250000000000000000e+02, 1.302499999999999991e+00
1.260000000000000000e+02, 1.182500000000000107e+00
1.270000000000000000e+02, 1.112500000000000044e+00
1.280000000000000000e+02, 1.090000000000000080e+00
1.290000000000000000e+02, 1.100000000000000089e+00
1.300000000000000000e+02, 1.100000000000000089e+00
1.310000000000000000e+02, 1.100000000000000089e+00
1.320000000000000000e+02, 1.110000000000000098e+00
1.330000000000000000e+02, 1.110000000000000098e+00
1.340000000000000000e+02, 1.110000000000000098e+00
1.350000000000000000e+02, 1.110000000000000098e+00
1.360000000000000000e+02, 1.110000000000000098e+00
1.370000000000000000e+02, 1.122500000000000053e+00
1.380000000000000000e+02, 1.150000000000000133e+00
1.390000000000000000e+02, 1.347500000000000142e+00
1.400000000000000000e+02, 1.772500000000000187e+00
1.410000000000000000e+02, 1.564999999999999947e+00
1.420000000000000000e+02, 1.460000000000000187e+00
1.430000000000000000e+02, 1.400000000000000133e+00
1.440000000000000000e+02, 1.392500000000000071e+00
1.450000000000000000e+02, 1.392500000000000071e+00
1.460000000000000000e+02, 1.340000000000000080e+00
1.470000000000000000e+02, 1.342500000000000027e+00
1.480000000000000000e+02, 1.362500000000000044e+00
1.490000000000000000e+02, 1.380000000000000115e+00
1.500000000000000000e+02, 1.382500000000000062e+00
1.510000000000000000e+02, 1.410000000000000142e+00
1.520000000000000000e+02, 1.422500000000000098e+00
1.530000000000000000e+02, 1.420000000000000151e+00
1.540000000000000000e+02, 1.460000000000000187e+00
1.550000000000000000e+02, 1.472500000000000142e+00
1.560000000000000000e+02, 1.500000000000000222e+00
1.570000000000000000e+02, 1.490000000000000213e+00
1.580000000000000000e+02, 1.470000000000000195e+00
1.590000000000000000e+02, 1.502500000000000169e+00
1.600000000000000000e+02, 1.500000000000000222e+00
1.610000000000000000e+02, 1.472500000000000142e+00
1.620000000000000000e+02, 1.500000000000000222e+00
1.630000000000000000e+02, 1.512500000000000178e+00
1.640000000000000000e+02, 1.512500000000000178e+00
1.650000000000000000e+02, 1.552499999999999991e+00
1.660000000000000000e+02, 1.604999999999999982e+00
1.670000000000000000e+02, 1.632500000000000062e+00
1.680000000000000000e+02, 1.592500000000000027e+00
1.690000000000000000e+02, 1.750000000000000222e+00
1.700000000000000000e+02, 1.957500000000000240e+00
1.710000000000000000e+02, 1.860000000000000098e+00
1.720000000000000000e+02, 1.662500000000000089e+00
1.730000000000000000e+02, 1.552499999999999991e+00
1.740000000000000000e+02, 1.582500000000000018e+00
1.750000000000000000e+02, 1.550000000000000044e+00
1.760000000000000000e+02, 1.570000000000000062e+00
1.770000000000000000e+02, 1.570000000000000062e+00
1.780000000000000000e+02, 1.570000000000000062e+00
1.790000000000000000e+02, 1.570000000000000062e+00
1.800000000000000000e+02, 1.580000000000000071e+00
1.810000000000000000e+02, 1.590000000000000080e+00
1.820000000000000000e+02, 1.600000000000000089e+00
1.830000000000000000e+02, 1.620000000000000107e+00
1.840000000000000000e+02, 1.680000000000000160e+00
1.850000000000000000e+02, 1.982500000000000151e+00
1.860000000000000000e+02, 2.012500000000000178e+00
1.870000000000000000e+02, 1.955000000000000071e+00
1.880000000000000000e+02, 1.922500000000000098e+00
1.890000000000000000e+02, 1.942500000000000115e+00
1.900000000000000000e+02, 1.942500000000000115e+00
1.910000000000000000e+02, 1.912500000000000089e+00
1.920000000000000000e+02, 1.892500000000000071e+00
1.930000000000000000e+02, 1.872500000000000053e+00
1.940000000000000000e+02, 1.890000000000000124e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=estimationmedian, color=estimationColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 2.000000000000010450e-02
1.100000000000000000e+01, -9.999999999999896125e-03
1.200000000000000000e+01, -1.499999999999989536e-02
1.300000000000000000e+01, -1.999999999999989633e-02
1.400000000000000000e+01, 2.000000000000010450e-02
1.500000000000000000e+01, 1.040834085586084257e-16
1.600000000000000000e+01, -1.499999999999989536e-02
1.700000000000000000e+01, 5.000000000000104187e-03
1.800000000000000000e+01, -2.499999999999989730e-02
1.900000000000000000e+01, -5.999999999999990064e-02
2.000000000000000000e+01, 1.040834085586084257e-16
2.100000000000000000e+01, 3.000000000000010297e-02
2.200000000000000000e+01, 3.000000000000010297e-02
2.300000000000000000e+01, 3.000000000000010297e-02
2.400000000000000000e+01, 3.000000000000010297e-02
2.500000000000000000e+01, 3.500000000000010048e-02
2.600000000000000000e+01, 3.500000000000010048e-02
2.700000000000000000e+01, 4.000000000000010492e-02
2.800000000000000000e+01, 4.000000000000010492e-02
2.900000000000000000e+01, 4.000000000000010492e-02
3.000000000000000000e+01, 4.000000000000010492e-02
3.100000000000000000e+01, 4.000000000000010492e-02
3.200000000000000000e+01, 4.000000000000010492e-02
3.300000000000000000e+01, 5.000000000000010686e-02
3.400000000000000000e+01, 8.000000000000009881e-02
3.500000000000000000e+01, 1.350000000000001199e-01
3.600000000000000000e+01, 1.800000000000001044e-01
3.700000000000000000e+01, 1.750000000000000999e-01
3.800000000000000000e+01, 1.850000000000001088e-01
3.900000000000000000e+01, 2.200000000000001121e-01
4.000000000000000000e+01, 2.100000000000001033e-01
4.100000000000000000e+01, 2.300000000000001210e-01
4.200000000000000000e+01, 2.500000000000001110e-01
4.300000000000000000e+01, 2.400000000000001021e-01
4.400000000000000000e+01, 2.500000000000001110e-01
4.500000000000000000e+01, 2.850000000000001421e-01
4.600000000000000000e+01, 2.950000000000000955e-01
4.700000000000000000e+01, 2.500000000000001110e-01
4.800000000000000000e+01, 2.200000000000001121e-01
4.900000000000000000e+01, 2.600000000000001199e-01
5.000000000000000000e+01, 3.000000000000000999e-01
5.100000000000000000e+01, 2.950000000000000955e-01
5.200000000000000000e+01, 3.350000000000001310e-01
5.300000000000000000e+01, 2.900000000000000910e-01
5.400000000000000000e+01, 3.200000000000001177e-01
5.500000000000000000e+01, 3.200000000000001177e-01
5.600000000000000000e+01, 3.200000000000001177e-01
5.700000000000000000e+01, 3.200000000000001177e-01
5.800000000000000000e+01, 3.200000000000001177e-01
5.900000000000000000e+01, 3.250000000000001221e-01
6.000000000000000000e+01, 3.200000000000001177e-01
6.100000000000000000e+01, 3.300000000000001266e-01
6.200000000000000000e+01, 3.300000000000001266e-01
6.300000000000000000e+01, 3.500000000000000888e-01
6.400000000000000000e+01, 3.550000000000000933e-01
6.500000000000000000e+01, 4.350000000000001088e-01
6.600000000000000000e+01, 5.000000000000001110e-01
6.700000000000000000e+01, 4.700000000000001399e-01
6.800000000000000000e+01, 4.650000000000001354e-01
6.900000000000000000e+01, 4.650000000000001354e-01
7.000000000000000000e+01, 4.600000000000001310e-01
7.100000000000000000e+01, 4.600000000000001310e-01
7.200000000000000000e+01, 5.000000000000001110e-01
7.300000000000000000e+01, 5.050000000000001155e-01
7.400000000000000000e+01, 5.050000000000001155e-01
7.500000000000000000e+01, 5.200000000000001288e-01
7.600000000000000000e+01, 5.250000000000001332e-01
7.700000000000000000e+01, 5.000000000000001110e-01
7.800000000000000000e+01, 5.650000000000001688e-01
7.900000000000000000e+01, 5.350000000000001421e-01
8.000000000000000000e+01, 5.850000000000000755e-01
8.100000000000000000e+01, 6.000000000000000888e-01
8.200000000000000000e+01, 6.000000000000000888e-01
8.300000000000000000e+01, 6.100000000000000977e-01
8.400000000000000000e+01, 6.200000000000001066e-01
8.500000000000000000e+01, 6.300000000000001155e-01
8.600000000000000000e+01, 6.500000000000001332e-01
8.700000000000000000e+01, 6.400000000000001243e-01
8.800000000000000000e+01, 6.350000000000001199e-01
8.900000000000000000e+01, 6.300000000000001155e-01
9.000000000000000000e+01, 6.700000000000001510e-01
9.100000000000000000e+01, 6.750000000000001554e-01
9.200000000000000000e+01, 6.800000000000001599e-01
9.300000000000000000e+01, 6.800000000000001599e-01
9.400000000000000000e+01, 7.850000000000001421e-01
9.500000000000000000e+01, 7.900000000000001465e-01
9.600000000000000000e+01, 7.850000000000001421e-01
9.700000000000000000e+01, 7.900000000000001465e-01
9.800000000000000000e+01, 7.750000000000001332e-01
9.900000000000000000e+01, 8.000000000000001554e-01
1.000000000000000000e+02, 8.000000000000001554e-01
1.010000000000000000e+02, 8.050000000000001599e-01
1.020000000000000000e+02, 8.050000000000001599e-01
1.030000000000000000e+02, 8.050000000000001599e-01
1.040000000000000000e+02, 8.100000000000001643e-01
1.050000000000000000e+02, 8.100000000000001643e-01
1.060000000000000000e+02, 8.100000000000001643e-01
1.070000000000000000e+02, 8.300000000000000711e-01
1.080000000000000000e+02, 8.150000000000001688e-01
1.090000000000000000e+02, 8.200000000000001732e-01
1.100000000000000000e+02, 9.300000000000001599e-01
1.110000000000000000e+02, 1.010000000000000231e+00
1.120000000000000000e+02, 9.500000000000001776e-01
1.130000000000000000e+02, 9.250000000000001554e-01
1.140000000000000000e+02, 9.500000000000001776e-01
1.150000000000000000e+02, 9.250000000000001554e-01
1.160000000000000000e+02, 9.350000000000001643e-01
1.170000000000000000e+02, 9.550000000000000711e-01
1.180000000000000000e+02, 9.400000000000001688e-01
1.190000000000000000e+02, 9.600000000000000755e-01
1.200000000000000000e+02, 9.650000000000000799e-01
1.210000000000000000e+02, 9.750000000000000888e-01
1.220000000000000000e+02, 9.650000000000000799e-01
1.230000000000000000e+02, 9.450000000000001732e-01
1.240000000000000000e+02, 1.000000000000000222e+00
1.250000000000000000e+02, 1.055000000000000160e+00
1.260000000000000000e+02, 1.064999999999999947e+00
1.270000000000000000e+02, 1.060000000000000053e+00
1.280000000000000000e+02, 1.060000000000000053e+00
1.290000000000000000e+02, 1.060000000000000053e+00
1.300000000000000000e+02, 1.070000000000000062e+00
1.310000000000000000e+02, 1.070000000000000062e+00
1.320000000000000000e+02, 1.070000000000000062e+00
1.330000000000000000e+02, 1.070000000000000062e+00
1.340000000000000000e+02, 1.070000000000000062e+00
1.350000000000000000e+02, 1.070000000000000062e+00
1.360000000000000000e+02, 1.070000000000000062e+00
1.370000000000000000e+02, 1.080000000000000071e+00
1.380000000000000000e+02, 1.080000000000000071e+00
1.390000000000000000e+02, 1.104999999999999982e+00
1.400000000000000000e+02, 1.294999999999999929e+00
1.410000000000000000e+02, 1.280000000000000249e+00
1.420000000000000000e+02, 1.205000000000000071e+00
1.430000000000000000e+02, 1.185000000000000053e+00
1.440000000000000000e+02, 1.175000000000000266e+00
1.450000000000000000e+02, 1.190000000000000169e+00
1.460000000000000000e+02, 1.215000000000000302e+00
1.470000000000000000e+02, 1.250000000000000222e+00
1.480000000000000000e+02, 1.230000000000000204e+00
1.490000000000000000e+02, 1.235000000000000320e+00
1.500000000000000000e+02, 1.250000000000000222e+00
1.510000000000000000e+02, 1.255000000000000338e+00
1.520000000000000000e+02, 1.260000000000000231e+00
1.530000000000000000e+02, 1.280000000000000027e+00
1.540000000000000000e+02, 1.290000000000000036e+00
1.550000000000000000e+02, 1.314999999999999947e+00
1.560000000000000000e+02, 1.320000000000000062e+00
1.570000000000000000e+02, 1.345000000000000195e+00
1.580000000000000000e+02, 1.350000000000000089e+00
1.590000000000000000e+02, 1.340000000000000080e+00
1.600000000000000000e+02, 1.370000000000000107e+00
1.610000000000000000e+02, 1.360000000000000098e+00
1.620000000000000000e+02, 1.390000000000000124e+00
1.630000000000000000e+02, 1.375000000000000000e+00
1.640000000000000000e+02, 1.360000000000000098e+00
1.650000000000000000e+02, 1.370000000000000107e+00
1.660000000000000000e+02, 1.410000000000000142e+00
1.670000000000000000e+02, 1.400000000000000133e+00
1.680000000000000000e+02, 1.420000000000000151e+00
1.690000000000000000e+02, 1.470000000000000195e+00
1.700000000000000000e+02, 1.610000000000000098e+00
1.710000000000000000e+02, 1.615000000000000213e+00
1.720000000000000000e+02, 1.564999999999999947e+00
1.730000000000000000e+02, 1.520000000000000240e+00
1.740000000000000000e+02, 1.560000000000000053e+00
1.750000000000000000e+02, 1.520000000000000240e+00
1.760000000000000000e+02, 1.540000000000000036e+00
1.770000000000000000e+02, 1.540000000000000036e+00
1.780000000000000000e+02, 1.540000000000000036e+00
1.790000000000000000e+02, 1.544999999999999929e+00
1.800000000000000000e+02, 1.550000000000000044e+00
1.810000000000000000e+02, 1.550000000000000044e+00
1.820000000000000000e+02, 1.544999999999999929e+00
1.830000000000000000e+02, 1.564999999999999947e+00
1.840000000000000000e+02, 1.564999999999999947e+00
1.850000000000000000e+02, 1.705000000000000071e+00
1.860000000000000000e+02, 1.705000000000000071e+00
1.870000000000000000e+02, 1.720000000000000195e+00
1.880000000000000000e+02, 1.725000000000000089e+00
1.890000000000000000e+02, 1.745000000000000107e+00
1.900000000000000000e+02, 1.735000000000000320e+00
1.910000000000000000e+02, 1.775000000000000355e+00
1.920000000000000000e+02, 1.775000000000000355e+00
1.930000000000000000e+02, 1.715000000000000302e+00
1.940000000000000000e+02, 1.710000000000000187e+00
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addlegendentry{estimation}

\addplot [backGray, fill opacity=0.3, forget plot] fill between[of=estimationlower and estimationupper];

\addplot [name path=ground-truth, color=ground-truthColor, line width=1.5pt]
	table[col sep=comma]{%
0.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+00, 0.000000000000000000e+00
2.000000000000000000e+00, 0.000000000000000000e+00
3.000000000000000000e+00, 0.000000000000000000e+00
4.000000000000000000e+00, 0.000000000000000000e+00
5.000000000000000000e+00, 0.000000000000000000e+00
6.000000000000000000e+00, 0.000000000000000000e+00
7.000000000000000000e+00, 0.000000000000000000e+00
8.000000000000000000e+00, 0.000000000000000000e+00
9.000000000000000000e+00, 0.000000000000000000e+00
1.000000000000000000e+01, 0.000000000000000000e+00
1.100000000000000000e+01, 0.000000000000000000e+00
1.200000000000000000e+01, 0.000000000000000000e+00
1.300000000000000000e+01, 0.000000000000000000e+00
1.400000000000000000e+01, 0.000000000000000000e+00
1.500000000000000000e+01, 0.000000000000000000e+00
1.600000000000000000e+01, 0.000000000000000000e+00
1.700000000000000000e+01, 0.000000000000000000e+00
1.800000000000000000e+01, 0.000000000000000000e+00
1.900000000000000000e+01, 0.000000000000000000e+00
2.000000000000000000e+01, 0.000000000000000000e+00
2.100000000000000000e+01, 1.000000000000000021e-02
2.200000000000000000e+01, 2.000000000000000042e-02
2.300000000000000000e+01, 2.999999999999999889e-02
2.400000000000000000e+01, 4.000000000000000083e-02
2.500000000000000000e+01, 5.000000000000000278e-02
2.600000000000000000e+01, 5.999999999999999778e-02
2.700000000000000000e+01, 7.000000000000000666e-02
2.800000000000000000e+01, 8.000000000000000167e-02
2.900000000000000000e+01, 8.999999999999999667e-02
3.000000000000000000e+01, 1.000000000000000056e-01
3.100000000000000000e+01, 1.100000000000000006e-01
3.200000000000000000e+01, 1.199999999999999956e-01
3.300000000000000000e+01, 1.300000000000000044e-01
3.400000000000000000e+01, 1.400000000000000133e-01
3.500000000000000000e+01, 1.499999999999999944e-01
3.600000000000000000e+01, 1.600000000000000033e-01
3.700000000000000000e+01, 1.700000000000000122e-01
3.800000000000000000e+01, 1.799999999999999933e-01
3.900000000000000000e+01, 1.900000000000000022e-01
4.000000000000000000e+01, 2.000000000000000111e-01
4.100000000000000000e+01, 2.099999999999999922e-01
4.200000000000000000e+01, 2.200000000000000011e-01
4.300000000000000000e+01, 2.300000000000000100e-01
4.400000000000000000e+01, 2.399999999999999911e-01
4.500000000000000000e+01, 2.500000000000000000e-01
4.600000000000000000e+01, 2.600000000000000089e-01
4.700000000000000000e+01, 2.700000000000000178e-01
4.800000000000000000e+01, 2.800000000000000266e-01
4.900000000000000000e+01, 2.899999999999999800e-01
5.000000000000000000e+01, 2.999999999999999889e-01
5.100000000000000000e+01, 3.099999999999999978e-01
5.200000000000000000e+01, 3.200000000000000067e-01
5.300000000000000000e+01, 3.300000000000000155e-01
5.400000000000000000e+01, 3.400000000000000244e-01
5.500000000000000000e+01, 3.499999999999999778e-01
5.600000000000000000e+01, 3.599999999999999867e-01
5.700000000000000000e+01, 3.699999999999999956e-01
5.800000000000000000e+01, 3.800000000000000044e-01
5.900000000000000000e+01, 3.900000000000000133e-01
6.000000000000000000e+01, 4.000000000000000222e-01
6.100000000000000000e+01, 4.099999999999999756e-01
6.200000000000000000e+01, 4.199999999999999845e-01
6.300000000000000000e+01, 4.299999999999999933e-01
6.400000000000000000e+01, 4.400000000000000022e-01
6.500000000000000000e+01, 4.500000000000000111e-01
6.600000000000000000e+01, 4.600000000000000200e-01
6.700000000000000000e+01, 4.699999999999999734e-01
6.800000000000000000e+01, 4.799999999999999822e-01
6.900000000000000000e+01, 4.899999999999999911e-01
7.000000000000000000e+01, 5.000000000000000000e-01
7.100000000000000000e+01, 5.100000000000000089e-01
7.200000000000000000e+01, 5.200000000000000178e-01
7.300000000000000000e+01, 5.300000000000000266e-01
7.400000000000000000e+01, 5.400000000000000355e-01
7.500000000000000000e+01, 5.500000000000000444e-01
7.600000000000000000e+01, 5.600000000000000533e-01
7.700000000000000000e+01, 5.699999999999999512e-01
7.800000000000000000e+01, 5.799999999999999600e-01
7.900000000000000000e+01, 5.899999999999999689e-01
8.000000000000000000e+01, 5.999999999999999778e-01
8.100000000000000000e+01, 6.099999999999999867e-01
8.200000000000000000e+01, 6.199999999999999956e-01
8.300000000000000000e+01, 6.300000000000000044e-01
8.400000000000000000e+01, 6.400000000000000133e-01
8.500000000000000000e+01, 6.500000000000000222e-01
8.600000000000000000e+01, 6.600000000000000311e-01
8.700000000000000000e+01, 6.700000000000000400e-01
8.800000000000000000e+01, 6.800000000000000488e-01
8.900000000000000000e+01, 6.899999999999999467e-01
9.000000000000000000e+01, 6.999999999999999556e-01
9.100000000000000000e+01, 7.099999999999999645e-01
9.200000000000000000e+01, 7.199999999999999734e-01
9.300000000000000000e+01, 7.299999999999999822e-01
9.400000000000000000e+01, 7.399999999999999911e-01
9.500000000000000000e+01, 7.500000000000000000e-01
9.600000000000000000e+01, 7.600000000000000089e-01
9.700000000000000000e+01, 7.700000000000000178e-01
9.800000000000000000e+01, 7.800000000000000266e-01
9.900000000000000000e+01, 7.900000000000000355e-01
1.000000000000000000e+02, 8.000000000000000444e-01
1.010000000000000000e+02, 8.100000000000000533e-01
1.020000000000000000e+02, 8.199999999999999512e-01
1.030000000000000000e+02, 8.299999999999999600e-01
1.040000000000000000e+02, 8.399999999999999689e-01
1.050000000000000000e+02, 8.499999999999999778e-01
1.060000000000000000e+02, 8.599999999999999867e-01
1.070000000000000000e+02, 8.699999999999999956e-01
1.080000000000000000e+02, 8.800000000000000044e-01
1.090000000000000000e+02, 8.900000000000000133e-01
1.100000000000000000e+02, 9.000000000000000222e-01
1.110000000000000000e+02, 9.100000000000000311e-01
1.120000000000000000e+02, 9.200000000000000400e-01
1.130000000000000000e+02, 9.300000000000000488e-01
1.140000000000000000e+02, 9.399999999999999467e-01
1.150000000000000000e+02, 9.499999999999999556e-01
1.160000000000000000e+02, 9.599999999999999645e-01
1.170000000000000000e+02, 9.699999999999999734e-01
1.180000000000000000e+02, 9.799999999999999822e-01
1.190000000000000000e+02, 9.899999999999999911e-01
1.200000000000000000e+02, 1.000000000000000000e+00
1.210000000000000000e+02, 1.010000000000000009e+00
1.220000000000000000e+02, 1.020000000000000018e+00
1.230000000000000000e+02, 1.030000000000000027e+00
1.240000000000000000e+02, 1.040000000000000036e+00
1.250000000000000000e+02, 1.050000000000000044e+00
1.260000000000000000e+02, 1.060000000000000053e+00
1.270000000000000000e+02, 1.070000000000000062e+00
1.280000000000000000e+02, 1.080000000000000071e+00
1.290000000000000000e+02, 1.090000000000000080e+00
1.300000000000000000e+02, 1.100000000000000089e+00
1.310000000000000000e+02, 1.110000000000000098e+00
1.320000000000000000e+02, 1.120000000000000107e+00
1.330000000000000000e+02, 1.129999999999999893e+00
1.340000000000000000e+02, 1.139999999999999902e+00
1.350000000000000000e+02, 1.149999999999999911e+00
1.360000000000000000e+02, 1.159999999999999920e+00
1.370000000000000000e+02, 1.169999999999999929e+00
1.380000000000000000e+02, 1.179999999999999938e+00
1.390000000000000000e+02, 1.189999999999999947e+00
1.400000000000000000e+02, 1.199999999999999956e+00
1.410000000000000000e+02, 1.209999999999999964e+00
1.420000000000000000e+02, 1.219999999999999973e+00
1.430000000000000000e+02, 1.229999999999999982e+00
1.440000000000000000e+02, 1.239999999999999991e+00
1.450000000000000000e+02, 1.250000000000000000e+00
1.460000000000000000e+02, 1.260000000000000009e+00
1.470000000000000000e+02, 1.270000000000000018e+00
1.480000000000000000e+02, 1.280000000000000027e+00
1.490000000000000000e+02, 1.290000000000000036e+00
1.500000000000000000e+02, 1.300000000000000044e+00
1.510000000000000000e+02, 1.310000000000000053e+00
1.520000000000000000e+02, 1.320000000000000062e+00
1.530000000000000000e+02, 1.330000000000000071e+00
1.540000000000000000e+02, 1.340000000000000080e+00
1.550000000000000000e+02, 1.350000000000000089e+00
1.560000000000000000e+02, 1.360000000000000098e+00
1.570000000000000000e+02, 1.370000000000000107e+00
1.580000000000000000e+02, 1.379999999999999893e+00
1.590000000000000000e+02, 1.389999999999999902e+00
1.600000000000000000e+02, 1.399999999999999911e+00
1.610000000000000000e+02, 1.409999999999999920e+00
1.620000000000000000e+02, 1.419999999999999929e+00
1.630000000000000000e+02, 1.429999999999999938e+00
1.640000000000000000e+02, 1.439999999999999947e+00
1.650000000000000000e+02, 1.449999999999999956e+00
1.660000000000000000e+02, 1.459999999999999964e+00
1.670000000000000000e+02, 1.469999999999999973e+00
1.680000000000000000e+02, 1.479999999999999982e+00
1.690000000000000000e+02, 1.489999999999999991e+00
1.700000000000000000e+02, 1.500000000000000000e+00
1.710000000000000000e+02, 1.510000000000000009e+00
1.720000000000000000e+02, 1.520000000000000018e+00
1.730000000000000000e+02, 1.530000000000000027e+00
1.740000000000000000e+02, 1.540000000000000036e+00
1.750000000000000000e+02, 1.550000000000000044e+00
1.760000000000000000e+02, 1.560000000000000053e+00
1.770000000000000000e+02, 1.570000000000000062e+00
1.780000000000000000e+02, 1.580000000000000071e+00
1.790000000000000000e+02, 1.590000000000000080e+00
1.800000000000000000e+02, 1.600000000000000089e+00
1.810000000000000000e+02, 1.610000000000000098e+00
1.820000000000000000e+02, 1.620000000000000107e+00
1.830000000000000000e+02, 1.629999999999999893e+00
1.840000000000000000e+02, 1.639999999999999902e+00
1.850000000000000000e+02, 1.649999999999999911e+00
1.860000000000000000e+02, 1.659999999999999920e+00
1.870000000000000000e+02, 1.669999999999999929e+00
1.880000000000000000e+02, 1.679999999999999938e+00
1.890000000000000000e+02, 1.689999999999999947e+00
1.900000000000000000e+02, 1.699999999999999956e+00
1.910000000000000000e+02, 1.709999999999999964e+00
1.920000000000000000e+02, 1.719999999999999973e+00
1.930000000000000000e+02, 1.729999999999999982e+00
1.940000000000000000e+02, 1.739999999999999991e+00
};

\addlegendentry{ground-truth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> img/raw/ramp_high_rotation.tex <==
\addplot [name path=sensor-rotation-0, color=sensor-rotation-0Color, line width=1.5pt, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 3.603968319886034777e-02
1.000000000000000000e+00, 6.968005850386729816e-02
2.000000000000000000e+00, 1.006973187716466156e-01
3.000000000000000000e+00, 2.797303863632699672e-01
4.000000000000000000e+00, 3.641014566618053228e-01
5.000000000000000000e+00, 4.749890916918136363e-01
6.000000000000000000e+00, 5.617608542928149706e-01
7.000000000000000000e+00, 6.313103086683544696e-01
8.000000000000000000e+00, 5.200726922512388661e-01
9.000000000000000000e+00, 4.628728552448689304e-01
1.000000000000000000e+01, 3.448337932786055826e-01
1.100000000000000000e+01, 1.525092923341857254e-01
1.200000000000000000e+01, 2.071674448845038929e-01
1.300000000000000000e+01, 1.169639402581168081e-01
1.400000000000000000e+01, 1.008369056198770708e-01
1.500000000000000000e+01, 9.259132321531997334e-02
1.600000000000000000e+01, 9.073109311119861853e-02
1.700000000000000000e+01, 1.388850136763981891e-01
1.800000000000000000e+01, 1.862412327101962972e-01
1.900000000000000000e+01, 2.049173528268569411e-01
2.000000000000000000e+01, 3.621670224881584077e-01
2.100000000000000000e+01, 7.292713389682395908e-01
2.200000000000000000e+01, 1.508520637102003015e+00
2.300000000000000000e+01, 1.182662897742465358e+00
2.400000000000000000e+01, 5.849211248254123641e-01
2.500000000000000000e+01, 2.026093820294030678e-01
2.600000000000000000e+01, 1.694879255701543241e-01
2.700000000000000000e+01, 6.036157755372583561e-02
2.800000000000000000e+01, 1.176183441988401107e-01
2.900000000000000000e+01, 7.335360963640601140e-02
3.000000000000000000e+01, 7.617579472511923355e-02
3.100000000000000000e+01, 1.111969354391711406e-01
3.200000000000000000e+01, 1.790362609400961147e-01
3.300000000000000000e+01, 2.469477979607435092e-01
3.400000000000000000e+01, 2.996378856738441954e-01
3.500000000000000000e+01, 3.247417877983769796e-01
3.600000000000000000e+01, 4.084349347267392516e-01
3.700000000000000000e+01, 5.103758162028028122e-01
3.800000000000000000e+01, 5.409171520025302105e-01
3.900000000000000000e+01, 4.061961998251444883e-01
4.000000000000000000e+01, 2.497715797099263058e-01
4.100000000000000000e+01, 2.943235177222511822e-01
4.200000000000000000e+01, 1.851798142246881274e-01
4.300000000000000000e+01, 9.612944120429675610e-02
4.400000000000000000e+01, 8.331710031796013549e-02
4.500000000000000000e+01, 6.763872433659331995e-02
4.600000000000000000e+01, 8.000306765715967106e-02
4.700000000000000000e+01, 1.022718122804931185e-01
4.800000000000000000e+01, 1.134555902374125846e-01
4.900000000000000000e+01, 2.202730641747351337e-01
5.000000000000000000e+01, 3.571360725209722364e-01
5.100000000000000000e+01, 9.230928147648486126e-01
5.200000000000000000e+01, 1.581130304213752558e+00
5.300000000000000000e+01, 1.067481732261403637e+00
5.400000000000000000e+01, 4.574820494544787342e-01
5.500000000000000000e+01, 2.299925167446194574e-01
5.600000000000000000e+01, 1.086160526017978523e-01
5.700000000000000000e+01, 1.515195603699596993e-01
5.800000000000000000e+01, 1.537924828490186413e-01
5.900000000000000000e+01, 1.357283644136054179e-01
6.000000000000000000e+01, 9.825663723794504645e-02
6.100000000000000000e+01, 1.430109679758660157e-01
6.200000000000000000e+01, 1.454920261011947435e-01
6.300000000000000000e+01, 1.975469644230705979e-01
6.400000000000000000e+01, 3.468237429549403394e-01
6.500000000000000000e+01, 3.227987233824367030e-01
6.600000000000000000e+01, 4.528849940193764856e-01
6.700000000000000000e+01, 5.927807411558745354e-01
6.800000000000000000e+01, 6.682847652003039984e-01
6.900000000000000000e+01, 5.310888104183214553e-01
7.000000000000000000e+01, 3.846692949345139612e-01
7.100000000000000000e+01, 2.600973440495178979e-01
7.200000000000000000e+01, 2.500495640302564659e-01
7.300000000000000000e+01, 7.790726216765216094e-02
7.400000000000000000e+01, 6.218445585277915244e-02
7.500000000000000000e+01, 8.997497998083300863e-02
7.600000000000000000e+01, 9.797581040701176802e-02
7.700000000000000000e+01, 1.288784772232110520e-01
7.800000000000000000e+01, 2.389676925924916762e-01
7.900000000000000000e+01, 2.781797021824595206e-01
8.000000000000000000e+01, 4.599818219679236986e-01
8.100000000000000000e+01, 5.299940357890980946e-01
8.200000000000000000e+01, 6.269701669315576043e-01
8.300000000000000000e+01, 5.606266905907778542e-01
8.400000000000000000e+01, 4.370201747341995180e-01
8.500000000000000000e+01, 3.206118383040609254e-01
8.600000000000000000e+01, 2.754984542760027799e-01
8.700000000000000000e+01, 1.430329382066507782e-01
8.800000000000000000e+01, 1.304634627657362267e-01
8.900000000000000000e+01, 8.063403375757424718e-02
9.000000000000000000e+01, 1.448601997537598274e-01
9.100000000000000000e+01, 1.045922545762313083e-01
9.200000000000000000e+01, 1.088707708713627237e-01
9.300000000000000000e+01, 7.002534450721786818e-02
9.400000000000000000e+01, 1.940101697992956120e-01
9.500000000000000000e+01, 2.941739190001240178e-01
9.600000000000000000e+01, 5.784347256552954120e-01
9.700000000000000000e+01, 1.316065466331806766e+00
9.800000000000000000e+01, 1.490832560416871067e+00
9.900000000000000000e+01, 8.047123524454907750e-01
1.000000000000000000e+02, 3.119456505226919640e-01
1.010000000000000000e+02, 1.302414858223648608e-01
1.020000000000000000e+02, 1.319759682623836972e-01
1.030000000000000000e+02, 5.435651629302664517e-02
1.040000000000000000e+02, 4.528786799793130258e-02
1.050000000000000000e+02, 3.409047283283697660e-02
1.060000000000000000e+02, 4.513198036409617198e-02
1.070000000000000000e+02, 9.510171929108618416e-02
1.080000000000000000e+02, 1.603512064761200284e-01
1.090000000000000000e+02, 2.936220651505271340e-01
1.100000000000000000e+02, 3.556206161889248762e-01
1.110000000000000000e+02, 4.540224353178858863e-01
1.120000000000000000e+02, 5.410665303316664065e-01
1.130000000000000000e+02, 4.649078637313243667e-01
1.140000000000000000e+02, 3.941438309230588799e-01
1.150000000000000000e+02, 3.557104579575472436e-01
1.160000000000000000e+02, 3.137546633281094177e-01
1.170000000000000000e+02, 1.821154865814181567e-01
1.180000000000000000e+02, 1.598439807090157316e-01
1.190000000000000000e+02, 8.656934168846439070e-02
1.200000000000000000e+02, 2.298965018526853352e-02
1.210000000000000000e+02, 4.130084710879962373e-02
1.220000000000000000e+02, 3.233377022458515382e-02
1.230000000000000000e+02, 1.214161383459033267e-01
1.240000000000000000e+02, 1.146719149040993507e-01
1.250000000000000000e+02, 3.162652376000384957e-01
1.260000000000000000e+02, 6.585476419420245309e-01
1.270000000000000000e+02, 1.469622545388833856e+00
1.280000000000000000e+02, 1.387338045811733256e+00
1.290000000000000000e+02, 6.348771278656917261e-01
1.300000000000000000e+02, 3.029567575949824731e-01
1.310000000000000000e+02, 2.260601060411659424e-01
1.320000000000000000e+02, 1.364345127235446764e-01
1.330000000000000000e+02, 1.004537463586576279e-01
1.340000000000000000e+02, 1.350029740935140554e-01
1.350000000000000000e+02, 1.682760676664696864e-01
1.360000000000000000e+02, 1.454814965386179160e-01
1.370000000000000000e+02, 1.119367342571959967e-01
1.380000000000000000e+02, 1.455911297851635311e-01
1.390000000000000000e+02, 2.210028965782560306e-01
1.400000000000000000e+02, 2.863702399216347949e-01
1.410000000000000000e+02, 4.590093061913201877e-01
1.420000000000000000e+02, 5.254223455261670672e-01
1.430000000000000000e+02, 6.583475314772879727e-01
1.440000000000000000e+02, 6.462529850837192003e-01
1.450000000000000000e+02, 3.616950607287373609e-01
1.460000000000000000e+02, 2.739748116625772001e-01
1.470000000000000000e+02, 2.282937646319331271e-01
1.480000000000000000e+02, 1.175745976112831659e-01
1.490000000000000000e+02, 9.299401120100427021e-02
1.500000000000000000e+02, 6.611059682010955729e-02
1.510000000000000000e+02, 5.352313798971500280e-02
1.520000000000000000e+02, 9.232765167270691464e-02
1.530000000000000000e+02, 1.241198027416724192e-01
1.540000000000000000e+02, 2.433994646932467476e-01
1.550000000000000000e+02, 3.608489860700280216e-01
1.560000000000000000e+02, 5.303111814575496297e-01
1.570000000000000000e+02, 6.467021803446274530e-01
1.580000000000000000e+02, 5.994482065983453012e-01
1.590000000000000000e+02, 5.217753961736570911e-01
1.600000000000000000e+02, 3.962363054405113605e-01
1.610000000000000000e+02, 3.548471555913704778e-01
1.620000000000000000e+02, 2.508512210745221793e-01
1.630000000000000000e+02, 1.540560414751746543e-01
1.640000000000000000e+02, 1.920326873333602635e-01
1.650000000000000000e+02, 1.558415183707223817e-01
1.660000000000000000e+02, 6.953919118463736115e-02
1.670000000000000000e+02, 1.005988680915474998e-01
1.680000000000000000e+02, 7.895919583061229707e-02
1.690000000000000000e+02, 1.269211831594811712e-01
1.700000000000000000e+02, 2.718866047900347360e-01
1.710000000000000000e+02, 4.203899795668841755e-01
1.720000000000000000e+02, 9.884832908353629044e-01
1.730000000000000000e+02, 1.564592900561045052e+00
1.740000000000000000e+02, 1.022085787277681179e+00
1.750000000000000000e+02, 4.739960995076346051e-01
1.760000000000000000e+02, 2.003577878078063867e-01
1.770000000000000000e+02, 1.403449945868644189e-01
1.780000000000000000e+02, 4.492129479008501874e-02
1.790000000000000000e+02, 4.739900686875486019e-02
1.800000000000000000e+02, 8.077966138988841582e-02
1.810000000000000000e+02, 5.841202888818329553e-02
1.820000000000000000e+02, 1.637668319471531353e-01
1.830000000000000000e+02, 2.238340859836203400e-01
1.840000000000000000e+02, 1.829365978290799499e-01
1.850000000000000000e+02, 3.000705735964960819e-01
1.860000000000000000e+02, 3.851015569265767713e-01
1.870000000000000000e+02, 5.473845746903936993e-01
1.880000000000000000e+02, 4.948176266491214892e-01
1.890000000000000000e+02, 4.658279955813790507e-01
1.900000000000000000e+02, 3.168032871683897356e-01
1.910000000000000000e+02, 3.076487733893951138e-01
1.920000000000000000e+02, 2.518525157519301838e-01
1.930000000000000000e+02, 2.042224477418986828e-01
1.940000000000000000e+02, 1.366662102729497008e-01
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [name path=sensor-rotation-1, color=sensor-rotation-1Color, line width=1.5pt, forget plot]
	table[col sep=comma]{%
0.000000000000000000e+00, 8.032558956365398739e-02
1.000000000000000000e+00, 5.922868758064615130e-02
2.000000000000000000e+00, 1.556649527029239921e-01
3.000000000000000000e+00, 1.817011988135305289e-01
4.000000000000000000e+00, 3.493210535316342846e-01
5.000000000000000000e+00, 5.076710848528052100e-01
6.000000000000000000e+00, 6.101107757680001020e-01
7.000000000000000000e+00, 6.321658149853615072e-01
8.000000000000000000e+00, 5.693861758362172010e-01
9.000000000000000000e+00, 4.264098833585181492e-01
1.000000000000000000e+01, 2.677139691657791087e-01
1.100000000000000000e+01, 2.078143495663322404e-01
1.200000000000000000e+01, 2.150686717286353911e-01
1.300000000000000000e+01, 1.241481540420088236e-01
1.400000000000000000e+01, 1.348015391087526160e-01
1.500000000000000000e+01, 8.842547649554281797e-02
1.600000000000000000e+01, 7.639517763718321752e-02
1.700000000000000000e+01, 1.846947852247808053e-01
1.800000000000000000e+01, 1.878058842451579002e-01
1.900000000000000000e+01, 1.586021975562675879e-01
2.000000000000000000e+01, 4.390351300693545733e-01
2.100000000000000000e+01, 8.118414480874853734e-01
2.200000000000000000e+01, 1.521896590510996239e+00
2.300000000000000000e+01, 1.200461475925660215e+00
2.400000000000000000e+01, 5.319258346463807685e-01
2.500000000000000000e+01, 1.890062096045207196e-01
2.600000000000000000e+01, 1.318693087919298179e-01
2.700000000000000000e+01, 8.161189408798413814e-02
2.800000000000000000e+01, 2.323156937147380363e-02
2.900000000000000000e+01, 2.748709513372582514e-02
3.000000000000000000e+01, 5.276692432185617343e-02
3.100000000000000000e+01, 4.920643105741047407e-02
3.200000000000000000e+01, 1.543318365539842751e-01
3.300000000000000000e+01, 2.200876072523548499e-01
3.400000000000000000e+01, 3.139318319802774093e-01
3.500000000000000000e+01, 3.451836895318802223e-01
3.600000000000000000e+01, 5.216563920570079782e-01
3.700000000000000000e+01, 4.653673822893071299e-01
3.800000000000000000e+01, 4.999546652566868588e-01
3.900000000000000000e+01, 4.065428629322530019e-01
4.000000000000000000e+01, 3.082051455388496453e-01
4.100000000000000000e+01, 2.020541637758081766e-01
4.200000000000000000e+01, 1.786144100558120784e-01
4.300000000000000000e+01, 1.776140024784899352e-01
4.400000000000000000e+01, 6.787346626689141904e-02
4.500000000000000000e+01, 7.266096757491243008e-02
4.600000000000000000e+01, 2.531565875075340172e-02
4.700000000000000000e+01, 5.443461323840321359e-02
4.800000000000000000e+01, 1.337562380850313981e-01
4.900000000000000000e+01, 2.013252374050372440e-01
5.000000000000000000e+01, 5.986376016891054030e-01
5.100000000000000000e+01, 1.150040782447746768e+00
5.200000000000000000e+01, 1.541447539152750679e+00
5.300000000000000000e+01, 8.522684838772344174e-01
5.400000000000000000e+01, 2.559835074900134178e-01
5.500000000000000000e+01, 2.471197992847059821e-01
5.600000000000000000e+01, 1.009554549568526249e-01
5.700000000000000000e+01, 1.527495996523794419e-01
5.800000000000000000e+01, 1.093926130337030816e-01
5.900000000000000000e+01, 8.023159586268173438e-02
6.000000000000000000e+01, 9.513460987716040873e-02
6.100000000000000000e+01, 1.153426865005249546e-01
6.200000000000000000e+01, 2.376390560822303766e-01
6.300000000000000000e+01, 2.407900996664398274e-01
6.400000000000000000e+01, 2.587563849243424974e-01
6.500000000000000000e+01, 4.431313630383685864e-01
6.600000000000000000e+01, 5.186759403565142090e-01
6.700000000000000000e+01, 6.409263642906196656e-01
6.800000000000000000e+01, 6.208884084306879325e-01
6.900000000000000000e+01, 5.046862016929318795e-01
7.000000000000000000e+01, 3.105400663021794516e-01
7.100000000000000000e+01, 2.181085834111087807e-01
7.200000000000000000e+01, 1.375121762335342890e-01
7.300000000000000000e+01, 1.317453626164351022e-01
7.400000000000000000e+01, 1.016818845910245489e-01
7.500000000000000000e+01, 1.289904545979655426e-01
7.600000000000000000e+01, 8.134635350979675661e-02
7.700000000000000000e+01, 1.618813803887995117e-01
7.800000000000000000e+01, 2.713495634790952793e-01
7.900000000000000000e+01, 4.005598912479939044e-01
8.000000000000000000e+01, 5.252975745195544999e-01
8.100000000000000000e+01, 5.995883096896584830e-01
8.200000000000000000e+01, 6.580191297619241153e-01
8.300000000000000000e+01, 4.822480299196419962e-01
8.400000000000000000e+01, 3.312564272017623490e-01
8.500000000000000000e+01, 3.449583185475484925e-01
8.600000000000000000e+01, 1.401200205302882695e-01
8.700000000000000000e+01, 1.438577837572069806e-01
8.800000000000000000e+01, 1.026055159276167417e-01
8.900000000000000000e+01, 1.599018683799175999e-01
9.000000000000000000e+01, 8.227718388060797916e-02
9.100000000000000000e+01, 1.348924943140384636e-01
9.200000000000000000e+01, 1.967187229016565952e-01
9.300000000000000000e+01, 1.485878738479505801e-01
9.400000000000000000e+01, 3.274381019751141930e-01
9.500000000000000000e+01, 4.665885798953523511e-01
9.600000000000000000e+01, 1.116089246709455862e+00
9.700000000000000000e+01, 1.542739208060529998e+00
9.800000000000000000e+01, 8.904929686852030013e-01
9.900000000000000000e+01, 4.217439310773839489e-01
1.000000000000000000e+02, 1.938939369004950009e-01
1.010000000000000000e+02, 5.251389001890351127e-02
1.020000000000000000e+02, 5.288315602071921862e-02
1.030000000000000000e+02, 4.922251634705442080e-02
1.040000000000000000e+02, 4.896294021845492422e-02
1.050000000000000000e+02, 7.703434867004195497e-02
1.060000000000000000e+02, 1.673548682142445010e-01
1.070000000000000000e+02, 1.433109709640965068e-01
1.080000000000000000e+02, 2.975442375631316416e-01
1.090000000000000000e+02, 3.769687667393071817e-01
1.100000000000000000e+02, 3.574385707542601653e-01
1.110000000000000000e+02, 4.743889986801863023e-01
1.120000000000000000e+02, 5.000847016209121199e-01
1.130000000000000000e+02, 4.464751418979305275e-01
1.140000000000000000e+02, 3.413774590836788914e-01
1.150000000000000000e+02, 2.607997236137024055e-01
1.160000000000000000e+02, 2.934963301360822840e-01
1.170000000000000000e+02, 6.464369670920362687e-02
1.180000000000000000e+02, 1.126906433032750926e-01
1.190000000000000000e+02, 5.618300342847007411e-02
1.200000000000000000e+02, 1.729398111878861777e-02
1.210000000000000000e+02, 5.887516676679496741e-02
1.220000000000000000e+02, 5.729321105633971428e-02
1.230000000000000000e+02, 1.536565812741261805e-01
1.240000000000000000e+02, 3.190435007740128337e-01
1.250000000000000000e+02, 7.425859410124355797e-01
1.260000000000000000e+02, 1.482798183692209726e+00
1.270000000000000000e+02, 1.325288510047307078e+00
1.280000000000000000e+02, 5.753530537911535347e-01
1.290000000000000000e+02, 3.467167405678112102e-01
1.300000000000000000e+02, 1.268303820135905369e-01
1.310000000000000000e+02, 1.414281753079041637e-01
1.320000000000000000e+02, 1.432296812137833775e-01
1.330000000000000000e+02, 1.259516625204885332e-01
1.340000000000000000e+02, 7.936635100801824050e-02
1.350000000000000000e+02, 1.419612991186181838e-01
1.360000000000000000e+02, 1.597015189526852785e-01
1.370000000000000000e+02, 2.400678617432416284e-01
1.380000000000000000e+02, 2.887719485002254727e-01
1.390000000000000000e+02, 3.203329310074994329e-01
1.400000000000000000e+02, 4.666697675165862313e-01
1.410000000000000000e+02, 5.295906530965350800e-01
1.420000000000000000e+02, 5.905258470293601736e-01
1.430000000000000000e+02, 4.940749239679912419e-01
1.440000000000000000e+02, 3.543738438923534351e-01
1.450000000000000000e+02, 2.803471942406298156e-01
1.460000000000000000e+02, 2.232846829374217912e-01
1.470000000000000000e+02, 4.861111099711824118e-02
1.480000000000000000e+02, 3.312708986717483040e-02
1.490000000000000000e+02, 4.465447035744701809e-02
1.500000000000000000e+02, 6.665567615776142596e-02
1.510000000000000000e+02, 8.009150603582922134e-02
1.520000000000000000e+02, 2.413484861695125994e-01
1.530000000000000000e+02, 2.790743076315234106e-01
1.540000000000000000e+02, 3.467494093558714519e-01
1.550000000000000000e+02, 5.311527310895070020e-01
1.560000000000000000e+02, 6.180392974040708198e-01
1.570000000000000000e+02, 5.926020606988580131e-01
1.580000000000000000e+02, 4.781080017705205409e-01
1.590000000000000000e+02, 4.140882353793172710e-01
1.600000000000000000e+02, 2.576182392376314412e-01
1.610000000000000000e+02, 2.111151206201626052e-01
1.620000000000000000e+02, 2.279030355565377086e-01
1.630000000000000000e+02, 2.046035807102913051e-01
1.640000000000000000e+02, 9.101396363212334306e-02
1.650000000000000000e+02, 9.918663851423707711e-02
1.660000000000000000e+02, 6.177419626834976946e-02
1.670000000000000000e+02, 7.617883909570298540e-02
1.680000000000000000e+02, 1.914119174700800452e-01
1.690000000000000000e+02, 2.760525603659990668e-01
1.700000000000000000e+02, 6.974445633976070757e-01
1.710000000000000000e+02, 1.368590594507399949e+00
1.720000000000000000e+02, 1.418528491913119582e+00
1.730000000000000000e+02, 6.586213088160114415e-01
1.740000000000000000e+02, 2.938033349880910250e-01
1.750000000000000000e+02, 9.865493231877424385e-02
1.760000000000000000e+02, 1.183492842574922488e-01
1.770000000000000000e+02, 6.083602444614630289e-02
1.780000000000000000e+02, 3.623015574385404780e-02
1.790000000000000000e+02, 9.351576199415337354e-02
1.800000000000000000e+02, 7.633764828233868815e-02
1.810000000000000000e+02, 1.552447262292309671e-01
1.820000000000000000e+02, 1.970587731833020606e-01
1.830000000000000000e+02, 2.593957657677585238e-01
1.840000000000000000e+02, 3.818843931797705205e-01
1.850000000000000000e+02, 4.682664050469090844e-01
1.860000000000000000e+02, 4.539713822750144345e-01
1.870000000000000000e+02, 5.125383874399286332e-01
1.880000000000000000e+02, 3.382077853772590403e-01
1.890000000000000000e+02, 2.924925797095426772e-01
1.900000000000000000e+02, 2.378366927578807466e-01
1.910000000000000000e+02, 1.215694411492478783e-01
1.920000000000000000e+02, 1.155775029730453790e-01
1.930000000000000000e+02, 7.063187313581402449e-02
1.940000000000000000e+02, 8.172952093346848301e-02
};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

